Equilibrium Microcanonical Annealing for First-Order Phase Transitions

A framework is presented for carrying out simulations of equilibrium systems in the microcanonical ensemble using annealing in an energy ceiling. The framework encompasses an equilibrium version of simulated annealing, population annealing and hybrid algorithms that interpolate between these extremes. These equilibrium, microcanonical annealing algorithms are applied to the thermal first-order transition in the 20-state, two-dimensional Potts model. All of these algorithms are observed to perform well at the first-order transition though for the system sizes studied here, equilibrium simulated annealing is most efficient.

==> Plots/PA_hist_1600.tex <==
e pe 
0.0 0.0
-0.000625 0.0
-0.00125 0.0
-0.001875 0.0
-0.0025 0.0
-0.003125 0.0
-0.00375 0.0
-0.004375 0.0
-0.005 0.0
-0.005625 0.0
-0.00625 0.0
-0.006875 0.0
-0.0075 0.0
-0.008125 0.0
-0.00875 0.0
-0.009375 0.0
-0.01 0.0
-0.010625 0.0
-0.01125 0.0
-0.011875 0.0
-0.0125 0.0
-0.013125 0.0
-0.01375 0.0
-0.014375 0.0
-0.015 0.0
-0.015625 0.0
-0.01625 0.0
-0.016875 0.0
-0.0175 0.0
-0.018125 0.0
-0.01875 0.0
-0.019375 0.0
-0.02 0.0
-0.020625 0.0
-0.02125 0.0
-0.021875 0.0
-0.0225 0.0
-0.023125 0.0
-0.02375 0.0
-0.024375 0.0
-0.025 0.0
-0.025625 0.0
-0.02625 0.0
-0.026875 0.0
-0.0275 0.0
-0.028125 0.0
-0.02875 0.0
-0.029375 0.0
-0.03 0.0
-0.030625 0.0
-0.03125 0.0
-0.031875 0.0
-0.0325 0.0
-0.033125 0.0
-0.03375 0.0
-0.034375 0.0
-0.035 0.0
-0.035625 0.0
-0.03625 0.0
-0.036875 0.0
-0.0375 0.0
-0.038125 0.0
-0.03875 0.0
-0.039375 0.0
-0.04 0.0
-0.040625 0.0
-0.04125 0.0
-0.041875 0.0
-0.0425 0.0
-0.043125 0.0
-0.04375 0.0
-0.044375 0.0
-0.045 0.0
-0.045625 0.0
-0.04625 0.0
-0.046875 0.0
-0.0475 0.0
-0.048125 0.0
-0.04875 0.0
-0.049375 0.0
-0.05 0.0
-0.050625 0.0
-0.05125 0.0
-0.051875 0.0
-0.0525 0.0
-0.053125 0.0
-0.05375 0.0
-0.054375 0.0
-0.055 0.0
-0.055625 0.0
-0.05625 0.0
-0.056875 0.0
-0.0575 0.0
-0.058125 0.0
-0.05875 0.0
-0.059375 0.0
-0.06 0.0
-0.060625 0.0
-0.06125 0.0
-0.061875 2.4320738261847158e-234
-0.0625 0.0
-0.063125 7.282667995649076e-233
-0.06375 0.0
-0.064375 6.542214817049833e-231
-0.065 5.9666580987130895e-230
-0.065625 5.2240517600463986e-229
-0.06625 3.9306701816799836e-228
-0.066875 1.9553769077600968e-227
-0.0675 8.560080256130614e-227
-0.068125 8.197296261020814e-226
-0.06875 1.121417589589482e-224
-0.069375 7.363817335894241e-224
-0.07 6.907825321226716e-223
-0.070625 5.2500324002182993e-222
-0.07125 4.2805493070105136e-221
-0.071875 3.5213549512641594e-220
-0.0725 2.434409300956214e-219
-0.073125 1.816918078033678e-218
-0.07375 1.334178154960531e-217
-0.074375 9.315675750601757e-217
-0.075 7.210156378635703e-216
-0.075625 5.12224151456868e-215
-0.07625 3.9567748330702946e-214
-0.076875 2.8770621210158424e-213
-0.0775 2.0022880480691488e-212
-0.078125 1.4138903377102984e-211
-0.07875 9.734430326996946e-211
-0.079375 7.228619668268943e-210
-0.08 4.810413163925597e-209
-0.080625 3.290415660986331e-208
-0.08125 2.2362824463151358e-207
-0.081875 1.517347433269362e-206
-0.0825 1.0189676214557557e-205
-0.083125 6.78383749783043e-205
-0.08375 4.4963076344482446e-204
-0.084375 2.936476249013e-203
-0.085 1.8741000308712655e-202
-0.085625 1.2285690111340508e-201
-0.08625 7.831450682688762e-201
-0.086875 4.9647389704395654e-200
-0.0875 3.109265281709056e-199
-0.088125 1.9643582263808635e-198
-0.08875 1.2139028286890898e-197
-0.089375 7.461506117210398e-197
-0.09 4.579680267660384e-196
-0.090625 2.7772650234377763e-195
-0.09125 1.6694020709161388e-194
-0.091875 1.0020933094646612e-193
-0.0925 5.905034215205183e-193
-0.093125 3.512019790129313e-192
-0.09375 2.050303860668107e-191
-0.094375 1.195074529905861e-190
-0.095 6.898012241844638e-190
-0.095625 3.9578446524555465e-189
-0.09625 2.254820208307558e-188
-0.096875 1.2760993338624832e-187
-0.0975 7.177651635930469e-187
-0.098125 4.003428565378724e-186
-0.09875 2.225417149325647e-185
-0.099375 1.2253743381394432e-184
-0.1 6.704718496935264e-184
-0.100625 3.6441836198151563e-183
-0.10125 1.9689185666087753e-182
-0.101875 1.0576212931407582e-181
-0.1025 5.643309476696798e-181
-0.103125 2.9904342007395143e-180
-0.10375 1.5782478903412233e-179
-0.104375 8.241948913445293e-179
-0.105 4.287072035893756e-178
-0.105625 2.21159615797926e-177
-0.10625 1.1356412407585651e-176
-0.106875 5.799487740918799e-176
-0.1075 2.9417343243680175e-175
-0.108125 1.4808232426489246e-174
-0.10875 7.418357120237835e-174
-0.109375 3.6995368318734156e-173
-0.11 1.8307278729908258e-172
-0.110625 9.002281397314076e-172
-0.11125 4.409086777927785e-171
-0.111875 2.1442477344748255e-170
-0.1125 1.0349036778110468e-169
-0.113125 4.9774279048249263e-169
-0.11375 2.3795794486947477e-168
-0.114375 1.129376815936851e-167
-0.115 5.3400575239932856e-167
-0.115625 2.504519223194142e-166
-0.11625 1.1691245660323966e-165
-0.116875 5.430658086282102e-165
-0.1175 2.5045869774629418e-164
-0.118125 1.1511292295461554e-163
-0.11875 5.2466133777746294e-163
-0.119375 2.3817289068344154e-162
-0.12 1.0751253123890028e-161
-0.120625 4.821698946229529e-161
-0.12125 2.1562989210815985e-160
-0.121875 9.55937959515773e-160
-0.1225 4.2278243092015103e-159
-0.123125 1.8551947980759944e-158
-0.12375 8.099808064152528e-158
-0.124375 3.5228559737224426e-157
-0.125 1.5238233819833702e-156
-0.125625 6.540491429243616e-156
-0.12625 2.7927163276488392e-155
-0.126875 1.188538674987701e-154
-0.1275 5.0360996415430966e-154
-0.128125 2.116306715193191e-153
-0.12875 8.876362938615208e-153
-0.129375 3.6931811851282915e-152
-0.13 1.5326557216388847e-151
-0.130625 6.320125480140662e-151
-0.13125 2.590614449931164e-150
-0.131875 1.0571101651811769e-149
-0.1325 4.298609664704695e-149
-0.133125 1.7350490394036893e-148
-0.13375 6.977903671370619e-148
-0.134375 2.791138623812816e-147
-0.135 1.1093943846153903e-146
-0.135625 4.400425359379763e-146
-0.13625 1.7323027288343146e-145
-0.136875 6.797300197914577e-145
-0.1375 2.6525651797333025e-144
-0.138125 1.031096917733335e-143
-0.13875 3.987208776204805e-143
-0.139375 1.5325094690854828e-142
-0.14 5.8708002435636925e-142
-0.140625 2.23683854929111e-141
-0.14125 8.486580442471721e-141
-0.141875 3.203291405156401e-140
-0.1425 1.2034481007075154e-139
-0.143125 4.497195816037058e-139
-0.14375 1.674861636101868e-138
-0.144375 6.201592775243381e-138
-0.145 2.2889042530569005e-137
-0.145625 8.40274982334011e-137
-0.14625 3.069239104801598e-136
-0.146875 1.1150718654250623e-135
-0.1475 4.039663302402316e-135
-0.148125 1.456944766612589e-134
-0.14875 5.225116377930171e-134
-0.149375 1.8661941213242884e-133
-0.15 6.6340826301125535e-133
-0.150625 2.3480067184495303e-132
-0.15125 8.277713245319389e-132
-0.151875 2.9040297984225066e-131
-0.1525 1.0144226723320486e-130
-0.153125 3.5272302931532763e-130
-0.15375 1.220941435927904e-129
-0.154375 4.209281094835623e-129
-0.155 1.4450123751372937e-128
-0.155625 4.937192707656359e-128
-0.15625 1.681880826840277e-127
-0.156875 5.693786107513319e-127
-0.1575 1.9197117180342183e-126
-0.158125 6.443819848330301e-126
-0.15875 2.1581187642559262e-125
-0.159375 7.185281294649744e-125
-0.16 2.3865689684398914e-124
-0.160625 7.869106515397488e-124
-0.16125 2.5874660419513212e-123
-0.161875 8.483340577165601e-123
-0.1625 2.765962748318938e-122
-0.163125 8.991778293150873e-122
-0.16375 2.905926831155934e-121
-0.164375 9.373361885379993e-121
-0.165 3.006026615915939e-120
-0.165625 9.602332292332931e-120
-0.16625 3.0566355236738276e-119
-0.166875 9.686272250176531e-119
-0.1675 3.057415885881149e-118
-0.168125 9.613847674095681e-118
-0.16875 3.0141618305972748e-117
-0.169375 9.40414813827782e-117
-0.17 2.91840969985169e-116
-0.170625 9.030978134014442e-116
-0.17125 2.784582909712574e-115
-0.171875 8.552997398661824e-115
-0.1725 2.613406787609509e-114
-0.173125 7.965526020811612e-114
-0.17375 2.4172490193559243e-113
-0.174375 7.308186631420068e-113
-0.175 2.200756499980716e-112
-0.175625 6.603433604946334e-112
-0.17625 1.971923993745448e-111
-0.176875 5.868274676862265e-111
-0.1775 1.740676466419083e-110
-0.178125 5.137542505504333e-110
-0.17875 1.5122801291569334e-109
-0.179375 4.434489447160759e-109
-0.18 1.2940473069383537e-108
-0.180625 3.763563050286576e-108
-0.18125 1.0920053922039166e-107
-0.181875 3.1544381385700015e-107
-0.1825 9.076134535796332e-107
-0.183125 2.603544263839364e-106
-0.18375 7.44178353316305e-106
-0.184375 2.1187177683264494e-105
-0.185 6.010005654121964e-105
-0.185625 1.6980835433441375e-104
-0.18625 4.781169419857965e-104
-0.186875 1.3405112825969915e-103
-0.1875 3.752406897345001e-103
-0.188125 1.0435783824457725e-102
-0.18875 2.8961131440568853e-102
-0.189375 8.008700850105858e-102
-0.19 2.2068526416694165e-101
-0.190625 6.060774604916249e-101
-0.19125 1.6572365573398438e-100
-0.191875 4.5197715603168833e-100
-0.1925 1.2267393468875335e-99
-0.193125 3.3246802779192693e-99
-0.19375 8.956930357611725e-99
-0.194375 2.4090687026752694e-98
-0.195 6.448928024517889e-98
-0.195625 1.7211396618973605e-97
-0.19625 4.5817601205129197e-97
-0.196875 1.215625438194079e-96
-0.1975 3.2156435661476393e-96
-0.198125 8.462187569744997e-96
-0.19875 2.220126735036657e-95
-0.199375 5.814127643928825e-95
-0.2 1.5140643330798483e-94
-0.200625 3.930364612722023e-94
-0.20125 1.0182528164336748e-93
-0.201875 2.6308685542536616e-93
-0.2025 6.759748477626157e-93
-0.203125 1.734440478261025e-92
-0.20375 4.424946529396025e-92
-0.204375 1.1282557805206739e-91
-0.205 2.861223566071041e-91
-0.205625 7.241255517117852e-91
-0.20625 1.8285257799447929e-90
-0.206875 4.59498882411374e-90
-0.2075 1.1500984244339227e-89
-0.208125 2.874243181551892e-89
-0.20875 7.157297759384581e-89
-0.209375 1.7737066475415452e-88
-0.21 4.391938440958548e-88
-0.210625 1.082074537245264e-87
-0.21125 2.659737210869978e-87
-0.211875 6.521496108862878e-87
-0.2125 1.5925362573814678e-86
-0.213125 3.877656186469945e-86
-0.21375 9.416832199988892e-86
-0.214375 2.2784714528946198e-85
-0.215 5.488539055736399e-85
-0.215625 1.3212426129698882e-84
-0.21625 3.161523226021079e-84
-0.216875 7.557553913855945e-84
-0.2175 1.801097364388167e-83
-0.218125 4.272647047203743e-83
-0.21875 1.0124360993490743e-82
-0.219375 2.3898371087205768e-82
-0.22 5.627971989216956e-82
-0.220625 1.3203481786800253e-81
-0.22125 3.0850187601634844e-81
-0.221875 7.2077106206747545e-81
-0.2225 1.6743656489851461e-80
-0.223125 3.8796522681112174e-80
-0.22375 8.97200167828322e-80
-0.224375 2.0662292191731156e-79
-0.225 4.7516638207646036e-79
-0.225625 1.0880862705711416e-78
-0.22625 2.4864024463478956e-78
-0.226875 5.661610363522764e-78
-0.2275 1.2845042503984292e-77
-0.228125 2.907888367346557e-77
-0.22875 6.56679914012365e-77
-0.229375 1.4781243596809473e-76
-0.23 3.316866712134598e-76
-0.230625 7.415165886636938e-76
-0.23125 1.654222484828563e-75
-0.231875 3.679538291603224e-75
-0.2325 8.164503301156437e-75
-0.233125 1.8065251537397626e-74
-0.23375 3.985766518429061e-74
-0.234375 8.769751539604928e-74
-0.235 1.922883362783438e-73
-0.235625 4.2078229853996356e-73
-0.23625 9.164710043266434e-73
-0.236875 1.9937833546535645e-72
-0.2375 4.3209706618160813e-72
-0.238125 9.355999817789276e-72
-0.23875 2.0167497198906908e-71
-0.239375 4.3322764976644256e-71
-0.24 9.306918768773407e-71
-0.240625 1.9900677195021637e-70
-0.24125 4.2437199278693334e-70
-0.241875 9.023634427877898e-70
-0.2425 1.9169746818477132e-69
-0.243125 4.054377893482765e-69
-0.24375 8.560537432349204e-69
-0.244375 1.7995782535494346e-68
-0.245 3.774604815212219e-68
-0.245625 7.894841548444271e-68
-0.24625 1.649705142924976e-67
-0.246875 3.431217362660877e-67
-0.2475 7.121583223010647e-67
-0.248125 1.4748332635157549e-66
-0.24875 3.0460594687735653e-66
-0.249375 6.268625616278177e-66
-0.25 1.2881327192014735e-65
-0.250625 2.6391725597211336e-65
-0.25125 5.395831992984956e-65
-0.251875 1.0999560581800335e-64
-0.2525 2.237199874197874e-64
-0.253125 4.538936330703414e-64
-0.25375 9.173957541617249e-64
-0.254375 1.852003612515028e-63
-0.255 3.724228908381122e-63
-0.255625 7.472248849872072e-63
-0.25625 1.4922684961516982e-62
-0.256875 2.9825696127168077e-62
-0.2575 5.9341972248823786e-62
-0.258125 1.1779802240141105e-61
-0.25875 2.334348180297672e-61
-0.259375 4.6132486393696684e-61
-0.26 9.092724340679135e-61
-0.260625 1.7886642055606865e-60
-0.26125 3.507234453661819e-60
-0.261875 6.86306964515133e-60
-0.2625 1.3402752979875501e-59
-0.263125 2.6105737906444295e-59
-0.26375 5.067482268544121e-59
-0.264375 9.824844238188514e-59
-0.265 1.8967862964761675e-58
-0.265625 3.657611679494454e-58
-0.26625 7.035231061765059e-58
-0.266875 1.34894048486032e-57
-0.2675 2.5788431573101575e-57
-0.268125 4.9222521728018634e-57
-0.26875 9.37249229311621e-57
-0.269375 1.782885862880091e-56
-0.27 3.3804831008951272e-56
-0.270625 6.395857567796317e-56
-0.27125 1.2068413188133235e-55
-0.271875 2.272173806388351e-55
-0.2725 4.264628026436993e-55
-0.273125 7.988558719898137e-55
-0.27375 1.4931541691362078e-54
-0.274375 2.7828810455709476e-54
-0.275 5.173884475669535e-54
-0.275625 9.599979608528481e-54
-0.27625 1.7784134477389627e-53
-0.276875 3.2829880731906063e-53
-0.2775 6.0470498787739265e-53
-0.278125 1.1116781450370077e-52
-0.27875 2.0391536241308964e-52
-0.279375 3.727989637262211e-52
-0.28 6.810102675604128e-52
-0.280625 1.239451476404602e-51
-0.28125 2.2525982055401836e-51
-0.281875 4.083040863818782e-51
-0.2825 7.383901284977859e-51
-0.283125 1.3320789460675722e-50
-0.28375 2.3987451989730986e-50
-0.284375 4.314100192121605e-50
-0.285 7.726463514934217e-50
-0.285625 1.3843632391932435e-49
-0.28625 2.471862242668601e-49
-0.286875 4.3993094048329595e-49
-0.2875 7.816161836462635e-49
-0.288125 1.38448444309849e-48
-0.28875 2.448989553044047e-48
-0.289375 4.3265137974875536e-48
-0.29 7.619021738634041e-48
-0.290625 1.3395846164543456e-47
-0.29125 2.3509294139822934e-47
-0.291875 4.1139600102832517e-47
-0.2925 7.175679822307433e-47
-0.293125 1.2496721663630939e-46
-0.29375 2.1725095918683093e-46
-0.294375 3.769199509236624e-46
-0.295 6.5365771223175446e-46
-0.295625 1.1298002381093586e-45
-0.29625 1.9460670836750353e-45
-0.296875 3.3454720338388356e-45
-0.2975 5.739461071533515e-45
-0.298125 9.850949147776941e-45
-0.29875 1.682853458636288e-44
-0.299375 2.8700963619343194e-44
-0.3 4.890142189141848e-44
-0.300625 8.307373350771292e-44
-0.30125 1.4097811126629227e-43
-0.301875 2.3843369173056453e-43
-0.3025 4.019342360968832e-43
-0.303125 6.776637731474815e-43
-0.30375 1.1396369997268933e-42
-0.304375 1.9124898510539525e-42
-0.305 3.2010122277195474e-42
-0.305625 5.3607610641000046e-42
-0.30625 8.933400196004209e-42
-0.306875 1.4877918287608339e-41
-0.3075 2.4696528378143664e-41
-0.308125 4.096958720372845e-41
-0.30875 6.762518526275772e-41
-0.309375 1.1164706296510812e-40
-0.31 1.838483889000007e-40
-0.310625 3.0276019073073527e-40
-0.31125 4.977677134178924e-40
-0.311875 8.139386240955485e-40
-0.3125 1.3346535199565278e-39
-0.313125 2.1753740919111522e-39
-0.31375 3.5443612511409495e-39
-0.314375 5.758964560538481e-39
-0.315 9.33917908832039e-39
-0.315625 1.512622934201113e-38
-0.31625 2.4437224748906704e-38
-0.316875 3.942759449569123e-38
-0.3175 6.346250932522888e-38
-0.318125 1.0202469579456245e-37
-0.31875 1.6358446223929423e-37
-0.319375 2.6206072895259382e-37
-0.32 4.185586510679187e-37
-0.320625 6.6757186598313545e-37
-0.32125 1.0626787653601563e-36
-0.321875 1.68713486678188e-36
-0.3225 2.6781289331449338e-36
-0.323125 4.234947431705401e-36
-0.32375 6.68676570797994e-36
-0.324375 1.0549848654220932e-35
-0.325 1.659595678452618e-35
-0.325625 2.607063925175257e-35
-0.32625 4.0923754479606597e-35
-0.326875 6.401827062560893e-35
-0.3275 9.994101356471781e-35
-0.328125 1.5583055687475504e-34
-0.32875 2.4259150866642983e-34
-0.329375 3.765472097587372e-34
-0.33 5.842810322509377e-34
-0.330625 9.04178832516268e-34
-0.33125 1.3969350968051486e-33
-0.331875 2.152150054387664e-33
-0.3325 3.313439272331201e-33
-0.333125 5.094210103663161e-33
-0.33375 7.821479199114092e-33
-0.334375 1.1963250842501447e-32
-0.335 1.8304256178956524e-32
-0.335625 2.790284613458784e-32
-0.33625 4.2564490345151107e-32
-0.336875 6.468298848407103e-32
-0.3375 9.835240244170445e-32
-0.338125 1.4902773164306842e-31
-0.33875 2.2539824737079156e-31
-0.339375 3.4014605592489104e-31
-0.34 5.130144110217695e-31
-0.340625 7.7236896281666e-31
-0.34125 1.1616582461685924e-30
-0.341875 1.7404986062736077e-30
-0.3425 2.604609808618093e-30
-0.343125 3.891080843444525e-30
-0.34375 5.810466444479026e-30
-0.344375 8.646694245995026e-30
-0.345 1.284974337576884e-29
-0.345625 1.9084299967770532e-29
-0.34625 2.828826637011123e-29
-0.346875 4.1832930761209264e-29
-0.3475 6.18616459493928e-29
-0.348125 9.11040470896847e-29
-0.34875 1.3419070022613346e-28
-0.349375 1.9726397863215125e-28
-0.35 2.8978909266105087e-28
-0.350625 4.2464117224905085e-28
-0.35125 6.2109193411560445e-28
-0.351875 9.070364928006104e-28
-0.3525 1.3212899686943508e-27
-0.353125 1.9213296260765383e-27
-0.35375 2.7912757146132962e-27
-0.354375 4.042759051721754e-27
-0.355 5.857985005303217e-27
-0.355625 8.469245293845527e-27
-0.35625 1.2239608527232051e-26
-0.356875 1.7636177517365477e-26
-0.3575 2.5383117727378796e-26
-0.358125 3.648106260649751e-26
-0.35875 5.236824443355669e-26
-0.359375 7.491874110757977e-26
-0.36 1.070592102845985e-25
-0.360625 1.5286184550378045e-25
-0.36125 2.1815729453484575e-25
-0.361875 3.0997211329589556e-25
-0.3625 4.410679047999972e-25
-0.363125 6.259066247670944e-25
-0.36375 8.86638125085371e-25
-0.364375 1.2539690964293366e-24
-0.365 1.7694951617349357e-24
-0.365625 2.496086171628763e-24
-0.36625 3.51922367162018e-24
-0.366875 4.9542678320404265e-24
-0.3675 6.945871001343746e-24
-0.368125 9.731689301486587e-24
-0.36875 1.3626871490704217e-23
-0.369375 1.9057062418957394e-23
-0.37 2.655268642469313e-23
-0.370625 3.6971934689992626e-23
-0.37125 5.148178048521506e-23
-0.371875 7.154310233157252e-23
-0.3725 9.938169611986797e-23
-0.373125 1.3748932457774748e-22
-0.37375 1.899993684682245e-22
-0.374375 2.6221301696825186e-22
-0.375 3.62168025330432e-22
-0.375625 4.979965547509699e-22
-0.37625 6.847852598550598e-22
-0.376875 9.41060558875242e-22
-0.3775 1.2917549185231636e-21
-0.378125 1.7702163332313774e-21
-0.37875 2.4186315015172143e-21
-0.379375 3.3009594265756384e-21
-0.38 4.5042037036240604e-21
-0.380625 6.126874369606296e-21
-0.38125 8.334751933442367e-21
-0.381875 1.1301988264472111e-20
-0.3825 1.533122608737208e-20
-0.383125 2.077021574846145e-20
-0.38375 2.806177904241505e-20
-0.384375 3.791852941835801e-20
-0.385 5.111832478560138e-20
-0.385625 6.87941048697437e-20
-0.38625 9.253073914768686e-20
-0.386875 1.2425844662665812e-19
-0.3875 1.666776419819634e-19
-0.388125 2.230948391152668e-19
-0.38875 2.9818576558688736e-19
-0.389375 3.978470168975572e-19
-0.39 5.301544552496503e-19
-0.390625 7.069431198795278e-19
-0.39125 9.398469877476237e-19
-0.391875 1.2467653068520897e-18
-0.3925 1.655194683697956e-18
-0.393125 2.191969781189919e-18
-0.39375 2.8964593656191892e-18
-0.394375 3.829836580105787e-18
-0.395 5.047962676570452e-18
-0.395625 6.6465459379839664e-18
-0.39625 8.742621513672027e-18
-0.396875 1.1477148749978765e-17
-0.3975 1.506350703652542e-17
-0.398125 1.9764862710000747e-17
-0.39875 2.588687705554664e-17
-0.399375 3.3795553734754445e-17
-0.4 4.409784695087947e-17
-0.400625 5.754857505107046e-17
-0.40125 7.498626134090561e-17
-0.401875 9.751646218185415e-17
-0.4025 1.266321725309536e-16
-0.403125 1.6433051761057015e-16
-0.40375 2.1256653592931022e-16
-0.404375 2.7464041779506365e-16
-0.405 3.545185892525253e-16
-0.405625 4.578527943509499e-16
-0.40625 5.906287613968633e-16
-0.406875 7.594762796429922e-16
-0.4075 9.756133693103773e-16
-0.408125 1.2528938819260195e-15
-0.40875 1.6075268269281146e-15
-0.409375 2.0581315567412336e-15
-0.41 2.6324831141985847e-15
-0.410625 3.3633633374011795e-15
-0.41125 4.290700602370571e-15
-0.411875 5.466269952982372e-15
-0.4125 6.957526191121262e-15
-0.413125 8.845558278479694e-15
-0.41375 1.1236556487069627e-14
-0.414375 1.423060586074388e-14
-0.415 1.8026976421409273e-14
-0.415625 2.2821854043316663e-14
-0.41625 2.8786266300091896e-14
-0.416875 3.6353546627835585e-14
-0.4175 4.5831275190192644e-14
-0.418125 5.773341235317753e-14
-0.41875 7.260264015594406e-14
-0.419375 9.126182059098022e-14
-0.42 1.1450092476276357e-13
-0.420625 1.4348282372962393e-13
-0.42125 1.796387035300147e-13
-0.421875 2.246181289796834e-13
-0.4225 2.806638991382816e-13
-0.423125 3.4962378526724e-13
-0.42375 4.358691120216818e-13
-0.424375 5.424268253867001e-13
-0.425 6.738350261119405e-13
-0.425625 8.376663614779526e-13
-0.42625 1.0395548378417127e-12
-0.426875 1.2881367612591351e-12
-0.4275 1.592881633559038e-12
-0.428125 1.9685474015829824e-12
-0.42875 2.433486571976045e-12
-0.429375 2.999392822926876e-12
-0.43 3.69682720272894e-12
-0.430625 4.549316231998119e-12
-0.43125 5.5942991466715064e-12
-0.431875 6.871780242015934e-12
-0.4325 8.436019204111865e-12
-0.433125 1.0323638713887351e-11
-0.43375 1.2640500027202762e-11
-0.434375 1.543577401450335e-11
-0.435 1.8838766650387347e-11
-0.435625 2.300875389710692e-11
-0.43625 2.8018368472681833e-11
-0.436875 3.412530769644774e-11
-0.4375 4.146027531545738e-11
-0.438125 5.0323412046983845e-11
-0.43875 6.105894688040097e-11
-0.439375 7.39670980681294e-11
-0.44 8.97059681437201e-11
-0.440625 1.086350072866943e-10
-0.44125 1.313949397947942e-10
-0.441875 1.584979537725917e-10
-0.4425 1.91062024886003e-10
-0.443125 2.3031245507188885e-10
-0.44375 2.769184031285042e-10
-0.444375 3.3296639213544294e-10
-0.445 3.996084150491681e-10
-0.445625 4.797566561885913e-10
-0.44625 5.74954321130449e-10
-0.446875 6.879760996738458e-10
-0.4475 8.226053141931894e-10
-0.448125 9.817902226531774e-10
-0.44875 1.1723466488175628e-09
-0.449375 1.3985691501831676e-09
-0.45 1.6650553584423693e-09
-0.450625 1.9814848399790923e-09
-0.45125 2.356659684976073e-09
-0.451875 2.795221468677862e-09
-0.4525 3.318898769099675e-09
-0.453125 3.9334130613164864e-09
-0.45375 4.6555822188202925e-09
-0.454375 5.507822571418386e-09
-0.455 6.507044956796281e-09
-0.455625 7.67697840084815e-09
-0.45625 9.036069073844922e-09
-0.456875 1.0648789036893354e-08
-0.4575 1.253610842309806e-08
-0.458125 1.475046532041193e-08
-0.45875 1.7308605664460104e-08
-0.459375 2.030905451407075e-08
-0.46 2.380493758426626e-08
-0.460625 2.791250979267577e-08
-0.46125 3.264623684560151e-08
-0.461875 3.827188435644287e-08
-0.4625 4.467543125912921e-08
-0.463125 5.218249833505426e-08
-0.46375 6.079687579780163e-08
-0.464375 7.074214483652522e-08
-0.465 8.235092766437999e-08
-0.465625 9.576422471716907e-08
-0.46625 1.1108398586943161e-07
-0.466875 1.289206041250325e-07
-0.4675 1.4939093461782667e-07
-0.468125 1.7299808354954508e-07
-0.46875 2.004779973835658e-07
-0.469375 2.3179749953174685e-07
-0.47 2.676725936332774e-07
-0.470625 3.0912682327966686e-07
-0.47125 3.561270479102792e-07
-0.471875 4.104688304344833e-07
-0.4725 4.72956869618368e-07
-0.473125 5.440667148170701e-07
-0.47375 6.244229238507714e-07
-0.474375 7.17097710013863e-07
-0.475 8.211923811437755e-07
-0.475625 9.40883750246711e-07
-0.47625 1.0767584798463605e-06
-0.476875 1.2321357073440536e-06
-0.4775 1.4085485664170976e-06
-0.478125 1.6083151133190453e-06
-0.47875 1.8351580784798276e-06
-0.479375 2.0878488664705266e-06
-0.48 2.3743078784571118e-06
-0.480625 2.7021595943196125e-06
-0.48125 3.06786623159685e-06
-0.481875 3.48558558512413e-06
-0.4825 3.957961461929791e-06
-0.483125 4.487927826236402e-06
-0.48375 5.085716440735612e-06
-0.484375 5.744854602801493e-06
-0.485 6.504654339564461e-06
-0.485625 7.348137117082885e-06
-0.48625 8.294133322721238e-06
-0.486875 9.356053947138406e-06
-0.4875 1.0540008703337481e-05
-0.488125 1.1898125930947457e-05
-0.48875 1.3393114174334079e-05
-0.489375 1.507018734352143e-05
-0.49 1.6931776706762015e-05
-0.490625 1.9020794847974753e-05
-0.49125 2.134445729297772e-05
-0.491875 2.388569919942125e-05
-0.4925 2.6728073576636092e-05
-0.493125 2.993559734196052e-05
-0.49375 3.342935491996698e-05
-0.494375 3.734506934326376e-05
-0.495 4.1644139069533514e-05
-0.495625 4.647361009480694e-05
-0.49625 5.183439457872296e-05
-0.496875 5.7753747832437625e-05
-0.4975 6.434690004581314e-05
-0.498125 7.154353187522448e-05
-0.49875 7.953236983073682e-05
-0.499375 8.833008143892803e-05
-0.5 9.779466590377156e-05
-0.500625 0.00010818404569519662
-0.50125 0.00011999286773140469
-0.501875 0.0001327416186318584
-0.5025 0.00014677068788372877
-0.503125 0.00016240140157825823
-0.50375 0.00017933715765910537
-0.504375 0.00019819908858843236
-0.505 0.00021868056015661032
-0.505625 0.00024095785522212156
-0.50625 0.0002651531655747545
-0.506875 0.0002919322725851043
-0.5075 0.0003210499982385921
-0.508125 0.00035264331005824344
-0.50875 0.00038789248072495006
-0.509375 0.0004257769297318794
-0.51 0.0004665661337722891
-0.510625 0.0005117301999324027
-0.51125 0.0005606752830313628
-0.511875 0.0006128684248697723
-0.5125 0.0006701345710964882
-0.513125 0.0007318572837859262
-0.51375 0.0007995159011067565
-0.514375 0.0008724486043955567
-0.515 0.0009510740394592326
-0.515625 0.0010372417756554322
-0.51625 0.0011288715983564408
-0.516875 0.001228458986778549
-0.5175 0.0013324966357592279
-0.518125 0.0014476878531161403
-0.51875 0.001573726741722439
-0.519375 0.0017074901424188784
-0.52 0.0018509716548233324
-0.520625 0.002003571724889444
-0.52125 0.0021710036927508132
-0.521875 0.002350257947202782
-0.5225 0.002537513261314711
-0.523125 0.002742744221606489
-0.52375 0.0029634306721944927
-0.524375 0.0031948211891328713
-0.525 0.0034497305812912758
-0.525625 0.0037127174347486953
-0.52625 0.003996776209011001
-0.526875 0.004306329401158012
-0.5275 0.004636727544954976
-0.528125 0.004974916956894759
-0.52875 0.0053494555461348434
-0.529375 0.0057449170021668374
-0.53 0.0061600165320804265
-0.530625 0.006602136714874432
-0.53125 0.007074715821353832
-0.531875 0.00757725017658087
-0.5325 0.008107326150110887
-0.533125 0.008674608467026697
-0.53375 0.009278705482854624
-0.534375 0.00990370215246301
-0.535 0.010562762361882892
-0.535625 0.011280195692658278
-0.53625 0.012023880969087635
-0.536875 0.012807205347199329
-0.5375 0.013649099610475132
-0.538125 0.01451289560673514
-0.53875 0.015444756307365373
-0.539375 0.016404950058171806
-0.54 0.017397352487440745
-0.540625 0.018456245219565792
-0.54125 0.01957809658540908
-0.541875 0.02074730162554827
-0.5425 0.021963211005325237
-0.543125 0.023272193121942487
-0.54375 0.024626334889467204
-0.544375 0.026034299186995923
-0.545 0.027517692612794957
-0.545625 0.029017371612899866
-0.54625 0.030622984802615917
-0.546875 0.03233420430132301
-0.5475 0.03405743108738941
-0.548125 0.03585867279302183
-0.54875 0.03774770534034556
-0.549375 0.03974201856667357
-0.55 0.04181424255740529
-0.550625 0.04399397403482783
-0.55125 0.04614959033213925
-0.551875 0.04846768532630546
-0.5525 0.05081019403425558
-0.553125 0.053321535862460655
-0.55375 0.05592469388622718
-0.554375 0.0585631321394168
-0.555 0.06139450330901078
-0.555625 0.06426829111885679
-0.55625 0.06732516330762775
-0.556875 0.07038781473399147
-0.5575 0.0735128543742286
-0.558125 0.07669535952387273
-0.55875 0.08010773016633153
-0.559375 0.08348620180935093
-0.56 0.08706933745592393
-0.560625 0.0908252283097084
-0.56125 0.09465271020344303
-0.561875 0.09857171932855383
-0.5625 0.10245618604592098
-0.563125 0.10665947893898338
-0.56375 0.11089342695185414
-0.564375 0.11532527987180928
-0.565 0.11968370544745677
-0.565625 0.1240406585596782
-0.56625 0.12872588095553655
-0.566875 0.13362877928106542
-0.5675 0.13850191771593737
-0.568125 0.1434021256274226
-0.56875 0.14844486221085887
-0.569375 0.15360562046331155
-0.57 0.15899942191939256
-0.570625 0.16443590802079405
-0.57125 0.1698597301624021
-0.571875 0.17556366188324257
-0.5725 0.1813872499168257
-0.573125 0.18726506189542574
-0.57375 0.19285527023737714
-0.574375 0.19896480266453298
-0.575 0.20462991432995437
-0.575625 0.21064990904486233
-0.57625 0.21641477142260176
-0.576875 0.22277159517889877
-0.5775 0.22944121890003466
-0.578125 0.23555842559588894
-0.57875 0.24176449909307274
-0.579375 0.24817031742792342
-0.58 0.25479901086892615
-0.580625 0.2609266860323717
-0.58125 0.2676467100266296
-0.581875 0.2737909706063049
-0.5825 0.2805922947371339
-0.583125 0.287554448707881
-0.58375 0.2941442368906307
-0.584375 0.30119084064240603
-0.585 0.30763658714296693
-0.585625 0.3143201979046446
-0.58625 0.32128798468169306
-0.586875 0.3281947798849739
-0.5875 0.33499433947060564
-0.588125 0.34177420696742206
-0.58875 0.34885810679785584
-0.589375 0.35574957081069053
-0.59 0.362097408600469
-0.590625 0.36956031886147783
-0.59125 0.37617896921650346
-0.591875 0.3825914592437907
-0.5925 0.38965366515569877
-0.593125 0.39616401868105033
-0.59375 0.4024840322497757
-0.594375 0.4092493124045795
-0.595 0.4155958063863036
-0.595625 0.4220269659368924
-0.59625 0.4287099383723663
-0.596875 0.43455694292398256
-0.5975 0.4409986550820377
-0.598125 0.4471869974305224
-0.59875 0.4526722161484304
-0.599375 0.45797882001753526
-0.6 0.46453780434944836
-0.600625 0.4696969731861818
-0.60125 0.47456952173899725
-0.601875 0.48011918793762376
-0.6025 0.4859409992349761
-0.603125 0.4898673252164567
-0.60375 0.49490941080584094
-0.604375 0.4992596549585261
-0.605 0.5035927054756096
-0.605625 0.5079251605330598
-0.60625 0.5127676007347914
-0.606875 0.5163523378910195
-0.6075 0.5210233193426403
-0.608125 0.5243922405562923
-0.60875 0.5274278402510381
-0.609375 0.5301938548965037
-0.61 0.534470858721525
-0.610625 0.5375398090799096
-0.61125 0.5401706723233108
-0.611875 0.5426619845782662
-0.6125 0.5450375011158821
-0.613125 0.547210945293706
-0.61375 0.5496905336388318
-0.614375 0.55131011578535
-0.615 0.5525963861097754
-0.615625 0.5543483488089246
-0.61625 0.5549312451066478
-0.616875 0.5555662731641774
-0.6175 0.5570008307601914
-0.618125 0.558167749254618
-0.61875 0.5592494973708199
-0.619375 0.5595355123879617
-0.62 0.5601915451672691
-0.620625 0.5599659983556688
-0.62125 0.5599181428069563
-0.621875 0.5595801600314744
-0.6225 0.5596558785632666
-0.623125 0.5589602451924743
-0.62375 0.5577538628630068
-0.624375 0.5564920962639435
-0.625 0.5554122176537718
-0.625625 0.5536253968658845
-0.62625 0.5528520251222608
-0.626875 0.5506669603103831
-0.6275 0.5484328619228865
-0.628125 0.546851982604282
-0.62875 0.5436922826902465
-0.629375 0.5420912508660679
-0.63 0.5396586241897631
-0.630625 0.5373467479825441
-0.63125 0.5341338573142231
-0.631875 0.5314506052029322
-0.6325 0.5284394004164253
-0.633125 0.5246960437438578
-0.63375 0.5210542379325583
-0.634375 0.5175311995033859
-0.635 0.5135475818827254
-0.635625 0.5099535331174576
-0.63625 0.5055394567169939
-0.636875 0.5010187958298541
-0.6375 0.4960584871908798
-0.638125 0.4907340441506326
-0.63875 0.48677680695361225
-0.639375 0.48210318642404604
-0.64 0.4774101432291198
-0.640625 0.47238891563092567
-0.64125 0.4680326108093963
-0.641875 0.4630056855146208
-0.6425 0.4585886247632253
-0.643125 0.45420486570974317
-0.64375 0.44917198937854813
-0.644375 0.4438921543091702
-0.645 0.43879766482497534
-0.645625 0.4339229987884668
-0.64625 0.4287626220686538
-0.646875 0.42351753626286637
-0.6475 0.41856803114683216
-0.648125 0.41292635257549787
-0.64875 0.40782543605286703
-0.649375 0.402444693939116
-0.65 0.39676148717543297
-0.650625 0.3911938129680744
-0.65125 0.3863188900777881
-0.651875 0.3808900110419305
-0.6525 0.3756630034534844
-0.653125 0.36998734658665433
-0.65375 0.3639389335891146
-0.654375 0.35822731149007386
-0.655 0.3529296126052396
-0.655625 0.3479415752441112
-0.65625 0.3431094157907517
-0.656875 0.3372402671948241
-0.6575 0.33176644047313425
-0.658125 0.3266538725970102
-0.65875 0.3204802562764495
-0.659375 0.3152573341246399
-0.66 0.309746128619112
-0.660625 0.30514981130447494
-0.66125 0.2994775920788232
-0.661875 0.294201807549774
-0.6625 0.28930537289494274
-0.663125 0.2837679575760733
-0.66375 0.2787738069905125
-0.664375 0.2736967036001768
-0.665 0.26855060837250716
-0.665625 0.26336291081369806
-0.66625 0.2584464229268485
-0.666875 0.2532721236919608
-0.6675 0.24867838464325992
-0.668125 0.24374479395993667
-0.66875 0.23909591095243327
-0.669375 0.23426233707052874
-0.67 0.2295098756198606
-0.670625 0.22472070704613692
-0.67125 0.22016061592949485
-0.671875 0.21526704933707458
-0.6725 0.21080824943182855
-0.673125 0.20613462480383654
-0.67375 0.20191769045850594
-0.674375 0.19769688388833725
-0.675 0.1932756518640657
-0.675625 0.1890493205283121
-0.67625 0.18509132145942178
-0.676875 0.18077579859357398
-0.6775 0.17714124875115217
-0.678125 0.1730969027602601
-0.67875 0.16915991008853198
-0.679375 0.1653728199021644
-0.68 0.16117018879091538
-0.680625 0.15745005496248923
-0.68125 0.153790173319427
-0.681875 0.1500395933370501
-0.6825 0.14669732830190663
-0.683125 0.1431335338466477
-0.68375 0.1396140572748736
-0.684375 0.13648147487965034
-0.685 0.13310916831206276
-0.685625 0.12988099964754368
-0.68625 0.12663158861644716
-0.686875 0.12356802483614454
-0.6875 0.1204873825445636
-0.688125 0.11731439857337886
-0.68875 0.11440831501579225
-0.689375 0.1116557706154713
-0.69 0.10878283664976961
-0.690625 0.10593889131353998
-0.69125 0.10322245547889153
-0.691875 0.10049041502528987
-0.6925 0.09801734762258162
-0.693125 0.09547140718324974
-0.69375 0.09296135379206279
-0.694375 0.09048257060971274
-0.695 0.08807574342077061
-0.695625 0.0857674965962244
-0.69625 0.08344417150849656
-0.696875 0.08119308132103109
-0.6975 0.0791320602826828
-0.698125 0.07692216299357628
-0.69875 0.07486354721837812
-0.699375 0.07289021683591221
-0.7 0.07107093735920884
-0.700625 0.06906629147262947
-0.70125 0.06721872525935323
-0.701875 0.06539405621040768
-0.7025 0.06372756849239067
-0.703125 0.06193915415374258
-0.70375 0.06026704542551988
-0.704375 0.05865898524489134
-0.705 0.056952983854999056
-0.705625 0.055377757609981856
-0.70625 0.05385679698877481
-0.706875 0.052377208212158195
-0.7075 0.050894796682215755
-0.708125 0.04944942503831782
-0.70875 0.048103364815800256
-0.709375 0.04674108887132586
-0.71 0.04547068713701014
-0.710625 0.044213104573647265
-0.71125 0.04292568274768489
-0.711875 0.041724108825345205
-0.7125 0.04054189076090527
-0.713125 0.03938647289170683
-0.71375 0.03822409812005427
-0.714375 0.037192566596237535
-0.715 0.0360653327554828
-0.715625 0.03503632644604807
-0.71625 0.0339925406822881
-0.716875 0.03307239311915192
-0.7175 0.03209872122879953
-0.718125 0.03115997682395896
-0.71875 0.03021195503107412
-0.719375 0.029383483972095243
-0.72 0.02856118707723768
-0.720625 0.027697515842603618
-0.72125 0.026864114333476276
-0.721875 0.026064042195788412
-0.7225 0.025289932230131342
-0.723125 0.024526157448120336
-0.72375 0.0238004104462392
-0.724375 0.02306903823641418
-0.725 0.022343673300408456
-0.725625 0.021706677166595696
-0.72625 0.021089500472308037
-0.726875 0.020447020448886057
-0.7275 0.0198719645010462
-0.728125 0.019257400663518283
-0.72875 0.018649363316285694
-0.729375 0.018102517961750747
-0.73 0.017573630376929134
-0.730625 0.017039657920539103
-0.73125 0.016522867183913627
-0.731875 0.0160039056224515
-0.7325 0.015529654813550238
-0.733125 0.015046533734417833
-0.73375 0.014598675549963663
-0.734375 0.014149945989462199
-0.735 0.013708077586171555
-0.735625 0.013295784818554028
-0.73625 0.012890510570138139
-0.736875 0.012500283101604068
-0.7375 0.012118429730855631
-0.738125 0.011757854249747901
-0.73875 0.01138945320068537
-0.739375 0.011052084347040202
-0.74 0.010714481070023905
-0.740625 0.010402859352673492
-0.74125 0.010092239232004065
-0.741875 0.009778451050683246
-0.7425 0.009485933156820245
-0.743125 0.009196613161755254
-0.74375 0.008931343497569175
-0.744375 0.008661063449545677
-0.745 0.008393631680791684
-0.745625 0.00813703062975408
-0.74625 0.007876639020896546
-0.746875 0.007637799149585037
-0.7475 0.007404013091111971
-0.748125 0.0071724409722470385
-0.74875 0.006956272667579306
-0.749375 0.006743918377115198
-0.75 0.006537621565723603
-0.750625 0.006337327037952505
-0.75125 0.006139660530486414
-0.751875 0.005943004511583824
-0.7525 0.005754334584696412
-0.753125 0.0055775795481245475
-0.75375 0.005407589240295626
-0.754375 0.005243501890627961
-0.755 0.005077847045272047
-0.755625 0.004926259264020244
-0.75625 0.00476634809637564
-0.756875 0.0046200322122016795
-0.7575 0.004478261620218159
-0.758125 0.004340801017464531
-0.75875 0.004210778037842225
-0.759375 0.004076886647489029
-0.76 0.003952117254297891
-0.760625 0.0038293459256591366
-0.76125 0.003709851637779959
-0.761875 0.003598537382417855
-0.7625 0.0034906954590186116
-0.763125 0.003381060467083548
-0.76375 0.0032848899833066206
-0.764375 0.0031881479809835406
-0.765 0.003090598797628059
-0.765625 0.0029947914115692493
-0.76625 0.00290557972739925
-0.766875 0.0028159480255085362
-0.7675 0.002731456392903505
-0.768125 0.002651632809234493
-0.76875 0.002572340024180595
-0.769375 0.0024947935821796356
-0.77 0.0024180981799429876
-0.770625 0.0023449372018108836
-0.77125 0.0022748509325207283
-0.771875 0.0022094627054267714
-0.7725 0.002141699393630659
-0.773125 0.002077281116199192
-0.77375 0.002014472511374412
-0.774375 0.0019577686378284857
-0.775 0.0018987935409498623
-0.775625 0.0018419873902571146
-0.77625 0.0017839275676003429
-0.776875 0.001731054495827591
-0.7775 0.0016818654691500496
-0.778125 0.0016291886956173525
-0.77875 0.001583008591104826
-0.779375 0.0015365618021212855
-0.78 0.0014909498288527131
-0.780625 0.0014481453619775981
-0.78125 0.0014053196960287847
-0.781875 0.0013650347293008647
-0.7825 0.0013258302746492808
-0.783125 0.0012875978771615267
-0.78375 0.001250427965451446
-0.784375 0.0012142739675118396
-0.785 0.0011798018847099035
-0.785625 0.0011438936541327415
-0.78625 0.0011131219529724888
-0.786875 0.001080303169281824
-0.7875 0.0010499000247301974
-0.788125 0.0010203997327947949
-0.78875 0.000992913496347356
-0.789375 0.0009649548446910685
-0.79 0.0009377833871712065
-0.790625 0.0009109688159511003
-0.79125 0.0008855690376800494
-0.791875 0.0008606543811143348
-0.7925 0.0008362716296874661
-0.793125 0.0008120414660025987
-0.79375 0.000789851361892227
-0.794375 0.0007685449216420132
-0.795 0.000747358449181795
-0.795625 0.0007262094235531917
-0.79625 0.0007062247185418902
-0.796875 0.0006874635025798337
-0.7975 0.0006678618018808026
-0.798125 0.0006497595429277711
-0.79875 0.0006313534406862237
-0.799375 0.0006146107552673818
-0.8 0.0005979874236831169
-0.800625 0.0005814496957140289
-0.80125 0.0005659428471359876
-0.801875 0.0005501738210331329
-0.8025 0.000536190806994971
-0.803125 0.0005214830867831183
-0.80375 0.0005078752260574866
-0.804375 0.0004941002383865471
-0.805 0.00048056098281804883
-0.805625 0.000468769594128516
-0.80625 0.0004563293328470712
-0.806875 0.00044446389882891855
-0.8075 0.00043295347935722896
-0.808125 0.0004214710764062407
-0.80875 0.00041049824225146127
-0.809375 0.00039964971500526677
-0.81 0.00038913001421254283
-0.810625 0.0003792437956489069
-0.81125 0.00036905340553141313
-0.811875 0.00035973192936276157
-0.8125 0.0003500492631626622
-0.813125 0.00034096446123288297
-0.81375 0.0003313915281619879
-0.814375 0.00032277286294888166
-0.815 0.00031429666155426746
-0.815625 0.00030632082922133413
-0.81625 0.00029810778416970447
-0.816875 0.00029028814050566356
-0.8175 0.0002828868583684988
-0.818125 0.0002757762294628793
-0.81875 0.000268962207231983
-0.819375 0.00026215641798952395
-0.82 0.00025539842730523107
-0.820625 0.0002489625014133231
-0.82125 0.00024302105897411685
-0.821875 0.0002368170330153587
-0.8225 0.0002308455550150621
-0.823125 0.00022499755108953357
-0.82375 0.0002194109255404359
-0.824375 0.00021337487605072893
-0.825 0.00020812174759048143
-0.825625 0.0002031024342373825
-0.82625 0.00019781174842045546
-0.826875 0.0001928224228033093
-0.8275 0.00018788290191431006
-0.828125 0.00018321715423604877
-0.82875 0.0001787686852260144
-0.829375 0.00017438702459030817
-0.83 0.00017027125485907845
-0.830625 0.00016600888051362866
-0.83125 0.00016189065393858285
-0.831875 0.0001581128431535458
-0.8325 0.00015416496830769204
-0.833125 0.0001505050926479999
-0.83375 0.00014705152442002123
-0.834375 0.00014355564083707572
-0.835 0.00014018286882839538
-0.835625 0.00013681480643917384
-0.83625 0.00013365981635465713
-0.836875 0.00013031183259693208
-0.8375 0.00012746588605146318
-0.838125 0.00012464341733550756
-0.83875 0.00012150559365633137
-0.839375 0.00011862861431765925
-0.84 0.00011593898465077239
-0.840625 0.00011319551059964286
-0.84125 0.0001106421867743334
-0.841875 0.00010814731638083797
-0.8425 0.00010546536648662785
-0.843125 0.00010293263758047695
-0.84375 0.00010054224410623669
-0.844375 9.819127331242602e-05
-0.845 9.605870853513178e-05
-0.845625 9.370285218152721e-05
-0.84625 9.163142236922354e-05
-0.846875 8.940384812206071e-05
-0.8475 8.73865521195415e-05
-0.848125 8.529612997310749e-05
-0.84875 8.329597114212922e-05
-0.849375 8.141355122664908e-05
-0.85 7.954381704460009e-05
-0.850625 7.788766783795397e-05
-0.85125 7.603468968083956e-05
-0.851875 7.424793390758605e-05
-0.8525 7.257961339836347e-05
-0.853125 7.10164156184062e-05
-0.85375 6.933846290973396e-05
-0.854375 6.79089594298139e-05
-0.855 6.641233703640166e-05
-0.855625 6.493523486126305e-05
-0.85625 6.340776530589477e-05
-0.856875 6.21255647035379e-05
-0.8575 6.070189997996383e-05
-0.858125 5.938885015240798e-05
-0.85875 5.8089201139942625e-05
-0.859375 5.6739123394546635e-05
-0.86 5.552031646339149e-05
-0.860625 5.4295893254850954e-05
-0.86125 5.313592145377797e-05
-0.861875 5.196317966502833e-05
-0.8625 5.0756692000988683e-05
-0.863125 4.967068156455779e-05
-0.86375 4.857588644856726e-05
-0.864375 4.757937877234476e-05
-0.865 4.660727348029371e-05
-0.865625 4.559905033068506e-05
-0.86625 4.4620828427248624e-05
-0.866875 4.375019269358138e-05
-0.8675 4.279326633606011e-05
-0.868125 4.191262027105008e-05
-0.86875 4.101211586009769e-05
-0.869375 4.013472934824437e-05
-0.87 3.9312450536116544e-05
-0.870625 3.855133507619071e-05
-0.87125 3.767381889814684e-05
-0.871875 3.6916845372398417e-05
-0.8725 3.610059433482456e-05
-0.873125 3.534302036176377e-05
-0.87375 3.4609808682315895e-05
-0.874375 3.389892587762644e-05
-0.875 3.318735500889817e-05
-0.875625 3.255996552934212e-05
-0.87625 3.192251662517724e-05
-0.876875 3.12029194828342e-05
-0.8775 3.0575939792028694e-05
-0.878125 3.0010919390306852e-05
-0.87875 2.937542136363062e-05
-0.879375 2.878804331292188e-05
-0.88 2.821172925616326e-05
-0.880625 2.7664147218447612e-05
-0.88125 2.7084594518013467e-05
-0.881875 2.6525507435911684e-05
-0.8825 2.5988269757196357e-05
-0.883125 2.5460362690375366e-05
-0.88375 2.4979520158906645e-05
-0.884375 2.4457139924305547e-05
-0.885 2.399607245711986e-05
-0.885625 2.3495069011264955e-05
-0.88625 2.300381259904359e-05
-0.886875 2.2581934357926085e-05
-0.8875 2.212663333365582e-05
-0.888125 2.166951043283645e-05
-0.88875 2.1273556070696367e-05
-0.889375 2.0882757227642326e-05
-0.89 2.048528667102426e-05
-0.890625 2.0060570593124203e-05
-0.89125 1.968389331172908e-05
-0.891875 1.927613741858046e-05
-0.8925 1.8908552687154305e-05
-0.893125 1.8546967536254923e-05
-0.89375 1.8188355001248757e-05
-0.894375 1.7864265367143743e-05
-0.895 1.7518348961587895e-05
-0.895625 1.7181911632327363e-05
-0.89625 1.681684815940867e-05
-0.896875 1.649411643343272e-05
-0.8975 1.6177587625346244e-05
-0.898125 1.588283850018684e-05
-0.89875 1.5578157629162648e-05
-0.899375 1.5307401607688167e-05
-0.9 1.5045120076040242e-05
-0.900625 1.475149102699639e-05
-0.90125 1.4475263130459544e-05
-0.901875 1.4204779749398076e-05
-0.9025 1.3929823084753171e-05
-0.903125 1.3651926121417675e-05
-0.90375 1.3407105817659918e-05
-0.904375 1.3145215067827403e-05
-0.905 1.2912461939845641e-05
-0.905625 1.2663953122171097e-05
-0.90625 1.2438783676962538e-05
-0.906875 1.2209769814459221e-05
-0.9075 1.1964182091256721e-05
-0.908125 1.1761184209173812e-05
-0.90875 1.1566746594774626e-05
-0.909375 1.137526152168562e-05
-0.91 1.1178808917551372e-05
-0.910625 1.0978752902139968e-05
-0.91125 1.0803687825730867e-05
-0.911875 1.0599549038508969e-05
-0.9125 1.0410906361966754e-05
-0.913125 1.0226352080932251e-05
-0.91375 1.0054695782939418e-05
-0.914375 9.88032837329497e-06
-0.915 9.72718413349138e-06
-0.915625 9.550578024964058e-06
-0.91625 9.384511258809153e-06
-0.916875 9.214724700722221e-06
-0.9175 9.058409856667375e-06
-0.918125 8.911212496731708e-06
-0.91875 8.76088985816069e-06
-0.919375 8.610730483837153e-06
-0.92 8.463124216073733e-06
-0.920625 8.31457724901401e-06
-0.92125 8.18291739010605e-06
-0.921875 8.049285451853077e-06
-0.9225 7.914764385629156e-06
-0.923125 7.78554061791351e-06
-0.92375 7.651827176056356e-06
-0.924375 7.5189343529997685e-06
-0.925 7.385262797387841e-06
-0.925625 7.2713809169758685e-06
-0.92625 7.1600231215965394e-06
-0.926875 7.037538142007927e-06
-0.9275 6.917421028941584e-06
-0.928125 6.799164818892265e-06
-0.92875 6.686468018049463e-06
-0.929375 6.576462548839133e-06
-0.93 6.469600444909209e-06
-0.930625 6.353319592499036e-06
-0.93125 6.254079740533255e-06
-0.931875 6.1540999531657874e-06
-0.9325 6.052349865546538e-06
-0.933125 5.959390869544343e-06
-0.93375 5.8518282074673606e-06
-0.934375 5.7690455179091094e-06
-0.935 5.6847652834138134e-06
-0.935625 5.592521793508717e-06
-0.93625 5.512309939042497e-06
-0.936875 5.425709455901928e-06
-0.9375 5.343575544462624e-06
-0.938125 5.265175563153743e-06
-0.93875 5.184390913457586e-06
-0.939375 5.105893447061866e-06
-0.94 5.02231286869698e-06
-0.940625 4.941135473847037e-06
-0.94125 4.867788052667974e-06
-0.941875 4.8020555923184725e-06
-0.9425 4.735263993398565e-06
-0.943125 4.661507379586268e-06
-0.94375 4.591089022858389e-06
-0.944375 4.5163478869559145e-06
-0.945 4.4494193070849514e-06
-0.945625 4.380553601021437e-06
-0.94625 4.3115383048754875e-06
-0.946875 4.246990584827882e-06
-0.9475 4.186540812780161e-06
-0.948125 4.1290404005092e-06
-0.94875 4.069067964817036e-06
-0.949375 4.005689189043366e-06
-0.95 3.9501515620119094e-06
-0.950625 3.890978702762772e-06
-0.95125 3.837082589781017e-06
-0.951875 3.784201339739413e-06
-0.9525 3.7283191579177677e-06
-0.953125 3.6790005098812322e-06
-0.95375 3.6238276791603832e-06
-0.954375 3.573428180411985e-06
-0.955 3.5246359259551735e-06
-0.955625 3.4762316795962537e-06
-0.95625 3.4322429067369317e-06
-0.956875 3.3847811768453186e-06
-0.9575 3.341425837414498e-06
-0.958125 3.298679802751044e-06
-0.95875 3.2481090218023997e-06
-0.959375 3.205417510773386e-06
-0.96 3.1643163749603344e-06
-0.960625 3.1200862490132095e-06
-0.96125 3.080139840130958e-06
-0.961875 3.03706328231282e-06
-0.9625 2.9966088276959305e-06
-0.963125 2.9545170585047402e-06
-0.96375 2.9153017018637254e-06
-0.964375 2.8772604600981543e-06
-0.965 2.8430294464086807e-06
-0.965625 2.8078991463483426e-06
-0.96625 2.7768464488207594e-06
-0.966875 2.741266647527556e-06
-0.9675 2.707282500689158e-06
-0.968125 2.674774391125366e-06
-0.96875 2.6389342216626057e-06
-0.969375 2.6092350975893364e-06
-0.97 2.57802210434629e-06
-0.970625 2.5431455831415732e-06
-0.97125 2.5136172280461372e-06
-0.971875 2.4840318149379825e-06
-0.9725 2.4531701347136244e-06
-0.973125 2.42284629845386e-06
-0.97375 2.3962649275533266e-06
-0.974375 2.365277028181028e-06
-0.975 2.339386285008999e-06
-0.975625 2.3112339996981137e-06
-0.97625 2.2872819706750973e-06
-0.976875 2.2630211807744748e-06
-0.9775 2.2363881270244785e-06
-0.978125 2.211141075339224e-06
-0.97875 2.187324580025785e-06
-0.979375 2.1640989014267906e-06
-0.98 2.139512674651292e-06
-0.980625 2.1151168731782462e-06
-0.98125 2.094449690581166e-06
-0.981875 2.072853657023722e-06
-0.9825 2.048554528891778e-06
-0.983125 2.026539520826603e-06
-0.98375 2.0065181599088084e-06
-0.984375 1.9870348481914235e-06
-0.985 1.964456141676096e-06
-0.985625 1.942567513191194e-06
-0.98625 1.9228491604879774e-06
-0.986875 1.8994952768191687e-06
-0.9875 1.8784500458934942e-06
-0.988125 1.8626904477230946e-06
-0.98875 1.8398226202277816e-06
-0.989375 1.8233751767569325e-06
-0.99 1.8070387672339854e-06
-0.990625 1.7917381636435648e-06
-0.99125 1.7732988335168592e-06
-0.991875 1.759972741218098e-06
-0.9925 1.7409198157944696e-06
-0.993125 1.7242639071501567e-06
-0.99375 1.7084811506574588e-06
-0.994375 1.6914538450882587e-06
-0.995 1.6777140028770014e-06
-0.995625 1.6621072378174321e-06
-0.99625 1.6465248886797794e-06
-0.996875 1.6305682007595247e-06
-0.9975 1.617574132192351e-06
-0.998125 1.6059308401255138e-06
-0.99875 1.5903103543441574e-06
-0.999375 1.5782453394509347e-06
-1.0 1.5626600923108354e-06
-1.000625 1.549010074800797e-06
-1.00125 1.5369609485247997e-06
-1.001875 1.524125674335013e-06
-1.0025 1.510420780272739e-06
-1.003125 1.500190505003795e-06
-1.00375 1.4881907909752795e-06
-1.004375 1.4774185287253718e-06
-1.005 1.46437663755296e-06
-1.005625 1.4551193535008964e-06
-1.00625 1.4456773769471258e-06
-1.006875 1.4336132568332074e-06
-1.0075 1.423644793848525e-06
-1.008125 1.4127026734705993e-06
-1.00875 1.4025648358917022e-06
-1.009375 1.3925027402258834e-06
-1.01 1.383393123863707e-06
-1.010625 1.372946392485669e-06
-1.01125 1.3632571430869426e-06
-1.011875 1.3555347305639833e-06
-1.0125 1.3450250052909664e-06
-1.013125 1.3360695179237016e-06
-1.01375 1.3290896731819275e-06
-1.014375 1.3208183092247068e-06
-1.015 1.3109106623246099e-06
-1.015625 1.3024869864318202e-06
-1.01625 1.2940808043568898e-06
-1.016875 1.2844093927033195e-06
-1.0175 1.277393869860335e-06
-1.018125 1.2696274931921987e-06
-1.01875 1.263081938002589e-06
-1.019375 1.254416260700625e-06
-1.02 1.2489332081905392e-06
-1.020625 1.2430076123013109e-06
-1.02125 1.2345868434840777e-06
-1.021875 1.2264234825956826e-06
-1.0225 1.2204964358187038e-06
-1.023125 1.2141516478829753e-06
-1.02375 1.2093060481361755e-06
-1.024375 1.2000295191374146e-06
-1.025 1.194618362149551e-06
-1.025625 1.187071906010794e-06
-1.02625 1.1802203059815172e-06
-1.026875 1.1735575315075708e-06
-1.0275 1.167483050054487e-06
-1.028125 1.1603320395814119e-06
-1.02875 1.1546155173503927e-06
-1.029375 1.1483936427305014e-06
-1.03 1.141800633566508e-06
-1.030625 1.1360679618566831e-06
-1.03125 1.1290373972998396e-06
-1.031875 1.1236230923735268e-06
-1.0325 1.115975097414503e-06
-1.033125 1.1110960856679513e-06
-1.03375 1.1067231927251974e-06
-1.034375 1.1002563301421123e-06
-1.035 1.0940243346536314e-06
-1.035625 1.0902577636794432e-06
-1.03625 1.0849454501457596e-06
-1.036875 1.080283601053315e-06
-1.0375 1.0770366460196465e-06
-1.038125 1.072539025929294e-06
-1.03875 1.068588399660417e-06
-1.039375 1.0667689184052293e-06
-1.04 1.0626421199085595e-06
-1.040625 1.0591502279156673e-06
-1.04125 1.0556702949565083e-06
-1.041875 1.0503793963594098e-06
-1.0425 1.0467751347090872e-06
-1.043125 1.0420334169691645e-06
-1.04375 1.0366959903256344e-06
-1.044375 1.0335042646543132e-06
-1.045 1.028380855410646e-06
-1.045625 1.0244980691098201e-06
-1.04625 1.0211891082068314e-06
-1.046875 1.0147917535340298e-06
-1.0475 1.0118804933804182e-06
-1.048125 1.0068114345531373e-06
-1.04875 1.0032684752472348e-06
-1.049375 9.993788418518845e-07
-1.05 9.956522742298425e-07
-1.050625 9.91871433937794e-07
-1.05125 9.88273319192622e-07
-1.051875 9.857377024735879e-07
-1.0525 9.832437652688e-07
-1.053125 9.792815325956103e-07
-1.05375 9.772947093671167e-07
-1.054375 9.739149725725811e-07
-1.055 9.689672360902782e-07
-1.055625 9.67033807366897e-07
-1.05625 9.63456252251979e-07
-1.056875 9.601668820936974e-07
-1.0575 9.590296926925847e-07
-1.058125 9.549405793745102e-07
-1.05875 9.51365305011164e-07
-1.059375 9.483190572937151e-07
-1.06 9.459513612014108e-07
-1.060625 9.451855937330017e-07
-1.06125 9.428445672665014e-07
-1.061875 9.410467280265664e-07
-1.0625 9.395349719330356e-07
-1.063125 9.359470007556611e-07
-1.06375 9.341115985777242e-07
-1.064375 9.319324838317322e-07
-1.065 9.282996255796325e-07
-1.065625 9.260440828548903e-07
-1.06625 9.227612609896002e-07
-1.066875 9.211210582084338e-07
-1.0675 9.205844501544954e-07
-1.068125 9.175027328119841e-07
-1.06875 9.152132382978809e-07
-1.069375 9.128257049700341e-07
-1.07 9.117149670063312e-07
-1.070625 9.100610636736045e-07
-1.07125 9.091190334035327e-07
-1.071875 9.07810736844485e-07
-1.0725 9.056931904732352e-07
-1.073125 9.02962069350904e-07
-1.07375 9.007813756035863e-07
-1.074375 8.999981237313125e-07
-1.075 8.979110995035954e-07
-1.075625 8.970698669378164e-07
-1.07625 8.960445062265695e-07
-1.076875 8.938760251186702e-07
-1.0775 8.931399167851039e-07
-1.078125 8.907831161251611e-07
-1.07875 8.887021493636465e-07
-1.079375 8.877072048957853e-07
-1.08 8.863840838185067e-07
-1.080625 8.842716261714228e-07
-1.08125 8.827182347539517e-07
-1.081875 8.807809556722708e-07
-1.0825 8.789340641191811e-07
-1.083125 8.772043945614038e-07
-1.08375 8.753163988338298e-07
-1.084375 8.745004087171354e-07
-1.085 8.73710884933835e-07
-1.085625 8.725734355296319e-07
-1.08625 8.693205090425315e-07
-1.086875 8.681719455535278e-07
-1.0875 8.658336517833676e-07
-1.088125 8.648110213964722e-07
-1.08875 8.637948831203479e-07
-1.089375 8.621537081552182e-07
-1.09 8.614332814593402e-07
-1.090625 8.605782579034914e-07
-1.09125 8.591228807322114e-07
-1.091875 8.569264250893052e-07
-1.0925 8.54295492605658e-07
-1.093125 8.533214689072946e-07
-1.09375 8.5181609121747e-07
-1.094375 8.507548275809017e-07
-1.095 8.488883013268053e-07
-1.095625 8.477210943532921e-07
-1.09625 8.472412117606002e-07
-1.096875 8.475611439658951e-07
-1.0975 8.470813120436027e-07
-1.098125 8.460716585583031e-07
-1.09875 8.45434333878471e-07
-1.099375 8.442188858201858e-07
-1.1 8.423468289993332e-07
-1.100625 8.421837577323892e-07
-1.10125 8.405770867670973e-07
-1.101875 8.391631798907065e-07
-1.1025 8.391897233877739e-07
-1.103125 8.389892608032379e-07
-1.10375 8.372698616415288e-07
-1.104375 8.37111774273707e-07
-1.105 8.361240933392666e-07
-1.105625 8.359661228127954e-07
-1.10625 8.344475760977985e-07
-1.106875 8.32921891839448e-07
-1.1075 8.335622850769105e-07
-1.108125 8.330382965202268e-07
-1.10875 8.33297501184489e-07
-1.109375 8.328220360656071e-07
-1.11 8.310689933310126e-07
-1.110625 8.294264383924208e-07
-1.11125 8.307614331070891e-07
-1.111875 8.300539109679912e-07
-1.1125 8.283057940302429e-07
-1.113125 8.276615794839325e-07
-1.11375 8.283330972447643e-07
-1.114375 8.275231379114381e-07
-1.115 8.263891242762937e-07
-1.115625 8.259389512233843e-07
-1.11625 8.261049112112664e-07
-1.116875 8.26505134772417e-07
-1.1175 8.250073825707084e-07
-1.118125 8.261264940382838e-07
-1.11875 8.267469147497403e-07
-1.119375 8.273153923968693e-07
-1.12 8.265955832072893e-07
-1.120625 8.267783934962494e-07
-1.12125 8.256259559569193e-07
-1.121875 8.267264279444393e-07
-1.1225 8.263637103360864e-07
-1.123125 8.275822710712353e-07
-1.12375 8.268417585922965e-07
-1.124375 8.263694029816864e-07
-1.125 8.267790898554058e-07
-1.125625 8.272317856579786e-07
-1.12625 8.279245796106712e-07
-1.126875 8.281774680692185e-07
-1.1275 8.277662792561972e-07
-1.128125 8.270255259918485e-07
-1.12875 8.276893253558235e-07
-1.129375 8.267720175018684e-07
-1.13 8.267567079202788e-07
-1.130625 8.27234387330059e-07
-1.13125 8.269122993873942e-07
-1.131875 8.260830773751863e-07
-1.1325 8.269684148454676e-07
-1.133125 8.258513309890835e-07
-1.13375 8.255431377592399e-07
-1.134375 8.243996366205137e-07
-1.135 8.248151614194961e-07
-1.135625 8.237334717261111e-07
-1.13625 8.238962307740577e-07
-1.136875 8.231925367967657e-07
-1.1375 8.236328818286472e-07
-1.138125 8.237991380582241e-07
-1.13875 8.251985340590369e-07
-1.139375 8.246430813147552e-07
-1.14 8.228612316748268e-07
-1.140625 8.232703536785239e-07
-1.14125 8.228146853979754e-07
-1.141875 8.230982206169396e-07
-1.1425 8.237705367511917e-07
-1.143125 8.250727680482845e-07
-1.14375 8.253712565991636e-07
-1.144375 8.242962111342047e-07
-1.145 8.243698103779915e-07
-1.145625 8.239667686314417e-07
-1.14625 8.23636652804482e-07
-1.146875 8.224479780278659e-07
-1.1475 8.219156780888208e-07
-1.148125 8.213837237674339e-07
-1.14875 8.207653424241057e-07
-1.149375 8.197645507534847e-07
-1.15 8.201889278313598e-07
-1.150625 8.205566299693117e-07
-1.15125 8.215930950493979e-07
-1.151875 8.211621729211845e-07
-1.1525 8.2124739468276e-07
-1.153125 8.207523070486017e-07
-1.15375 8.212751498778556e-07
-1.154375 8.205587956374022e-07
-1.155 8.208118909437547e-07
-1.155625 8.202593974577618e-07
-1.15625 8.202656120051568e-07
-1.156875 8.199506648560909e-07
-1.1575 8.196966043675996e-07
-1.158125 8.203065824690814e-07
-1.15875 8.203519547845739e-07
-1.159375 8.201196684377465e-07
-1.16 8.213807645456399e-07
-1.160625 8.218384488857993e-07
-1.16125 8.223951638100911e-07
-1.161875 8.219911414051446e-07
-1.1625 8.219214609555193e-07
-1.163125 8.216241625243834e-07
-1.16375 8.214559125930287e-07
-1.164375 8.225625551479753e-07
-1.165 8.220691102224426e-07
-1.165625 8.228117098577854e-07
-1.16625 8.229443344239829e-07
-1.166875 8.231974122845887e-07
-1.1675 8.243811743860645e-07
-1.168125 8.245362299754259e-07
-1.16875 8.241751009438659e-07
-1.169375 8.261266742732299e-07
-1.17 8.257088415378079e-07
-1.170625 8.258206930651957e-07
-1.17125 8.267033938443973e-07
-1.171875 8.261092837637912e-07
-1.1725 8.260605574485705e-07
-1.173125 8.266716000035647e-07
-1.17375 8.275734106310928e-07
-1.174375 8.27332236001868e-07
-1.175 8.26635212613641e-07
-1.175625 8.260605666031331e-07
-1.17625 8.256461203491224e-07
-1.176875 8.247859159625362e-07
-1.1775 8.262665624001101e-07
-1.178125 8.249245722812788e-07
-1.17875 8.250572717921857e-07
-1.179375 8.250722442517223e-07
-1.18 8.251810523305887e-07
-1.180625 8.250305402426249e-07
-1.18125 8.261582494731224e-07
-1.181875 8.266378961354676e-07
-1.1825 8.269978757125528e-07
-1.183125 8.271658849592658e-07
-1.18375 8.276937836852296e-07
-1.184375 8.281431876203904e-07
-1.185 8.281927486030413e-07
-1.185625 8.28648907946138e-07
-1.18625 8.284202926058307e-07
-1.186875 8.292913038444904e-07
-1.1875 8.304581780583955e-07
-1.188125 8.311900877572612e-07
-1.18875 8.319104828319504e-07
-1.189375 8.325783990917527e-07
-1.19 8.338613906949095e-07
-1.190625 8.34711677879912e-07
-1.19125 8.348540335442928e-07
-1.191875 8.352109430893638e-07
-1.1925 8.366960587333015e-07
-1.193125 8.367677145100979e-07
-1.19375 8.394887596880301e-07
-1.194375 8.390556647615479e-07
-1.195 8.404054708867728e-07
-1.195625 8.414519481736013e-07
-1.19625 8.411942427566484e-07
-1.196875 8.415822444684445e-07
-1.1975 8.43143433295306e-07
-1.198125 8.43199700518173e-07
-1.19875 8.445589269522318e-07
-1.199375 8.456725311855786e-07
-1.2 8.47046503175214e-07
-1.200625 8.475390747483339e-07
-1.20125 8.486731858970059e-07
-1.201875 8.479213300996483e-07
-1.2025 8.488028125699824e-07
-1.203125 8.487873954534404e-07
-1.20375 8.499742399796544e-07
-1.204375 8.506626978833876e-07
-1.205 8.532465326101673e-07
-1.205625 8.527227759184646e-07
-1.20625 8.541021681748937e-07
-1.206875 8.559650477046383e-07
-1.2075 8.57416332785821e-07
-1.208125 8.599676047114314e-07
-1.20875 8.611426900297212e-07
-1.209375 8.634205594363413e-07
-1.21 8.627892588989599e-07
-1.210625 8.631690365952913e-07
-1.21125 8.647904053286548e-07
-1.211875 8.662875247554924e-07
-1.2125 8.677172905861549e-07
-1.213125 8.695853156092097e-07
-1.21375 8.706404872102516e-07
-1.214375 8.713675798325585e-07
-1.215 8.726432802416708e-07
-1.215625 8.733346729648804e-07
-1.21625 8.739083729147315e-07
-1.216875 8.759349727903014e-07
-1.2175 8.769671942837421e-07
-1.218125 8.794746501391269e-07
-1.21875 8.804623184188188e-07
-1.219375 8.825019644596855e-07
-1.22 8.843940009301136e-07
-1.220625 8.867707575679384e-07
-1.22125 8.893519050539155e-07
-1.221875 8.90487522003885e-07
-1.2225 8.918053652897403e-07
-1.223125 8.943765544343343e-07
-1.22375 8.955687427761029e-07
-1.224375 8.977996970950425e-07
-1.225 8.99398594637711e-07
-1.225625 8.99856576730293e-07
-1.22625 9.021175960216952e-07
-1.226875 9.045534631978431e-07
-1.2275 9.065090241348523e-07
-1.228125 9.067033800070842e-07
-1.22875 9.073172978241714e-07
-1.229375 9.094693814063645e-07
-1.23 9.121442163028259e-07
-1.230625 9.131977246211018e-07
-1.23125 9.149034355225364e-07
-1.231875 9.150723529620902e-07
-1.2325 9.189042248061098e-07
-1.233125 9.207731903673083e-07
-1.23375 9.235359771237888e-07
-1.234375 9.244418233933331e-07
-1.235 9.26878752974117e-07
-1.235625 9.28998473581863e-07
-1.23625 9.300684419095059e-07
-1.236875 9.327475479723538e-07
-1.2375 9.34445740278164e-07
-1.238125 9.362516465692667e-07
-1.23875 9.376158327980458e-07
-1.239375 9.394812188572988e-07
-1.24 9.432947390896592e-07
-1.240625 9.459358198592934e-07
-1.24125 9.472403625033864e-07
-1.241875 9.488823017398463e-07
-1.2425 9.520425405985708e-07
-1.243125 9.533944230916919e-07
-1.24375 9.56227312647473e-07
-1.244375 9.575025867644762e-07
-1.245 9.602211939872724e-07
-1.245625 9.61807722160537e-07
-1.24625 9.645211441113983e-07
-1.246875 9.66823459783784e-07
-1.2475 9.697245791285564e-07
-1.248125 9.717622022995113e-07
-1.24875 9.743409985590112e-07
-1.249375 9.755196412526373e-07
-1.25 9.772966235095425e-07
-1.250625 9.806764060759608e-07
-1.25125 9.831380809274054e-07
-1.251875 9.857369354104141e-07
-1.2525 9.89018647524665e-07
-1.253125 9.908015608761822e-07
-1.25375 9.938364629230049e-07
-1.254375 9.970571507935284e-07
-1.255 9.982840312125583e-07
-1.255625 9.998499297658161e-07
-1.25625 1.0016786933289935e-06
-1.256875 1.0044701518694996e-06
-1.2575 1.0072031531398866e-06
-1.258125 1.0123535223126678e-06
-1.25875 1.0140445919442037e-06
-1.259375 1.0163563459555832e-06
-1.26 1.0190997525181585e-06
-1.260625 1.0224956494356574e-06
-1.26125 1.0262961258794777e-06
-1.261875 1.0284910484140093e-06
-1.2625 1.0307668683397238e-06
-1.263125 1.0333855372856363e-06
-1.26375 1.0359587729130395e-06
-1.264375 1.0397439227284878e-06
-1.265 1.044084386031055e-06
-1.265625 1.0484319400886388e-06
-1.26625 1.0506149430308068e-06
-1.266875 1.0521016789513406e-06
-1.2675 1.0569161452463778e-06
-1.268125 1.0608468708805116e-06
-1.26875 1.0641241451573888e-06
-1.269375 1.0686965749520795e-06
-1.27 1.0702912145852085e-06
-1.270625 1.0756234573034498e-06
-1.27125 1.0806751674855183e-06
-1.271875 1.0833669951750265e-06
-1.2725 1.0877137703016652e-06
-1.273125 1.093863975366642e-06
-1.27375 1.0972659547741854e-06
-1.274375 1.0996441532034901e-06
-1.275 1.1034448628781241e-06
-1.275625 1.1099182469271526e-06
-1.27625 1.1145766602219776e-06
-1.276875 1.1180871162113313e-06
-1.2775 1.122431335066896e-06
-1.278125 1.1267686264899144e-06
-1.27875 1.1341019701352487e-06
-1.279375 1.1376508484586143e-06
-1.28 1.1437299460729096e-06
-1.280625 1.1479466279819042e-06
-1.28125 1.1541028657015838e-06
-1.281875 1.1580202261894974e-06
-1.2825 1.1630062111951014e-06
-1.283125 1.1690706180835845e-06
-1.28375 1.174201055481767e-06
-1.284375 1.1794400102639395e-06
-1.285 1.186231020027158e-06
-1.285625 1.191517761561827e-06
-1.28625 1.1978792275157939e-06
-1.286875 1.2025584152954794e-06
-1.2875 1.208962960765026e-06
-1.288125 1.2142653087420471e-06
-1.28875 1.2199909519575185e-06
-1.289375 1.2255305705682567e-06
-1.29 1.2321536676828894e-06
-1.290625 1.2379091595151745e-06
-1.29125 1.2447619113978316e-06
-1.291875 1.253245876638978e-06
-1.2925 1.2566196586899296e-06
-1.293125 1.262284257009992e-06
-1.29375 1.2695705336072413e-06
-1.294375 1.2767674096079385e-06
-1.295 1.283144187895908e-06
-1.295625 1.2900193962513701e-06
-1.29625 1.2987548919471394e-06
-1.296875 1.3073381558672484e-06
-1.2975 1.3143459830561885e-06
-1.298125 1.322002500886484e-06
-1.29875 1.3284371269535423e-06
-1.299375 1.3335622872147302e-06
-1.3 1.340944204314134e-06
-1.300625 1.3493544680062487e-06
-1.30125 1.3588251301739627e-06
-1.301875 1.3681005402606154e-06
-1.3025 1.3766971442469718e-06
-1.303125 1.3846267148370816e-06
-1.30375 1.3922572849925312e-06
-1.304375 1.4010911035266625e-06
-1.305 1.413232021790187e-06
-1.305625 1.4230029663953138e-06
-1.30625 1.4318097486217014e-06
-1.306875 1.439594613523436e-06
-1.3075 1.4505504693533368e-06
-1.308125 1.4591571150479824e-06
-1.30875 1.4679365663363702e-06
-1.309375 1.478022637975509e-06
-1.31 1.4878027901668328e-06
-1.310625 1.4961821620156147e-06
-1.31125 1.5074484240331025e-06
-1.311875 1.5146217280890468e-06
-1.3125 1.5260905645657834e-06
-1.313125 1.5381814224029811e-06
-1.31375 1.5499059452883038e-06
-1.314375 1.561007833034685e-06
-1.315 1.5709313221209343e-06
-1.315625 1.5815267597730626e-06
-1.31625 1.5954578954236461e-06
-1.316875 1.605617750183297e-06
-1.3175 1.6176735371196663e-06
-1.318125 1.6316805766088941e-06
-1.31875 1.6442774581354681e-06
-1.319375 1.6602288028443397e-06
-1.32 1.6727639971959548e-06
-1.320625 1.688828223608933e-06
-1.32125 1.6996899496159946e-06
-1.321875 1.7122184837054166e-06
-1.3225 1.7264687635041023e-06
-1.323125 1.7372432338444134e-06
-1.32375 1.7520533478298043e-06
-1.324375 1.7644038982709785e-06
-1.325 1.7772208378213746e-06
-1.325625 1.7922439331404372e-06
-1.32625 1.8079191972928252e-06
-1.326875 1.8252724221574808e-06
-1.3275 1.8410382518355666e-06
-1.328125 1.8557762832869755e-06
-1.32875 1.871388210288366e-06
-1.329375 1.885945188964272e-06
-1.33 1.9000462950535254e-06
-1.330625 1.916993146836473e-06
-1.33125 1.9334216651032844e-06
-1.331875 1.9468136032330506e-06
-1.3325 1.960382610638074e-06
-1.333125 1.980109145456711e-06
-1.33375 1.997533936813207e-06
-1.334375 2.0134835739568507e-06
-1.335 2.033098953569518e-06
-1.335625 2.0526818130561196e-06
-1.33625 2.0712259311956713e-06
-1.336875 2.091936667535681e-06
-1.3375 2.1099870106642015e-06
-1.338125 2.1256667931110362e-06
-1.33875 2.142781061693032e-06
-1.339375 2.1637309907348524e-06
-1.34 2.184419742165879e-06
-1.340625 2.2057372772105926e-06
-1.34125 2.2237035060675125e-06
-1.341875 2.2438195967754425e-06
-1.3425 2.265483534978636e-06
-1.343125 2.2857090412321015e-06
-1.34375 2.306005404319782e-06
-1.344375 2.321023577573597e-06
-1.345 2.344288311526732e-06
-1.345625 2.3665487686965093e-06
-1.34625 2.3880943112401316e-06
-1.346875 2.4134385604885175e-06
-1.3475 2.4363679374684127e-06
-1.348125 2.4570681305063563e-06
-1.34875 2.483871090456883e-06
-1.349375 2.5060365881173483e-06
-1.35 2.5313279626194104e-06
-1.350625 2.555133014244053e-06
-1.35125 2.5802838093763767e-06
-1.351875 2.606426001607697e-06
-1.3525 2.633498589132909e-06
-1.353125 2.664707338276767e-06
-1.35375 2.6921499545121125e-06
-1.354375 2.7224813233937923e-06
-1.355 2.744178291503711e-06
-1.355625 2.772778736148009e-06
-1.35625 2.8001620421776004e-06
-1.356875 2.8324545771052738e-06
-1.3575 2.868932497209193e-06
-1.358125 2.900356885007382e-06
-1.35875 2.929445674712459e-06
-1.359375 2.9592806143509325e-06
-1.36 2.991367101992161e-06
-1.360625 3.023494027800982e-06
-1.36125 3.0568941287872144e-06
-1.361875 3.0899530960496253e-06
-1.3625 3.12574484531233e-06
-1.363125 3.1574701883779564e-06
-1.36375 3.188569573222596e-06
-1.364375 3.2248497716226546e-06
-1.365 3.2589942803126984e-06
-1.365625 3.296938131847359e-06
-1.36625 3.324095534851078e-06
-1.366875 3.358812535733447e-06
-1.3675 3.401552788000433e-06
-1.368125 3.4349560452985933e-06
-1.36875 3.4782922223666333e-06
-1.369375 3.5167337968034793e-06
-1.37 3.5573094240342588e-06
-1.370625 3.5940310746928857e-06
-1.37125 3.6409746842966987e-06
-1.371875 3.6826351162803527e-06
-1.3725 3.72467629857352e-06
-1.373125 3.766631916760906e-06
-1.37375 3.808797840037031e-06
-1.374375 3.856095196422084e-06
-1.375 3.8992147947783e-06
-1.375625 3.945307389327541e-06
-1.37625 3.993385195370052e-06
-1.376875 4.039566804947866e-06
-1.3775 4.083445811427848e-06
-1.378125 4.126732068113209e-06
-1.37875 4.173949743379185e-06
-1.379375 4.218724950210842e-06
-1.38 4.265416250249622e-06
-1.380625 4.318077375912894e-06
-1.38125 4.361470465653119e-06
-1.381875 4.411837658973364e-06
-1.3825 4.459952223894875e-06
-1.383125 4.509162963238553e-06
-1.38375 4.565407465643377e-06
-1.384375 4.618380156331198e-06
-1.385 4.669712815021565e-06
-1.385625 4.7322366947759335e-06
-1.38625 4.7896848741580445e-06
-1.386875 4.849187083568782e-06
-1.3875 4.89680698497442e-06
-1.388125 4.958114301299786e-06
-1.38875 5.025537410084557e-06
-1.389375 5.07942022183058e-06
-1.39 5.143618851986312e-06
-1.390625 5.203955220324509e-06
-1.39125 5.268857656631184e-06
-1.391875 5.335617338826266e-06
-1.3925 5.40289949996727e-06
-1.393125 5.474642133136853e-06
-1.39375 5.536692529286929e-06
-1.394375 5.615113954313336e-06
-1.395 5.685620675482134e-06
-1.395625 5.7627513484137055e-06
-1.39625 5.837501714303683e-06
-1.396875 5.915589205705836e-06
-1.3975 5.9921356174053854e-06
-1.398125 6.061419307320687e-06
-1.39875 6.143743716585901e-06
-1.399375 6.221392203538605e-06
-1.4 6.307646204954234e-06
-1.400625 6.396038978665352e-06
-1.40125 6.466613931130035e-06
-1.401875 6.552538922641645e-06
-1.4025 6.628733227552e-06
-1.403125 6.722508042771852e-06
-1.40375 6.8123229524604685e-06
-1.404375 6.89899530556635e-06
-1.405 6.996718552183582e-06
-1.405625 7.0802350235014555e-06
-1.40625 7.178068374627922e-06
-1.406875 7.285299738837038e-06
-1.4075 7.388423034147335e-06
-1.408125 7.498701733088608e-06
-1.40875 7.599151039736988e-06
-1.409375 7.699621860186648e-06
-1.41 7.79394872156933e-06
-1.410625 7.886280945091857e-06
-1.41125 8.006173754277241e-06
-1.411875 8.106208067407575e-06
-1.4125 8.209465337185818e-06
-1.413125 8.330526244478344e-06
-1.41375 8.438579884862938e-06
-1.414375 8.565267904277015e-06
-1.415 8.680278441306876e-06
-1.415625 8.796183835652611e-06
-1.41625 8.923843063343658e-06
-1.416875 9.03704852149808e-06
-1.4175 9.17012641524231e-06
-1.418125 9.285700173205691e-06
-1.41875 9.415700521596913e-06
-1.419375 9.54087648723195e-06
-1.42 9.67320888902782e-06
-1.420625 9.797999913560356e-06
-1.42125 9.93588180155118e-06
-1.421875 1.0067261968636073e-05
-1.4225 1.0207009928058039e-05
-1.423125 1.035405462059411e-05
-1.42375 1.0493561664410964e-05
-1.424375 1.064972311888477e-05
-1.425 1.0808460292935522e-05
-1.425625 1.0951436081151764e-05
-1.42625 1.112080045539232e-05
-1.426875 1.1281371854419346e-05
-1.4275 1.144745344256415e-05
-1.428125 1.1602110269467778e-05
-1.42875 1.1759262112865206e-05
-1.429375 1.1912391074572572e-05
-1.43 1.2087587854045552e-05
-1.430625 1.22480898808362e-05
-1.43125 1.2411417057033663e-05
-1.431875 1.2603806815485328e-05
-1.4325 1.2761785950173487e-05
-1.433125 1.2959029549575647e-05
-1.43375 1.3157646285774442e-05
-1.434375 1.3353695818219285e-05
-1.435 1.3571382568931186e-05
-1.435625 1.375455797016788e-05
-1.43625 1.3984694158873784e-05
-1.436875 1.416711127419649e-05
-1.4375 1.436623926982355e-05
-1.438125 1.4557708689625184e-05
-1.43875 1.478625541756978e-05
-1.439375 1.4995485401424284e-05
-1.44 1.5195602655414253e-05
-1.440625 1.5425801751004402e-05
-1.44125 1.564998876958883e-05
-1.441875 1.589263156813774e-05
-1.4425 1.61450887529054e-05
-1.443125 1.63898333251315e-05
-1.44375 1.6630259711982763e-05
-1.444375 1.6884053618282838e-05
-1.445 1.7135017955663104e-05
-1.445625 1.738748171459219e-05
-1.44625 1.7672929755831047e-05
-1.446875 1.7913741081040358e-05
-1.4475 1.8186097965568497e-05
-1.448125 1.8415133924807834e-05
-1.44875 1.869909316583523e-05
-1.449375 1.898080450542358e-05
-1.45 1.927105937053809e-05
-1.450625 1.9556767365344323e-05
-1.45125 1.985015018515246e-05
-1.451875 2.0138475018987167e-05
-1.4525 2.0457868580552477e-05
-1.453125 2.078436035560326e-05
-1.45375 2.1104397672006944e-05
-1.454375 2.1431621293716417e-05
-1.455 2.1776882879129976e-05
-1.455625 2.21416576702613e-05
-1.45625 2.2453008868972715e-05
-1.456875 2.2813707809918864e-05
-1.4575 2.315764931552701e-05
-1.458125 2.3504887259174887e-05
-1.45875 2.3887242013977818e-05
-1.459375 2.4216557624123187e-05
-1.46 2.45997133299791e-05
-1.460625 2.5037185442120614e-05
-1.46125 2.5473524668843082e-05
-1.461875 2.5864408944670338e-05
-1.4625 2.6274392031287068e-05
-1.463125 2.664539408690771e-05
-1.46375 2.7078089139051342e-05
-1.464375 2.7517016339175507e-05
-1.465 2.7923254747566314e-05
-1.465625 2.8315520961131922e-05
-1.46625 2.8774534572823798e-05
-1.466875 2.9237091100271727e-05
-1.4675 2.967864826541028e-05
-1.468125 3.0097061963141042e-05
-1.46875 3.061291749425388e-05
-1.469375 3.1090544358423764e-05
-1.47 3.157900222252566e-05
-1.470625 3.210546846409062e-05
-1.47125 3.257090026377185e-05
-1.471875 3.3130462142227986e-05
-1.4725 3.368649841547274e-05
-1.473125 3.422115159546122e-05
-1.47375 3.475003055481866e-05
-1.474375 3.536978896722735e-05
-1.475 3.592232435855852e-05
-1.475625 3.650664997811387e-05
-1.47625 3.7118395179454304e-05
-1.476875 3.7731951342537525e-05
-1.4775 3.8364331849806925e-05
-1.478125 3.901145443141618e-05
-1.47875 3.962364247090227e-05
-1.479375 4.017430396101826e-05
-1.48 4.0845984652304855e-05
-1.480625 4.157357284165075e-05
-1.48125 4.231165347459251e-05
-1.481875 4.295428265147146e-05
-1.4825 4.3600811808209186e-05
-1.483125 4.431269971872951e-05
-1.48375 4.49928524628275e-05
-1.484375 4.575161699625498e-05
-1.485 4.649261832367441e-05
-1.485625 4.7320038801408444e-05
-1.48625 4.8113542647319086e-05
-1.486875 4.888156210585179e-05
-1.4875 4.967217569866984e-05
-1.488125 5.0463236255400254e-05
-1.48875 5.1318700132813716e-05
-1.489375 5.2170315528241044e-05
-1.49 5.3005814670855154e-05
-1.490625 5.3848178671190165e-05
-1.49125 5.472687541864814e-05
-1.491875 5.558114528151056e-05
-1.4925 5.644524998595176e-05
-1.493125 5.745573074539297e-05
-1.49375 5.843137799687522e-05
-1.494375 5.937403936010924e-05
-1.495 6.0356964951612676e-05
-1.495625 6.134547495463537e-05
-1.49625 6.232090394772363e-05
-1.496875 6.338668922260292e-05
-1.4975 6.442902173072614e-05
-1.498125 6.557878071138069e-05
-1.49875 6.67219420018106e-05
-1.499375 6.800874451036276e-05
-1.5 6.915513439979024e-05
-1.500625 7.02658280478447e-05
-1.50125 7.145370678628886e-05
-1.501875 7.261893507007268e-05
-1.5025 7.38469776604513e-05
-1.503125 7.516565531839237e-05
-1.50375 7.645047466271587e-05
-1.504375 7.78333351726737e-05
-1.505 7.919977915084048e-05
-1.505625 8.051216449440556e-05
-1.50625 8.183003490129341e-05
-1.506875 8.323707172723115e-05
-1.5075 8.481303389088241e-05
-1.508125 8.618445944322064e-05
-1.50875 8.776157748548206e-05
-1.509375 8.941384316009049e-05
-1.51 9.094596464197875e-05
-1.510625 9.260018388523625e-05
-1.51125 9.41416409146659e-05
-1.511875 9.563542592551307e-05
-1.5125 9.737128191830565e-05
-1.513125 9.9074627946037e-05
-1.51375 0.00010078447285570617
-1.514375 0.00010246703993356385
-1.515 0.0001041906892849212
-1.515625 0.0001060914817303581
-1.51625 0.00010790482492317744
-1.516875 0.00010982138866358877
-1.5175 0.00011184477246326227
-1.518125 0.0001137882555192734
-1.51875 0.00011578111393357238
-1.519375 0.000117911358757243
-1.52 0.00011999037530817115
-1.520625 0.0001220116644901095
-1.52125 0.0001240974321608263
-1.521875 0.0001264614455988135
-1.5225 0.00012877072847801332
-1.523125 0.00013108801757224383
-1.52375 0.00013344124272761246
-1.524375 0.0001359957085592909
-1.525 0.00013851333054887489
-1.525625 0.0001408387141557067
-1.52625 0.0001433737061142299
-1.526875 0.0001457883146319579
-1.5275 0.00014854144235968466
-1.528125 0.00015148601434949224
-1.52875 0.00015434465808453231
-1.529375 0.00015721236005411624
-1.53 0.00015996323664890322
-1.530625 0.00016295426386308748
-1.53125 0.0001658818685300138
-1.531875 0.0001691946557829095
-1.5325 0.0001723175512377559
-1.533125 0.00017560742545436042
-1.53375 0.00017874341361304226
-1.534375 0.0001818793981705466
-1.535 0.00018530130181703352
-1.535625 0.00018908734216765098
-1.53625 0.00019236416688778285
-1.536875 0.00019564447615606903
-1.5375 0.00019921436006958907
-1.538125 0.0002029189397562487
-1.53875 0.00020656343700717922
-1.539375 0.00021051384616712157
-1.54 0.00021415418600415097
-1.540625 0.00021826575576723217
-1.54125 0.0002225751920945022
-1.541875 0.00022678957902469893
-1.5425 0.0002314902125310226
-1.543125 0.0002358416370966028
-1.54375 0.0002401572865784021
-1.544375 0.00024518850286849475
-1.545 0.00024983255538934125
-1.545625 0.00025469346397551324
-1.54625 0.0002592528151436252
-1.546875 0.0002639861885420749
-1.5475 0.0002691900642412517
-1.548125 0.0002740845018911738
-1.54875 0.0002795171598490406
-1.549375 0.0002852612754645148
-1.55 0.0002905390325007754
-1.550625 0.00029681948334510876
-1.55125 0.0003023211846901298
-1.551875 0.00030790370133631834
-1.5525 0.000314267787559432
-1.553125 0.00032048460961886456
-1.55375 0.00032636457882753733
-1.554375 0.00033268766957556494
-1.555 0.0003390630066964737
-1.555625 0.0003457366805254515
-1.55625 0.0003528987861387999
-1.556875 0.00035986760210588196
-1.5575 0.00036684728199377176
-1.558125 0.00037403034241709096
-1.55875 0.00038168001989322706
-1.559375 0.00038898129193382384
-1.56 0.00039707129360625165
-1.560625 0.00040468807401721255
-1.56125 0.00041283147425806116
-1.561875 0.00042094543690188917
-1.5625 0.00043002545784223114
-1.563125 0.00043826877634812724
-1.56375 0.0004465335266583467
-1.564375 0.00045505856818418085
-1.565 0.00046479968213211165
-1.565625 0.00047448327884871386
-1.56625 0.0004845408098083557
-1.566875 0.0004941825562655741
-1.5675 0.0005034775621047752
-1.568125 0.0005141818774678257
-1.56875 0.00052524703428702
-1.569375 0.0005367193038692495
-1.57 0.0005469376445540852
-1.570625 0.0005593158980136467
-1.57125 0.0005704286181637518
-1.571875 0.0005819089940223998
-1.5725 0.0005944686857690364
-1.573125 0.0006066291663698616
-1.57375 0.0006203221202459981
-1.574375 0.0006320763774475247
-1.575 0.000645535700968565
-1.575625 0.000658687273353955
-1.57625 0.0006724907158916576
-1.576875 0.0006862897628931657
-1.5775 0.0007002665647387943
-1.578125 0.0007167040568269154
-1.57875 0.000732470705309391
-1.579375 0.0007481620947710229
-1.58 0.0007639348570191534
-1.580625 0.0007797896733723411
-1.58125 0.0007968073752597482
-1.581875 0.0008120062991319477
-1.5825 0.0008274890298111113
-1.583125 0.00084592789537668
-1.58375 0.0008654873542859274
-1.584375 0.0008853638848110448
-1.585 0.0009054151216845072
-1.585625 0.0009243979768363154
-1.58625 0.0009434613808527565
-1.586875 0.0009648114132183503
-1.5875 0.00098714196131573
-1.588125 0.0010073831794708648
-1.58875 0.001029035125458027
-1.589375 0.00105332359749281
-1.59 0.0010769792007838902
-1.590625 0.0010996777230316427
-1.59125 0.00112431913588372
-1.591875 0.001149165445581469
-1.5925 0.001175738859045252
-1.593125 0.0012006410329232606
-1.59375 0.0012277324186936737
-1.594375 0.001255055205543993
-1.595 0.0012842158544940662
-1.595625 0.0013116381655403672
-1.59625 0.0013415845193435376
-1.596875 0.0013734971335421524
-1.5975 0.001402823185317043
-1.598125 0.00143512289100513
-1.59875 0.0014700020296295703
-1.599375 0.0015040493337526916
-1.6 0.0015383526070885023
-1.600625 0.0015764575818200002
-1.60125 0.0016112854070522255
-1.601875 0.001648615029961645
-1.6025 0.0016884223793686274
-1.603125 0.0017266657533324525
-1.60375 0.0017665830663463958
-1.604375 0.0018088964854198778
-1.605 0.0018470452448452366
-1.605625 0.001890053340451619
-1.60625 0.0019369113859609153
-1.606875 0.0019824536120454355
-1.6075 0.0020267502296197953
-1.608125 0.002073778145224043
-1.60875 0.0021233090743620663
-1.609375 0.002173541453331034
-1.61 0.0022237245882799853
-1.610625 0.002274169700561924
-1.61125 0.002327939152785732
-1.611875 0.0023856725266850278
-1.6125 0.0024433585093455055
-1.613125 0.002502154115599102
-1.61375 0.0025665013698822456
-1.614375 0.002627961623291527
-1.615 0.00268607268925275
-1.615625 0.002753288893526224
-1.61625 0.002820749659793207
-1.616875 0.0028904857559363217
-1.6175 0.0029653290640911266
-1.618125 0.003037749640820185
-1.61875 0.003108977815075337
-1.619375 0.003183683487014216
-1.62 0.0032648405466057582
-1.620625 0.003348719212639281
-1.62125 0.0034317473101043872
-1.621875 0.0035227987470116758
-1.6225 0.0036077943947820075
-1.623125 0.0037044071744684786
-1.62375 0.003792598905500297
-1.624375 0.0038839396317894535
-1.625 0.003973541365555775
-1.625625 0.004076623958122864
-1.62625 0.004182139373328776
-1.626875 0.00428592969370282
-1.6275 0.004398220055703426
-1.628125 0.004508727121303512
-1.62875 0.004626316510633354
-1.629375 0.004745005997442828
-1.63 0.004864000747549894
-1.630625 0.004997066697829802
-1.63125 0.00511820924833533
-1.631875 0.005255726281330336
-1.6325 0.005387589605810946
-1.633125 0.005529138928686801
-1.63375 0.005673613781803756
-1.634375 0.005820504201183155
-1.635 0.005974959883231871
-1.635625 0.00612793107904814
-1.63625 0.006296035296008961
-1.636875 0.006469975231624785
-1.6375 0.006632619648210244
-1.638125 0.006806022117381414
-1.63875 0.006976057827972148
-1.639375 0.00717160418424444
-1.64 0.007363511140195863
-1.640625 0.007563068957286339
-1.64125 0.007757885315161128
-1.641875 0.007969991190577091
-1.6425 0.008195440959837055
-1.643125 0.00841141509944336
-1.64375 0.008651687105250013
-1.644375 0.008883620058184872
-1.645 0.009135047248580809
-1.645625 0.009373852492225688
-1.64625 0.009630831242327238
-1.646875 0.009900014866715346
-1.6475 0.010173533784571752
-1.648125 0.010441979844821911
-1.64875 0.01073472281690958
-1.649375 0.011035561487319856
-1.65 0.011335700072395228
-1.650625 0.011644222399169499
-1.65125 0.011981090643739228
-1.651875 0.01231724660907717
-1.6525 0.012669017689626515
-1.653125 0.013031064072166003
-1.65375 0.0133855447067753
-1.654375 0.013775365656881393
-1.655 0.014157535111093475
-1.655625 0.01456141144349785
-1.65625 0.015004939283790033
-1.656875 0.015413663108693625
-1.6575 0.015850002189768564
-1.658125 0.016299689286968344
-1.65875 0.016764569841703
-1.659375 0.017253162471694127
-1.66 0.017741325472464722
-1.660625 0.018253110586021783
-1.66125 0.018759599167329465
-1.661875 0.01930352074978976
-1.6625 0.019831333319960377
-1.663125 0.020407236099612376
-1.66375 0.020996227466091963
-1.664375 0.021617122863656697
-1.665 0.022235925799754683
-1.665625 0.022884403903724843
-1.66625 0.023599029053884817
-1.666875 0.02430099359859239
-1.6675 0.024999840716622233
-1.668125 0.0257115546467479
-1.66875 0.0264953883737586
-1.669375 0.027241076769320725
-1.67 0.028058126723454938
-1.670625 0.028857972564452283
-1.67125 0.029710017734712886
-1.671875 0.030663872898123327
-1.6725 0.03156630002115495
-1.673125 0.03251937380344237
-1.67375 0.033510669550278885
-1.674375 0.03449570934561854
-1.675 0.035505773913033924
-1.675625 0.0366260806982642
-1.67625 0.037772471893184
-1.676875 0.03882111295229076
-1.6775 0.040043147735375685
-1.678125 0.041199621271976045
-1.67875 0.04241821721028495
-1.679375 0.043688468506544814
-1.68 0.04503954617100639
-1.680625 0.04638010648496962
-1.68125 0.047783099341020686
-1.681875 0.04923567011267673
-1.6825 0.0508597506251491
-1.683125 0.05237944005881557
-1.68375 0.05405146671679848
-1.684375 0.055611117864054246
-1.685 0.05733011444946836
-1.685625 0.05915784006675451
-1.68625 0.06108040579752102
-1.686875 0.06289880135770617
-1.6875 0.06480628915963187
-1.688125 0.06687508464405699
-1.68875 0.06884117922993253
-1.689375 0.07096018050499235
-1.69 0.07313112900950057
-1.690625 0.07547348360245744
-1.69125 0.0776994438056997
-1.691875 0.08007223697567586
-1.6925 0.08261464020141462
-1.693125 0.08516842024936533
-1.69375 0.08779494645825318
-1.694375 0.0905922299360899
-1.695 0.09339852837142364
-1.695625 0.09638322834506721
-1.69625 0.09934420341670656
-1.696875 0.10253372676583103
-1.6975 0.1057446778295972
-1.698125 0.10911167756180921
-1.69875 0.1125889850451858
-1.699375 0.11614785475566418
-1.7 0.11970559708553356
-1.700625 0.12361089455019537
-1.70125 0.12754246008694997
-1.701875 0.13159740870858838
-1.7025 0.13553989664811808
-1.703125 0.139650166860317
-1.70375 0.1441270679787486
-1.704375 0.14884327909702852
-1.705 0.15321467816722412
-1.705625 0.15787499359471044
-1.70625 0.16300508733533442
-1.706875 0.16819677994167176
-1.7075 0.17327413069954561
-1.708125 0.17876445754733442
-1.70875 0.18435177058754004
-1.709375 0.1904314589139037
-1.71 0.1967032017759966
-1.710625 0.20304229199630378
-1.71125 0.20927289905417215
-1.711875 0.2162229761604171
-1.7125 0.2228785548359049
-1.713125 0.2300966861090762
-1.71375 0.2378668146419071
-1.714375 0.24524838044685535
-1.715 0.2531111264089521
-1.715625 0.2616812929992453
-1.71625 0.2698382948795548
-1.716875 0.27846205209353825
-1.7175 0.28755546023548445
-1.718125 0.29613831960970527
-1.71875 0.3055640507820607
-1.719375 0.3151589279860317
-1.72 0.3252027128386222
-1.720625 0.3357993237413436
-1.72125 0.34602927474353373
-1.721875 0.35681378466164504
-1.7225 0.3680925565377977
-1.723125 0.3790415437189533
-1.72375 0.39073249994839254
-1.724375 0.4030906260204399
-1.725 0.4155901054834121
-1.725625 0.4286833740760761
-1.72625 0.4421323862461016
-1.726875 0.45632126690856467
-1.7275 0.4704726295043533
-1.728125 0.4850611433555155
-1.72875 0.4999173920896889
-1.729375 0.5152297047070747
-1.73 0.5312489469976163
-1.730625 0.5473588807715886
-1.73125 0.5646489399753524
-1.731875 0.5827839391884598
-1.7325 0.5995649367768578
-1.733125 0.6194549216461278
-1.73375 0.6378474746067869
-1.734375 0.6572049140491331
-1.735 0.6779392948540764
-1.735625 0.6986427042126879
-1.73625 0.720307079487042
-1.736875 0.7433967970798816
-1.7375 0.7656894324700236
-1.738125 0.7898439808657735
-1.73875 0.8147441337773386
-1.739375 0.8401371855192787
-1.74 0.8647076923074348
-1.740625 0.8910108362873174
-1.74125 0.9169480440229002
-1.741875 0.9437784574687681
-1.7425 0.9725124166926555
-1.743125 1.0011477636233
-1.74375 1.02934919161526
-1.744375 1.058392089986467
-1.745 1.089841207551828
-1.745625 1.1241099562516255
-1.74625 1.155224133731413
-1.746875 1.18853618984343
-1.7475 1.2226362299565867
-1.748125 1.256661545415759
-1.74875 1.2931038965060437
-1.749375 1.3310848393489745
-1.75 1.3706631786614218
-1.750625 1.4128092612465248
-1.75125 1.45472348170382
-1.751875 1.4963037563126533
-1.7525 1.538009942986811
-1.753125 1.5829641436213955
-1.75375 1.6274200010330098
-1.754375 1.6746570370277682
-1.755 1.7207154173083181
-1.755625 1.767643031957997
-1.75625 1.8140328619714887
-1.756875 1.8634975051081717
-1.7575 1.9138808786924162
-1.758125 1.9649891372838815
-1.75875 2.0194895360495444
-1.759375 2.0746895634269693
-1.76 2.130574035794121
-1.760625 2.1871848069974242
-1.76125 2.2437301616243266
-1.761875 2.303694291822444
-1.7625 2.371457595576376
-1.763125 2.4336410203331527
-1.76375 2.4997480450647847
-1.764375 2.5588543614826045
-1.765 2.6255676981692964
-1.765625 2.694151911560092
-1.76625 2.7626542567934878
-1.766875 2.8307472966508658
-1.7675 2.9048422616626466
-1.768125 2.982239089143058
-1.76875 3.056582049488217
-1.769375 3.132221445359124
-1.77 3.2111766017851826
-1.770625 3.2904431415654676
-1.77125 3.3721747290002018
-1.771875 3.449085591029845
-1.7725 3.5370220369946805
-1.773125 3.618663723135629
-1.77375 3.706504065012571
-1.774375 3.790967893363195
-1.775 3.8849058584264724
-1.775625 3.9715115104937153
-1.77625 4.06720700410506
-1.776875 4.158467380589145
-1.7775 4.256611890163363
-1.778125 4.3524889370394755
-1.77875 4.448545173658204
-1.779375 4.547352103744797
-1.78 4.645062621947666
-1.780625 4.742133435473588
-1.78125 4.844115231604744
-1.781875 4.950328070673481
-1.7825 5.058481577105726
-1.783125 5.159741129461383
-1.78375 5.267508556159268
-1.784375 5.37507976654394
-1.785 5.485111133293176
-1.785625 5.60397812764895
-1.78625 5.715340624693746
-1.786875 5.829432660780971
-1.7875 5.9374373146153
-1.788125 6.052409331785885
-1.78875 6.17455469493998
-1.789375 6.279303052241887
-1.79 6.390841824442364
-1.790625 6.497004576013262
-1.79125 6.620668732488455
-1.791875 6.757490479742957
-1.7925 6.859595978161333
-1.793125 6.986734831175423
-1.79375 7.109670383526925
-1.794375 7.2142768370362
-1.795 7.329419729251837
-1.795625 7.4547391784999455
-1.79625 7.574621152800148
-1.796875 7.691679447689821
-1.7975 7.809255875651343
-1.798125 7.937329823263524
-1.79875 8.071280608847639
-1.799375 8.184035881647716
-1.8 8.314123070867671
-1.800625 8.43047101065431
-1.80125 8.535084190726645
-1.801875 8.648328405574034
-1.8025 8.765899503293678
-1.803125 8.87559950839797
-1.80375 8.982422329113462
-1.804375 9.096789901433452
-1.805 9.211955484736515
-1.805625 9.321827289927349
-1.80625 9.427543836372385
-1.806875 9.549974390928341
-1.8075 9.657023258319011
-1.808125 9.766181188456526
-1.80875 9.857854064256232
-1.809375 9.953717128871231
-1.81 10.042005730359776
-1.810625 10.136289531727218
-1.81125 10.249131684287425
-1.811875 10.338803483755548
-1.8125 10.438669191303308
-1.813125 10.521086439110254
-1.81375 10.619961894589046
-1.814375 10.70092362820001
-1.815 10.787902346029119
-1.815625 10.865133557555312
-1.81625 10.93392272538817
-1.816875 11.015206385140196
-1.8175 11.085964800698028
-1.818125 11.13605570391539
-1.81875 11.217309517928255
-1.819375 11.267347149431059
-1.82 11.32579786111005
-1.820625 11.347967190988086
-1.82125 11.401261721365827
-1.821875 11.442083661336609
-1.8225 11.492057053045054
-1.823125 11.520316564950171
-1.82375 11.534819254782507
-1.824375 11.565211986509382
-1.825 11.581925528395058
-1.825625 11.597898724171223
-1.82625 11.604429838438127
-1.826875 11.602862494203912
-1.8275 11.593376223452452
-1.828125 11.624223473842331
-1.82875 11.633747934728635
-1.829375 11.606620211650785
-1.83 11.609011524619811
-1.830625 11.595741857587907
-1.83125 11.57927801492195
-1.831875 11.549729214476839
-1.8325 11.523408203095046
-1.833125 11.49322436794013
-1.83375 11.448071610571693
-1.834375 11.413764870493164
-1.835 11.371777990083979
-1.835625 11.319134529354114
-1.83625 11.24494321105268
-1.836875 11.18360730118059
-1.8375 11.129260939074172
-1.838125 11.050599904694797
-1.83875 10.972748365981476
-1.839375 10.8905096051038
-1.84 10.837591705834521
-1.840625 10.739734135615574
-1.84125 10.646565386331451
-1.841875 10.554071166050296
-1.8425 10.450187153289965
-1.843125 10.365260147857857
-1.84375 10.24232058484849
-1.844375 10.135063827861366
-1.845 10.013060124422669
-1.845625 9.896114294427374
-1.84625 9.778919335261348
-1.846875 9.655526148181435
-1.8475 9.536592118636824
-1.848125 9.406445058441976
-1.84875 9.277326692962133
-1.849375 9.139385632432232
-1.85 9.007960876256742
-1.850625 8.867455283804587
-1.85125 8.718273335847616
-1.851875 8.582898207784485
-1.8525 8.427870677416237
-1.853125 8.277990576317658
-1.85375 8.129687720475639
-1.854375 7.978615671200025
-1.855 7.8021648965443156
-1.855625 7.648070973346307
-1.85625 7.496075866439243
-1.856875 7.3363989278131525
-1.8575 7.166120446803753
-1.858125 6.998224136757042
-1.85875 6.840991353244935
-1.859375 6.6900647696342785
-1.86 6.513633957378194
-1.860625 6.357175266892748
-1.86125 6.187434253183626
-1.861875 6.025864754559436
-1.8625 5.8712177384131286
-1.863125 5.703809438760436
-1.86375 5.5437410178250985
-1.864375 5.392167600655258
-1.865 5.235582281229874
-1.865625 5.0762030988200335
-1.86625 4.924114720692364
-1.866875 4.7766880627315444
-1.8675 4.625500131185548
-1.868125 4.479371429568046
-1.86875 4.331507652022703
-1.869375 4.1869041618569085
-1.87 4.0466278302309595
-1.870625 3.9093440408024356
-1.87125 3.7677752638714814
-1.871875 3.6287252205171865
-1.8725 3.493265399788522
-1.873125 3.363838199473045
-1.87375 3.2312785430388007
-1.874375 3.106849912034986
-1.875 2.9863200970580337
-1.875625 2.872446825667562
-1.87625 2.75819605248435
-1.876875 2.645928126821359
-1.8775 2.537430266351568
-1.878125 2.424717277424644
-1.87875 2.323229187777794
-1.879375 2.221730884550779
-1.88 2.1210917652412666
-1.880625 2.0262262655647154
-1.88125 1.9329955194432251
-1.881875 1.8434561482867569
-1.8825 1.7532021397542052
-1.883125 1.6668905193671382
-1.88375 1.5840364957153932
-1.884375 1.5042558184838821
-1.885 1.4297044557209269
-1.885625 1.3554460034726434
-1.88625 1.285671311096686
-1.886875 1.2179244084187606
-1.8875 1.1515105654992994
-1.888125 1.088385400808687
-1.88875 1.0283378505387395
-1.889375 0.9701256016659798
-1.89 0.9133634310082444
-1.890625 0.859568401859258
-1.89125 0.8094300980205301
-1.891875 0.7619170730041843
-1.8925 0.7162246756390459
-1.893125 0.6722948483105817
-1.89375 0.629870401005224
-1.894375 0.5903002569598261
-1.895 0.5522006358396304
-1.895625 0.5159453380947386
-1.89625 0.4812630291987372
-1.896875 0.44980795342546676
-1.8975 0.4196995647321155
-1.898125 0.3906414644167565
-1.89875 0.3638137642958563
-1.899375 0.33799967838261474
-1.9 0.3141125050465091
-1.900625 0.29195438628870635
-1.90125 0.27075831102449477
-1.901875 0.25062238017712535
-1.9025 0.2317728303343119
-1.903125 0.2142146744893175
-1.90375 0.19774730846774205
-1.904375 0.18239071655869082
-1.905 0.16800479640277372
-1.905625 0.15457242672378999
-1.90625 0.14230327809328355
-1.906875 0.13060303363182238
-1.9075 0.11985574845427927
-1.908125 0.10985187484315032
-1.90875 0.10055146560237686
-1.909375 0.09191462099245283
-1.91 0.08393658742467817
-1.910625 0.0764511418218798
-1.91125 0.06957870694810726
-1.911875 0.06329617399581236
-1.9125 0.05740020059125715
-1.913125 0.05218639570125438
-1.91375 0.04731271582140252
-1.914375 0.042878971783827664
-1.915 0.038737185211593875
-1.915625 0.03496819273905801
-1.91625 0.03155436756627317
-1.916875 0.028437689773108368
-1.9175 0.025578943849333464
-1.918125 0.02297183060169247
-1.91875 0.02058852456854702
-1.919375 0.018451020970993926
-1.92 0.016510809449468977
-1.920625 0.01473655373992144
-1.92125 0.013154116675995009
-1.921875 0.011725741401495798
-1.9225 0.010427590966343213
-1.923125 0.009273962535118268
-1.92375 0.008230675017882112
-1.924375 0.007305987429978342
-1.925 0.0064478054183816896
-1.925625 0.005695432219189583
-1.92625 0.005026534295776604
-1.926875 0.0044237578341453036
-1.9275 0.003894945726656252
-1.928125 0.003423970730579477
-1.92875 0.0030072966042234556
-1.929375 0.0026326506813057625
-1.93 0.0023018437557317437
-1.930625 0.0020105577413377803
-1.93125 0.0017525743223938315
-1.931875 0.0015235845296003674
-1.9325 0.0013232951087098874
-1.933125 0.0011472819067676109
-1.93375 0.0009944713138695328
-1.934375 0.0008593154538786347
-1.935 0.000740498676838313
-1.935625 0.0006378562738401066
-1.93625 0.0005498935256199081
-1.936875 0.0004724091063461487
-1.9375 0.0004039344349036164
-1.938125 0.00034485964728278096
-1.93875 0.0002949779827774431
-1.939375 0.00025154476202427417
-1.94 0.0002128558715597699
-1.940625 0.00018040393042088613
-1.94125 0.00015331805425032417
-1.941875 0.00012952550026531533
-1.9425 0.0001087233435568765
-1.943125 9.152091335002815e-05
-1.94375 7.747271185588071e-05
-1.944375 6.466209442450825e-05
-1.945 5.384811946916788e-05
-1.945625 4.4977821518013494e-05
-1.94625 3.78151280781186e-05
-1.946875 3.113554633677814e-05
-1.9475 2.5615114641089395e-05
-1.948125 2.1332361014881406e-05
-1.94875 1.7859539571349274e-05
-1.949375 1.444215499697856e-05
-1.95 1.1780650221564426e-05
-1.950625 9.760716149731407e-06
-1.95125 8.123786873329346e-06
-1.951875 6.419564593100939e-06
-1.9525 5.2066094689132306e-06
-1.953125 4.311294074463897e-06
-1.95375 3.550840037402664e-06
-1.954375 2.726618225872516e-06
-1.955 2.2145277564464304e-06
-1.955625 1.833850559400455e-06
-1.95625 1.49293351706598e-06
-1.956875 1.1026644429531567e-06
-1.9575 9.027727746194392e-07
-1.958125 7.46461404382879e-07
-1.95875 5.965616922742643e-07
-1.959375 4.1892716683033607e-07
-1.96 3.5233812169140716e-07
-1.960625 2.9038708002339885e-07
-1.96125 2.2623633690804017e-07
-1.961875 1.499905202862383e-07
-1.9625 1.3263445739965726e-07
-1.963125 1.081600821467992e-07
-1.96375 8.131840340481432e-08
-1.964375 5.025134979614818e-08
-1.965 4.825686936280297e-08
-1.965625 3.8248109659842144e-08
-1.96625 2.7420072050854465e-08
-1.966875 1.5589298922577156e-08
-1.9675 1.6795221078757914e-08
-1.968125 1.2706228512280752e-08
-1.96875 8.607897839641162e-09
-1.969375 4.426644617883899e-09
-1.97 5.633080766582662e-09
-1.970625 3.934539169147498e-09
-1.97125 2.493055017399149e-09
-1.971875 1.1464279286347502e-09
-1.9725 1.7936038682790978e-09
-1.973125 1.1229493957423092e-09
-1.97375 6.614965991477436e-10
-1.974375 2.679567608495697e-10
-1.975 5.430167432877973e-10
-1.975625 2.9406893435708355e-10
-1.97625 1.5907196553717516e-10
-1.976875 5.536443203006765e-11
-1.9775 1.5363384337146623e-10
-1.978125 6.90108057851876e-11
-1.97875 3.411512046568607e-11
-1.979375 9.912708294711182e-12
-1.98 3.973955251944748e-11
-1.980625 1.4162991980411335e-11
-1.98125 6.410887284876384e-12
-1.981875 1.50764737120516e-12
-1.9825 9.235958624838484e-12
-1.983125 2.503020378083016e-12
-1.98375 1.0371584099365662e-12
-1.984375 1.8792784254414102e-13
-1.985 1.9048936822093646e-12
-1.985625 3.701079170161408e-13
-1.98625 1.4033404866412778e-13
-1.986875 1.846266831438509e-14
-1.9875 3.364608311144815e-13
-1.988125 4.380536432211938e-14
-1.98875 1.5402177692486458e-14
-1.989375 1.3357672702113689e-15
-1.99 4.977915615633213e-14
-1.990625 3.88453377852541e-15
-1.99125 1.2758225620165395e-15
-1.991875 6.11076840440698e-17
-1.9925 5.866229326807305e-15
-1.993125 2.2773550735730926e-16
-1.99375 7.152077134130789e-17
-1.994375 1.320412702670808e-18
-1.995 5.186982890377519e-16
-1.995625 6.72326719587342e-18
-1.99625 2.042316326455983e-18
-1.996875 0.0
-1.9975 3.0601391499289336e-17
-1.998125 0.0
-1.99875 0.0
-1.999375 0.0
-2.0 8.52029952429918e-19


==> Plots/PA_hist_2500.tex <==
e pe 
0.0 0.0
-0.0004 0.0
-0.0008 0.0
-0.0012 0.0
-0.0016 0.0
-0.002 0.0
-0.0024 0.0
-0.0028 0.0
-0.0032 0.0
-0.0036 0.0
-0.004 0.0
-0.0044 0.0
-0.0048 0.0
-0.0052 0.0
-0.0056 0.0
-0.006 0.0
-0.0064 0.0
-0.0068 0.0
-0.0072 0.0
-0.0076 0.0
-0.008 0.0
-0.0084 0.0
-0.0088 0.0
-0.0092 0.0
-0.0096 0.0
-0.01 0.0
-0.0104 0.0
-0.0108 0.0
-0.0112 0.0
-0.0116 0.0
-0.012 0.0
-0.0124 0.0
-0.0128 0.0
-0.0132 0.0
-0.0136 0.0
-0.014 0.0
-0.0144 0.0
-0.0148 0.0
-0.0152 0.0
-0.0156 0.0
-0.016 0.0
-0.0164 0.0
-0.0168 0.0
-0.0172 0.0
-0.0176 0.0
-0.018 0.0
-0.0184 0.0
-0.0188 0.0
-0.0192 0.0
-0.0196 0.0
-0.02 0.0
-0.0204 0.0
-0.0208 0.0
-0.0212 0.0
-0.0216 0.0
-0.022 0.0
-0.0224 0.0
-0.0228 0.0
-0.0232 0.0
-0.0236 0.0
-0.024 0.0
-0.0244 0.0
-0.0248 0.0
-0.0252 0.0
-0.0256 0.0
-0.026 0.0
-0.0264 0.0
-0.0268 0.0
-0.0272 0.0
-0.0276 0.0
-0.028 0.0
-0.0284 0.0
-0.0288 0.0
-0.0292 0.0
-0.0296 0.0
-0.03 0.0
-0.0304 0.0
-0.0308 0.0
-0.0312 0.0
-0.0316 0.0
-0.032 0.0
-0.0324 0.0
-0.0328 0.0
-0.0332 0.0
-0.0336 0.0
-0.034 0.0
-0.0344 0.0
-0.0348 0.0
-0.0352 0.0
-0.0356 0.0
-0.036 0.0
-0.0364 0.0
-0.0368 0.0
-0.0372 0.0
-0.0376 0.0
-0.038 0.0
-0.0384 0.0
-0.0388 0.0
-0.0392 0.0
-0.0396 0.0
-0.04 0.0
-0.0404 0.0
-0.0408 0.0
-0.0412 0.0
-0.0416 0.0
-0.042 0.0
-0.0424 0.0
-0.0428 0.0
-0.0432 0.0
-0.0436 0.0
-0.044 0.0
-0.0444 0.0
-0.0448 0.0
-0.0452 0.0
-0.0456 0.0
-0.046 0.0
-0.0464 0.0
-0.0468 0.0
-0.0472 0.0
-0.0476 0.0
-0.048 0.0
-0.0484 0.0
-0.0488 0.0
-0.0492 0.0
-0.0496 0.0
-0.05 0.0
-0.0504 0.0
-0.0508 0.0
-0.0512 0.0
-0.0516 0.0
-0.052 0.0
-0.0524 0.0
-0.0528 0.0
-0.0532 0.0
-0.0536 0.0
-0.054 0.0
-0.0544 0.0
-0.0548 0.0
-0.0552 0.0
-0.0556 0.0
-0.056 0.0
-0.0564 0.0
-0.0568 0.0
-0.0572 0.0
-0.0576 0.0
-0.058 0.0
-0.0584 0.0
-0.0588 0.0
-0.0592 0.0
-0.0596 0.0
-0.06 0.0
-0.0604 0.0
-0.0608 0.0
-0.0612 0.0
-0.0616 0.0
-0.062 0.0
-0.0624 0.0
-0.0628 0.0
-0.0632 0.0
-0.0636 0.0
-0.064 0.0
-0.0644 0.0
-0.0648 0.0
-0.0652 0.0
-0.0656 0.0
-0.066 0.0
-0.0664 0.0
-0.0668 0.0
-0.0672 0.0
-0.0676 0.0
-0.068 0.0
-0.0684 0.0
-0.0688 0.0
-0.0692 0.0
-0.0696 0.0
-0.07 0.0
-0.0704 0.0
-0.0708 0.0
-0.0712 0.0
-0.0716 0.0
-0.072 0.0
-0.0724 0.0
-0.0728 0.0
-0.0732 0.0
-0.0736 0.0
-0.074 0.0
-0.0744 0.0
-0.0748 0.0
-0.0752 0.0
-0.0756 0.0
-0.076 0.0
-0.0764 0.0
-0.0768 0.0
-0.0772 0.0
-0.0776 0.0
-0.078 0.0
-0.0784 0.0
-0.0788 0.0
-0.0792 0.0
-0.0796 0.0
-0.08 0.0
-0.0804 0.0
-0.0808 0.0
-0.0812 0.0
-0.0816 0.0
-0.082 0.0
-0.0824 0.0
-0.0828 1.235e-320
-0.0832 9.8813e-320
-0.0836 6.42285e-319
-0.084 4.15015e-318
-0.0844 2.760592e-317
-0.0848 1.80729213e-316
-0.0852 1.160202004e-315
-0.0856 7.56733176e-315
-0.086 4.800598729e-314
-0.0864 3.0213723662e-313
-0.0868 1.92084774822e-312
-0.0872 1.204518123026e-311
-0.0876 7.72665209846e-311
-0.088 4.74462012419856e-310
-0.0884 2.940155983004097e-309
-0.0888 1.8412437958949806e-308
-0.0892 1.1409840785828035e-307
-0.0896 6.982433953985181e-307
-0.09 4.2996748345815564e-306
-0.0904 2.6033318836810425e-305
-0.0908 1.5830276481606598e-304
-0.0912 9.45308508436037e-304
-0.0916 5.683002762336e-303
-0.092 3.4140332968587937e-302
-0.0924 2.0181463123128557e-301
-0.0928 1.2018582390512461e-300
-0.0932 7.035944109562381e-300
-0.0936 4.1326683527812503e-299
-0.094 2.417159524887511e-298
-0.0944 1.4141628807400085e-297
-0.0948 8.131913096957076e-297
-0.0952 4.6863854968485496e-296
-0.0956 2.6853248375136086e-295
-0.096 1.5373061965330448e-294
-0.0964 8.709032181711095e-294
-0.0968 4.9575305290656095e-293
-0.0972 2.794472319421253e-292
-0.0976 1.5650636588255339e-291
-0.098 8.779552288143077e-291
-0.0984 4.8916873729325717e-290
-0.0988 2.7034405229461805e-289
-0.0992 1.4985756459221599e-288
-0.0996 8.233553426230042e-288
-0.1 4.510803223969179e-287
-0.1004 2.452582334456058e-286
-0.1008 1.3298614989220165e-285
-0.1012 7.193897521309767e-285
-0.1016 3.86749493626723e-284
-0.102 2.069292734844178e-283
-0.1024 1.105441185229442e-282
-0.1028 5.895847378926068e-282
-0.1032 3.116520201931007e-281
-0.1036 1.6420219855890324e-280
-0.104 8.611223140747361e-280
-0.1044 4.501463553564761e-279
-0.1048 2.3522277456556068e-278
-0.1052 1.2192698773054426e-277
-0.1056 6.311431147589356e-277
-0.106 3.2372789410442302e-276
-0.1064 1.664063855283033e-275
-0.1068 8.493389408513235e-275
-0.1072 4.3160179083417984e-274
-0.1076 2.191394303955164e-273
-0.108 1.1047003877478408e-272
-0.1084 5.5481429415535944e-272
-0.1088 2.7822105810431686e-271
-0.1092 1.3819300578201073e-270
-0.1096 6.882571913442108e-270
-0.11 3.4125737322720624e-269
-0.1104 1.6792652206050364e-268
-0.1108 8.238460309632504e-268
-0.1112 4.039657820390914e-267
-0.1116 1.9741432398583854e-266
-0.112 9.545491828161437e-266
-0.1124 4.6166638077623636e-265
-0.1128 2.228265126962659e-264
-0.1132 1.0710278170502613e-263
-0.1136 5.117209025625671e-263
-0.114 2.4367476044976432e-262
-0.1144 1.1583577648671497e-261
-0.1148 5.476176706308568e-261
-0.1152 2.5808538550092796e-260
-0.1156 1.2150759025337486e-259
-0.116 5.664604247248453e-259
-0.1164 2.64510801834312e-258
-0.1168 1.2282551247818711e-257
-0.1172 5.685217732103533e-257
-0.1176 2.6227745082876492e-256
-0.118 1.2043135314104567e-255
-0.1184 5.512483406068395e-255
-0.1188 2.5229382034053193e-254
-0.1192 1.1460367367937122e-253
-0.1196 5.1686470277192384e-253
-0.12 2.3383979554333555e-252
-0.1204 1.049013042504903e-251
-0.1208 4.7046196722415565e-251
-0.1212 2.1022802704829898e-250
-0.1216 9.350416881989979e-250
-0.122 4.147109265605458e-249
-0.1224 1.829589177333656e-248
-0.1228 8.073169529814261e-248
-0.1232 3.5496540139268583e-247
-0.1236 1.5517371915015388e-246
-0.124 6.747487766748643e-246
-0.1244 2.9357336336458245e-245
-0.1248 1.2703757088007337e-244
-0.1252 5.4772278099637195e-244
-0.1256 2.3545118611246704e-243
-0.126 1.0085636635825953e-242
-0.1264 4.307019528858135e-242
-0.1268 1.8341164029307842e-241
-0.1272 7.781518457746615e-241
-0.1276 3.2875335503525493e-240
-0.128 1.3870573369377403e-239
-0.1284 5.824592516229956e-239
-0.1288 2.4375016970140846e-238
-0.1292 1.0173834435455154e-237
-0.1296 4.2266914355608915e-237
-0.13 1.7506975818181865e-236
-0.1304 7.237421726449185e-236
-0.1308 2.9802661091355888e-235
-0.1312 1.2214452301586508e-234
-0.1316 4.999866935655563e-234
-0.132 2.0394009917771275e-233
-0.1324 8.284174246600135e-233
-0.1328 3.360248218243458e-232
-0.1332 1.3557895893758524e-231
-0.1336 5.460333608148641e-231
-0.134 2.189574043131922e-230
-0.1344 8.749987783023039e-230
-0.1348 3.494302322257437e-229
-0.1352 1.3860227624567802e-228
-0.1356 5.507100918800812e-228
-0.136 2.1714651710711556e-227
-0.1364 8.529623459140722e-227
-0.1368 3.3541305917500797e-226
-0.1372 1.313480346781109e-225
-0.1376 5.1113117809193816e-225
-0.138 1.9873905592585458e-224
-0.1384 7.708750772005629e-224
-0.1388 2.978558271518165e-223
-0.1392 1.1468036871702465e-222
-0.1396 4.4076234586669796e-222
-0.14 1.6882235378526758e-221
-0.1404 6.440833109965742e-221
-0.1408 2.4495654903693473e-220
-0.1412 9.300240495967748e-220
-0.1416 3.510196813581044e-219
-0.142 1.3248457091937085e-218
-0.1424 4.978599384380468e-218
-0.1428 1.864893582266543e-217
-0.1432 6.957941920237673e-217
-0.1436 2.5944147961454885e-216
-0.144 9.651128124288356e-216
-0.1444 3.5726210052676277e-215
-0.1448 1.3200338760323994e-214
-0.1452 4.8589914597767465e-214
-0.1456 1.781467995090747e-213
-0.146 6.530108635686534e-213
-0.1464 2.3790164490653563e-212
-0.1468 8.661612391880624e-212
-0.1472 3.1364204565639296e-211
-0.1476 1.1348879125452407e-210
-0.148 4.096668599721551e-210
-0.1484 1.4739451987645005e-209
-0.1488 5.288768454118159e-209
-0.1492 1.8904248844342784e-208
-0.1496 6.737198527507954e-208
-0.15 2.391039629677861e-207
-0.1504 8.488708540324327e-207
-0.1508 2.996383527220318e-206
-0.1512 1.0570689659276193e-205
-0.1516 3.7140220607801315e-205
-0.152 1.3033009963051788e-204
-0.1524 4.552502935378481e-204
-0.1528 1.5852003618184733e-203
-0.1532 5.508223987280075e-203
-0.1536 1.9107920076840903e-202
-0.154 6.609513782069001e-202
-0.1544 2.274811797822829e-201
-0.1548 7.830071353549606e-201
-0.1552 2.6817339561701484e-200
-0.1556 9.170982949401326e-200
-0.156 3.1217128168146357e-199
-0.1564 1.0612258912941727e-198
-0.1568 3.596638169565919e-198
-0.1572 1.2148974540961268e-197
-0.1576 4.1032797433759143e-197
-0.158 1.3789856605599865e-196
-0.1584 4.630414279385441e-196
-0.1588 1.5474724742460834e-195
-0.1592 5.1643620190419116e-195
-0.1596 1.7162211931376685e-194
-0.16 5.703671467214526e-194
-0.1604 1.88635687449676e-193
-0.1608 6.221764211516609e-193
-0.1612 2.044241767268494e-192
-0.1616 6.7116127850997815e-192
-0.162 2.1955777584136495e-191
-0.1624 7.172485091769883e-191
-0.1628 2.336176379110849e-190
-0.1632 7.580850071662521e-190
-0.1636 2.450878448943892e-189
-0.164 7.911622626167038e-189
-0.1644 2.551527176656269e-188
-0.1648 8.183119248931429e-188
-0.1652 2.625730615899883e-187
-0.1656 8.383315360481818e-187
-0.166 2.6772814339065813e-186
-0.1664 8.511579532252356e-186
-0.1668 2.6985240463161468e-185
-0.1672 8.543290682823948e-185
-0.1676 2.6928648740042674e-184
-0.168 8.45817561307318e-184
-0.1684 2.6549606015608202e-183
-0.1688 8.302879006962688e-183
-0.1692 2.5929922781802867e-182
-0.1696 8.086237590609325e-182
-0.17 2.5113806225108825e-181
-0.1704 7.787902480176986e-181
-0.1708 2.405536838206161e-180
-0.1712 7.426527679244034e-180
-0.1716 2.2810850453731436e-179
-0.172 7.00193845853265e-179
-0.1724 2.1420461246254787e-178
-0.1728 6.542153734370771e-178
-0.1732 1.9925122950406147e-177
-0.1736 6.049000640980843e-177
-0.174 1.832465361360147e-176
-0.1744 5.5477808204351336e-176
-0.1748 1.6703292906387477e-175
-0.1752 5.0234860899135973e-175
-0.1756 1.5067772065280116e-174
-0.176 4.512633180030893e-174
-0.1764 1.3479050651119087e-173
-0.1768 4.014570134385657e-173
-0.1772 1.1920186426941382e-172
-0.1776 3.5384075172669596e-172
-0.178 1.0429558755240168e-171
-0.1784 3.079908912831941e-171
-0.1788 9.073697494062162e-171
-0.1792 2.6588800397479377e-170
-0.1796 7.781060180015883e-170
-0.18 2.2718721073989047e-169
-0.1804 6.63713204459925e-169
-0.1808 1.9287136070600758e-168
-0.1812 5.589326802680965e-168
-0.1816 1.6191232136955056e-167
-0.182 4.676502127614648e-167
-0.1824 1.3462776420819933e-166
-0.1828 3.866605806441486e-166
-0.1832 1.107016454358635e-165
-0.1836 3.1728087630312826e-165
-0.184 9.037097335926065e-165
-0.1844 2.5716626435367164e-164
-0.1848 7.299941049798377e-164
-0.1852 2.0675073290954597e-163
-0.1856 5.837257685979149e-163
-0.186 1.6442546380871828e-162
-0.1864 4.630129872520828e-162
-0.1868 1.2995414426576025e-161
-0.1872 3.640349925635384e-161
-0.1876 1.0180403640418307e-160
-0.188 2.832493451544562e-160
-0.1884 7.879278730325646e-160
-0.1888 2.186892115803202e-159
-0.1892 6.047422954296459e-159
-0.1896 1.6696605755916745e-158
-0.19 4.6003759361486245e-158
-0.1904 1.263717541234144e-157
-0.1908 3.471183365480035e-157
-0.1912 9.487495745298745e-157
-0.1916 2.591995711235865e-156
-0.192 7.059617507600173e-156
-0.1924 1.9143071857384644e-155
-0.1928 5.199550246208531e-155
-0.1932 1.4072628267507314e-154
-0.1936 3.7967841071054295e-154
-0.194 1.0226154369486188e-153
-0.1944 2.7511098049399465e-153
-0.1948 7.381810874978018e-153
-0.1952 1.976332558071747e-152
-0.1956 5.271373075709231e-152
-0.196 1.4035042246735866e-151
-0.1964 3.732713506141039e-151
-0.1968 9.905507561066816e-151
-0.1972 2.625928006857674e-150
-0.1976 6.926347561899644e-150
-0.198 1.825904281011809e-149
-0.1984 4.800097750714537e-149
-0.1988 1.2604297326123663e-148
-0.1992 3.299786019965621e-148
-0.1996 8.631886825198569e-148
-0.2 2.2469280719934963e-147
-0.2004 5.847894942064089e-147
-0.2008 1.516014178902231e-146
-0.2012 3.9288416936272208e-146
-0.2016 1.015987296272687e-145
-0.202 2.621603439830812e-145
-0.2024 6.748826479055724e-145
-0.2028 1.7316002876134668e-144
-0.2032 4.4377471239043985e-144
-0.2036 1.1337887860902997e-143
-0.204 2.893882500792901e-143
-0.2044 7.368389623288266e-143
-0.2048 1.870748125217134e-142
-0.2052 4.7515959883829126e-142
-0.2056 1.2004751904722308e-141
-0.206 3.03486397995324e-141
-0.2064 7.636985494629099e-141
-0.2068 1.9242722444068484e-140
-0.2072 4.826556879091965e-140
-0.2076 1.210010570593143e-139
-0.208 3.0222697521688877e-139
-0.2084 7.541632908953869e-139
-0.2088 1.8777268547726467e-138
-0.2092 4.663091104444022e-138
-0.2096 1.1578492501725596e-137
-0.21 2.864482293577567e-137
-0.2104 7.071119851306999e-137
-0.2108 1.7414662867251376e-136
-0.2112 4.2839011063131075e-136
-0.2116 1.0516835122158768e-135
-0.212 2.5757321731613662e-135
-0.2124 6.296741033528368e-135
-0.2128 1.535422048520595e-134
-0.2132 3.7394422608007327e-134
-0.2136 9.07394999579886e-134
-0.214 2.2008774847450018e-133
-0.2144 5.328675942906733e-133
-0.2148 1.2846538165132538e-132
-0.2152 3.091444341714659e-132
-0.2156 7.449513194922298e-132
-0.216 1.788602378228533e-131
-0.2164 4.2804231394867897e-131
-0.2168 1.0230351526279421e-130
-0.2172 2.442316553420311e-130
-0.2176 5.808951884147854e-130
-0.218 1.3783585357573613e-129
-0.2184 3.2687546347454144e-129
-0.2188 7.740873895349716e-129
-0.2192 1.8264604842760315e-128
-0.2196 4.308226918508419e-128
-0.22 1.0151445905645288e-127
-0.2204 2.383090660284416e-127
-0.2208 5.585337598305656e-127
-0.2212 1.3056530773883957e-126
-0.2216 3.051011929089415e-126
-0.222 7.10643328826768e-126
-0.2224 1.653513025912404e-125
-0.2228 3.836214974306117e-125
-0.2232 8.878220848727042e-125
-0.2236 2.0529517458738213e-124
-0.224 4.742400469828285e-124
-0.2244 1.0929097499923064e-123
-0.2248 2.5078333400612497e-123
-0.2252 5.767747173729095e-123
-0.2256 1.3222571647609462e-122
-0.226 3.019276189154614e-122
-0.2264 6.898581782080973e-122
-0.2268 1.5718633191453467e-121
-0.2272 3.570982727280556e-121
-0.2276 8.105980684514115e-121
-0.228 1.8358354546475944e-120
-0.2284 4.141785142616625e-120
-0.2288 9.35672609910665e-120
-0.2292 2.1050110143633085e-119
-0.2296 4.736373560271683e-119
-0.23 1.0644101922901163e-118
-0.2304 2.380094666291387e-118
-0.2308 5.320140125537262e-118
-0.2312 1.188124595746045e-117
-0.2316 2.649152899533925e-117
-0.232 5.885276069653031e-117
-0.2324 1.306594924208994e-116
-0.2328 2.8943974059409904e-116
-0.2332 6.398168071120893e-116
-0.2336 1.413274097985036e-115
-0.234 3.1168483625317726e-115
-0.2344 6.850083959477505e-115
-0.2348 1.5027913545645096e-114
-0.2352 3.2959650322594165e-114
-0.2356 7.221800951078665e-114
-0.236 1.5756912703272148e-113
-0.2364 3.439285440032425e-113
-0.2368 7.477820905706861e-113
-0.2372 1.6235325879977161e-112
-0.2376 3.521287168206171e-112
-0.238 7.610192657631831e-112
-0.2384 1.6443776663534318e-111
-0.2388 3.543004019817857e-111
-0.2392 7.63085075930077e-111
-0.2396 1.6389908503687485e-110
-0.24 3.517105264976901e-110
-0.2404 7.529025239636827e-110
-0.2408 1.6103620315046927e-109
-0.2412 3.433013759936524e-109
-0.2416 7.298574389008042e-109
-0.242 1.5533415427777762e-108
-0.2424 3.3009486967926533e-108
-0.2428 6.991599861851637e-108
-0.2432 1.477007613738727e-107
-0.2436 3.121061563580319e-107
-0.244 6.570214999016837e-107
-0.2444 1.3826316952309625e-106
-0.2448 2.899532859732957e-106
-0.2452 6.079435504000819e-106
-0.2456 1.2711687506387664e-105
-0.246 2.6564010352668596e-105
-0.2464 5.549866222798312e-105
-0.2468 1.1559720123013612e-104
-0.2472 2.4015996918178052e-104
-0.2476 4.9851104194455347e-104
-0.248 1.034295290236593e-103
-0.2484 2.1383275616259467e-103
-0.2488 4.4129429881600875e-103
-0.2492 9.098188096905826e-103
-0.2496 1.870434117908407e-102
-0.25 3.844178785375613e-102
-0.2504 7.877480713120124e-102
-0.2508 1.6133369910683224e-101
-0.2512 3.295818205368016e-101
-0.2516 6.735023274938841e-101
-0.252 1.3711655143828277e-100
-0.2524 2.789047342775385e-100
-0.2528 5.674522796938472e-100
-0.2532 1.1481321680398541e-99
-0.2536 2.3223740587220043e-99
-0.254 4.699319796507631e-99
-0.2544 9.473661493583578e-99
-0.2548 1.9080559307286666e-98
-0.2552 3.834411956807953e-98
-0.2556 7.698284869914919e-98
-0.256 1.5440688991924103e-97
-0.2564 3.080769900642404e-97
-0.2568 6.158286870373999e-97
-0.2572 1.2275595589804563e-96
-0.2576 2.447590177270637e-96
-0.258 4.862152999428721e-96
-0.2584 9.655722911443256e-96
-0.2588 1.911372978309901e-95
-0.2592 3.78020599671085e-95
-0.2596 7.466111171946009e-95
-0.26 1.4704602531631068e-94
-0.2604 2.8948118147257414e-94
-0.2608 5.689591984446173e-94
-0.2612 1.1160647171718435e-93
-0.2616 2.1884918410780943e-93
-0.262 4.274546592350299e-93
-0.2624 8.330752058129604e-93
-0.2628 1.6259160531796437e-92
-0.2632 3.163419521722391e-92
-0.2636 6.146001051189615e-92
-0.264 1.1923041641666912e-91
-0.2644 2.308373616502322e-91
-0.2648 4.459605162998254e-91
-0.2652 8.616553752974826e-91
-0.2656 1.6627181442259396e-90
-0.266 3.1988850531256096e-90
-0.2664 6.1455686263727635e-90
-0.2668 1.1818265561367814e-89
-0.2672 2.265299436468034e-89
-0.2676 4.3325804905464524e-89
-0.268 8.270214934676216e-89
-0.2684 1.5759517615374018e-88
-0.2688 3.006044387391385e-88
-0.2692 5.716855980285637e-88
-0.2696 1.0851537376477154e-87
-0.27 2.0547084098308236e-87
-0.2704 3.8925091530104534e-87
-0.2708 7.353582697755188e-87
-0.2712 1.3881955172026871e-86
-0.2716 2.6152224584004118e-86
-0.272 4.917971410994107e-86
-0.2724 9.219817394781653e-86
-0.2728 1.729576352399817e-85
-0.2732 3.237055806527578e-85
-0.2736 6.058703684923671e-85
-0.274 1.1316624684711913e-84
-0.2744 2.1098767146409953e-84
-0.2748 3.9296031774014682e-84
-0.2752 7.30363180783107e-84
-0.2756 1.3545421065163266e-83
-0.276 2.5103611395309633e-83
-0.2764 4.645569429895835e-83
-0.2768 8.581602499037668e-83
-0.2772 1.5830775520536255e-82
-0.2776 2.915209472938832e-82
-0.278 5.354843708589453e-82
-0.2784 9.825736409430143e-82
-0.2788 1.8032830844109517e-81
-0.2792 3.3010553280300687e-81
-0.2796 6.039243258503234e-81
-0.28 1.1036055632630728e-80
-0.2804 2.010764482404738e-80
-0.2808 3.66337026664743e-80
-0.2812 6.6552475836100195e-80
-0.2816 1.2079050497356414e-79
-0.282 2.1919668550983336e-79
-0.2824 3.971774992826609e-79
-0.2828 7.173841606004716e-79
-0.2832 1.2956769088845503e-78
-0.2836 2.3337479210270597e-78
-0.284 4.195319375223737e-78
-0.2844 7.543451622751039e-78
-0.2848 1.352846599963301e-77
-0.2852 2.4276346119548247e-77
-0.2856 4.337752368056518e-77
-0.286 7.747005427214545e-77
-0.2864 1.3808429324911065e-76
-0.2868 2.4625604045470493e-76
-0.2872 4.384568389366546e-76
-0.2876 7.787569389040058e-76
-0.288 1.3808465233092216e-75
-0.2884 2.4462714512858507e-75
-0.2888 4.329485312090502e-75
-0.2892 7.650536080248114e-75
-0.2896 1.348011276233247e-74
-0.29 2.376174627120203e-74
-0.2904 4.1849983323899714e-74
-0.2908 7.353750162516141e-74
-0.2912 1.2900799351910805e-73
-0.2916 2.259734577895913e-73
-0.292 3.950048654589759e-73
-0.2924 6.900849975533733e-73
-0.2928 1.2033853146956648e-72
-0.2932 2.0956521493942845e-72
-0.2936 3.6455907924471683e-72
-0.294 6.340479065469641e-72
-0.2944 1.0972665318791084e-71
-0.2948 1.9005281270810784e-71
-0.2952 3.2942117307627413e-71
-0.2956 5.689772687784744e-71
-0.296 9.83195099337025e-71
-0.2964 1.6953179848997873e-70
-0.2968 2.9202857247428415e-70
-0.2972 5.013172716281255e-70
-0.2976 8.603348336347867e-70
-0.298 1.474200189897749e-69
-0.2984 2.5210104193586416e-69
-0.2988 4.309376819940184e-69
-0.2992 7.361580374280162e-69
-0.2996 1.2551212564061816e-68
-0.3 2.1380753432904945e-68
-0.3004 3.639412183189007e-68
-0.3008 6.166999478642959e-68
-0.3012 1.0473002190888472e-67
-0.3016 1.771792576494655e-67
-0.302 2.993587112998274e-67
-0.3024 5.0507315052461414e-67
-0.3028 8.518929988150193e-67
-0.3032 1.436744660190354e-66
-0.3036 2.419117177104928e-66
-0.304 4.0572117084248837e-66
-0.3044 6.822152774975361e-66
-0.3048 1.1424038115371383e-65
-0.3052 1.914327767445404e-65
-0.3056 3.1944343238991286e-65
-0.306 5.32760306129764e-65
-0.3064 8.884620172722175e-65
-0.3068 1.4788024329747877e-64
-0.3072 2.4628540807789048e-64
-0.3076 4.0897617825026135e-64
-0.308 6.780704948776025e-64
-0.3084 1.1233655472875344e-63
-0.3088 1.860528678122778e-63
-0.3092 3.067623788467007e-63
-0.3096 5.062090363196651e-63
-0.31 8.348830184660895e-63
-0.3104 1.37512822751812e-62
-0.3108 2.260266570575269e-62
-0.3112 3.713991680035843e-62
-0.3116 6.091426347589478e-62
-0.312 9.977198442176419e-62
-0.3124 1.631498159807846e-61
-0.3128 2.6701379346029467e-61
-0.3132 4.3567684439618624e-61
-0.3136 7.094333119786614e-61
-0.314 1.1569021841518584e-60
-0.3144 1.8787154488773345e-60
-0.3148 3.0464801148477813e-60
-0.3152 4.946970603964878e-60
-0.3156 8.009791339712827e-60
-0.316 1.2961554276890959e-59
-0.3164 2.0920920455452895e-59
-0.3168 3.3773174957281935e-59
-0.3172 5.444337914431249e-59
-0.3176 8.767038203266443e-59
-0.318 1.4094943499609245e-58
-0.3184 2.2636749615631717e-58
-0.3188 3.6252996448852815e-58
-0.3192 5.80474231529129e-58
-0.3196 9.290071903042244e-58
-0.32 1.4824922171124194e-57
-0.3204 2.3723942514801366e-57
-0.3208 3.770332611300675e-57
-0.3212 6.001375268024734e-57
-0.3216 9.552946705528433e-57
-0.322 1.5149726634897692e-56
-0.3224 2.4030381950068543e-56
-0.3228 3.8050832896126057e-56
-0.3232 6.039059645272016e-56
-0.3236 9.539679772184788e-56
-0.324 1.5054288273971508e-55
-0.3244 2.3732583709986913e-55
-0.3248 3.7379183313087434e-55
-0.3252 5.876625424204002e-55
-0.3256 9.225539195063796e-55
-0.326 1.4509281115878307e-54
-0.3264 2.2751054180394363e-54
-0.3268 3.5552586543398675e-54
-0.3272 5.557927767324425e-54
-0.3276 8.682957254855602e-54
-0.328 1.3505823729342132e-53
-0.3284 2.1097959605551185e-53
-0.3288 3.28563689635081e-53
-0.3292 5.105293146687442e-53
-0.3296 7.929652309355914e-53
-0.33 1.2293383701874731e-52
-0.3304 1.9038502283306065e-52
-0.3308 2.9485321737806824e-52
-0.3312 4.5565453434261745e-52
-0.3316 7.038593727764044e-52
-0.332 1.0847233554562019e-51
-0.3324 1.6678506642977063e-51
-0.3328 2.5625545137172443e-51
-0.3332 3.9422956793367483e-51
-0.3336 6.053238904455801e-51
-0.334 9.289140723561188e-51
-0.3344 1.4229375980896327e-50
-0.3348 2.176741664421975e-50
-0.3352 3.323649772802091e-50
-0.3356 5.074059469408309e-50
-0.336 7.7418052206217865e-50
-0.3364 1.1782973151837964e-49
-0.3368 1.795334925238353e-49
-0.3372 2.7260152720894717e-49
-0.3376 4.13550264675959e-49
-0.338 6.269645441943899e-49
-0.3384 9.505269941851252e-49
-0.3388 1.4381614050334647e-48
-0.3392 2.171108816181512e-48
-0.3396 3.279575049010838e-48
-0.34 4.944175917566442e-48
-0.3404 7.458442295828455e-48
-0.3408 1.120920853314162e-47
-0.3412 1.682928283027859e-47
-0.3416 2.526609043255016e-47
-0.342 3.784902677615028e-47
-0.3424 5.668415070304358e-47
-0.3428 8.48994551187876e-47
-0.3432 1.2706192352680268e-46
-0.3436 1.8958846491662966e-46
-0.344 2.8289056712077925e-46
-0.3444 4.219587426639438e-46
-0.3448 6.286323478842281e-46
-0.3452 9.33422762914853e-46
-0.3456 1.3846351674358221e-45
-0.346 2.0573328520964846e-45
-0.3464 3.044899228398797e-45
-0.3468 4.5048045800614024e-45
-0.3472 6.665108037938603e-45
-0.3476 9.840889222114649e-45
-0.348 1.4511545384119986e-44
-0.3484 2.1390923624570277e-44
-0.3488 3.1510310805583233e-44
-0.3492 4.630451702319262e-44
-0.3496 6.806036303699025e-44
-0.35 9.985461306637236e-44
-0.3504 1.465830879563806e-43
-0.3508 2.14723766381362e-43
-0.3512 3.1434067804318887e-43
-0.3516 4.596336501188709e-43
-0.352 6.713793666681748e-43
-0.3524 9.800241305572153e-43
-0.3528 1.4255652799970033e-42
-0.3532 2.072063714048574e-42
-0.3536 3.0125078143486405e-42
-0.354 4.3769741100843446e-42
-0.3544 6.344082236474148e-42
-0.3548 9.194048847855266e-42
-0.3552 1.3310996590559574e-41
-0.3556 1.9256235637681954e-41
-0.356 2.787303273249752e-41
-0.3564 4.017934399678683e-41
-0.3568 5.796234421377479e-41
-0.3572 8.353311690745053e-41
-0.3576 1.2026362615567396e-40
-0.358 1.7306875459212206e-40
-0.3584 2.484524195078507e-40
-0.3588 3.5659727502689226e-40
-0.3592 5.10643224905494e-40
-0.3596 7.310786376251256e-40
-0.36 1.0435374912664584e-39
-0.3604 1.491572894995565e-39
-0.3608 2.1287179116310214e-39
-0.3612 3.036609162037381e-39
-0.3616 4.3240868165232196e-39
-0.362 6.160026059969206e-39
-0.3624 8.757566806994298e-39
-0.3628 1.2437402204825734e-38
-0.3632 1.7649947513057537e-38
-0.3636 2.502185751251108e-38
-0.364 3.5481407597603984e-38
-0.3644 5.014450231830519e-38
-0.3648 7.08213120310136e-38
-0.3652 9.983834389003376e-38
-0.3656 1.4100520324009325e-37
-0.366 1.988962629358405e-37
-0.3664 2.80038502842097e-37
-0.3668 3.932277366662434e-37
-0.3672 5.529602280462498e-37
-0.3676 7.763885314080262e-37
-0.368 1.0882343422984668e-36
-0.3684 1.5244763423571863e-36
-0.3688 2.1294405347632372e-36
-0.3692 2.976745430574406e-36
-0.3696 4.156460894503001e-36
-0.37 5.8103179533273284e-36
-0.3704 8.090830890287717e-36
-0.3708 1.1281405232782471e-35
-0.3712 1.5710351249848377e-35
-0.3716 2.1862033789538167e-35
-0.372 3.0388291262212606e-35
-0.3724 4.2196370181409774e-35
-0.3728 5.857652042325034e-35
-0.3732 8.109708698182393e-35
-0.3736 1.1223018920951276e-34
-0.374 1.5502163738698192e-34
-0.3744 2.1423297239903805e-34
-0.3748 2.9571295281409594e-34
-0.3752 4.075144357538162e-34
-0.3756 5.624984305019694e-34
-0.376 7.726562918292765e-34
-0.3764 1.0604969661906856e-33
-0.3768 1.4580462716032567e-33
-0.3772 2.0016092298921607e-33
-0.3776 2.7433988056058372e-33
-0.378 3.756191849562073e-33
-0.3784 5.132893789955056e-33
-0.3788 7.003539850151892e-33
-0.3792 9.574185716149959e-33
-0.3796 1.304301841299264e-32
-0.38 1.778979512914066e-32
-0.3804 2.4210940847704622e-32
-0.3808 3.297533885279848e-32
-0.3812 4.4892617908826313e-32
-0.3816 6.096465366440093e-32
-0.382 8.275824293703398e-32
-0.3824 1.12252454276506e-31
-0.3828 1.5225625971688577e-31
-0.3832 2.0625632826746673e-31
-0.3836 2.7875858064809214e-31
-0.384 3.763323754957036e-31
-0.3844 5.085566460416042e-31
-0.3848 6.866935719054772e-31
-0.3852 9.257031542395852e-31
-0.3856 1.2467976173290283e-30
-0.386 1.67884718378051e-30
-0.3864 2.2566661790345034e-30
-0.3868 3.033907711434759e-30
-0.3872 4.071123789474427e-30
-0.3876 5.463385874574219e-30
-0.388 7.324390471718276e-30
-0.3884 9.795097282445462e-30
-0.3888 1.3093676021852982e-29
-0.3892 1.7510078558002317e-29
-0.3896 2.3412099171098145e-29
-0.39 3.123472462204237e-29
-0.3904 4.158899569764611e-29
-0.3908 5.543070633810142e-29
-0.3912 7.370993650232262e-29
-0.3916 9.789502864495525e-29
-0.392 1.2992384884319472e-28
-0.3924 1.7219374452143323e-28
-0.3928 2.2792925009203553e-28
-0.3932 3.020721476638943e-28
-0.3936 3.9951399740313995e-28
-0.394 5.2847559435666275e-28
-0.3944 6.976052971378495e-28
-0.3948 9.200140857757772e-28
-0.3952 1.2139504310973905e-27
-0.3956 1.599261475398548e-27
-0.396 2.1073240740155764e-27
-0.3964 2.76925117204868e-27
-0.3968 3.6316134414164786e-27
-0.3972 4.7778604711880275e-27
-0.3976 6.261620416401261e-27
-0.398 8.204018781623613e-27
-0.3984 1.0740971395965892e-26
-0.3988 1.4047760755431257e-26
-0.3992 1.8362582834457302e-26
-0.3996 2.3985977279255298e-26
-0.4 3.1284082120884505e-26
-0.4004 4.0844299078942824e-26
-0.4008 5.323690908161911e-26
-0.4012 6.937722499380832e-26
-0.4016 9.034362633723304e-26
-0.402 1.1742615566498282e-25
-0.4024 1.5252621244881145e-25
-0.4028 1.9806225101027393e-25
-0.4032 2.56518433948745e-25
-0.4036 3.323925171628264e-25
-0.404 4.308171170879083e-25
-0.4044 5.572190769729096e-25
-0.4048 7.197482256700337e-25
-0.4052 9.283837145922343e-25
-0.4056 1.1981534198398783e-24
-0.406 1.5460637020034654e-24
-0.4064 1.9924256269185202e-24
-0.4068 2.5688657387935068e-24
-0.4072 3.3044464778963198e-24
-0.4076 4.2545037806085625e-24
-0.408 5.469950336658215e-24
-0.4084 7.01390223229431e-24
-0.4088 8.990389569836916e-24
-0.4092 1.15324084258938e-23
-0.4096 1.4744022850955163e-23
-0.41 1.8925004898245885e-23
-0.4104 2.4194583141012467e-23
-0.4108 3.089057259428221e-23
-0.4112 3.941353667519367e-23
-0.4116 5.0158106362876155e-23
-0.412 6.389707934677589e-23
-0.4124 8.138074143422302e-23
-0.4128 1.0375368624700523e-22
-0.4132 1.3187537131141685e-22
-0.4136 1.675318550366093e-22
-0.414 2.122138244307593e-22
-0.4144 2.696650502979325e-22
-0.4148 3.4149259848364805e-22
-0.4152 4.322673656661208e-22
-0.4156 5.466095005275035e-22
-0.416 6.927617761229187e-22
-0.4164 8.752666869070035e-22
-0.4168 1.1032435708635386e-21
-0.4172 1.390784228240951e-21
-0.4176 1.7520908732004404e-21
-0.418 2.2075176139073112e-21
-0.4184 2.7785395761397255e-21
-0.4188 3.49562414015904e-21
-0.4192 4.387541361736654e-21
-0.4196 5.509021021782201e-21
-0.42 6.915632544269702e-21
-0.4204 8.686339295162424e-21
-0.4208 1.0903359203724082e-20
-0.4212 1.364831048141871e-20
-0.4216 1.706061568864649e-20
-0.422 2.1324201771554837e-20
-0.4224 2.661523146243735e-20
-0.4228 3.323039127063112e-20
-0.4232 4.148978746821295e-20
-0.4236 5.169632716126447e-20
-0.424 6.43974128217879e-20
-0.4244 8.021816142487172e-20
-0.4248 9.969144144616027e-20
-0.4252 1.2411547283739502e-19
-0.4256 1.5376874180689848e-19
-0.426 1.9077835280319453e-19
-0.4264 2.365746793577746e-19
-0.4268 2.934796124227848e-19
-0.4272 3.6290959033965444e-19
-0.4276 4.4945266106893205e-19
-0.428 5.556314225549028e-19
-0.4284 6.864504746631842e-19
-0.4288 8.480979595971133e-19
-0.4292 1.0466640779863906e-18
-0.4296 1.2892351629883049e-18
-0.43 1.5910116203069164e-18
-0.4304 1.956794956300733e-18
-0.4308 2.406287735529766e-18
-0.4312 2.9628923701938544e-18
-0.4316 3.6364358672586485e-18
-0.432 4.476321330872089e-18
-0.4324 5.4888771645923294e-18
-0.4328 6.730153412629037e-18
-0.4332 8.257955204775527e-18
-0.4336 1.0116387303746577e-17
-0.434 1.2354271614312905e-17
-0.4344 1.5115250657617834e-17
-0.4348 1.8485550393397812e-17
-0.4352 2.251097132025512e-17
-0.4356 2.7473771102244825e-17
-0.436 3.3555310608974405e-17
-0.4364 4.0866268172192574e-17
-0.4368 4.9813698673485955e-17
-0.4372 6.057124924271914e-17
-0.4376 7.359878743583487e-17
-0.438 8.94542734912145e-17
-0.4384 1.085648064883421e-16
-0.4388 1.3191471181226953e-16
-0.4392 1.6000093480867312e-16
-0.4396 1.9423861636799974e-16
-0.44 2.354503972222657e-16
-0.4404 2.853330947153665e-16
-0.4408 3.4526449819015177e-16
-0.4412 4.17490233106167e-16
-0.4416 5.046372065292761e-16
-0.442 6.085210247513027e-16
-0.4424 7.329465500905185e-16
-0.4428 8.847069257994444e-16
-0.4432 1.0660242860288412e-15
-0.4436 1.286707414325335e-15
-0.444 1.548123218025479e-15
-0.4444 1.8615109310527005e-15
-0.4448 2.2380680077494233e-15
-0.4452 2.6890394135655765e-15
-0.4456 3.2277817118919396e-15
-0.446 3.867778864017168e-15
-0.4464 4.634348580269398e-15
-0.4468 5.5512560079610235e-15
-0.4472 6.640950792586579e-15
-0.4476 7.933130890104991e-15
-0.448 9.46237725549217e-15
-0.4484 1.1307147979606924e-14
-0.4488 1.3506017238714384e-14
-0.4492 1.607102985218922e-14
-0.4496 1.9162756708390157e-14
-0.45 2.282860531115223e-14
-0.4504 2.7135273097157795e-14
-0.4508 3.226543388613033e-14
-0.4512 3.8358602176639133e-14
-0.4516 4.545278758329132e-14
-0.452 5.395951556374473e-14
-0.4524 6.404568956592984e-14
-0.4528 7.607200220146256e-14
-0.4532 9.01919112810622e-14
-0.4536 1.0691616080373493e-13
-0.454 1.2648187633169463e-13
-0.4544 1.4939436719669444e-13
-0.4548 1.7652280229960279e-13
-0.4552 2.0883368420254055e-13
-0.4556 2.4605798325043863e-13
-0.456 2.9092814803568126e-13
-0.4564 3.4313409137963087e-13
-0.4568 4.0406212803015167e-13
-0.4572 4.760830861020179e-13
-0.4576 5.598765758734579e-13
-0.458 6.574912268158211e-13
-0.4584 7.731057928907287e-13
-0.4588 9.069428906544733e-13
-0.4592 1.0645965193993597e-12
-0.4596 1.2492496928052008e-12
-0.46 1.4651892921299501e-12
-0.4604 1.7187789194247119e-12
-0.4608 2.013512960995518e-12
-0.4612 2.360223724211058e-12
-0.4616 2.7583666212660124e-12
-0.462 3.224419855457698e-12
-0.4624 3.767874433412676e-12
-0.4628 4.4012475704358576e-12
-0.4632 5.139519690352701e-12
-0.4636 5.993315555190002e-12
-0.464 6.987370991498206e-12
-0.4644 8.148467330407836e-12
-0.4648 9.491036329707452e-12
-0.4652 1.1041301678694726e-11
-0.4656 1.2838766359980352e-11
-0.466 1.4893722045430106e-11
-0.4664 1.730510111150386e-11
-0.4668 2.005165869282492e-11
-0.4672 2.329968255633055e-11
-0.4676 2.701290504683978e-11
-0.468 3.132421860265425e-11
-0.4684 3.6302594974989954e-11
-0.4688 4.1966728598641094e-11
-0.4692 4.85445437195848e-11
-0.4696 5.6161664073953276e-11
-0.47 6.497747983280661e-11
-0.4704 7.514022615668088e-11
-0.4708 8.669169491378204e-11
-0.4712 1.0016822365656782e-10
-0.4716 1.1534337947164751e-10
-0.472 1.329284101709873e-10
-0.4724 1.5315249461647247e-10
-0.4728 1.7608688777054958e-10
-0.4732 2.025338962061646e-10
-0.4736 2.3306384025546523e-10
-0.474 2.679617709253128e-10
-0.4744 3.078148983481835e-10
-0.4748 3.5342163935072895e-10
-0.4752 4.052089564010256e-10
-0.4756 4.642547739182809e-10
-0.476 5.311938149691286e-10
-0.4764 6.078220127065471e-10
-0.4768 6.95305552942569e-10
-0.4772 7.950382907792957e-10
-0.4776 9.095173397732267e-10
-0.478 1.0391481043378767e-09
-0.4784 1.1875398125954725e-09
-0.4788 1.355304378471581e-09
-0.4792 1.5466843898870508e-09
-0.4796 1.7670813540452874e-09
-0.48 2.0087652551670648e-09
-0.4804 2.288038012069229e-09
-0.4808 2.6056314635015396e-09
-0.4812 2.9595504018428206e-09
-0.4816 3.3774001028521448e-09
-0.482 3.835105354988547e-09
-0.4824 4.3547441520936275e-09
-0.4828 4.946296275884199e-09
-0.4832 5.599174460956293e-09
-0.4836 6.356623562389769e-09
-0.484 7.1978023546264965e-09
-0.4844 8.151037097636386e-09
-0.4848 9.216763043952862e-09
-0.4852 1.0426819362747668e-08
-0.4856 1.1775349494196258e-08
-0.486 1.3280012875111875e-08
-0.4864 1.5013765734707302e-08
-0.4868 1.690786229624634e-08
-0.4872 1.907714516353013e-08
-0.4876 2.151521326223931e-08
-0.488 2.4271356328918597e-08
-0.4884 2.732377963057385e-08
-0.4888 3.079286302813814e-08
-0.4892 3.461904075117572e-08
-0.4896 3.893651500443665e-08
-0.49 4.367808364619758e-08
-0.4904 4.8971922984894744e-08
-0.4908 5.504101717692642e-08
-0.4912 6.17947120215689e-08
-0.4916 6.933874055441814e-08
-0.492 7.776288094687739e-08
-0.4924 8.720764219617169e-08
-0.4928 9.756386874657579e-08
-0.4932 1.0914597820496019e-07
-0.4936 1.2224013925057957e-07
-0.494 1.3657796867858717e-07
-0.4944 1.5252759828689803e-07
-0.4948 1.704068692180553e-07
-0.4952 1.9049301736129493e-07
-0.4956 2.1253861499795974e-07
-0.496 2.3740732350460837e-07
-0.4964 2.6439717710436943e-07
-0.4968 2.941576116502884e-07
-0.4972 3.2737836577233153e-07
-0.4976 3.643862160142e-07
-0.498 4.056927387225036e-07
-0.4984 4.5091330612728436e-07
-0.4988 5.00273241784829e-07
-0.4992 5.55034058254849e-07
-0.4996 6.160382159464827e-07
-0.5 6.841689045271095e-07
-0.5004 7.583075650100609e-07
-0.5008 8.413847701957725e-07
-0.5012 9.32129007815857e-07
-0.5016 1.0340103951725585e-06
-0.502 1.146050993460967e-06
-0.5024 1.2698146611089054e-06
-0.5028 1.404299315225801e-06
-0.5032 1.5536045932862377e-06
-0.5036 1.7201394763156302e-06
-0.504 1.899249859924697e-06
-0.5044 2.099344458351744e-06
-0.5048 2.3158528169037173e-06
-0.5052 2.557896008355175e-06
-0.5056 2.822317447524105e-06
-0.506 3.106386728473304e-06
-0.5064 3.425902843808914e-06
-0.5068 3.777715551971411e-06
-0.5072 4.163546823209225e-06
-0.5076 4.574013147992467e-06
-0.508 5.039585901261849e-06
-0.5084 5.53689004521786e-06
-0.5088 6.082065686096025e-06
-0.5092 6.678392179542857e-06
-0.5096 7.329053272011505e-06
-0.51 8.032844583301688e-06
-0.5104 8.803301655048988e-06
-0.5108 9.648645589537443e-06
-0.5112 1.0573443998807703e-05
-0.5116 1.1559479374822675e-05
-0.512 1.2623781331104724e-05
-0.5124 1.3799705066092942e-05
-0.5128 1.5093011306196613e-05
-0.5132 1.6479526413197933e-05
-0.5136 1.8041558446526525e-05
-0.514 1.969516593668265e-05
-0.5144 2.146849823875908e-05
-0.5148 2.347092675742925e-05
-0.5152 2.5574545157177677e-05
-0.5156 2.7869632054931793e-05
-0.516 3.0367885524288824e-05
-0.5164 3.3132034590981515e-05
-0.5168 3.605901541645827e-05
-0.5172 3.9302281912424615e-05
-0.5176 4.273619346386898e-05
-0.518 4.648855384260886e-05
-0.5184 5.053045836560419e-05
-0.5188 5.475109418487071e-05
-0.5192 5.948429627245064e-05
-0.5196 6.448163699900279e-05
-0.52 6.997161662262961e-05
-0.5204 7.588216936114435e-05
-0.5208 8.213889953449109e-05
-0.5212 8.903878302070094e-05
-0.5216 9.625255488072134e-05
-0.522 0.00010408948110002458
-0.5224 0.00011265686509495617
-0.5228 0.00012188788249839407
-0.5232 0.00013158515225310792
-0.5236 0.00014199702171253307
-0.524 0.0001534281466081947
-0.5244 0.0001656674990209124
-0.5248 0.0001789893805391281
-0.5252 0.00019343769815950823
-0.5256 0.00020848375852441174
-0.526 0.00022430898609891023
-0.5264 0.00024171025794961256
-0.5268 0.0002604068404599012
-0.5272 0.00028039760994164384
-0.5276 0.0003012328501942779
-0.528 0.00032478865313073917
-0.5284 0.000349324426604304
-0.5288 0.00037481218974244374
-0.5292 0.0004020544192928185
-0.5296 0.00043150664039408386
-0.53 0.0004635912546851676
-0.5304 0.0004962984036410141
-0.5308 0.0005319306118297229
-0.5312 0.0005705167670628074
-0.5316 0.0006122245507664759
-0.532 0.0006543613146336463
-0.5324 0.0007011056283913775
-0.5328 0.0007505304026095644
-0.5332 0.0008014935887697409
-0.5336 0.0008576208849789884
-0.534 0.0009186499756154181
-0.5344 0.000982222548459914
-0.5348 0.0010487222695501949
-0.5352 0.0011180453505904462
-0.5356 0.0011931123473080526
-0.536 0.0012743804255757035
-0.5364 0.0013594894407059463
-0.5368 0.0014480161011005005
-0.5372 0.0015464122540072246
-0.5376 0.0016467300494958023
-0.538 0.001750497538686176
-0.5384 0.001862001460267769
-0.5388 0.0019803910812872137
-0.5392 0.0021046732986175283
-0.5396 0.0022329277149283396
-0.54 0.0023697796094216414
-0.5404 0.0025168237021466755
-0.5408 0.002668608989925708
-0.5412 0.002832436868537044
-0.5416 0.00300802182345282
-0.542 0.003189712227403487
-0.5424 0.003383680255024023
-0.5428 0.003576690807657786
-0.5432 0.003791932307494799
-0.5436 0.0040161182738496825
-0.544 0.0042488398733721115
-0.5444 0.004500389170908045
-0.5448 0.004762832755894177
-0.5452 0.00503034415462798
-0.5456 0.005325614170553081
-0.546 0.005622938978821191
-0.5464 0.005934004337144493
-0.5468 0.006261397402176943
-0.5472 0.0065981859556623985
-0.5476 0.006968955222029159
-0.548 0.007357688165202626
-0.5484 0.00775799557715153
-0.5488 0.00817453674899614
-0.5492 0.008602096961191692
-0.5496 0.009050473027611014
-0.55 0.009518832148640397
-0.5504 0.010000791432398974
-0.5508 0.01050917357911952
-0.5512 0.01104966925249972
-0.5516 0.01159057119308383
-0.552 0.012173671940657035
-0.5524 0.01279593700311402
-0.5528 0.013406376526510989
-0.5532 0.014097045259093346
-0.5536 0.01478314933355358
-0.554 0.01548484775568598
-0.5544 0.016258192401404695
-0.5548 0.017056036791554496
-0.5552 0.017883731434604616
-0.5556 0.018721346166803855
-0.556 0.019615136952999688
-0.5564 0.02051479940458166
-0.5568 0.02146750908917262
-0.5572 0.022446391266722505
-0.5576 0.023511088669597856
-0.558 0.024567343311858048
-0.5584 0.025648475850439386
-0.5588 0.0268046013392156
-0.5592 0.02793070969783883
-0.5596 0.029121221163820512
-0.56 0.03032300046447954
-0.5604 0.03160173086063983
-0.5608 0.03294335929127979
-0.5612 0.034383558028916565
-0.5616 0.03589722724276626
-0.562 0.03738668595811018
-0.5624 0.03888753333202476
-0.5628 0.04050869978267672
-0.5632 0.042274056231159325
-0.5636 0.04394554980892808
-0.564 0.04570445895280525
-0.5644 0.047519071846329385
-0.5648 0.04933509983557735
-0.5652 0.051217085857038235
-0.5656 0.053358284711488936
-0.566 0.05544728968916273
-0.5664 0.05756971325372903
-0.5668 0.05977283422314353
-0.5672 0.06197590198488709
-0.5676 0.0642568011435334
-0.568 0.06666623280569532
-0.5684 0.0691596825628893
-0.5688 0.07157661526008764
-0.5692 0.07414674099791976
-0.5696 0.07686843679500857
-0.57 0.07965748885655402
-0.5704 0.08226874760816393
-0.5708 0.08514340440692081
-0.5712 0.08800120918191172
-0.5716 0.09113457627338674
-0.572 0.09406975778574107
-0.5724 0.09723684063545575
-0.5728 0.1006514780359581
-0.5732 0.10358579245891963
-0.5736 0.10690488695516115
-0.574 0.11037494676833201
-0.5744 0.11365788097199023
-0.5748 0.11706529245509657
-0.5752 0.1205584092603919
-0.5756 0.12424946242192117
-0.576 0.1280325030395401
-0.5764 0.13171120101533032
-0.5768 0.13558523953808133
-0.5772 0.1394445062309404
-0.5776 0.1433404280498275
-0.578 0.14777326642381225
-0.5784 0.15207266100961098
-0.5788 0.15597103641237123
-0.5792 0.16039475827061278
-0.5796 0.16441163610214143
-0.58 0.1688828959665291
-0.5804 0.1734051381078601
-0.5808 0.1777365837443538
-0.5812 0.1824639379065678
-0.5816 0.18719016235595473
-0.582 0.19224805188432942
-0.5824 0.1966412742282122
-0.5828 0.20112485086954532
-0.5832 0.20597863479984135
-0.5836 0.21125837861367514
-0.584 0.216260212580404
-0.5844 0.22174160845571475
-0.5848 0.22693202567949528
-0.5852 0.23239428150432168
-0.5856 0.23742495164802707
-0.586 0.2424428576873048
-0.5864 0.2477143282228373
-0.5868 0.25349848622882976
-0.5872 0.25878804364592034
-0.5876 0.26406756719526553
-0.588 0.26957289178001276
-0.5884 0.2748550813899536
-0.5888 0.2804299594288014
-0.5892 0.28587271045781387
-0.5896 0.2921331198843702
-0.59 0.2982681912206372
-0.5904 0.3040594134933785
-0.5908 0.3097569736971745
-0.5912 0.315011254455033
-0.5916 0.3209244339869534
-0.592 0.32688026064783166
-0.5924 0.33292156290303654
-0.5928 0.33898323288761295
-0.5932 0.3446754169644315
-0.5936 0.35058466323693366
-0.594 0.35664029808110076
-0.5944 0.36209851997343545
-0.5948 0.367962860311245
-0.5952 0.37390227054157327
-0.5956 0.37957819318377006
-0.596 0.3858070938450824
-0.5964 0.3918367043147662
-0.5968 0.39806900441119364
-0.5972 0.40383982350521663
-0.5976 0.40970618470048004
-0.598 0.41514066396654553
-0.5984 0.42140007214196096
-0.5988 0.42678019523252764
-0.5992 0.4319171143918143
-0.5996 0.4366016678910041
-0.6 0.4425216090347187
-0.6004 0.44831563983425676
-0.6008 0.4536698547113787
-0.6012 0.4592310010913381
-0.6016 0.46475805242506785
-0.602 0.4704008762198831
-0.6024 0.4757678326964749
-0.6028 0.4803239459373156
-0.6032 0.4853286500838508
-0.6036 0.4912127040391056
-0.604 0.49643588052548016
-0.6044 0.5005264644123889
-0.6048 0.5063817503652887
-0.6052 0.5116513679103382
-0.6056 0.5157115489113351
-0.606 0.5206696526182732
-0.6064 0.5248132947331161
-0.6068 0.5299123457489748
-0.6072 0.5345369170319386
-0.6076 0.5390428328427525
-0.608 0.5431175338085361
-0.6084 0.5468925271554251
-0.6088 0.551399840543453
-0.6092 0.5552155030863509
-0.6096 0.5596888724796416
-0.61 0.5624095211217286
-0.6104 0.5661724050717626
-0.6108 0.5701264583669585
-0.6112 0.5730073430722684
-0.6116 0.5763860888141642
-0.612 0.5800875641764022
-0.6124 0.5833103169273696
-0.6128 0.5844607493159002
-0.6132 0.5872929045478998
-0.6136 0.5895704798526239
-0.614 0.592932448942799
-0.6144 0.5946531775837088
-0.6148 0.5971902378374637
-0.6152 0.5983976894411005
-0.6156 0.6008160441665796
-0.616 0.6037738446098978
-0.6164 0.6051413065519159
-0.6168 0.6068178257139876
-0.6172 0.6086238552222515
-0.6176 0.6097677623124665
-0.618 0.6102153754057675
-0.6184 0.6110871814726276
-0.6188 0.6121204599611728
-0.6192 0.6127125593847425
-0.6196 0.6146309786803121
-0.62 0.6148365512893954
-0.6204 0.6157269266767416
-0.6208 0.6163710133292712
-0.6212 0.6161898147318421
-0.6216 0.6161868253360497
-0.622 0.6164131514073921
-0.6224 0.6154554815517169
-0.6228 0.6166827584734306
-0.6232 0.6160396384463885
-0.6236 0.6157298723137733
-0.624 0.6145420558640342
-0.6244 0.6146820122884277
-0.6248 0.6145792237697895
-0.6252 0.613549122180533
-0.6256 0.6128737400143415
-0.626 0.6115439576145856
-0.6264 0.6104049274575398
-0.6268 0.6071857144507986
-0.6272 0.6058446036592176
-0.6276 0.6046522671673286
-0.628 0.603178690290229
-0.6284 0.6012695959624978
-0.6288 0.5998108607364064
-0.6292 0.5987988099913989
-0.6296 0.5977944817707608
-0.63 0.5962372929402785
-0.6304 0.5941686203065751
-0.6308 0.592170170560764
-0.6312 0.5902732262626902
-0.6316 0.5885931200748296
-0.632 0.5851600328148711
-0.6324 0.582493166704059
-0.6328 0.5785724755978816
-0.6332 0.5756735967764264
-0.6336 0.5725206985117084
-0.634 0.5688776910927554
-0.6344 0.5654328637524441
-0.6348 0.5624109086403192
-0.6352 0.5601488387130181
-0.6356 0.5560127648559811
-0.636 0.5519748760806533
-0.6364 0.5475893565817569
-0.6368 0.5444942121245561
-0.6372 0.539963000271959
-0.6376 0.5364914847705609
-0.638 0.5340985433646646
-0.6384 0.5288284210392531
-0.6388 0.5257518125685572
-0.6392 0.5224107255165789
-0.6396 0.5190895215004567
-0.64 0.5137533401581043
-0.6404 0.5103688682502698
-0.6408 0.5053269253965127
-0.6412 0.5010119977405136
-0.6416 0.49588023799866104
-0.642 0.491256260464745
-0.6424 0.48662872254997547
-0.6428 0.4817430448402206
-0.6432 0.47740580779379455
-0.6436 0.47305025916648075
-0.644 0.46829224238267253
-0.6444 0.4636119230077563
-0.6448 0.45871190563304254
-0.6452 0.4538187154949331
-0.6456 0.4500009768226634
-0.646 0.4442426666890929
-0.6464 0.4391221093618524
-0.6468 0.4329888174241682
-0.6472 0.4284398690087759
-0.6476 0.4240228910629451
-0.648 0.4191160940902824
-0.6484 0.4142617107024742
-0.6488 0.40986635471361627
-0.6492 0.4052083286907486
-0.6496 0.4003313123519128
-0.65 0.39495606828924695
-0.6504 0.3908651748710746
-0.6508 0.3862086427422598
-0.6512 0.38129439736503395
-0.6516 0.3759293551523921
-0.652 0.370989401593048
-0.6524 0.36672800084777457
-0.6528 0.36216132650837024
-0.6532 0.35693186997188586
-0.6536 0.35175621783999145
-0.654 0.3469829828872256
-0.6544 0.34280110222330346
-0.6548 0.33839828417925333
-0.6552 0.3331809967773108
-0.6556 0.3285491742924126
-0.656 0.3236298080042833
-0.6564 0.31889204785506214
-0.6568 0.31465712668431695
-0.6572 0.309859804774529
-0.6576 0.3053248343839863
-0.658 0.3006385043421163
-0.6584 0.2958479463321368
-0.6588 0.29100483319139797
-0.6592 0.28627301975339065
-0.6596 0.2819718877625782
-0.66 0.27728426970309644
-0.6604 0.27237149466264327
-0.6608 0.26763311061486506
-0.6612 0.26315889920805074
-0.6616 0.258964007662738
-0.662 0.2547233614327798
-0.6624 0.2505649865583136
-0.6628 0.24615620047135467
-0.6632 0.24225942066914938
-0.6636 0.2384830731559247
-0.664 0.23436498505169023
-0.6644 0.23017942204395925
-0.6648 0.22613000894096597
-0.6652 0.22233370997382115
-0.6656 0.2179971907185505
-0.666 0.21461371748472982
-0.6664 0.21069480382043027
-0.6668 0.20691704786464024
-0.6672 0.2035266660775337
-0.6676 0.19955530654456424
-0.668 0.19587756463982792
-0.6684 0.1923126210367615
-0.6688 0.18847496303641928
-0.6692 0.18518756035386508
-0.6696 0.1817582772796376
-0.67 0.17815504064642143
-0.6704 0.17506599849338544
-0.6708 0.17181233104128882
-0.6712 0.1688352943821023
-0.6716 0.1654172013698768
-0.672 0.16217200537157123
-0.6724 0.1586828651074609
-0.6728 0.15552399051178423
-0.6732 0.15292468570485612
-0.6736 0.14999300505839092
-0.674 0.14715656353957066
-0.6744 0.14409256801210726
-0.6748 0.14129697107391093
-0.6752 0.13826150040379628
-0.6756 0.1354392224132313
-0.676 0.13257231625711235
-0.6764 0.12978018004248332
-0.6768 0.1271617905189696
-0.6772 0.12441912188258324
-0.6776 0.12198052473954954
-0.678 0.11933866225327203
-0.6784 0.11671616416090502
-0.6788 0.11446195731366676
-0.6792 0.1120548243947445
-0.6796 0.1097028022628595
-0.68 0.10744984397261144
-0.6804 0.10515110401400048
-0.6808 0.1028875294185992
-0.6812 0.10055443288858047
-0.6816 0.09859933126270841
-0.682 0.09660960895364117
-0.6824 0.09446203534288349
-0.6828 0.09251032358262637
-0.6832 0.09029293623934156
-0.6836 0.08842320333514403
-0.684 0.08658914674377247
-0.6844 0.084675676429637
-0.6848 0.08291309060511111
-0.6852 0.08114311531743276
-0.6856 0.0791509735999596
-0.686 0.07742138296267594
-0.6864 0.07560844914190495
-0.6868 0.07403734309346975
-0.6872 0.07245603192660155
-0.6876 0.07078853663018596
-0.688 0.0692221913648601
-0.6884 0.06770384095403015
-0.6888 0.06606576647575155
-0.6892 0.06450073366945196
-0.6896 0.06304191078670694
-0.69 0.0616346920695967
-0.6904 0.05999703535148706
-0.6908 0.058586845331272064
-0.6912 0.057260884977722776
-0.6916 0.055903558436234756
-0.692 0.05461442494758053
-0.6924 0.05338753446381289
-0.6928 0.05212664213896638
-0.6932 0.05109063231649364
-0.6936 0.04995582576396388
-0.694 0.048799617812196355
-0.6944 0.047648231753941624
-0.6948 0.04645658403977296
-0.6952 0.04538790904806071
-0.6956 0.04415609935495982
-0.696 0.043062723213381233
-0.6964 0.04211239119718484
-0.6968 0.04114310067199429
-0.6972 0.04011719674235644
-0.6976 0.03916191120003542
-0.698 0.038206221129220445
-0.6984 0.03727221371852036
-0.6988 0.03638937717707803
-0.6992 0.03551846036102766
-0.6996 0.03460222507019788
-0.7 0.033701394547306515
-0.7004 0.03285153921858616
-0.7008 0.031972178188864935
-0.7012 0.031164145019509388
-0.7016 0.030396356725396093
-0.702 0.029611467310846313
-0.7024 0.028834238083621185
-0.7028 0.028139375623533806
-0.7032 0.02747690710394366
-0.7036 0.026785597223591258
-0.704 0.026127788189458486
-0.7044 0.025497443968062455
-0.7048 0.024865558781657523
-0.7052 0.024232016394883964
-0.7056 0.023637760047759877
-0.706 0.023015017813640383
-0.7064 0.022447763443090518
-0.7068 0.02191567568101357
-0.7072 0.021313413346094094
-0.7076 0.02074913750181137
-0.708 0.020245756447555226
-0.7084 0.019727041605297802
-0.7088 0.019224566211884595
-0.7092 0.018728994802707805
-0.7096 0.018257960605054635
-0.71 0.017830073782776984
-0.7104 0.01735142431233696
-0.7108 0.01691419343981796
-0.7112 0.016455864299316773
-0.7116 0.016035485571625402
-0.712 0.015603519425758827
-0.7124 0.015212236058146918
-0.7128 0.014838185652936675
-0.7132 0.01442180379484578
-0.7136 0.014083128127225526
-0.714 0.01365906031413265
-0.7144 0.01329019971408682
-0.7148 0.012981633279416475
-0.7152 0.012646091208174169
-0.7156 0.012327851301108049
-0.716 0.011978155543107842
-0.7164 0.011662701037817778
-0.7168 0.011390469684692995
-0.7172 0.011075747358887765
-0.7176 0.010785404361037464
-0.718 0.010473279462170549
-0.7184 0.010191396694319822
-0.7188 0.009947525533539833
-0.7192 0.009680647194145584
-0.7196 0.009422935577824742
-0.72 0.009196221564508935
-0.7204 0.008968318109330213
-0.7208 0.008716174245093265
-0.7212 0.008484293224004708
-0.7216 0.008252732556815714
-0.722 0.008028597875922978
-0.7224 0.007820923001951823
-0.7228 0.0076018185904413674
-0.7232 0.0074002836492063975
-0.7236 0.007190201944451071
-0.724 0.006986288666880217
-0.7244 0.006797973185437684
-0.7248 0.006610467263769211
-0.7252 0.0064228886782745805
-0.7256 0.006246133535164886
-0.726 0.006078094238409869
-0.7264 0.005927123857682095
-0.7268 0.005766777757758237
-0.7272 0.005623272635856439
-0.7276 0.005478144845527494
-0.728 0.005331970671322194
-0.7284 0.005182342775108191
-0.7288 0.005052472690022385
-0.7292 0.004909322831878178
-0.7296 0.004782806849473154
-0.73 0.004650533762123917
-0.7304 0.004529423841555962
-0.7308 0.0044173779122810225
-0.7312 0.004297765111539717
-0.7316 0.00418310584208451
-0.732 0.004069339627225001
-0.7324 0.003960987543360193
-0.7328 0.0038579646933051925
-0.7332 0.003751279633897203
-0.7336 0.0036500768947918833
-0.734 0.0035538536568004405
-0.7344 0.0034594452634523517
-0.7348 0.003367767337881092
-0.7352 0.0032788501620100163
-0.7356 0.003192276124826348
-0.736 0.003112637311309198
-0.7364 0.0030308918857687023
-0.7368 0.002949462381917419
-0.7372 0.0028712351226102143
-0.7376 0.002798941688668218
-0.738 0.0027273782315635183
-0.7384 0.002654860571437563
-0.7388 0.002589176567938669
-0.7392 0.002523855037640066
-0.7396 0.0024599297158972877
-0.74 0.002392121567399411
-0.7404 0.002322701401709923
-0.7408 0.002264026826769307
-0.7412 0.0022008049390189804
-0.7416 0.0021422595514805284
-0.742 0.002087768130544314
-0.7424 0.002031160082244471
-0.7428 0.0019793257061807186
-0.7432 0.001927117218053408
-0.7436 0.0018712139446761557
-0.744 0.0018212701456019236
-0.7444 0.0017707206625509823
-0.7448 0.0017201391306801627
-0.7452 0.0016780716175288592
-0.7456 0.0016330940372161302
-0.746 0.001587455501380573
-0.7464 0.0015431642692946331
-0.7468 0.0015015230553001625
-0.7472 0.0014612191137155345
-0.7476 0.0014237454983195264
-0.748 0.0013865587292155963
-0.7484 0.0013506541198520918
-0.7488 0.0013134533444388635
-0.7492 0.001280596212962808
-0.7496 0.0012477942155437623
-0.75 0.0012154562483588822
-0.7504 0.0011828782811286402
-0.7508 0.0011505190036308656
-0.7512 0.0011194909341880287
-0.7516 0.0010905711917338144
-0.752 0.0010597009375724643
-0.7524 0.0010339955601921076
-0.7528 0.0010075684562535624
-0.7532 0.0009823104352990166
-0.7536 0.0009567041133071104
-0.754 0.0009332858358403903
-0.7544 0.0009093163326604271
-0.7548 0.0008866665704717933
-0.7552 0.000866090505521955
-0.7556 0.0008435672001924319
-0.756 0.0008222393686034191
-0.7564 0.0008001242294314592
-0.7568 0.0007789013081304708
-0.7572 0.0007607290196789128
-0.7576 0.0007410943037502942
-0.758 0.0007227290458380536
-0.7584 0.0007055140062445648
-0.7588 0.0006879428862141108
-0.7592 0.0006704330411779904
-0.7596 0.00065338738439862
-0.76 0.0006365306417694642
-0.7604 0.0006214130041654322
-0.7608 0.0006057396326881679
-0.7612 0.0005897446550956146
-0.7616 0.0005744960140390124
-0.762 0.0005603224334873138
-0.7624 0.0005467561179633207
-0.7628 0.0005323010203609147
-0.7632 0.0005193156180654347
-0.7636 0.0005063261652715935
-0.764 0.000494221208295105
-0.7644 0.00048198930131485566
-0.7648 0.0004698301545595294
-0.7652 0.0004581149358001265
-0.7656 0.00044643075178312235
-0.766 0.0004350985308821192
-0.7664 0.0004239578515685171
-0.7668 0.00041391091025105126
-0.7672 0.00040377349451658796
-0.7676 0.0003932274325931409
-0.768 0.0003832486427650569
-0.7684 0.00037295224128500653
-0.7688 0.00036332529347303115
-0.7692 0.0003542989409852639
-0.7696 0.0003462509544331437
-0.77 0.0003372684528706627
-0.7704 0.00032943814651248074
-0.7708 0.00032100111156448417
-0.7712 0.0003131630098860555
-0.7716 0.0003057237852813695
-0.772 0.00029804404152604727
-0.7724 0.00029053690027366403
-0.7728 0.00028386572168929394
-0.7732 0.00027704512492415713
-0.7736 0.0002699939602185531
-0.774 0.00026383847437909294
-0.7744 0.00025715347332673906
-0.7748 0.0002513144262663467
-0.7752 0.00024530196459422005
-0.7756 0.0002393559128946611
-0.776 0.00023363689291771425
-0.7764 0.00022836364140551814
-0.7768 0.0002229492493990544
-0.7772 0.00021765204248380216
-0.7776 0.0002127910862418866
-0.778 0.00020786378239369838
-0.7784 0.0002028393103102439
-0.7788 0.0001983626344407946
-0.7792 0.00019360658601949807
-0.7796 0.00018906953212966413
-0.78 0.00018446815661569892
-0.7804 0.0001801935956249281
-0.7808 0.0001758086728200998
-0.7812 0.00017153093249674302
-0.7816 0.00016735953236956378
-0.782 0.0001637517785074456
-0.7824 0.00015989253146607812
-0.7828 0.00015643932779036353
-0.7832 0.00015301586310751056
-0.7836 0.00014977953659509939
-0.784 0.00014619846349771381
-0.7844 0.00014279112068504802
-0.7848 0.00013952984080836306
-0.7852 0.0001364027942663285
-0.7856 0.00013322586405358256
-0.786 0.0001301520617658009
-0.7864 0.00012726812178061447
-0.7868 0.00012430273078796803
-0.7872 0.00012155515866010796
-0.7876 0.00011902597363795954
-0.788 0.00011639959360286114
-0.7884 0.00011373975716211563
-0.7888 0.00011114884606646534
-0.7892 0.00010870913272401207
-0.7896 0.00010619283463385414
-0.79 0.00010380999705597712
-0.7904 0.00010142592452227345
-0.7908 9.908114826440517e-05
-0.7912 9.69921709724162e-05
-0.7916 9.480473067062194e-05
-0.792 9.24967695593112e-05
-0.7924 9.055969248057149e-05
-0.7928 8.861138647347423e-05
-0.7932 8.65580508545193e-05
-0.7936 8.469383750572907e-05
-0.794 8.300463009968285e-05
-0.7944 8.1134055834032e-05
-0.7948 7.941734862267052e-05
-0.7952 7.76827930629638e-05
-0.7956 7.587558950719691e-05
-0.796 7.440424339141058e-05
-0.7964 7.272970920212917e-05
-0.7968 7.1359566794779e-05
-0.7972 6.970317559566563e-05
-0.7976 6.818317311374413e-05
-0.798 6.672981930029604e-05
-0.7984 6.52430137216677e-05
-0.7988 6.389279926552311e-05
-0.7992 6.245619810676434e-05
-0.7996 6.110836050055184e-05
-0.8 5.982408955956464e-05
-0.8004 5.8565446623193316e-05
-0.8008 5.727753474781474e-05
-0.8012 5.621892063763155e-05
-0.8016 5.507341905946482e-05
-0.802 5.3970637986883016e-05
-0.8024 5.278692923319113e-05
-0.8028 5.167311064999186e-05
-0.8032 5.069853730699113e-05
-0.8036 4.970776070172754e-05
-0.804 4.865999695999374e-05
-0.8044 4.770231309708982e-05
-0.8048 4.6740310232707216e-05
-0.8052 4.567314705106463e-05
-0.8056 4.4710516884432646e-05
-0.806 4.379994359668711e-05
-0.8064 4.2821802415673886e-05
-0.8068 4.1943465087493415e-05
-0.8072 4.1167876021749655e-05
-0.8076 4.030523410557394e-05
-0.808 3.9453036123409605e-05
-0.8084 3.8670057653036365e-05
-0.8088 3.7956944220714244e-05
-0.8092 3.7130692369337954e-05
-0.8096 3.641630473774734e-05
-0.81 3.566639679095139e-05
-0.8104 3.497518548191407e-05
-0.8108 3.432389270188326e-05
-0.8112 3.3612214218418655e-05
-0.8116 3.2912978222309565e-05
-0.812 3.2242682726362194e-05
-0.8124 3.157688985614642e-05
-0.8128 3.092095830976446e-05
-0.8132 3.029499009634853e-05
-0.8136 2.9646726350862998e-05
-0.814 2.9016648844253928e-05
-0.8144 2.851118333590657e-05
-0.8148 2.7937596267758865e-05
-0.8152 2.737380214719476e-05
-0.8156 2.6796461932197617e-05
-0.816 2.6321379433150685e-05
-0.8164 2.5795895427683924e-05
-0.8168 2.529090818500338e-05
-0.8172 2.4820059808964967e-05
-0.8176 2.4307572871912112e-05
-0.818 2.380828226987836e-05
-0.8184 2.3366150543673186e-05
-0.8188 2.293854788689674e-05
-0.8192 2.246704847002056e-05
-0.8196 2.2001303750265522e-05
-0.82 2.159333820148461e-05
-0.8204 2.116779908486587e-05
-0.8208 2.0744575911456572e-05
-0.8212 2.035143411228972e-05
-0.8216 1.9932480880870136e-05
-0.822 1.953827642077821e-05
-0.8224 1.9153760425186118e-05
-0.8228 1.8785636260614833e-05
-0.8232 1.8411020880339247e-05
-0.8236 1.8089659499799724e-05
-0.824 1.7716432354947306e-05
-0.8244 1.7366921459127235e-05
-0.8248 1.704198211944364e-05
-0.8252 1.6708567459800144e-05
-0.8256 1.6404640914427627e-05
-0.826 1.6117473871651813e-05
-0.8264 1.5804931109274673e-05
-0.8268 1.5526435699457138e-05
-0.8272 1.5233590598526061e-05
-0.8276 1.4952473206829268e-05
-0.828 1.4667212435676398e-05
-0.8284 1.4394423258212607e-05
-0.8288 1.4138452193618309e-05
-0.8292 1.387929787921583e-05
-0.8296 1.3594574386183233e-05
-0.83 1.3358766198502097e-05
-0.8304 1.3135963902583063e-05
-0.8308 1.2907856809292254e-05
-0.8312 1.2668093403645471e-05
-0.8316 1.2449776025575796e-05
-0.832 1.2201020477140842e-05
-0.8324 1.197909971942642e-05
-0.8328 1.173571294730058e-05
-0.8332 1.1521743487753612e-05
-0.8336 1.1306817898486499e-05
-0.834 1.1086056847587161e-05
-0.8344 1.0897697718942234e-05
-0.8348 1.0695150506654369e-05
-0.8352 1.0509781395599701e-05
-0.8356 1.032317277744804e-05
-0.836 1.0139994279349521e-05
-0.8364 9.960051433120407e-06
-0.8368 9.795825656764538e-06
-0.8372 9.605716633887124e-06
-0.8376 9.439389979924652e-06
-0.838 9.270655522585552e-06
-0.8384 9.101879856120265e-06
-0.8388 8.931740049894205e-06
-0.8392 8.762785712048966e-06
-0.8396 8.617638050990004e-06
-0.84 8.479883240916438e-06
-0.8404 8.342129492857191e-06
-0.8408 8.178122600299633e-06
-0.8412 8.029871951636202e-06
-0.8416 7.88199019958843e-06
-0.842 7.737831285146432e-06
-0.8424 7.584118509402317e-06
-0.8428 7.465393560482313e-06
-0.8432 7.339874772489433e-06
-0.8436 7.219600039472723e-06
-0.844 7.092815015080542e-06
-0.8444 6.966510046068342e-06
-0.8448 6.83871385308816e-06
-0.8452 6.740234607143113e-06
-0.8456 6.619025626878386e-06
-0.846 6.497482799335586e-06
-0.8464 6.386305382891007e-06
-0.8468 6.2730252350549005e-06
-0.8472 6.173850228565066e-06
-0.8476 6.060874759848705e-06
-0.848 5.960323144289937e-06
-0.8484 5.859010148201258e-06
-0.8488 5.760711249869632e-06
-0.8492 5.666877833879697e-06
-0.8496 5.57347320907157e-06
-0.85 5.477905252069664e-06
-0.8504 5.385541841200543e-06
-0.8508 5.294997924892955e-06
-0.8512 5.1980202648606785e-06
-0.8516 5.109812098372111e-06
-0.852 5.029187514237259e-06
-0.8524 4.937555030260019e-06
-0.8528 4.869108896723294e-06
-0.8532 4.788533849262638e-06
-0.8536 4.714230174801669e-06
-0.854 4.64255717656438e-06
-0.8544 4.552316571814016e-06
-0.8548 4.466074491793635e-06
-0.8552 4.3920802592440254e-06
-0.8556 4.324977494835112e-06
-0.856 4.253886717405152e-06
-0.8564 4.184976344119666e-06
-0.8568 4.114659642868355e-06
-0.8572 4.0507169382955165e-06
-0.8576 3.981168061395867e-06
-0.858 3.918132764825893e-06
-0.8584 3.857040117445947e-06
-0.8588 3.790863914798893e-06
-0.8592 3.725620856474869e-06
-0.8596 3.664539481005861e-06
-0.86 3.605403700725552e-06
-0.8604 3.5451095789093754e-06
-0.8608 3.4860552106454458e-06
-0.8612 3.4292320700375297e-06
-0.8616 3.3817791895844732e-06
-0.862 3.329088654394569e-06
-0.8624 3.273836142064886e-06
-0.8628 3.217545960437745e-06
-0.8632 3.167257725611217e-06
-0.8636 3.122208370118121e-06
-0.864 3.0694256189263946e-06
-0.8644 3.0159343899443968e-06
-0.8648 2.968170334020257e-06
-0.8652 2.921807129981963e-06
-0.8656 2.8746633158661037e-06
-0.866 2.8303996053244066e-06
-0.8664 2.785752702778418e-06
-0.8668 2.7388670125746093e-06
-0.8672 2.7035900566930925e-06
-0.8676 2.657072197893961e-06
-0.868 2.6203773997838886e-06
-0.8684 2.576780810009597e-06
-0.8688 2.5298079606430386e-06
-0.8692 2.488084473259019e-06
-0.8696 2.448586072523758e-06
-0.87 2.413394521920408e-06
-0.8704 2.382761432300047e-06
-0.8708 2.3412464674271263e-06
-0.8712 2.30340497824445e-06
-0.8716 2.2690247216516915e-06
-0.872 2.233957873176611e-06
-0.8724 2.2020870988654623e-06
-0.8728 2.163753691888196e-06
-0.8732 2.132033264050346e-06
-0.8736 2.0988054104553756e-06
-0.874 2.0624233023284755e-06
-0.8744 2.031310231000092e-06
-0.8748 1.9977558502675234e-06
-0.8752 1.967846002084877e-06
-0.8756 1.9398625554721697e-06
-0.876 1.909277803293207e-06
-0.8764 1.8798945126933073e-06
-0.8768 1.8465911526985082e-06
-0.8772 1.8206238268950184e-06
-0.8776 1.791134643067676e-06
-0.878 1.7627488591280953e-06
-0.8784 1.7396167561713211e-06
-0.8788 1.710552281077665e-06
-0.8792 1.6872791389168863e-06
-0.8796 1.6595622814703265e-06
-0.88 1.6342355193330446e-06
-0.8804 1.6079832162225276e-06
-0.8808 1.5803563301298818e-06
-0.8812 1.5557826657957406e-06
-0.8816 1.534796639056961e-06
-0.882 1.5120322713527991e-06
-0.8824 1.4868897116514973e-06
-0.8828 1.4630812113751062e-06
-0.8832 1.4412203565861987e-06
-0.8836 1.4234815883515014e-06
-0.884 1.3990632195106376e-06
-0.8844 1.3776136053561202e-06
-0.8848 1.3578360909096685e-06
-0.8852 1.3378104703203036e-06
-0.8856 1.3202750534318266e-06
-0.886 1.2994033027755475e-06
-0.8864 1.2816500534589903e-06
-0.8868 1.2630852647395709e-06
-0.8872 1.24649533479952e-06
-0.8876 1.2264520728017307e-06
-0.888 1.2104841837842096e-06
-0.8884 1.1928024287186653e-06
-0.8888 1.175684461451777e-06
-0.8892 1.1571091355257964e-06
-0.8896 1.1401933751224917e-06
-0.89 1.1218511490797532e-06
-0.8904 1.1077082307533899e-06
-0.8908 1.0923001471756574e-06
-0.8912 1.0779970252572217e-06
-0.8916 1.0629233182343839e-06
-0.892 1.0481446810902522e-06
-0.8924 1.0330919767351996e-06
-0.8928 1.0173618152271667e-06
-0.8932 1.0035924299374304e-06
-0.8936 9.878547805190946e-07
-0.894 9.742528102533737e-07
-0.8944 9.595104338230076e-07
-0.8948 9.473057093445117e-07
-0.8952 9.335631382942849e-07
-0.8956 9.206538327179922e-07
-0.896 9.066834676373443e-07
-0.8964 8.968706752737479e-07
-0.8968 8.828493323887058e-07
-0.8972 8.703828347550845e-07
-0.8976 8.597545512083843e-07
-0.898 8.455270582248781e-07
-0.8984 8.340751712355149e-07
-0.8988 8.232167932196014e-07
-0.8992 8.112545258153971e-07
-0.8996 8.006115783915755e-07
-0.9 7.886656306746751e-07
-0.9004 7.769300886282216e-07
-0.9008 7.671042738410673e-07
-0.9012 7.558719287364562e-07
-0.9016 7.46018234579637e-07
-0.902 7.347822473307493e-07
-0.9024 7.244281780664996e-07
-0.9028 7.143117157914563e-07
-0.9032 7.048718086551378e-07
-0.9036 6.95356428302811e-07
-0.904 6.85433288714311e-07
-0.9044 6.747425906418569e-07
-0.9048 6.649800035325905e-07
-0.9052 6.552254690607352e-07
-0.9056 6.480092679733745e-07
-0.906 6.391116269670039e-07
-0.9064 6.30444671030827e-07
-0.9068 6.219387875354967e-07
-0.9072 6.134492831730498e-07
-0.9076 6.052077064341082e-07
-0.908 5.971797253441904e-07
-0.9084 5.882527800279262e-07
-0.9088 5.808308484090443e-07
-0.9092 5.726621975066569e-07
-0.9096 5.639639163121082e-07
-0.91 5.568032676377414e-07
-0.9104 5.487325427669149e-07
-0.9108 5.407671948735516e-07
-0.9112 5.337213654285102e-07
-0.9116 5.261063835485853e-07
-0.912 5.195863854419431e-07
-0.9124 5.133226862764134e-07
-0.9128 5.065825174403124e-07
-0.9132 4.987823594207245e-07
-0.9136 4.928906961489245e-07
-0.914 4.863536007647998e-07
-0.9144 4.794145067939127e-07
-0.9148 4.736371060625717e-07
-0.9152 4.6688405070243006e-07
-0.9156 4.6097473277037164e-07
-0.916 4.5530213729124405e-07
-0.9164 4.5041380123680685e-07
-0.9168 4.4440168982785445e-07
-0.9172 4.3798564566611036e-07
-0.9176 4.322954064257082e-07
-0.918 4.2629692378104814e-07
-0.9184 4.1975114400647303e-07
-0.9188 4.1396231441818605e-07
-0.9192 4.079518051620599e-07
-0.9196 4.0317037615690133e-07
-0.92 3.9750994545943774e-07
-0.9204 3.9255576315077155e-07
-0.9208 3.8683127014549853e-07
-0.9212 3.816931848773457e-07
-0.9216 3.7688355199431264e-07
-0.922 3.7229613052626116e-07
-0.9224 3.6835857624231465e-07
-0.9228 3.628846795094372e-07
-0.9232 3.5780837831110307e-07
-0.9236 3.5224308702856937e-07
-0.924 3.4838307532786876e-07
-0.9244 3.4366585159813337e-07
-0.9248 3.3880056692573536e-07
-0.9252 3.34192228192411e-07
-0.9256 3.2991049327342775e-07
-0.926 3.255026753464622e-07
-0.9264 3.208496007508797e-07
-0.9268 3.16527910595361e-07
-0.9272 3.126924801465807e-07
-0.9276 3.084767584276431e-07
-0.928 3.0517885566410693e-07
-0.9284 3.014885178042536e-07
-0.9288 2.976408604913198e-07
-0.9292 2.938340160968619e-07
-0.9296 2.902138115280349e-07
-0.93 2.8683695268088595e-07
-0.9304 2.8278744465285334e-07
-0.9308 2.793379195035498e-07
-0.9312 2.7551081153448387e-07
-0.9316 2.713197576351091e-07
-0.932 2.683122528049396e-07
-0.9324 2.6483178037684974e-07
-0.9328 2.6131221874890826e-07
-0.9332 2.582702259547489e-07
-0.9336 2.551619396775345e-07
-0.934 2.520544741659247e-07
-0.9344 2.4896495469870594e-07
-0.9348 2.463901997845308e-07
-0.9352 2.430907411499676e-07
-0.9356 2.399202004290094e-07
-0.936 2.3717035414296914e-07
-0.9364 2.3405829311564376e-07
-0.9368 2.3143654422641714e-07
-0.9372 2.2882345155260766e-07
-0.9376 2.2603106818667474e-07
-0.938 2.2302414331166028e-07
-0.9384 2.200722312198553e-07
-0.9388 2.1779094265192272e-07
-0.9392 2.1497918558815063e-07
-0.9396 2.127549963278035e-07
-0.94 2.1020498268166926e-07
-0.9404 2.0753559274706563e-07
-0.9408 2.0491472962472243e-07
-0.9412 2.0256196506526136e-07
-0.9416 1.999096774011244e-07
-0.942 1.9771327263838332e-07
-0.9424 1.9574213793774e-07
-0.9428 1.9349805881954083e-07
-0.9432 1.9150499270917012e-07
-0.9436 1.8928930528023753e-07
-0.944 1.8708883907142053e-07
-0.9444 1.8516985523279407e-07
-0.9448 1.8309980150427216e-07
-0.9452 1.8065943699656586e-07
-0.9456 1.7844826326434203e-07
-0.946 1.7605778522939263e-07
-0.9464 1.7381742180989788e-07
-0.9468 1.7181819890382986e-07
-0.9472 1.6960881667533457e-07
-0.9476 1.67789459714404e-07
-0.948 1.657807810716889e-07
-0.9484 1.6410758027982013e-07
-0.9488 1.625840242425666e-07
-0.9492 1.607071440235027e-07
-0.9496 1.5889737398443e-07
-0.95 1.572264038197221e-07
-0.9504 1.5558680758941316e-07
-0.9508 1.5357795439042265e-07
-0.9512 1.518231400142444e-07
-0.9516 1.5025786286253534e-07
-0.952 1.4854677558280424e-07
-0.9524 1.4687861502912674e-07
-0.9528 1.4520729131922515e-07
-0.9532 1.4378074020144828e-07
-0.9536 1.422486529989955e-07
-0.954 1.406375196454048e-07
-0.9544 1.3894021388510798e-07
-0.9548 1.3747375516922534e-07
-0.9552 1.357511933919649e-07
-0.9556 1.344745102173572e-07
-0.956 1.329071044245465e-07
-0.9564 1.315194352945814e-07
-0.9568 1.2990970083138862e-07
-0.9572 1.2864864607883962e-07
-0.9576 1.272169178886079e-07
-0.958 1.2609281253197504e-07
-0.9584 1.2429899224241e-07
-0.9588 1.229860388141412e-07
-0.9592 1.215461627177667e-07
-0.9596 1.2026718567357607e-07
-0.96 1.1880962413818676e-07
-0.9604 1.1738145645300223e-07
-0.9608 1.1627612642459468e-07
-0.9612 1.1516518129373914e-07
-0.9616 1.1400626564662453e-07
-0.962 1.1267419627060277e-07
-0.9624 1.1171408394130577e-07
-0.9628 1.1062349591427261e-07
-0.9632 1.0933616227362855e-07
-0.9636 1.0833144130299229e-07
-0.964 1.0738075674909352e-07
-0.9644 1.063857132591585e-07
-0.9648 1.053334077160017e-07
-0.9652 1.0414563388779983e-07
-0.9656 1.0344545603733211e-07
-0.966 1.0251612202797017e-07
-0.9664 1.0145262795656067e-07
-0.9668 1.0021722855752977e-07
-0.9672 9.923970995285089e-08
-0.9676 9.810526344369079e-08
-0.968 9.713324629851366e-08
-0.9684 9.613029925751602e-08
-0.9688 9.518010977317831e-08
-0.9692 9.413777361825993e-08
-0.9696 9.331152603419417e-08
-0.97 9.239091025260072e-08
-0.9704 9.151550986344419e-08
-0.9708 9.050586649429462e-08
-0.9712 8.958213437545558e-08
-0.9716 8.880551931055193e-08
-0.972 8.784515634541715e-08
-0.9724 8.698841996023876e-08
-0.9728 8.612253392077264e-08
-0.9732 8.53270856226242e-08
-0.9736 8.45126421599743e-08
-0.974 8.37952888286977e-08
-0.9744 8.295791425992747e-08
-0.9748 8.241058589455431e-08
-0.9752 8.162010182741549e-08
-0.9756 8.093639176250952e-08
-0.976 8.024423668060062e-08
-0.9764 7.941172572726744e-08
-0.9768 7.879041765667641e-08
-0.9772 7.820500653988136e-08
-0.9776 7.737625150596143e-08
-0.978 7.667012496889741e-08
-0.9784 7.599426063311725e-08
-0.9788 7.530715904714013e-08
-0.9792 7.466107320131086e-08
-0.9796 7.409691934455133e-08
-0.98 7.339696834353684e-08
-0.9804 7.284720113856979e-08
-0.9808 7.22531808064815e-08
-0.9812 7.183147568563045e-08
-0.9816 7.127860465579181e-08
-0.982 7.073408061854187e-08
-0.9824 7.002463052332992e-08
-0.9828 6.949722324604307e-08
-0.9832 6.893342456617402e-08
-0.9836 6.822299732384591e-08
-0.984 6.774178506291986e-08
-0.9844 6.708136636373566e-08
-0.9848 6.657527924380972e-08
-0.9852 6.59985132859601e-08
-0.9856 6.54637580999214e-08
-0.986 6.499621969158212e-08
-0.9864 6.434181812522416e-08
-0.9868 6.372561418631754e-08
-0.9872 6.313146310493029e-08
-0.9876 6.257925129215799e-08
-0.988 6.203582874137511e-08
-0.9884 6.149561098522167e-08
-0.9888 6.091302042812679e-08
-0.9892 6.036086559180853e-08
-0.9896 6.004802480784104e-08
-0.99 5.962327763628399e-08
-0.9904 5.912639695080327e-08
-0.9908 5.863862340664639e-08
-0.9912 5.8204667131204775e-08
-0.9916 5.779242754250607e-08
-0.992 5.7272513000172735e-08
-0.9924 5.690711958360596e-08
-0.9928 5.6427257557770976e-08
-0.9932 5.6098453061196456e-08
-0.9936 5.568590912922966e-08
-0.994 5.5242170521479315e-08
-0.9944 5.489598738660074e-08
-0.9948 5.4421190941595926e-08
-0.9952 5.405780019642507e-08
-0.9956 5.3735269720945e-08
-0.996 5.3249763267885384e-08
-0.9964 5.290934589714388e-08
-0.9968 5.2409372054647815e-08
-0.9972 5.203808182204324e-08
-0.9976 5.1650108223678714e-08
-0.998 5.1273234955241857e-08
-0.9984 5.090554421516743e-08
-0.9988 5.047782656401253e-08
-0.9992 5.009416920199921e-08
-0.9996 4.979121831132551e-08
-1.0 4.94057982723635e-08
-1.0004 4.904283134618958e-08
-1.0008 4.877240337564636e-08
-1.0012 4.842471504677872e-08
-1.0016 4.803283339585026e-08
-1.002 4.772404805683496e-08
-1.0024 4.7356450580863566e-08
-1.0028 4.70460944908134e-08
-1.0032 4.670091302702074e-08
-1.0036 4.644279928492451e-08
-1.004 4.6126423105794466e-08
-1.0044 4.5889840547288426e-08
-1.0048 4.559587019885377e-08
-1.0052 4.525570223674424e-08
-1.0056 4.498350264848264e-08
-1.006 4.462029120863285e-08
-1.0064 4.4422973600352324e-08
-1.0068 4.4087755100192605e-08
-1.0072 4.3907333397886124e-08
-1.0076 4.358329580344194e-08
-1.008 4.336967141487167e-08
-1.0084 4.315140977981147e-08
-1.0088 4.2898103999068963e-08
-1.0092 4.2647100598305e-08
-1.0096 4.2282363565037376e-08
-1.01 4.209908092193958e-08
-1.0104 4.185072410120461e-08
-1.0108 4.158947016297258e-08
-1.0112 4.1349398430004153e-08
-1.0116 4.120489575707157e-08
-1.012 4.09762170106738e-08
-1.0124 4.0712863549098486e-08
-1.0128 4.0572117857422364e-08
-1.0132 4.031370946836159e-08
-1.0136 4.013416447954419e-08
-1.014 3.989426110584037e-08
-1.0144 3.962945582223231e-08
-1.0148 3.9482366897281615e-08
-1.0152 3.927963271109785e-08
-1.0156 3.903730357025642e-08
-1.016 3.88957864245007e-08
-1.0164 3.859390084420436e-08
-1.0168 3.844606397799157e-08
-1.0172 3.825203769107397e-08
-1.0176 3.8138737229951665e-08
-1.018 3.7891612621994426e-08
-1.0184 3.777229657429795e-08
-1.0188 3.7698193363633544e-08
-1.0192 3.74529631065376e-08
-1.0196 3.728833727415599e-08
-1.02 3.7107537487306854e-08
-1.0204 3.6854797562348826e-08
-1.0208 3.671754083750525e-08
-1.0212 3.6568343603549674e-08
-1.0216 3.633115482811499e-08
-1.022 3.6199059868105414e-08
-1.0224 3.6018391813255246e-08
-1.0228 3.584213430443664e-08
-1.0232 3.573867456983111e-08
-1.0236 3.5507707702500716e-08
-1.024 3.5353444776415316e-08
-1.0244 3.523425369209476e-08
-1.0248 3.509453139541565e-08
-1.0252 3.4923557844088016e-08
-1.0256 3.475875378876631e-08
-1.026 3.463688938300315e-08
-1.0264 3.448878289390209e-08
-1.0268 3.431258122288612e-08
-1.0272 3.4168559571175606e-08
-1.0276 3.3988878159957886e-08
-1.028 3.382813669362652e-08
-1.0284 3.3694242844087815e-08
-1.0288 3.349071790313648e-08
-1.0292 3.34140284342342e-08
-1.0296 3.3210739167374655e-08
-1.03 3.311375199039513e-08
-1.0304 3.301039061306861e-08
-1.0308 3.2853593842077735e-08
-1.0312 3.2736746287389725e-08
-1.0316 3.25381120938817e-08
-1.032 3.237543852462683e-08
-1.0324 3.218764879305264e-08
-1.0328 3.208202049793644e-08
-1.0332 3.201187673424123e-08
-1.0336 3.1872394140656454e-08
-1.034 3.172094253903292e-08
-1.0344 3.162721204791414e-08
-1.0348 3.153112328712303e-08
-1.0352 3.142024598561025e-08
-1.0356 3.1370879530080426e-08
-1.036 3.125614083111194e-08
-1.0364 3.1214879810805695e-08
-1.0368 3.1052688009042216e-08
-1.0372 3.0928453923124094e-08
-1.0376 3.085779361541521e-08
-1.038 3.084186495738512e-08
-1.0384 3.0730578937295965e-08
-1.0388 3.061167631601507e-08
-1.0392 3.056254333137015e-08
-1.0396 3.048861137815444e-08
-1.04 3.0391056477392456e-08
-1.0404 3.029247525292098e-08
-1.0408 3.023014511694551e-08
-1.0412 3.0166490020566547e-08
-1.0416 3.0010931200879294e-08
-1.042 2.9931118920135044e-08
-1.0424 2.9854697546935604e-08
-1.0428 2.9732627341452953e-08
-1.0432 2.9655749123669828e-08
-1.0436 2.94962026018689e-08
-1.044 2.94031854135623e-08
-1.0444 2.938659151257373e-08
-1.0448 2.930352024049875e-08
-1.0452 2.9154118249183953e-08
-1.0456 2.9061877740433043e-08
-1.046 2.8969188843375125e-08
-1.0464 2.8900103799331566e-08
-1.0468 2.881820615155896e-08
-1.0472 2.8672992352661508e-08
-1.0476 2.858696522676744e-08
-1.048 2.845876084666735e-08
-1.0484 2.836732909805173e-08
-1.0488 2.8357485521005654e-08
-1.0492 2.8239056661350756e-08
-1.0496 2.816602576650415e-08
-1.05 2.8080191358845894e-08
-1.0504 2.8084095159650056e-08
-1.0508 2.7947473730532235e-08
-1.0512 2.791892105747648e-08
-1.0516 2.7799295472438193e-08
-1.052 2.7699650891456352e-08
-1.0524 2.769274653698917e-08
-1.0528 2.763011617698752e-08
-1.0532 2.7529067259310418e-08
-1.0536 2.740342513209575e-08
-1.054 2.7352217399630302e-08
-1.0544 2.7307451956874654e-08
-1.0548 2.7250767537916133e-08
-1.0552 2.717636344396663e-08
-1.0556 2.7123199343096063e-08
-1.056 2.701737982445912e-08
-1.0564 2.6980519591440783e-08
-1.0568 2.6941739094595882e-08
-1.0572 2.684535447714081e-08
-1.0576 2.6748060000770057e-08
-1.058 2.6713262367887012e-08
-1.0584 2.6634616360196357e-08
-1.0588 2.6619511560523304e-08
-1.0592 2.6552306682173353e-08
-1.0596 2.6520324062524865e-08
-1.06 2.650523386220332e-08
-1.0604 2.6445216112273187e-08
-1.0608 2.6412368156985543e-08
-1.0612 2.6330977936541048e-08
-1.0616 2.631139789038729e-08
-1.062 2.622083878842829e-08
-1.0624 2.6165805343057947e-08
-1.0628 2.608330830378813e-08
-1.0632 2.609313301413244e-08
-1.0636 2.6046885600192225e-08
-1.064 2.596043555396908e-08
-1.0644 2.5935199233167823e-08
-1.0648 2.5860596514915785e-08
-1.0652 2.584089029531192e-08
-1.0656 2.5788004153975373e-08
-1.066 2.5772669866201097e-08
-1.0664 2.571415070885287e-08
-1.0668 2.5632594011964782e-08
-1.0672 2.5625829213350145e-08
-1.0676 2.5600942280158156e-08
-1.068 2.5532372291052498e-08
-1.0684 2.552724383038959e-08
-1.0688 2.5502086935115367e-08
-1.0692 2.539953636811366e-08
-1.0696 2.536862520788223e-08
-1.07 2.5349715429745693e-08
-1.0704 2.528882562740601e-08
-1.0708 2.5211218451329988e-08
-1.0712 2.514738577933458e-08
-1.0716 2.503686767402529e-08
-1.072 2.496666174134924e-08
-1.0724 2.494549506693299e-08
-1.0728 2.4928073824401997e-08
-1.0732 2.4933172605058022e-08
-1.0736 2.4904924020256627e-08
-1.074 2.4878144254544993e-08
-1.0744 2.4825195449412843e-08
-1.0748 2.479210895411327e-08
-1.0752 2.4779929740875477e-08
-1.0756 2.4745033782834303e-08
-1.076 2.474651257086391e-08
-1.0764 2.4745187861841837e-08
-1.0768 2.4657116971404622e-08
-1.0772 2.4631874806889142e-08
-1.0776 2.461440706967162e-08
-1.078 2.4588344522185683e-08
-1.0784 2.4541752222993083e-08
-1.0788 2.4574334190527372e-08
-1.0792 2.4562647375372136e-08
-1.0796 2.4509486911008013e-08
-1.08 2.4485032788135855e-08
-1.0804 2.443432490513741e-08
-1.0808 2.445255464907545e-08
-1.0812 2.4376696571837736e-08
-1.0816 2.433404482826837e-08
-1.082 2.425564645746914e-08
-1.0824 2.4279061146387342e-08
-1.0828 2.4307768534541152e-08
-1.0832 2.4267685131851612e-08
-1.0836 2.427013856963743e-08
-1.084 2.4228274103273246e-08
-1.0844 2.4222620920496633e-08
-1.0848 2.4156609179125148e-08
-1.0852 2.4105964427751714e-08
-1.0856 2.4042412839502355e-08
-1.086 2.399593372811167e-08
-1.0864 2.3967842681482604e-08
-1.0868 2.3941806507991706e-08
-1.0872 2.3880364198393006e-08
-1.0876 2.387935988565298e-08
-1.088 2.3859667555554725e-08
-1.0884 2.389030862101088e-08
-1.0888 2.3867753445290067e-08
-1.0892 2.382691579934725e-08
-1.0896 2.378703789058036e-08
-1.09 2.3774057589890536e-08
-1.0904 2.370592874174166e-08
-1.0908 2.368650399219538e-08
-1.0912 2.3689685849018245e-08
-1.0916 2.3684477208049264e-08
-1.092 2.3696792139757644e-08
-1.0924 2.3691697936269216e-08
-1.0928 2.3677938237068473e-08
-1.0932 2.3652727444001673e-08
-1.0936 2.364751359858205e-08
-1.094 2.3659899883005023e-08
-1.0944 2.3631185089219656e-08
-1.0948 2.3615166837728797e-08
-1.0952 2.3648796192328343e-08
-1.0956 2.3645875790556415e-08
-1.096 2.3673465774934703e-08
-1.0964 2.366225231448823e-08
-1.0968 2.3645037717162295e-08
-1.0972 2.3641117189686584e-08
-1.0976 2.3668872345009527e-08
-1.098 2.362102125888219e-08
-1.0984 2.3611012411867077e-08
-1.0988 2.364247758620469e-08
-1.0992 2.3610723474419177e-08
-1.0996 2.3555636124928806e-08
-1.1 2.355761044709922e-08
-1.1004 2.3505710390695286e-08
-1.1008 2.349676976591717e-08
-1.1012 2.350052439859243e-08
-1.1016 2.3452642420816685e-08
-1.102 2.3436867496172406e-08
-1.1024 2.3404251748448678e-08
-1.1028 2.342529211750153e-08
-1.1032 2.338733045794507e-08
-1.1036 2.337821238439605e-08
-1.104 2.3344746293719805e-08
-1.1044 2.3336609586433792e-08
-1.1048 2.3346609572214486e-08
-1.1052 2.334349916574053e-08
-1.1056 2.334227163639782e-08
-1.106 2.3307757483552238e-08
-1.1064 2.334224915202017e-08
-1.1068 2.3317065015918403e-08
-1.1072 2.3351457424924284e-08
-1.1076 2.33389516596496e-08
-1.108 2.33244573126062e-08
-1.1084 2.334239361697924e-08
-1.1088 2.330076210658319e-08
-1.1092 2.3316093141896625e-08
-1.1096 2.324920001266057e-08
-1.11 2.326718786805425e-08
-1.1104 2.323805902248075e-08
-1.1108 2.327229314109925e-08
-1.1112 2.3248446981990922e-08
-1.1116 2.3201773323685083e-08
-1.112 2.3200512440344375e-08
-1.1124 2.3145482810724564e-08
-1.1128 2.3135888419924022e-08
-1.1132 2.313689209007576e-08
-1.1136 2.3110779411940074e-08
-1.114 2.3123153895419453e-08
-1.1144 2.309970717312433e-08
-1.1148 2.308427533558757e-08
-1.1152 2.3078136707580927e-08
-1.1156 2.3060340392739636e-08
-1.116 2.3050395243140366e-08
-1.1164 2.3057445150757067e-08
-1.1168 2.3058723446226134e-08
-1.1172 2.305721447152172e-08
-1.1176 2.3019231102831596e-08
-1.118 2.300145520604884e-08
-1.1184 2.2983952102676818e-08
-1.1188 2.2990705086158487e-08
-1.1192 2.29768866557921e-08
-1.1196 2.29906854734941e-08
-1.12 2.2957358708328606e-08
-1.1204 2.2929430335004195e-08
-1.1208 2.2922044752814874e-08
-1.1212 2.2899843717759338e-08
-1.1216 2.293637907129368e-08
-1.122 2.2957871490001163e-08
-1.1224 2.2938898688678955e-08
-1.1228 2.2953775469645722e-08
-1.1232 2.2934498871802443e-08
-1.1236 2.290182996945809e-08
-1.124 2.2939595779806476e-08
-1.1244 2.2927635283555176e-08
-1.1248 2.292665112451931e-08
-1.1252 2.2935524656608153e-08
-1.1256 2.289557763503639e-08
-1.126 2.287880083306068e-08
-1.1264 2.2871073647417242e-08
-1.1268 2.2900168817347917e-08
-1.1272 2.293963744154856e-08
-1.1276 2.289747226122646e-08
-1.128 2.2926186621043484e-08
-1.1284 2.289365293646501e-08
-1.1288 2.28465654043674e-08
-1.1292 2.2895402510981966e-08
-1.1296 2.2888344050761665e-08
-1.13 2.2930870172628597e-08
-1.1304 2.2909975687932595e-08
-1.1308 2.2987674491607053e-08
-1.1312 2.2926438765946576e-08
-1.1316 2.2921772385340158e-08
-1.132 2.2941181961207686e-08
-1.1324 2.2937828436886076e-08
-1.1328 2.2958082031443497e-08
-1.1332 2.296402763926919e-08
-1.1336 2.2900063068875826e-08
-1.134 2.2926268274248317e-08
-1.1344 2.2891019890444497e-08
-1.1348 2.291195079265787e-08
-1.1352 2.2905160280360574e-08
-1.1356 2.28662141489797e-08
-1.136 2.288686304096944e-08
-1.1364 2.2869892402976852e-08
-1.1368 2.2836110357485734e-08
-1.1372 2.2906594930613732e-08
-1.1376 2.290680598128208e-08
-1.138 2.2882901960141785e-08
-1.1384 2.283736219967011e-08
-1.1388 2.2846153796695623e-08
-1.1392 2.2843072553013767e-08
-1.1396 2.2863483876441603e-08
-1.14 2.2842712173767733e-08
-1.1404 2.2890800863411443e-08
-1.1408 2.2830948702703993e-08
-1.1412 2.2839993817761824e-08
-1.1416 2.2876700872790707e-08
-1.142 2.286916912738518e-08
-1.1424 2.2855188075473186e-08
-1.1428 2.286536147973019e-08
-1.1432 2.2852663119871307e-08
-1.1436 2.2852829834619942e-08
-1.144 2.2856674233304657e-08
-1.1444 2.288364788366259e-08
-1.1448 2.2852325519251045e-08
-1.1452 2.2881570867888382e-08
-1.1456 2.2884345267029978e-08
-1.146 2.2851562167274407e-08
-1.1464 2.2824091991284758e-08
-1.1468 2.2839476143848333e-08
-1.1472 2.276927593961387e-08
-1.1476 2.2804207794025725e-08
-1.148 2.2761549062323206e-08
-1.1484 2.278482080726508e-08
-1.1488 2.283500835827601e-08
-1.1492 2.2826793997502176e-08
-1.1496 2.2825987574660766e-08
-1.15 2.2820683028120023e-08
-1.1504 2.282074859932361e-08
-1.1508 2.281427410280389e-08
-1.1512 2.2778883108567195e-08
-1.1516 2.2792571709570713e-08
-1.152 2.2809917900201887e-08
-1.1524 2.2851973597999024e-08
-1.1528 2.286015251909419e-08
-1.1532 2.286042112190002e-08
-1.1536 2.2844557684804666e-08
-1.154 2.2833514601629412e-08
-1.1544 2.282349856319008e-08
-1.1548 2.2817022782534835e-08
-1.1552 2.2789488207990694e-08
-1.1556 2.280550216225161e-08
-1.156 2.2838939158563784e-08
-1.1564 2.2850423814336293e-08
-1.1568 2.283500404673183e-08
-1.1572 2.2921186535573837e-08
-1.1576 2.2918837327529687e-08
-1.158 2.285367731729256e-08
-1.1584 2.2863680158602138e-08
-1.1588 2.286449354990265e-08
-1.1592 2.2850621946745225e-08
-1.1596 2.2847506913393716e-08
-1.16 2.285683619449691e-08
-1.1604 2.2873805396025183e-08
-1.1608 2.2838280146577648e-08
-1.1612 2.287051086676043e-08
-1.1616 2.2849152199612102e-08
-1.162 2.2853744878300598e-08
-1.1624 2.2879766756908422e-08
-1.1628 2.2917837665775323e-08
-1.1632 2.2896900202642678e-08
-1.1636 2.2867903114612497e-08
-1.164 2.2901340623889804e-08
-1.1644 2.2922520748965003e-08
-1.1648 2.293219077217493e-08
-1.1652 2.286272013609795e-08
-1.1656 2.2864857944472687e-08
-1.166 2.2925930707965858e-08
-1.1664 2.2862147588334454e-08
-1.1668 2.2817612634029878e-08
-1.1672 2.280027808008213e-08
-1.1676 2.2761409016305297e-08
-1.168 2.277681975623832e-08
-1.1684 2.2700916749976136e-08
-1.1688 2.2703539483953242e-08
-1.1692 2.2734267246919666e-08
-1.1696 2.2753722143953677e-08
-1.17 2.2763008417587752e-08
-1.1704 2.2776688836134842e-08
-1.1708 2.2754065114452618e-08
-1.1712 2.2754665003899134e-08
-1.1716 2.2739416422817664e-08
-1.172 2.2736148417977844e-08
-1.1724 2.271294471141061e-08
-1.1728 2.2683594411280738e-08
-1.1732 2.2673002236056768e-08
-1.1736 2.266148557516727e-08
-1.174 2.2663333937499037e-08
-1.1744 2.2725101505786172e-08
-1.1748 2.274175855582682e-08
-1.1752 2.2745951395686308e-08
-1.1756 2.2766736308723945e-08
-1.176 2.2726499441117588e-08
-1.1764 2.2705357938460974e-08
-1.1768 2.263685085658929e-08
-1.1772 2.2656311001916923e-08
-1.1776 2.272070653464183e-08
-1.178 2.27053005413586e-08
-1.1784 2.268632816873591e-08
-1.1788 2.2696979527458952e-08
-1.1792 2.274971899207485e-08
-1.1796 2.2769062525857416e-08
-1.18 2.2733091728884512e-08
-1.1804 2.2750028286485225e-08
-1.1808 2.274633999554269e-08
-1.1812 2.274803830341199e-08
-1.1816 2.2746064589258423e-08
-1.182 2.273837242187196e-08
-1.1824 2.2797522311545488e-08
-1.1828 2.2796699392193515e-08
-1.1832 2.2754461392302057e-08
-1.1836 2.2808807302444933e-08
-1.184 2.2819566174093275e-08
-1.1844 2.2799855716119402e-08
-1.1848 2.286004581481023e-08
-1.1852 2.2860138899747644e-08
-1.1856 2.2866509683651443e-08
-1.186 2.2874186145562817e-08
-1.1864 2.2893987466589653e-08
-1.1868 2.2859545303892063e-08
-1.1872 2.2881454738998074e-08
-1.1876 2.2886657430363324e-08
-1.188 2.2891601777831112e-08
-1.1884 2.2945236981451194e-08
-1.1888 2.29356490688045e-08
-1.1892 2.284661251659012e-08
-1.1896 2.2856280684264518e-08
-1.19 2.285693692592388e-08
-1.1904 2.289468395551487e-08
-1.1908 2.288673771867209e-08
-1.1912 2.29023439067252e-08
-1.1916 2.2891612948692448e-08
-1.192 2.2887334133991426e-08
-1.1924 2.287848292380435e-08
-1.1928 2.2907355565901966e-08
-1.1932 2.2954634951302457e-08
-1.1936 2.2998998723821793e-08
-1.194 2.3011053908007528e-08
-1.1944 2.2982275572007416e-08
-1.1948 2.3015104795288768e-08
-1.1952 2.2959244641641452e-08
-1.1956 2.2954224875364704e-08
-1.196 2.2955953603829322e-08
-1.1964 2.292323140468867e-08
-1.1968 2.2961029898288822e-08
-1.1972 2.298999449451799e-08
-1.1976 2.2991574698102825e-08
-1.198 2.298153563216008e-08
-1.1984 2.2987867868798138e-08
-1.1988 2.299921085971498e-08
-1.1992 2.3014127206698096e-08
-1.1996 2.3027439262187875e-08
-1.2 2.3092668232848977e-08
-1.2004 2.3104161065991815e-08
-1.2008 2.3070397873109106e-08
-1.2012 2.306708008637826e-08
-1.2016 2.3093576113540818e-08
-1.202 2.3096892644482366e-08
-1.2024 2.3058723331552405e-08
-1.2028 2.308017060748682e-08
-1.2032 2.3046846671893157e-08
-1.2036 2.305038400359994e-08
-1.204 2.3086220458981068e-08
-1.2044 2.308318465572327e-08
-1.2048 2.308474374168176e-08
-1.2052 2.3107648749591727e-08
-1.2056 2.3144480052578577e-08
-1.206 2.3154243262804937e-08
-1.2064 2.313260238667763e-08
-1.2068 2.312550989487589e-08
-1.2072 2.315630721456002e-08
-1.2076 2.3146666846891335e-08
-1.208 2.317959223692846e-08
-1.2084 2.3214544822085435e-08
-1.2088 2.3241086919036406e-08
-1.2092 2.3271684846017765e-08
-1.2096 2.328536449329861e-08
-1.21 2.3251392007127193e-08
-1.2104 2.3261738638703327e-08
-1.2108 2.3296444734608923e-08
-1.2112 2.330643218145476e-08
-1.2116 2.3332169205472757e-08
-1.212 2.3322540636665663e-08
-1.2124 2.334901828712633e-08
-1.2128 2.3408060885131182e-08
-1.2132 2.346802072761256e-08
-1.2136 2.347283034609602e-08
-1.214 2.347803943938662e-08
-1.2144 2.349300673650581e-08
-1.2148 2.3544135580540456e-08
-1.2152 2.3601144554654922e-08
-1.2156 2.3628243338557874e-08
-1.216 2.369340248614729e-08
-1.2164 2.36934229163117e-08
-1.2168 2.369205647657712e-08
-1.2172 2.3630225337299524e-08
-1.2176 2.3675962287239663e-08
-1.218 2.3674338886822366e-08
-1.2184 2.3708613169122168e-08
-1.2188 2.365235074226676e-08
-1.2192 2.370857678169773e-08
-1.2196 2.370609901440645e-08
-1.22 2.3758575151167146e-08
-1.2204 2.376834446703977e-08
-1.2208 2.3798982582159168e-08
-1.2212 2.379888612543813e-08
-1.2216 2.380835559556174e-08
-1.222 2.379068173226461e-08
-1.2224 2.382440099981211e-08
-1.2228 2.386844035990067e-08
-1.2232 2.389933086222581e-08
-1.2236 2.3936799564088834e-08
-1.224 2.3943491033143667e-08
-1.2244 2.3921749609833427e-08
-1.2248 2.394724668890964e-08
-1.2252 2.395730228180075e-08
-1.2256 2.3945167532496216e-08
-1.226 2.393508841620108e-08
-1.2264 2.395859198126145e-08
-1.2268 2.393222378634257e-08
-1.2272 2.393876425251196e-08
-1.2276 2.3935431319709172e-08
-1.228 2.3938136743421547e-08
-1.2284 2.391441064674292e-08
-1.2288 2.39376809587876e-08
-1.2292 2.3966485926060595e-08
-1.2296 2.397180385433706e-08
-1.23 2.3968582277851288e-08
-1.2304 2.3982169641153788e-08
-1.2308 2.396339855989237e-08
-1.2312 2.3984392701025343e-08
-1.2316 2.3999115716907622e-08
-1.232 2.4003815707594134e-08
-1.2324 2.4002900489859278e-08
-1.2328 2.4017479930718035e-08
-1.2332 2.4050552059435337e-08
-1.2336 2.402858798004741e-08
-1.234 2.411443251283738e-08
-1.2344 2.4111227151228243e-08
-1.2348 2.4140519366288598e-08
-1.2352 2.416078869639676e-08
-1.2356 2.4157813498530628e-08
-1.236 2.416249648502765e-08
-1.2364 2.417911421307543e-08
-1.2368 2.4187099101499232e-08
-1.2372 2.4205102943879998e-08
-1.2376 2.4227948559743023e-08
-1.238 2.4253577523843252e-08
-1.2384 2.4268616184536842e-08
-1.2388 2.432122811139443e-08
-1.2392 2.435063190835025e-08
-1.2396 2.4340779791945308e-08
-1.24 2.4350840235896293e-08
-1.2404 2.4428245508760024e-08
-1.2408 2.4451611805220457e-08
-1.2412 2.4479805451273216e-08
-1.2416 2.4506609905635835e-08
-1.242 2.45303143435671e-08
-1.2424 2.4503181050263566e-08
-1.2428 2.4533853606804546e-08
-1.2432 2.4627283368198056e-08
-1.2436 2.467557446396619e-08
-1.244 2.4712916670617247e-08
-1.2444 2.4752846776811908e-08
-1.2448 2.4694349481611626e-08
-1.2452 2.473448397223219e-08
-1.2456 2.4691581700469945e-08
-1.246 2.4767934152523538e-08
-1.2464 2.4790527520675025e-08
-1.2468 2.48247874795241e-08
-1.2472 2.4835140623000947e-08
-1.2476 2.4934288130624973e-08
-1.248 2.491311459372934e-08
-1.2484 2.495401872065871e-08
-1.2488 2.4968865694778335e-08
-1.2492 2.5007651841252473e-08
-1.2496 2.506178263998869e-08
-1.25 2.5085205181246805e-08
-1.2504 2.5176712693080294e-08
-1.2508 2.5198392026551863e-08
-1.2512 2.520666758953847e-08
-1.2516 2.5252706191909046e-08
-1.252 2.531118377349392e-08
-1.2524 2.531042054953118e-08
-1.2528 2.5358476962284817e-08
-1.2532 2.5397767278484877e-08
-1.2536 2.5476756951278995e-08
-1.254 2.5496374812396766e-08
-1.2544 2.5552095868887572e-08
-1.2548 2.5584517440199326e-08
-1.2552 2.5618072698211566e-08
-1.2556 2.5668329323241005e-08
-1.256 2.5733055454594517e-08
-1.2564 2.5818296902988283e-08
-1.2568 2.5915454764630128e-08
-1.2572 2.596181571620832e-08
-1.2576 2.605971574947156e-08
-1.258 2.60975287696275e-08
-1.2584 2.6158391860465997e-08
-1.2588 2.6224102191950775e-08
-1.2592 2.6231373205326945e-08
-1.2596 2.630094111976912e-08
-1.26 2.634836041377417e-08
-1.2604 2.631522312411994e-08
-1.2608 2.641148751878181e-08
-1.2612 2.6438079675376705e-08
-1.2616 2.6443022608253427e-08
-1.262 2.6483237467943152e-08
-1.2624 2.65359464100863e-08
-1.2628 2.658623984549855e-08
-1.2632 2.665460996620238e-08
-1.2636 2.6700734615072875e-08
-1.264 2.67519433353637e-08
-1.2644 2.679264252885339e-08
-1.2648 2.6851787564728807e-08
-1.2652 2.6910829060219063e-08
-1.2656 2.702253074483851e-08
-1.266 2.7023179417252166e-08
-1.2664 2.701573545310904e-08
-1.2668 2.7054532840707636e-08
-1.2672 2.7119426392251673e-08
-1.2676 2.7182317346364362e-08
-1.268 2.7179747207815214e-08
-1.2684 2.7269292949910708e-08
-1.2688 2.725634401613845e-08
-1.2692 2.7308662046565882e-08
-1.2696 2.733867780506783e-08
-1.27 2.741886670065e-08
-1.2704 2.743945356560865e-08
-1.2708 2.7522504432108956e-08
-1.2712 2.7513945702366648e-08
-1.2716 2.7581221417482103e-08
-1.272 2.7597131448219406e-08
-1.2724 2.768421309962076e-08
-1.2728 2.7764166216103797e-08
-1.2732 2.7822735737685754e-08
-1.2736 2.7896539305160636e-08
-1.274 2.7913254164437674e-08
-1.2744 2.8014073736947124e-08
-1.2748 2.8085547250215818e-08
-1.2752 2.8152831135457618e-08
-1.2756 2.8191362501127936e-08
-1.276 2.8259612434868576e-08
-1.2764 2.8307264534583723e-08
-1.2768 2.8345144706488314e-08
-1.2772 2.8408887677467476e-08
-1.2776 2.8513542366495313e-08
-1.278 2.85351695205086e-08
-1.2784 2.8564390408729736e-08
-1.2788 2.8589634230283353e-08
-1.2792 2.870337697120063e-08
-1.2796 2.8799927526407597e-08
-1.28 2.8822145550082484e-08
-1.2804 2.8863052885285688e-08
-1.2808 2.9017693385756294e-08
-1.2812 2.912823698898848e-08
-1.2816 2.91804171156202e-08
-1.282 2.9302648381979203e-08
-1.2824 2.9358033072187607e-08
-1.2828 2.9416671931669124e-08
-1.2832 2.9443421874386615e-08
-1.2836 2.9555130151072787e-08
-1.284 2.9636207721861523e-08
-1.2844 2.9712035096161824e-08
-1.2848 2.978529037285554e-08
-1.2852 2.9865716617652554e-08
-1.2856 2.988211050745298e-08
-1.286 2.994635154030977e-08
-1.2864 3.0035463561634165e-08
-1.2868 3.0046354030369443e-08
-1.2872 3.009810038362612e-08
-1.2876 3.020119374317596e-08
-1.288 3.03122820863214e-08
-1.2884 3.03491638705712e-08
-1.2888 3.041014294845428e-08
-1.2892 3.0491396138872566e-08
-1.2896 3.0499694663403705e-08
-1.29 3.0583276549476836e-08
-1.2904 3.0644438196676074e-08
-1.2908 3.078040523971509e-08
-1.2912 3.0877795421060486e-08
-1.2916 3.0982329929826495e-08
-1.292 3.1036902189632416e-08
-1.2924 3.1133454437695935e-08
-1.2928 3.12661886616679e-08
-1.2932 3.135961212533635e-08
-1.2936 3.1463010031326526e-08
-1.294 3.155790385714271e-08
-1.2944 3.1630448460852855e-08
-1.2948 3.1768656991916213e-08
-1.2952 3.185890912533137e-08
-1.2956 3.192876625107107e-08
-1.296 3.200574354940903e-08
-1.2964 3.213592405516408e-08
-1.2968 3.222452260026146e-08
-1.2972 3.236898207014614e-08
-1.2976 3.244628256802891e-08
-1.298 3.255333007569314e-08
-1.2984 3.2680226332771e-08
-1.2988 3.281920041946174e-08
-1.2992 3.300622685106715e-08
-1.2996 3.30648006304603e-08
-1.3 3.3235254674819834e-08
-1.3004 3.3321938261824335e-08
-1.3008 3.336829396039232e-08
-1.3012 3.348954893823424e-08
-1.3016 3.360827092647578e-08
-1.302 3.3713278787790644e-08
-1.3024 3.391523959474253e-08
-1.3028 3.4033953865141314e-08
-1.3032 3.4191673553110514e-08
-1.3036 3.425286699774604e-08
-1.304 3.433521036012655e-08
-1.3044 3.44786843934893e-08
-1.3048 3.4584348182389334e-08
-1.3052 3.469803581286497e-08
-1.3056 3.4852580741303356e-08
-1.306 3.491187490101657e-08
-1.3064 3.50324510524603e-08
-1.3068 3.522201533523144e-08
-1.3072 3.537938730851829e-08
-1.3076 3.561232338193291e-08
-1.308 3.5766658984536235e-08
-1.3084 3.5919333137476984e-08
-1.3088 3.606322735594901e-08
-1.3092 3.617802014092584e-08
-1.3096 3.628456773879837e-08
-1.31 3.64214886838791e-08
-1.3104 3.654734538155639e-08
-1.3108 3.671138808961017e-08
-1.3112 3.690853872560522e-08
-1.3116 3.7021994561723204e-08
-1.312 3.722136118627078e-08
-1.3124 3.7326305360886786e-08
-1.3128 3.7416845398399753e-08
-1.3132 3.758294800705647e-08
-1.3136 3.7722960642262256e-08
-1.314 3.78613941708197e-08
-1.3144 3.804147199516392e-08
-1.3148 3.8201879041723207e-08
-1.3152 3.837445150117591e-08
-1.3156 3.858430463553627e-08
-1.316 3.86225585967402e-08
-1.3164 3.876951225995027e-08
-1.3168 3.899912904766553e-08
-1.3172 3.9143308110593235e-08
-1.3176 3.9310658810612156e-08
-1.318 3.94233281967717e-08
-1.3184 3.958443974988789e-08
-1.3188 3.984321216474995e-08
-1.3192 4.0038659083059335e-08
-1.3196 4.0336648171108013e-08
-1.32 4.0442225444611433e-08
-1.3204 4.0619924682863316e-08
-1.3208 4.078657425866414e-08
-1.3212 4.098276410391786e-08
-1.3216 4.113828433165532e-08
-1.322 4.1359583176498165e-08
-1.3224 4.149710565213962e-08
-1.3228 4.167064218812975e-08
-1.3232 4.1936918384431674e-08
-1.3236 4.216562462595093e-08
-1.324 4.248584476950424e-08
-1.3244 4.265227975875057e-08
-1.3248 4.28961644096817e-08
-1.3252 4.3039039323721303e-08
-1.3256 4.324023996564583e-08
-1.326 4.348725879788297e-08
-1.3264 4.370788587176253e-08
-1.3268 4.402353797810342e-08
-1.3272 4.432658884755149e-08
-1.3276 4.453460077847266e-08
-1.328 4.470324584545842e-08
-1.3284 4.49952325744002e-08
-1.3288 4.520265974432489e-08
-1.3292 4.551367930238088e-08
-1.3296 4.569784572408699e-08
-1.33 4.583703597057461e-08
-1.3304 4.6169646075142975e-08
-1.3308 4.6323229291251274e-08
-1.3312 4.659457608866228e-08
-1.3316 4.687047022119099e-08
-1.332 4.712053491594896e-08
-1.3324 4.73946118583954e-08
-1.3328 4.7670500430651254e-08
-1.3332 4.7895153425634776e-08
-1.3336 4.817883558375291e-08
-1.334 4.8455891838364567e-08
-1.3344 4.872227528549793e-08
-1.3348 4.910451965171718e-08
-1.3352 4.933728568255867e-08
-1.3356 4.9647741489758615e-08
-1.336 4.996985568201996e-08
-1.3364 5.0327937440913315e-08
-1.3368 5.058837542595264e-08
-1.3372 5.083896797948641e-08
-1.3376 5.126834144840759e-08
-1.338 5.152933656363219e-08
-1.3384 5.192543303917444e-08
-1.3388 5.2217161915502576e-08
-1.3392 5.250566817537769e-08
-1.3396 5.278803338217724e-08
-1.34 5.308318832475513e-08
-1.3404 5.340459664023357e-08
-1.3408 5.374588937118574e-08
-1.3412 5.4065779137637906e-08
-1.3416 5.441829189538054e-08
-1.342 5.471464494972738e-08
-1.3424 5.488905336088124e-08
-1.3428 5.530334696725631e-08
-1.3432 5.5777422045947e-08
-1.3436 5.615298566272048e-08
-1.344 5.653434003271603e-08
-1.3444 5.7023087898847764e-08
-1.3448 5.7304880231215666e-08
-1.3452 5.766181295196006e-08
-1.3456 5.8037591950896166e-08
-1.346 5.823036434602038e-08
-1.3464 5.8653046823974795e-08
-1.3468 5.8988004462009767e-08
-1.3472 5.9321160355578876e-08
-1.3476 5.979056947385564e-08
-1.348 6.023623057555529e-08
-1.3484 6.053856572141036e-08
-1.3488 6.10984256569609e-08
-1.3492 6.147150561018677e-08
-1.3496 6.181639179089669e-08
-1.35 6.230931416641858e-08
-1.3504 6.288961607769345e-08
-1.3508 6.328466537292422e-08
-1.3512 6.385814958969276e-08
-1.3516 6.432272784513337e-08
-1.352 6.482864824962709e-08
-1.3524 6.529432290722073e-08
-1.3528 6.583561174186449e-08
-1.3532 6.638663245326115e-08
-1.3536 6.686717982217638e-08
-1.354 6.739612083752458e-08
-1.3544 6.773313254345708e-08
-1.3548 6.811904118477889e-08
-1.3552 6.863575272395662e-08
-1.3556 6.916060761227354e-08
-1.356 6.965732103575035e-08
-1.3564 7.009283199755749e-08
-1.3568 7.046658038547443e-08
-1.3572 7.09813703219099e-08
-1.3576 7.137535789547288e-08
-1.358 7.195123005206366e-08
-1.3584 7.231473597896999e-08
-1.3588 7.303827935951883e-08
-1.3592 7.358618401150226e-08
-1.3596 7.412942200933787e-08
-1.36 7.461157226713449e-08
-1.3604 7.516433247801685e-08
-1.3608 7.573141479751236e-08
-1.3612 7.625200849522443e-08
-1.3616 7.675472272161382e-08
-1.362 7.731502969771814e-08
-1.3624 7.779757654683386e-08
-1.3628 7.832012341657105e-08
-1.3632 7.90532119519587e-08
-1.3636 7.964999669357743e-08
-1.364 8.029817156551127e-08
-1.3644 8.096615990158784e-08
-1.3648 8.165541328876097e-08
-1.3652 8.22431323956052e-08
-1.3656 8.291540481055973e-08
-1.366 8.361285740531356e-08
-1.3664 8.422161565380795e-08
-1.3668 8.508976726596513e-08
-1.3672 8.552898487642537e-08
-1.3676 8.607335835085142e-08
-1.368 8.672509746294907e-08
-1.3684 8.740589781640703e-08
-1.3688 8.802139136306198e-08
-1.3692 8.867744522745498e-08
-1.3696 8.93980458114067e-08
-1.37 9.027240657611492e-08
-1.3704 9.109418813933028e-08
-1.3708 9.177739436907057e-08
-1.3712 9.268427448310216e-08
-1.3716 9.360698122634724e-08
-1.372 9.442620403999454e-08
-1.3724 9.512982560572911e-08
-1.3728 9.591477234813924e-08
-1.3732 9.691273675374922e-08
-1.3736 9.784900721339413e-08
-1.374 9.861613911999188e-08
-1.3744 9.95257732182891e-08
-1.3748 1.0035519055985269e-07
-1.3752 1.0088430447498189e-07
-1.3756 1.0183285218350003e-07
-1.376 1.0262483122245039e-07
-1.3764 1.0362318274908169e-07
-1.3768 1.0417835002932922e-07
-1.3772 1.0517172460251086e-07
-1.3776 1.0618125282161585e-07
-1.378 1.0695972609572995e-07
-1.3784 1.0749678583137433e-07
-1.3788 1.0839481016248794e-07
-1.3792 1.0944731557701182e-07
-1.3796 1.1032496573942876e-07
-1.38 1.1133231875826967e-07
-1.3804 1.1233733361312862e-07
-1.3808 1.133673407338671e-07
-1.3812 1.1445895663900623e-07
-1.3816 1.151856089372799e-07
-1.382 1.1644755388687189e-07
-1.3824 1.1770424916143249e-07
-1.3828 1.1870988784155335e-07
-1.3832 1.1994599946771508e-07
-1.3836 1.2075688160079279e-07
-1.384 1.2195929201161887e-07
-1.3844 1.2289352905675685e-07
-1.3848 1.2398935030489836e-07
-1.3852 1.2470009085768572e-07
-1.3856 1.2553440662642307e-07
-1.386 1.2673238946510334e-07
-1.3864 1.2815996762506578e-07
-1.3868 1.2934202479523395e-07
-1.3872 1.307091619137538e-07
-1.3876 1.3186447642929705e-07
-1.388 1.3329398368206398e-07
-1.3884 1.3438567114190303e-07
-1.3888 1.354994655985853e-07
-1.3892 1.3677161322559944e-07
-1.3896 1.3800280220826332e-07
-1.39 1.3939974412273906e-07
-1.3904 1.4065261245280682e-07
-1.3908 1.416970995392677e-07
-1.3912 1.4299859919227425e-07
-1.3916 1.4452853111369295e-07
-1.392 1.4581351721153317e-07
-1.3924 1.4716885065937444e-07
-1.3928 1.4866365961414044e-07
-1.3932 1.5058168538580147e-07
-1.3936 1.515757383926908e-07
-1.394 1.531983448366574e-07
-1.3944 1.548488501667136e-07
-1.3948 1.562232842916815e-07
-1.3952 1.5766673284517634e-07
-1.3956 1.5901285501379658e-07
-1.396 1.609759420512441e-07
-1.3964 1.6259481347889458e-07
-1.3968 1.6463903032297885e-07
-1.3972 1.6623771558796766e-07
-1.3976 1.6811183494503664e-07
-1.398 1.7001734631730227e-07
-1.3984 1.7200749261866879e-07
-1.3988 1.7328583656884922e-07
-1.3992 1.7524304092553796e-07
-1.3996 1.7720285646321911e-07
-1.4 1.7906133538118154e-07
-1.4004 1.8077076552294747e-07
-1.4008 1.8258234546573503e-07
-1.4012 1.8435212124778877e-07
-1.4016 1.8625683579043273e-07
-1.402 1.881205284126656e-07
-1.4024 1.900187355423413e-07
-1.4028 1.9245897389023822e-07
-1.4032 1.9424672210505543e-07
-1.4036 1.963421180695664e-07
-1.404 1.9814485163418992e-07
-1.4044 2.0001612920748763e-07
-1.4048 2.0178752232289552e-07
-1.4052 2.0361454575972162e-07
-1.4056 2.0574221785350148e-07
-1.406 2.078498735346747e-07
-1.4064 2.0987779443194566e-07
-1.4068 2.1177217135414163e-07
-1.4072 2.1378775375646012e-07
-1.4076 2.1601473966399302e-07
-1.408 2.176907176962333e-07
-1.4084 2.2001851246723222e-07
-1.4088 2.2175991499210015e-07
-1.4092 2.2376627607630845e-07
-1.4096 2.2651005367480218e-07
-1.41 2.2867234396092677e-07
-1.4104 2.3155511617082427e-07
-1.4108 2.3349161243190327e-07
-1.4112 2.358428262517122e-07
-1.4116 2.380087182220535e-07
-1.412 2.4026503722417554e-07
-1.4124 2.4246601219152814e-07
-1.4128 2.447041401585699e-07
-1.4132 2.4735344673163954e-07
-1.4136 2.496156213135604e-07
-1.414 2.5212328326001064e-07
-1.4144 2.5459674055702654e-07
-1.4148 2.575030139722525e-07
-1.4152 2.5990550444782e-07
-1.4156 2.6272894498513236e-07
-1.416 2.6542480082494084e-07
-1.4164 2.677779027336763e-07
-1.4168 2.702845419797651e-07
-1.4172 2.734396639518916e-07
-1.4176 2.763756363894086e-07
-1.418 2.793868658599802e-07
-1.4184 2.8251331404254547e-07
-1.4188 2.8544440983883234e-07
-1.4192 2.883338213182403e-07
-1.4196 2.912272718439585e-07
-1.42 2.9512286065559e-07
-1.4204 2.98040402832476e-07
-1.4208 3.017108689462724e-07
-1.4212 3.041974463084799e-07
-1.4216 3.0763118315538657e-07
-1.422 3.114376966864802e-07
-1.4224 3.1495615121822446e-07
-1.4228 3.1758860770593685e-07
-1.4232 3.2084111892362313e-07
-1.4236 3.2441057648785583e-07
-1.424 3.276858495238367e-07
-1.4244 3.315928023209247e-07
-1.4248 3.352151555672567e-07
-1.4252 3.377171876936807e-07
-1.4256 3.4207541770719035e-07
-1.426 3.4486793488036154e-07
-1.4264 3.4911970210965876e-07
-1.4268 3.532854557959031e-07
-1.4272 3.57418365229682e-07
-1.4276 3.610698822120083e-07
-1.428 3.6575890463070275e-07
-1.4284 3.693788341305379e-07
-1.4288 3.7387801892638577e-07
-1.4292 3.7881757597543985e-07
-1.4296 3.83757122939285e-07
-1.43 3.8793084220651456e-07
-1.4304 3.9128409341505124e-07
-1.4308 3.961843278891383e-07
-1.4312 4.0076615209037166e-07
-1.4316 4.064697253961124e-07
-1.432 4.1002969069883443e-07
-1.4324 4.15097404149477e-07
-1.4328 4.202393872845514e-07
-1.4332 4.2495429649748026e-07
-1.4336 4.2941670747367243e-07
-1.434 4.342479015327294e-07
-1.4344 4.4000827789641304e-07
-1.4348 4.442918852505951e-07
-1.4352 4.489783422862924e-07
-1.4356 4.5352788013805546e-07
-1.436 4.5783603029289004e-07
-1.4364 4.633950915819906e-07
-1.4368 4.676451509540908e-07
-1.4372 4.728453488679805e-07
-1.4376 4.785479424308144e-07
-1.438 4.842225523529486e-07
-1.4384 4.90199532536005e-07
-1.4388 4.964672365094856e-07
-1.4392 5.015838136590999e-07
-1.4396 5.061115051002395e-07
-1.44 5.119506326591382e-07
-1.4404 5.179300527816362e-07
-1.4408 5.227746476617978e-07
-1.4412 5.288358571551698e-07
-1.4416 5.345235683752757e-07
-1.442 5.408001054478528e-07
-1.4424 5.458288567584581e-07
-1.4428 5.509647964704822e-07
-1.4432 5.569427710569755e-07
-1.4436 5.632476778209141e-07
-1.444 5.697163564235671e-07
-1.4444 5.756610371771223e-07
-1.4448 5.834721666602743e-07
-1.4452 5.901637516833689e-07
-1.4456 5.971607364071918e-07
-1.446 6.037404574120873e-07
-1.4464 6.11785632987476e-07
-1.4468 6.193082944033701e-07
-1.4472 6.258924190709243e-07
-1.4476 6.317180446311159e-07
-1.448 6.384792224481605e-07
-1.4484 6.47526755701277e-07
-1.4488 6.552342517606763e-07
-1.4492 6.63844419043656e-07
-1.4496 6.71356880801876e-07
-1.45 6.794847044848699e-07
-1.4504 6.853442817854423e-07
-1.4508 6.938407998823489e-07
-1.4512 7.03567882733516e-07
-1.4516 7.115630794436951e-07
-1.452 7.197978494711636e-07
-1.4524 7.275762978407781e-07
-1.4528 7.381467177450281e-07
-1.4532 7.453400375663924e-07
-1.4536 7.550984166826673e-07
-1.454 7.644772558589223e-07
-1.4544 7.73486369219084e-07
-1.4548 7.828857733768106e-07
-1.4552 7.896398791576757e-07
-1.4556 7.98397516128378e-07
-1.456 8.068482651829756e-07
-1.4564 8.154023663395514e-07
-1.4568 8.256678787263125e-07
-1.4572 8.359887422187253e-07
-1.4576 8.475260613625964e-07
-1.458 8.548306727469177e-07
-1.4584 8.649162528033317e-07
-1.4588 8.746870897456698e-07
-1.4592 8.863939024535964e-07
-1.4596 8.963048588829561e-07
-1.46 9.083134331251693e-07
-1.4604 9.189267605123033e-07
-1.4608 9.296956276039676e-07
-1.4612 9.395667290564586e-07
-1.4616 9.522060882319306e-07
-1.462 9.626659836646656e-07
-1.4624 9.755222213008295e-07
-1.4628 9.903786262358144e-07
-1.4632 1.0048137372208887e-06
-1.4636 1.015522537242594e-06
-1.464 1.02735518439533e-06
-1.4644 1.0393420974740906e-06
-1.4648 1.0543399833154305e-06
-1.4652 1.0662939353644715e-06
-1.4656 1.0773500663710866e-06
-1.466 1.0920654569618755e-06
-1.4664 1.1031596414055847e-06
-1.4668 1.1180985745523051e-06
-1.4672 1.1320205103709917e-06
-1.4676 1.146828077826113e-06
-1.468 1.161768679894928e-06
-1.4684 1.176984759163138e-06
-1.4688 1.1869434114076448e-06
-1.4692 1.2006319406855427e-06
-1.4696 1.216095464595192e-06
-1.47 1.230950316640311e-06
-1.4704 1.2445691721906825e-06
-1.4708 1.257908616409483e-06
-1.4712 1.2756827918642784e-06
-1.4716 1.2893005195937103e-06
-1.472 1.305378506256148e-06
-1.4724 1.3187866803650286e-06
-1.4728 1.3317803176580586e-06
-1.4732 1.3492391674948183e-06
-1.4736 1.3666470102188575e-06
-1.474 1.3817578840179564e-06
-1.4744 1.4000493422392133e-06
-1.4748 1.4174684958765236e-06
-1.4752 1.4358600431876228e-06
-1.4756 1.4562409228618314e-06
-1.476 1.4752470595406442e-06
-1.4764 1.4928759171715042e-06
-1.4768 1.5061284470158548e-06
-1.4772 1.526342829743831e-06
-1.4776 1.5452568882406477e-06
-1.478 1.565641283855535e-06
-1.4784 1.5833395003702056e-06
-1.4788 1.5982104283908055e-06
-1.4792 1.6156573131785868e-06
-1.4796 1.639443415020645e-06
-1.48 1.6615771948298803e-06
-1.4804 1.6802219760762504e-06
-1.4808 1.7034228347183181e-06
-1.4812 1.723382582436578e-06
-1.4816 1.7437992260445913e-06
-1.482 1.7658973935325413e-06
-1.4824 1.7886755407310635e-06
-1.4828 1.8107574086206737e-06
-1.4832 1.8380023342069994e-06
-1.4836 1.8549579812166972e-06
-1.484 1.8850823079120307e-06
-1.4844 1.908651440176932e-06
-1.4848 1.930509779057351e-06
-1.4852 1.9570768405544637e-06
-1.4856 1.9749751013225314e-06
-1.486 2.0047416239218903e-06
-1.4864 2.02876428849696e-06
-1.4868 2.052667812370547e-06
-1.4872 2.0804085660682886e-06
-1.4876 2.1024945020615513e-06
-1.488 2.1295041205236474e-06
-1.4884 2.1546361450353084e-06
-1.4888 2.1816710707508707e-06
-1.4892 2.2099337061447205e-06
-1.4896 2.2406404875648018e-06
-1.49 2.2674931322826036e-06
-1.4904 2.2943963450048143e-06
-1.4908 2.3236190504879214e-06
-1.4912 2.3545228925491163e-06
-1.4916 2.3885586094967564e-06
-1.492 2.4181734463116844e-06
-1.4924 2.4454151323707838e-06
-1.4928 2.475206679542925e-06
-1.4932 2.5076339245635524e-06
-1.4936 2.5393913615478826e-06
-1.494 2.5784432183845615e-06
-1.4944 2.6051388128238336e-06
-1.4948 2.6404436677086547e-06
-1.4952 2.669770527646404e-06
-1.4956 2.7106748055254418e-06
-1.496 2.745779409391087e-06
-1.4964 2.7860037670219876e-06
-1.4968 2.8120263381562187e-06
-1.4972 2.849789424109747e-06
-1.4976 2.8859425322111957e-06
-1.498 2.9291785726075437e-06
-1.4984 2.963795747247379e-06
-1.4988 3.0021804584754797e-06
-1.4992 3.043765685380731e-06
-1.4996 3.081694127492409e-06
-1.5 3.117261645171436e-06
-1.5004 3.1616711213014445e-06
-1.5008 3.1901192907051258e-06
-1.5012 3.2310456573918603e-06
-1.5016 3.2795244332567235e-06
-1.502 3.3174138542461514e-06
-1.5024 3.362476532327584e-06
-1.5028 3.404901393033474e-06
-1.5032 3.457936768942194e-06
-1.5036 3.505675551963375e-06
-1.504 3.545378660891922e-06
-1.5044 3.5950664351782073e-06
-1.5048 3.6455071920171104e-06
-1.5052 3.6917091569887025e-06
-1.5056 3.7466945013161554e-06
-1.506 3.795134387590377e-06
-1.5064 3.843528163324155e-06
-1.5068 3.896132796835158e-06
-1.5072 3.94741749282235e-06
-1.5076 4.003151002830099e-06
-1.508 4.053544202482726e-06
-1.5084 4.1119937401911215e-06
-1.5088 4.168040886859586e-06
-1.5092 4.233094028421688e-06
-1.5096 4.285952912942765e-06
-1.51 4.350370772615676e-06
-1.5104 4.404398792721359e-06
-1.5108 4.459575917738583e-06
-1.5112 4.524204585447062e-06
-1.5116 4.585485047042318e-06
-1.512 4.651951248010529e-06
-1.5124 4.726178292929496e-06
-1.5128 4.781208388067428e-06
-1.5132 4.835306979710367e-06
-1.5136 4.895360692303127e-06
-1.514 4.96191610412272e-06
-1.5144 5.033583774974809e-06
-1.5148 5.097310202604548e-06
-1.5152 5.171863220872854e-06
-1.5156 5.233736224993442e-06
-1.516 5.293505935249793e-06
-1.5164 5.362426991366623e-06
-1.5168 5.425336610340442e-06
-1.5172 5.500049704145226e-06
-1.5176 5.577265744195209e-06
-1.518 5.6572354350847276e-06
-1.5184 5.729402178517612e-06
-1.5188 5.8187052020923926e-06
-1.5192 5.883588260569681e-06
-1.5196 5.969223871567147e-06
-1.52 6.038121831976411e-06
-1.5204 6.117904343745853e-06
-1.5208 6.2175425322734425e-06
-1.5212 6.307624817939317e-06
-1.5216 6.394670703741791e-06
-1.522 6.480110091115634e-06
-1.5224 6.562044706566625e-06
-1.5228 6.659375155154866e-06
-1.5232 6.742836483215329e-06
-1.5236 6.819823459373574e-06
-1.524 6.914569357709527e-06
-1.5244 7.00603759129067e-06
-1.5248 7.106779209354174e-06
-1.5252 7.1920122417773625e-06
-1.5256 7.303526691475461e-06
-1.526 7.4116721265499e-06
-1.5264 7.497747849514379e-06
-1.5268 7.585740560914975e-06
-1.5272 7.717902183276705e-06
-1.5276 7.821327459265655e-06
-1.528 7.931553669201828e-06
-1.5284 8.036992556473812e-06
-1.5288 8.150699012842841e-06
-1.5292 8.268497460159723e-06
-1.5296 8.38841567926721e-06
-1.53 8.506457884824635e-06
-1.5304 8.632961586365837e-06
-1.5308 8.77425702058137e-06
-1.5312 8.884078313035435e-06
-1.5316 9.007649561947113e-06
-1.532 9.152185588081905e-06
-1.5324 9.28603945330476e-06
-1.5328 9.40984722767425e-06
-1.5332 9.541008723224848e-06
-1.5336 9.672711119763584e-06
-1.534 9.814772524667918e-06
-1.5344 9.94717994138861e-06
-1.5348 1.0084536026868342e-05
-1.5352 1.024447955683011e-05
-1.5356 1.04128979092988e-05
-1.536 1.0528125196547316e-05
-1.5364 1.0676286380886074e-05
-1.5368 1.0851973783556268e-05
-1.5372 1.0973190390860185e-05
-1.5376 1.1149525046005757e-05
-1.538 1.1323587604745873e-05
-1.5384 1.149148743147852e-05
-1.5388 1.1651308444430144e-05
-1.5392 1.1804242393257417e-05
-1.5396 1.1952464502281921e-05
-1.54 1.2125437942157204e-05
-1.5404 1.2286067681257523e-05
-1.5408 1.245963599921173e-05
-1.5412 1.2633356096914614e-05
-1.5416 1.281122974399228e-05
-1.542 1.3017085980413335e-05
-1.5424 1.3219472186682734e-05
-1.5428 1.3407969861213181e-05
-1.5432 1.361557185391628e-05
-1.5436 1.3845468741204445e-05
-1.544 1.4016677131048556e-05
-1.5444 1.4257398789050403e-05
-1.5448 1.4455539038533154e-05
-1.5452 1.4694778082402747e-05
-1.5456 1.4875059805018799e-05
-1.546 1.5095010037765666e-05
-1.5464 1.531483170812447e-05
-1.5468 1.5514486873853616e-05
-1.5472 1.5733318454168834e-05
-1.5476 1.5992178964311007e-05
-1.548 1.620611635674512e-05
-1.5484 1.646273629437939e-05
-1.5488 1.669037869064398e-05
-1.5492 1.6941661295530033e-05
-1.5496 1.718820475743746e-05
-1.55 1.744376848578922e-05
-1.5504 1.770352283819933e-05
-1.5508 1.7971351644090092e-05
-1.5512 1.819724439154667e-05
-1.5516 1.847884230511179e-05
-1.552 1.8737325921543182e-05
-1.5524 1.8944313134558027e-05
-1.5528 1.921722402883032e-05
-1.5532 1.95034128740518e-05
-1.5536 1.9793698124362937e-05
-1.554 2.0082397552943868e-05
-1.5544 2.039566240989854e-05
-1.5548 2.0688742368149537e-05
-1.5552 2.101294382261222e-05
-1.5556 2.134922401502508e-05
-1.556 2.164928662576691e-05
-1.5564 2.187074670058857e-05
-1.5568 2.2228890300097464e-05
-1.5572 2.2519586509282712e-05
-1.5576 2.2872048343369927e-05
-1.558 2.3225368230008685e-05
-1.5584 2.359117461663109e-05
-1.5588 2.3931722835605663e-05
-1.5592 2.4264082545126865e-05
-1.5596 2.458908087529677e-05
-1.56 2.496489246393649e-05
-1.5604 2.5301638179783914e-05
-1.5608 2.5681175849520594e-05
-1.5612 2.610420383482214e-05
-1.5616 2.647539397987855e-05
-1.562 2.689790125919358e-05
-1.5624 2.7255209123585764e-05
-1.5628 2.7672425323193896e-05
-1.5632 2.8120855559482735e-05
-1.5636 2.8461875062087035e-05
-1.564 2.8984675795681712e-05
-1.5644 2.9435244521377767e-05
-1.5648 2.9967773058716447e-05
-1.5652 3.034812441580075e-05
-1.5656 3.0802964771374194e-05
-1.566 3.134914331883669e-05
-1.5664 3.183815896587494e-05
-1.5668 3.237235875546779e-05
-1.5672 3.278655681329696e-05
-1.5676 3.3309978371132064e-05
-1.568 3.375454673652519e-05
-1.5684 3.4395931147621626e-05
-1.5688 3.489901719408187e-05
-1.5692 3.539940496031569e-05
-1.5696 3.599189225495268e-05
-1.57 3.654015310138274e-05
-1.5704 3.720550989883794e-05
-1.5708 3.7835743771768214e-05
-1.5712 3.842625625384926e-05
-1.5716 3.898885279203709e-05
-1.572 3.952180816428056e-05
-1.5724 4.01671055854684e-05
-1.5728 4.090063642701714e-05
-1.5732 4.159149962591721e-05
-1.5736 4.218699838908135e-05
-1.574 4.289036312439053e-05
-1.5744 4.3501782368253545e-05
-1.5748 4.413853888442018e-05
-1.5752 4.493495700812363e-05
-1.5756 4.562891127823505e-05
-1.576 4.634184756075283e-05
-1.5764 4.700532007447566e-05
-1.5768 4.7749377747019265e-05
-1.5772 4.848037703329801e-05
-1.5776 4.918615985158338e-05
-1.578 4.995068144240328e-05
-1.5784 5.078945977768644e-05
-1.5788 5.15470086531185e-05
-1.5792 5.236846572122505e-05
-1.5796 5.3147799824135184e-05
-1.58 5.3910797456317476e-05
-1.5804 5.489508168377136e-05
-1.5808 5.579051270372853e-05
-1.5812 5.669998824726497e-05
-1.5816 5.771815216123413e-05
-1.582 5.878980845853969e-05
-1.5824 5.971551495351662e-05
-1.5828 6.0788710239263975e-05
-1.5832 6.182151146920589e-05
-1.5836 6.282630957624792e-05
-1.584 6.389729594465159e-05
-1.5844 6.499599259055991e-05
-1.5848 6.598716477035528e-05
-1.5852 6.697564623999872e-05
-1.5856 6.81403549729456e-05
-1.586 6.930394217420683e-05
-1.5864 7.03371955463325e-05
-1.5868 7.133222122306518e-05
-1.5872 7.261130873005765e-05
-1.5876 7.367188077896195e-05
-1.588 7.495091499984748e-05
-1.5884 7.597758940190098e-05
-1.5888 7.716770123083553e-05
-1.5892 7.829792381948445e-05
-1.5896 7.970485252110855e-05
-1.59 8.095458633081625e-05
-1.5904 8.223612237348681e-05
-1.5908 8.38624140562094e-05
-1.5912 8.536627054622672e-05
-1.5916 8.663021344196697e-05
-1.592 8.83420419226649e-05
-1.5924 8.966417633162415e-05
-1.5928 9.097858351802525e-05
-1.5932 9.279261244709708e-05
-1.5936 9.433799874090887e-05
-1.594 9.58231843742461e-05
-1.5944 9.75160991437951e-05
-1.5948 9.930903587697834e-05
-1.5952 0.0001008021912708165
-1.5956 0.00010220647513573222
-1.596 0.00010402182151636343
-1.5964 0.00010584921150824515
-1.5968 0.00010767322743290798
-1.5972 0.00010974964459310773
-1.5976 0.0001118066827266586
-1.598 0.00011359281416311741
-1.5984 0.00011565489092541247
-1.5988 0.00011712027119825725
-1.5992 0.00011907765049204728
-1.5996 0.00012118160213565818
-1.6 0.00012338142087476333
-1.6004 0.0001253663335663664
-1.6008 0.00012743969073031517
-1.6012 0.00012942863922929548
-1.6016 0.0001318083923697649
-1.602 0.0001341669971756644
-1.6024 0.00013683014249018496
-1.6028 0.00013903493722706626
-1.6032 0.00014149745900811787
-1.6036 0.00014400079191969397
-1.604 0.00014621289139848343
-1.6044 0.00014850517634759636
-1.6048 0.00015126415753220093
-1.6052 0.0001537348166373622
-1.6056 0.00015617019885504592
-1.606 0.0001591520745694653
-1.6064 0.00016206585108924785
-1.6068 0.00016468058559795321
-1.6072 0.000167350319288981
-1.6076 0.00017028736047963315
-1.608 0.0001736070174892739
-1.6084 0.00017671489557097446
-1.6088 0.00017972851952248906
-1.6092 0.00018317692367560785
-1.6096 0.00018613122943325448
-1.61 0.0001898869698146639
-1.6104 0.00019358539334224264
-1.6108 0.00019696670401682744
-1.6112 0.00020026030522229236
-1.6116 0.0002039033411579646
-1.612 0.00020770079062887385
-1.6124 0.00021130710283095332
-1.6128 0.00021487411301945294
-1.6132 0.00021920146827871206
-1.6136 0.00022263658034347346
-1.614 0.00022659809470502074
-1.6144 0.00023054594543409285
-1.6148 0.00023461321328201604
-1.6152 0.00023912531528386163
-1.6156 0.0002436059570632131
-1.616 0.00024803890951546973
-1.6164 0.0002525284737581905
-1.6168 0.00025674037896339857
-1.6172 0.00026151814504168843
-1.6176 0.0002663292202592828
-1.618 0.0002715691204364326
-1.6184 0.00027684771062948515
-1.6188 0.0002819227290232918
-1.6192 0.0002871509759798343
-1.6196 0.0002925492255894713
-1.62 0.0002982767583412619
-1.6204 0.0003035909133681599
-1.6208 0.0003095592050161222
-1.6212 0.0003150710447782918
-1.6216 0.00032203171843455774
-1.622 0.0003279106729708307
-1.6224 0.0003341781836774616
-1.6228 0.0003405991857060668
-1.6232 0.0003468598167675443
-1.6236 0.00035342067609401184
-1.624 0.0003595951888985429
-1.6244 0.0003668186308154234
-1.6248 0.0003735300399255612
-1.6252 0.00038058248494670223
-1.6256 0.00038762480291539426
-1.626 0.00039556260393266323
-1.6264 0.00040206203496301524
-1.6268 0.0004105292649986515
-1.6272 0.0004188714149527726
-1.6276 0.00042731638307611837
-1.628 0.00043523282908183473
-1.6284 0.0004424487142070209
-1.6288 0.00045205129786440743
-1.6292 0.0004601139277633976
-1.6296 0.00046923088156801906
-1.63 0.0004780687059112081
-1.6304 0.0004880591575756304
-1.6308 0.0004988564358329754
-1.6312 0.0005084535884338842
-1.6316 0.0005171634888909858
-1.632 0.0005268298399132525
-1.6324 0.0005377983024117604
-1.6328 0.0005468152780045163
-1.6332 0.000557542377998568
-1.6336 0.0005692318987525393
-1.634 0.0005800721614372331
-1.6344 0.0005920958670616293
-1.6348 0.0006034181352245545
-1.6352 0.0006145827005731427
-1.6356 0.0006276905621641467
-1.636 0.0006393179235532309
-1.6364 0.000651510148464813
-1.6368 0.0006641808332996899
-1.6372 0.0006770659225663386
-1.6376 0.0006903963501982878
-1.638 0.000704097646728982
-1.6384 0.000717959531058204
-1.6388 0.0007330687881073513
-1.6392 0.0007490381665516519
-1.6396 0.0007641070358124344
-1.64 0.0007798679030480157
-1.6404 0.0007966430537005561
-1.6408 0.000810189597865279
-1.6412 0.0008274989360350009
-1.6416 0.0008440335037620295
-1.642 0.0008597916108304246
-1.6424 0.0008768841496681684
-1.6428 0.0008961954415538832
-1.6432 0.0009120482127539932
-1.6436 0.0009319333129607088
-1.644 0.0009510306691578946
-1.6444 0.0009721066444388917
-1.6448 0.0009908914478961694
-1.6452 0.001009012757873943
-1.6456 0.0010296735040399817
-1.646 0.0010499403155302149
-1.6464 0.0010719140658253781
-1.6468 0.001095976570945041
-1.6472 0.0011166946444468129
-1.6476 0.0011407828321280315
-1.648 0.0011655634871545607
-1.6484 0.00119026129482535
-1.6488 0.0012167118605463266
-1.6492 0.00124320713700567
-1.6496 0.0012678702203576587
-1.65 0.0012960912989563793
-1.6504 0.0013247033321747445
-1.6508 0.0013518545842536854
-1.6512 0.0013844160832132202
-1.6516 0.0014120264138857326
-1.652 0.0014411500187738316
-1.6524 0.0014718617565579063
-1.6528 0.001506766989634947
-1.6532 0.0015354312459916778
-1.6536 0.0015688706060686284
-1.654 0.0016054801144339227
-1.6544 0.001637668784864559
-1.6548 0.0016753705066615472
-1.6552 0.0017103675957404762
-1.6556 0.0017492097328191197
-1.656 0.001785248419337792
-1.6564 0.001827464940177453
-1.6568 0.001866478019102442
-1.6572 0.001908429322333597
-1.6576 0.0019532580511866958
-1.658 0.0019960132413067064
-1.6584 0.0020418854846683543
-1.6588 0.002087338517450531
-1.6592 0.0021343056654620266
-1.6596 0.002180905105233533
-1.66 0.00222880088866906
-1.6604 0.002269386693943244
-1.6608 0.0023214896203237337
-1.6612 0.0023742119527106853
-1.6616 0.0024309154264702515
-1.662 0.002491703823041634
-1.6624 0.0025486458284570235
-1.6628 0.0026018428056225214
-1.6632 0.0026604855572973487
-1.6636 0.002719705629324438
-1.664 0.0027828210432550146
-1.6644 0.002849220816730142
-1.6648 0.002922720386861485
-1.6652 0.0029863450999467536
-1.6656 0.003052954483927065
-1.666 0.0031180922588327042
-1.6664 0.0031959256764222156
-1.6668 0.0032624891731717364
-1.6672 0.003339856745257083
-1.6676 0.0034128516191916994
-1.668 0.003491486863763152
-1.6684 0.003583334958993425
-1.6688 0.00366806687314499
-1.6692 0.003760628746427251
-1.6696 0.0038476644751665786
-1.67 0.003936752527491631
-1.6704 0.004019289429891469
-1.6708 0.004109450479707749
-1.6712 0.004215528991049749
-1.6716 0.004316431422900194
-1.672 0.0044135286547905845
-1.6724 0.0045219890365391395
-1.6728 0.004634144788834002
-1.6732 0.0047400328764958845
-1.6736 0.004858385649131964
-1.674 0.004978592569532868
-1.6744 0.005096760553682123
-1.6748 0.005213182455703111
-1.6752 0.005356744469930925
-1.6756 0.005483251585896448
-1.676 0.005608578877819774
-1.6764 0.005737136369412243
-1.6768 0.005873303995519811
-1.6772 0.006021224239399904
-1.6776 0.00618286972155309
-1.678 0.006330268092305613
-1.6784 0.006468038196156387
-1.6788 0.00662342840430471
-1.6792 0.006788314913323223
-1.6796 0.006960938329117543
-1.68 0.0071338001277424816
-1.6804 0.007308468642527895
-1.6808 0.007492752111552891
-1.6812 0.007681964847575654
-1.6816 0.00789199866578372
-1.682 0.008087878950837915
-1.6824 0.0082978033252691
-1.6828 0.008499752117583748
-1.6832 0.008720172477266048
-1.6836 0.008932787800130786
-1.684 0.009140131719239282
-1.6844 0.00936434328874332
-1.6848 0.009608681444721375
-1.6852 0.009876811050705585
-1.6856 0.010117103868786483
-1.686 0.010386013155905682
-1.6864 0.010634673256673966
-1.6868 0.010901384562788283
-1.6872 0.011210625741998265
-1.6876 0.011493241902848013
-1.688 0.01177902890207989
-1.6884 0.012091679898115486
-1.6888 0.012387540438486389
-1.6892 0.012703720432143377
-1.6896 0.01302839652558106
-1.69 0.013361777501053412
-1.6904 0.013707776174582785
-1.6908 0.01403181766899421
-1.6912 0.014376749551762128
-1.6916 0.01474565137346712
-1.692 0.015124110100585989
-1.6924 0.015519566157766986
-1.6928 0.015895706193565496
-1.6932 0.016312068154225992
-1.6936 0.01672936712721198
-1.694 0.01716348182068197
-1.6944 0.01764663197440399
-1.6948 0.018071177941751188
-1.6952 0.018591590912926954
-1.6956 0.019032754268334746
-1.696 0.019530881475932606
-1.6964 0.020030470320191694
-1.6968 0.02056016807150892
-1.6972 0.021090201780309115
-1.6976 0.02168299920195785
-1.698 0.022259090205628662
-1.6984 0.02284626889080946
-1.6988 0.023483003101249907
-1.6992 0.024109868642996204
-1.6996 0.02476379687666043
-1.7 0.02536964054206593
-1.7004 0.02606299911294837
-1.7008 0.026705834139201558
-1.7012 0.02747509758860168
-1.7016 0.028225757507858582
-1.702 0.029036103292926517
-1.7024 0.02984740395574713
-1.7028 0.03063028103460234
-1.7032 0.031431921132633274
-1.7036 0.03225888098218402
-1.704 0.03307902086643632
-1.7044 0.03389456979025825
-1.7048 0.034819218353244655
-1.7052 0.03581572055290755
-1.7056 0.03674530116334752
-1.706 0.03780903926243839
-1.7064 0.038880603319962785
-1.7068 0.03990065124808802
-1.7072 0.040981612330323755
-1.7076 0.042055192400040325
-1.708 0.04315518436055917
-1.7084 0.04426953511788632
-1.7088 0.04538935354118739
-1.7092 0.046752149324171814
-1.7096 0.047888817359557675
-1.71 0.04917122801047497
-1.7104 0.050507484624460024
-1.7108 0.05184006633169802
-1.7112 0.05323599606169792
-1.7116 0.05457939377730029
-1.712 0.05601940440950235
-1.7124 0.057599391283699695
-1.7128 0.0590776447597947
-1.7132 0.06081459398273138
-1.7136 0.06251618557076975
-1.714 0.06424694389147868
-1.7144 0.06593502471398925
-1.7148 0.06770079006983849
-1.7152 0.06948862912762067
-1.7156 0.07147194243185845
-1.716 0.07334337661397426
-1.7164 0.07541269907810198
-1.7168 0.0775570586398672
-1.7172 0.07969308223776204
-1.7176 0.08195768864973653
-1.718 0.08417941225222471
-1.7184 0.08680423128166516
-1.7188 0.08934020668125747
-1.7192 0.09170150403762346
-1.7196 0.09436393775539345
-1.72 0.09699199857604367
-1.7204 0.09945707666577591
-1.7208 0.10211297853144144
-1.7212 0.1049456897089843
-1.7216 0.10804214708335266
-1.722 0.1110580785681477
-1.7224 0.11439207245565786
-1.7228 0.11727454303555646
-1.7232 0.1206743864024945
-1.7236 0.12390023613527221
-1.724 0.1270656650879693
-1.7244 0.13080082820369285
-1.7248 0.1341954618679802
-1.7252 0.13835782066975694
-1.7256 0.14214199663596525
-1.726 0.14584266980968158
-1.7264 0.149824444121031
-1.7268 0.15395557230616874
-1.7272 0.15846009526929078
-1.7276 0.16256089868127124
-1.728 0.16666620454546408
-1.7284 0.17104587245332
-1.7288 0.17593534750819836
-1.7292 0.180689271785354
-1.7296 0.1855106315733579
-1.73 0.19061486344766226
-1.7304 0.1958945218860655
-1.7308 0.20144354287677133
-1.7312 0.20760786952203833
-1.7316 0.21353786164611688
-1.732 0.21927906464295982
-1.7324 0.2248899819114532
-1.7328 0.2312288282041333
-1.7332 0.23820007511579092
-1.7336 0.24485024599234154
-1.734 0.25149873389167676
-1.7344 0.2583770012505304
-1.7348 0.26543233997933435
-1.7352 0.2735119555012467
-1.7356 0.2812270959653023
-1.736 0.2889288717658781
-1.7364 0.29737298565248793
-1.7368 0.3046725238206177
-1.7372 0.31350213024505974
-1.7376 0.32157952201902473
-1.738 0.3300012834971735
-1.7384 0.339592448265976
-1.7388 0.3490882550765383
-1.7392 0.3583941975632967
-1.7396 0.36850183060955655
-1.74 0.37807585817522465
-1.7404 0.38809775052767187
-1.7408 0.39954816133898285
-1.7412 0.41101180108837476
-1.7416 0.4220244926529814
-1.742 0.4330239743290905
-1.7424 0.4468676659769581
-1.7428 0.4588900276687766
-1.7432 0.47031275954493784
-1.7436 0.48321915309531327
-1.744 0.49623556024443655
-1.7444 0.5100482355406007
-1.7448 0.5242220319527006
-1.7452 0.5375010553526791
-1.7456 0.5520547812109267
-1.746 0.5665002346464441
-1.7464 0.5822124434551527
-1.7468 0.5995073262877642
-1.7472 0.6133387343247624
-1.7476 0.629326866857009
-1.748 0.6461944271005241
-1.7484 0.6626392127154107
-1.7488 0.6799394040871692
-1.7492 0.696515662496188
-1.7496 0.7167322291349412
-1.75 0.7353132024493776
-1.7504 0.7526213816218547
-1.7508 0.7710189239397172
-1.7512 0.7903629435427861
-1.7516 0.8101317483880307
-1.752 0.8319132253063078
-1.7524 0.853467865806521
-1.7528 0.8766207394252398
-1.7532 0.9000070314392298
-1.7536 0.9207934880444179
-1.754 0.9431221614249284
-1.7544 0.9693483789957275
-1.7548 0.9933592636128399
-1.7552 1.0174065989516583
-1.7556 1.0431863516711293
-1.756 1.070607475707365
-1.7564 1.0982934869825578
-1.7568 1.1240634558512586
-1.7572 1.1539112881476217
-1.7576 1.1795420811549409
-1.758 1.2105011259621004
-1.7584 1.2375827853386276
-1.7588 1.268095213755387
-1.7592 1.2987878706743046
-1.7596 1.3291579547236816
-1.76 1.35964733579692
-1.7604 1.3933342124514976
-1.7608 1.4242296855448007
-1.7612 1.4592198329911172
-1.7616 1.4928019300004802
-1.762 1.5307285464094345
-1.7624 1.5720186833800114
-1.7628 1.610825833951063
-1.7632 1.6425468613753602
-1.7636 1.682370383748733
-1.764 1.719559567587435
-1.7644 1.7579436724677342
-1.7648 1.8033200712662398
-1.7652 1.8461136194946057
-1.7656 1.8924164341965104
-1.766 1.940716707623663
-1.7664 1.9820411234127076
-1.7668 2.029027346604125
-1.7672 2.0757017679130363
-1.7676 2.125096444525443
-1.768 2.170122468738839
-1.7684 2.223108169197337
-1.7688 2.2711718795189073
-1.7692 2.327075657179168
-1.7696 2.3804511020296024
-1.77 2.4334150796929737
-1.7704 2.4869473033833485
-1.7708 2.5436569471841906
-1.7712 2.6032964348635756
-1.7716 2.656981242444677
-1.772 2.7118743883376233
-1.7724 2.7719526382470194
-1.7728 2.834422688286167
-1.7732 2.8917732686776483
-1.7736 2.949218746951664
-1.774 3.0041300210881805
-1.7744 3.0718576541058016
-1.7748 3.1337376832398407
-1.7752 3.2025253157768816
-1.7756 3.275053086829859
-1.776 3.3438895958113264
-1.7764 3.4110344549376053
-1.7768 3.4850191769018295
-1.7772 3.5567349268500963
-1.7776 3.6209229325611374
-1.778 3.701710052152361
-1.7784 3.783033895429154
-1.7788 3.860060503773207
-1.7792 3.9308161994898887
-1.7796 4.015638808298399
-1.78 4.097320333725599
-1.7804 4.18641063748473
-1.7808 4.272175936350966
-1.7812 4.345751103580205
-1.7816 4.437947732258055
-1.782 4.516727002651222
-1.7824 4.605721248767454
-1.7828 4.6904058526611845
-1.7832 4.771514187343184
-1.7836 4.860659732113601
-1.784 4.946451352516378
-1.7844 5.040932056256097
-1.7848 5.125699075924613
-1.7852 5.224798103838052
-1.7856 5.3212371687413595
-1.786 5.417402090676524
-1.7864 5.507270485064017
-1.7868 5.6091061167734955
-1.7872 5.713405814041263
-1.7876 5.801256790414534
-1.788 5.897677753606075
-1.7884 5.992905826785158
-1.7888 6.0876770011263375
-1.7892 6.202251503605285
-1.7896 6.296886037698378
-1.79 6.404429765658848
-1.7904 6.512120494410352
-1.7908 6.632187992865572
-1.7912 6.745062740010697
-1.7916 6.840902910163538
-1.792 6.943522188032963
-1.7924 7.06076098278033
-1.7928 7.183253535316481
-1.7932 7.3075173560735225
-1.7936 7.397946873620893
-1.794 7.50076072194296
-1.7944 7.620241299270369
-1.7948 7.74602598429799
-1.7952 7.866565871277999
-1.7956 7.970490755979607
-1.796 8.08961538257056
-1.7964 8.202153437981716
-1.7968 8.313240577269504
-1.7972 8.451146469753244
-1.7976 8.526664085605162
-1.798 8.65152115177465
-1.7984 8.781270221087075
-1.7988 8.869515240619505
-1.7992 9.001090082910434
-1.7996 9.113903314513344
-1.8 9.237291959834925
-1.8004 9.37335915748109
-1.8008 9.500223297087754
-1.8012 9.609517132196167
-1.8016 9.750707859729891
-1.802 9.866311043173406
-1.8024 9.997396900907276
-1.8028 10.100888867153541
-1.8032 10.228651851238459
-1.8036 10.333626562445673
-1.804 10.434875168608412
-1.8044 10.555881377244113
-1.8048 10.69731425631893
-1.8052 10.817133299287907
-1.8056 10.938887283041153
-1.806 11.047575288711196
-1.8064 11.173647072037419
-1.8068 11.304183454348875
-1.8072 11.430704886435981
-1.8076 11.56694351124652
-1.808 11.65320005133547
-1.8084 11.737014061939119
-1.8088 11.865208603079656
-1.8092 11.972514228242106
-1.8096 12.073260484255002
-1.81 12.168591076456952
-1.8104 12.29183482751289
-1.8108 12.410895430838966
-1.8112 12.500663927278188
-1.8116 12.603921417750808
-1.812 12.712717815304021
-1.8124 12.78977988519635
-1.8128 12.882116429782425
-1.8132 12.98388502603595
-1.8136 13.044551087389957
-1.814 13.14220940794187
-1.8144 13.237886437121368
-1.8148 13.306289137805479
-1.8152 13.41975899014836
-1.8156 13.52108868601585
-1.816 13.560261935703172
-1.8164 13.629755957742264
-1.8168 13.695357729445144
-1.8172 13.766090908515194
-1.8176 13.834496656259024
-1.818 13.903769394129085
-1.8184 13.947706815358291
-1.8188 14.008241008515212
-1.8192 14.064050826395327
-1.8196 14.11298430614147
-1.82 14.184249593645028
-1.8204 14.226412679852588
-1.8208 14.274038181930274
-1.8212 14.352210117300386
-1.8216 14.358375497428437
-1.822 14.410658344557906
-1.8224 14.384695222711466
-1.8228 14.425462084932985
-1.8232 14.456253313049105
-1.8236 14.46844454409788
-1.824 14.501528400993045
-1.8244 14.512962428776255
-1.8248 14.539685400884544
-1.8252 14.534029376607393
-1.8256 14.508482689414466
-1.826 14.485899494383558
-1.8264 14.4597972918048
-1.8268 14.463529608408578
-1.8272 14.43514597752451
-1.8276 14.496822211479799
-1.828 14.44405371820184
-1.8284 14.423595683723363
-1.8288 14.413446390495334
-1.8292 14.380573399997209
-1.8296 14.331365677009321
-1.83 14.272803928010545
-1.8304 14.252815856338541
-1.8308 14.237807385734493
-1.8312 14.205572447394966
-1.8316 14.155157964412892
-1.832 14.122061375926583
-1.8324 14.055901812011669
-1.8328 13.982451406014718
-1.8332 13.91610640312176
-1.8336 13.862885647065998
-1.834 13.804253466558922
-1.8344 13.727261621784942
-1.8348 13.636525343155652
-1.8352 13.50992113058113
-1.8356 13.44014974241974
-1.836 13.358922583659854
-1.8364 13.2507206386106
-1.8368 13.146091835975657
-1.8372 13.071879530238139
-1.8376 12.988688978307865
-1.838 12.886235307173251
-1.8384 12.781655310366213
-1.8388 12.69097322185081
-1.8392 12.596057374548618
-1.8396 12.487067229994544
-1.84 12.37221920011005
-1.8404 12.228389265901022
-1.8408 12.0996466380622
-1.8412 11.978423158467649
-1.8416 11.854298094815066
-1.842 11.746605500766986
-1.8424 11.619580630980582
-1.8428 11.487472558595709
-1.8432 11.376246259430644
-1.8436 11.237069119223703
-1.844 11.112117739231035
-1.8444 10.954235999693005
-1.8448 10.839294718696411
-1.8452 10.695691352468247
-1.8456 10.552647631533244
-1.846 10.402545018692182
-1.8464 10.275720566788554
-1.8468 10.11911508169292
-1.8472 9.982613537593819
-1.8476 9.828768552182625
-1.848 9.680530354822475
-1.8484 9.519977877946157
-1.8488 9.373705507483283
-1.8492 9.239306906872423
-1.8496 9.067838702621836
-1.85 8.914606745916538
-1.8504 8.759444284845634
-1.8508 8.590804172167626
-1.8512 8.440560696418432
-1.8516 8.28908386489049
-1.852 8.137307572801339
-1.8524 7.980026529748459
-1.8528 7.82639170343974
-1.8532 7.674916838962079
-1.8536 7.533823468585464
-1.854 7.374831045893136
-1.8544 7.233917884178184
-1.8548 7.068306432387459
-1.8552 6.9016033303958855
-1.8556 6.7579807412241975
-1.856 6.594309679731695
-1.8564 6.4480201833170385
-1.8568 6.291059239105406
-1.8572 6.141592591315129
-1.8576 6.0039376191097125
-1.858 5.862189029921895
-1.8584 5.715291866339417
-1.8588 5.564655098539344
-1.8592 5.420808790919282
-1.8596 5.289359405954277
-1.86 5.165973104286053
-1.8604 5.019278591220279
-1.8608 4.892246821768287
-1.8612 4.757142260266849
-1.8616 4.625307813337629
-1.862 4.487362772274399
-1.8624 4.369054007675363
-1.8628 4.239329196813558
-1.8632 4.117490096730612
-1.8636 3.9914782021002386
-1.864 3.87034453906134
-1.8644 3.7644936462655774
-1.8648 3.6467740917643194
-1.8652 3.5337793082414946
-1.8656 3.4248148691925753
-1.866 3.3139900736665964
-1.8664 3.205509978456093
-1.8668 3.0992851767260663
-1.8672 2.995860010357386
-1.8676 2.8932149300369012
-1.868 2.8052089774874913
-1.8684 2.713376421139994
-1.8688 2.620607215229844
-1.8692 2.5320811749615815
-1.8696 2.4385591226657164
-1.87 2.34835152917247
-1.8704 2.2603351703750847
-1.8708 2.1745132604688813
-1.8712 2.0954478079421355
-1.8716 2.0209176587225732
-1.872 1.9455250411442524
-1.8724 1.8685455870626075
-1.8728 1.7965165108507022
-1.8732 1.7251724489089917
-1.8736 1.6602651911337265
-1.874 1.5921825659683384
-1.8744 1.5266919639563996
-1.8748 1.4656684179945116
-1.8752 1.4073351859778203
-1.8756 1.3494365644701496
-1.876 1.2920421042351418
-1.8764 1.238553078656121
-1.8768 1.1842871799859733
-1.8772 1.13596045153679
-1.8776 1.0868298635674374
-1.878 1.0385124844301146
-1.8784 0.9916986306539842
-1.8788 0.9459200553396312
-1.8792 0.903548718434779
-1.8796 0.8629921403716772
-1.88 0.8218177213104083
-1.8804 0.7857530174461687
-1.8808 0.7479272657919713
-1.8812 0.7149032095233636
-1.8816 0.6787258206758139
-1.882 0.6467168164630375
-1.8824 0.6142324188437204
-1.8828 0.5828844517405458
-1.8832 0.5534222992676725
-1.8836 0.5261301426038933
-1.884 0.5006525599482045
-1.8844 0.4752074110567575
-1.8848 0.4515697924042485
-1.8852 0.4275020267012166
-1.8856 0.4041617345037522
-1.886 0.3823868100617426
-1.8864 0.3619122670971372
-1.8868 0.34155667776167187
-1.8872 0.3222211475216118
-1.8876 0.3052591772494217
-1.888 0.2883709309497744
-1.8884 0.2717974076339306
-1.8888 0.2554663510119299
-1.8892 0.24130075665304226
-1.8896 0.2269389423567624
-1.89 0.21370928439306308
-1.8904 0.2011359381678182
-1.8908 0.18892822972824025
-1.8912 0.17767902167369345
-1.8916 0.16699582238373248
-1.892 0.15669087522061134
-1.8924 0.14675292044141444
-1.8928 0.13755357989295464
-1.8932 0.12913936947271093
-1.8936 0.12089976865860483
-1.894 0.11316973309816439
-1.8944 0.10570721502840111
-1.8948 0.09889803465925996
-1.8952 0.09259014632378804
-1.8956 0.08649920725765373
-1.896 0.08065995895878061
-1.8964 0.07523303470301776
-1.8968 0.07024968214592323
-1.8972 0.06539667897380591
-1.8976 0.06088049686684446
-1.898 0.05655826733564325
-1.8984 0.052704343380663043
-1.8988 0.0489397247519965
-1.8992 0.0454764496198438
-1.8996 0.04227247975498142
-1.9 0.039116625859014015
-1.9004 0.03646313675185544
-1.9008 0.03380222799399298
-1.9012 0.031200612099415107
-1.9016 0.028853435334485138
-1.902 0.02672464669854772
-1.9024 0.0247228730206434
-1.9028 0.022831085028496807
-1.9032 0.021054355988399366
-1.9036 0.01940474813844392
-1.904 0.017842269274974985
-1.9044 0.016425801899100517
-1.9048 0.015109041295656446
-1.9052 0.013902154277567203
-1.9056 0.01275826137015294
-1.906 0.011685698727941693
-1.9064 0.010748696775514219
-1.9068 0.009844329911302
-1.9072 0.009008742424939894
-1.9076 0.008217552355781152
-1.908 0.007524547127650825
-1.9084 0.0068786765387759945
-1.9088 0.006295243379374357
-1.9092 0.005753362666503697
-1.9096 0.005239742321871371
-1.91 0.004772480026049802
-1.9104 0.0043459432494869984
-1.9108 0.003936739921314962
-1.9112 0.0035823063055532164
-1.9116 0.0032571565527035776
-1.912 0.002954814831930753
-1.9124 0.002683131823454136
-1.9128 0.0024322771743958424
-1.9132 0.002203766945457758
-1.9136 0.001989570552746365
-1.914 0.0018030341678791325
-1.9144 0.001627474887599227
-1.9148 0.0014719780240220633
-1.9152 0.0013277924810118798
-1.9156 0.0011960483518320226
-1.916 0.0010773382982148887
-1.9164 0.0009706773481972529
-1.9168 0.0008725448739062121
-1.9172 0.0007849214525008372
-1.9176 0.0007040350720270086
-1.918 0.000633211137416907
-1.9184 0.000566699195107666
-1.9188 0.0005074976940360995
-1.9192 0.00045276202657861073
-1.9196 0.0004043231145997496
-1.92 0.00036073266020059184
-1.9204 0.00032255523643519334
-1.9208 0.00028735816537511804
-1.9212 0.00025544075178901907
-1.9216 0.0002269715303317604
-1.922 0.0002016928675062086
-1.9224 0.00017896830511434037
-1.9228 0.00015945322873761407
-1.9232 0.0001411702103904914
-1.9236 0.00012488920674808566
-1.924 0.00011043786991833904
-1.9244 9.790502589097722e-05
-1.9248 8.635378650258595e-05
-1.9252 7.62165208093732e-05
-1.9256 6.726246743714058e-05
-1.926 5.9227121500660756e-05
-1.9264 5.2195337756964044e-05
-1.9268 4.585047414750705e-05
-1.9272 4.0204821891038175e-05
-1.9276 3.523168571463877e-05
-1.928 3.097372282983937e-05
-1.9284 2.715867903830564e-05
-1.9288 2.377420200079769e-05
-1.9292 2.0747636817426994e-05
-1.9296 1.805441243405623e-05
-1.93 1.572610676165415e-05
-1.9304 1.3707077025076117e-05
-1.9308 1.1949323209190925e-05
-1.9312 1.0399077128654408e-05
-1.9316 9.013505769242793e-06
-1.932 7.828073290071867e-06
-1.9324 6.788172388866223e-06
-1.9328 5.88877842421735e-06
-1.9332 5.094839929039938e-06
-1.9336 4.391474923905906e-06
-1.934 3.784747922781051e-06
-1.9344 3.262197084880243e-06
-1.9348 2.8099828257121417e-06
-1.9352 2.4118529631534496e-06
-1.9356 2.071333024530622e-06
-1.936 1.777510020346812e-06
-1.9364 1.5230911861723774e-06
-1.9368 1.3060156505778597e-06
-1.9372 1.1164365884997414e-06
-1.9376 9.528604477788489e-07
-1.938 8.128914511053969e-07
-1.9384 6.938930470219299e-07
-1.9388 5.903287511161729e-07
-1.9392 5.010465578723382e-07
-1.9396 4.254448661393982e-07
-1.94 3.610233321059497e-07
-1.9404 3.0598610204656346e-07
-1.9408 2.581777913587989e-07
-1.9412 2.1782499756049686e-07
-1.9416 1.838578871845052e-07
-1.942 1.5488686654408533e-07
-1.9424 1.30443981378277e-07
-1.9428 1.0935872397383853e-07
-1.9432 9.183826250309346e-08
-1.9436 7.674631296655927e-08
-1.944 6.436206941316207e-08
-1.9444 5.379910899199424e-08
-1.9448 4.4806474394793e-08
-1.9452 3.733149846789156e-08
-1.9456 3.105299233359893e-08
-1.946 2.583366228333471e-08
-1.9464 2.139193797734166e-08
-1.9468 1.7720732599197596e-08
-1.9472 1.465288670950111e-08
-1.9476 1.2096374649014615e-08
-1.948 9.96140161982471e-09
-1.9484 8.213297104723492e-09
-1.9488 6.746272103662193e-09
-1.9492 5.5214340702880865e-09
-1.9496 4.540838821115642e-09
-1.95 3.7182937349184708e-09
-1.9504 3.032384517582379e-09
-1.9508 2.4714977456568234e-09
-1.9512 2.0084247114077262e-09
-1.9516 1.6321703092139254e-09
-1.952 1.32165865586057e-09
-1.9524 1.0683221732593595e-09
-1.9528 8.645482901551126e-10
-1.9532 7.003545278074914e-10
-1.9536 5.644385520240482e-10
-1.954 4.533115010642347e-10
-1.9544 3.6441728904391476e-10
-1.9548 2.9172136014334467e-10
-1.9552 2.329932954220943e-10
-1.9556 1.8573519600106346e-10
-1.956 1.4883877319728533e-10
-1.9564 1.1834128290350033e-10
-1.9568 9.383447966202248e-11
-1.9572 7.449390807412195e-11
-1.9576 5.948023368200988e-11
-1.958 4.683782408048028e-11
-1.9584 3.6673315724610826e-11
-1.9588 2.8993077615254397e-11
-1.9592 2.2950618095727066e-11
-1.9596 1.7858574186295454e-11
-1.96 1.3877051762674629e-11
-1.9604 1.0915828908257147e-11
-1.9608 8.632299000862521e-12
-1.9612 6.609610877233587e-12
-1.9616 5.124818079144927e-12
-1.962 4.010570974821021e-12
-1.9624 3.1501974071518098e-12
-1.9628 2.357640080249478e-12
-1.9632 1.8147854027551807e-12
-1.9636 1.4161486183537102e-12
-1.964 1.1030025522255144e-12
-1.9644 8.087873226361953e-13
-1.9648 6.234652277381205e-13
-1.9652 4.851943743832804e-13
-1.9656 3.7570909722593693e-13
-1.966 2.681614952136235e-13
-1.9664 2.073549720732779e-13
-1.9668 1.6149979461704182e-13
-1.9672 1.2340732194051364e-13
-1.9676 8.488090724595876e-14
-1.968 6.637643396680116e-14
-1.9684 5.1503540313323625e-14
-1.9688 3.860213446424206e-14
-1.9692 2.543711015781187e-14
-1.9696 2.039794304765574e-14
-1.97 1.5745695595504605e-14
-1.9704 1.1552293745131609e-14
-1.9708 7.247456177697583e-15
-1.9712 6.091351518203141e-15
-1.9716 4.637507057502741e-15
-1.972 3.305603102932437e-15
-1.9724 1.9571859470882786e-15
-1.9728 1.74630539939154e-15
-1.9732 1.3001141894326676e-15
-1.9736 8.968585285565674e-16
-1.974 4.967559492501088e-16
-1.9744 4.82665651391164e-16
-1.9748 3.459373384206821e-16
-1.9752 2.294458847507175e-16
-1.9756 1.177709202067376e-16
-1.976 1.285813649783799e-16
-1.9764 8.73632128023813e-17
-1.9768 5.531573126368824e-17
-1.9772 2.603744479553968e-17
-1.9776 3.291529684432852e-17
-1.978 2.079608173918694e-17
-1.9784 1.2398060550677793e-17
-1.9788 5.304857045085023e-18
-1.9792 8.024226686442443e-18
-1.9796 4.580014344341906e-18
-1.98 2.5776785151732186e-18
-1.9804 9.845528916470238e-19
-1.9808 1.8544576949490188e-18
-1.9812 9.331704592575267e-19
-1.9816 4.92009778677879e-19
-1.982 1.6644525445966568e-19
-1.9824 4.0103321676760813e-19
-1.9828 1.751800006741037e-19
-1.9832 8.59933928628937e-20
-1.9836 2.525871619584126e-20
-1.984 8.071890154722495e-20
-1.9844 2.940663411342479e-20
-1.9848 1.3532550739989621e-20
-1.9852 3.3454152197162873e-21
-1.9856 1.502433227760345e-20
-1.986 4.4546516325160254e-21
-1.9864 1.9085058972139064e-21
-1.9868 3.9301861814315418e-22
-1.9872 2.535690157326901e-21
-1.9876 5.894056417478642e-22
-1.988 2.358724351188469e-22
-1.9884 3.853873682903966e-23
-1.9888 3.848253413861199e-22
-1.9892 6.707838989852446e-23
-1.9896 2.5230398081353014e-23
-1.99 3.1843570372270826e-24
-1.9904 5.11494234044524e-23
-1.9908 6.441051634604884e-24
-1.9912 2.2707311765594917e-24
-1.9916 2.043198137022094e-25
-1.992 5.859842566017411e-24
-1.9924 4.939499827326726e-25
-1.9928 1.6501625257284535e-25
-1.9932 9.42999651609511e-27
-1.9936 5.610163360820488e-25
-1.994 2.7958897969718144e-26
-1.9944 8.956956771483712e-27
-1.9948 2.9539721411020955e-28
-1.9952 4.229794974406256e-26
-1.9956 1.0804955989157216e-27
-1.996 3.3651986127644324e-28
-1.9964 4.041012053977672e-30
-1.9968 2.467061453319359e-27
-1.9972 2.0688743648396666e-29
-1.9976 6.2969074599043786e-30
-1.998 0.0
-1.9984 9.428949328305728e-29
-1.9988 0.0
-1.9992 0.0
-1.9996 0.0
-2.0 2.26537738800185e-30


==> Plots/PA_hist_900.tex <==
e pe
0.0 0.0
-0.0011111111111111111 0.0
-0.0022222222222222222 0.0
-0.0033333333333333335 0.0
-0.0044444444444444444 0.0
-0.005555555555555556 0.0
-0.006666666666666667 0.0
-0.0077777777777777776 0.0
-0.008888888888888889 0.0
-0.01 0.0
-0.011111111111111112 8.577901311915642e-169
-0.012222222222222223 1.4081832656217747e-167
-0.013333333333333334 1.5411540558073414e-166
-0.014444444444444444 1.124453936129979e-165
-0.015555555555555555 7.691456017050389e-165
-0.016666666666666666 4.208869301719215e-165
-0.017777777777777778 0.0
-0.01888888888888889 0.0
-0.02 6.896616492894805e-163
-0.021111111111111112 0.0
-0.022222222222222223 0.0
-0.023333333333333334 3.390216434839181e-160
-0.024444444444444446 1.2367816832204338e-159
-0.025555555555555557 2.3687431310331397e-158
-0.02666666666666667 1.6665537157043362e-157
-0.027777777777777776 7.093028840058983e-157
-0.028888888888888888 5.5448597350756445e-157
-0.03 3.0342226321728e-156
-0.03111111111111111 1.6603658006388874e-155
-0.03222222222222222 1.8171494792261514e-154
-0.03333333333333333 9.943689000879273e-154
-0.034444444444444444 1.08826436214127e-152
-0.035555555555555556 1.0421478453082817e-151
-0.03666666666666667 4.88809259548567e-151
-0.03777777777777778 2.2290250463378928e-150
-0.03888888888888889 7.318518690028258e-150
-0.04 1.3349309753672347e-149
-0.04111111111111111 1.4609829313193406e-148
-0.042222222222222223 7.994697228110905e-148
-0.043333333333333335 1.0937017537821915e-146
-0.044444444444444446 8.378838567287397e-146
-0.04555555555555556 4.5850135597646415e-145
-0.04666666666666667 1.7921301453483426e-144
-0.04777777777777778 5.884060527555825e-144
-0.04888888888888889 3.2198406006240154e-143
-0.05 2.3492513774854185e-142
-0.051111111111111114 2.57108458601374e-141
-0.052222222222222225 2.4621312215491763e-140
-0.05333333333333334 1.4435481580486135e-139
-0.05444444444444444 4.7395686159718545e-139
-0.05555555555555555 4.034421321113722e-138
-0.056666666666666664 8.042291428436107e-137
-0.057777777777777775 5.4363361439875655e-136
-0.058888888888888886 5.524681926722497e-135
-0.06 4.806059096217409e-134
-0.06111111111111111 4.991192638305511e-133
-0.06222222222222222 4.085207020601924e-132
-0.06333333333333334 3.670679910499709e-131
-0.06444444444444444 3.380055614701188e-130
-0.06555555555555556 2.7774184800711135e-129
-0.06666666666666667 2.33053535584887e-128
-0.06777777777777778 1.913822024256044e-127
-0.06888888888888889 1.5330970101469316e-126
-0.07 1.228138862317755e-125
-0.07111111111111111 9.484540716733814e-125
-0.07222222222222222 7.313862637371504e-124
-0.07333333333333333 5.54309887600324e-123
-0.07444444444444444 4.1333527225379745e-122
-0.07555555555555556 3.0280489941704756e-121
-0.07666666666666666 2.1828552418159664e-120
-0.07777777777777778 1.5750147498844624e-119
-0.07888888888888888 1.0939300709952635e-118
-0.08 7.567552759034352e-118
-0.0811111111111111 5.167320187739219e-117
-0.08222222222222222 3.4699352580509245e-116
-0.08333333333333333 2.3022153806292507e-115
-0.08444444444444445 1.5000193534440509e-114
-0.08555555555555555 9.701319731114092e-114
-0.08666666666666667 6.168676098012548e-113
-0.08777777777777777 3.8688617292352604e-112
-0.08888888888888889 2.3965156693842063e-111
-0.09 1.4694310829413712e-110
-0.09111111111111111 8.852734395436571e-110
-0.09222222222222222 5.275243669808776e-109
-0.09333333333333334 3.104861488293443e-108
-0.09444444444444444 1.8069154176158945e-107
-0.09555555555555556 1.0375162450607751e-106
-0.09666666666666666 5.887347268422504e-106
-0.09777777777777778 3.3020460191057075e-105
-0.09888888888888889 1.8296738472458158e-104
-0.1 1.0013050406895228e-103
-0.10111111111111111 5.421170763400739e-103
-0.10222222222222223 2.896346191797694e-102
-0.10333333333333333 1.532519078318057e-101
-0.10444444444444445 8.021715226079213e-101
-0.10555555555555556 4.1526538666625564e-100
-0.10666666666666667 2.1211646673913764e-99
-0.10777777777777778 1.0742441040684592e-98
-0.10888888888888888 5.375480994158852e-98
-0.11 2.6615579833483973e-97
-0.1111111111111111 1.3043305979833875e-96
-0.11222222222222222 6.3238433244310755e-96
-0.11333333333333333 3.0309910592101e-95
-0.11444444444444445 1.4396672779782882e-94
-0.11555555555555555 6.775688955271864e-94
-0.11666666666666667 3.1466916912715055e-93
-0.11777777777777777 1.4501603451580862e-92
-0.11888888888888889 6.61173090357718e-92
-0.12 2.984920828975086e-91
-0.12111111111111111 1.3346156635892553e-90
-0.12222222222222222 5.905462147089311e-90
-0.12333333333333334 2.5915450507598237e-89
-0.12444444444444444 1.125334888386582e-88
-0.12555555555555556 4.841534499193979e-88
-0.12666666666666668 2.0635116597277883e-87
-0.12777777777777777 8.711075789820571e-87
-0.1288888888888889 3.644570466971302e-86
-0.13 1.5100181815753597e-85
-0.13111111111111112 6.205100835473243e-85
-0.1322222222222222 2.525729382779105e-84
-0.13333333333333333 1.0195787526854005e-83
-0.13444444444444445 4.078123283656038e-83
-0.13555555555555557 1.618391839022232e-82
-0.13666666666666666 6.352718092129363e-82
-0.13777777777777778 2.4750834483881976e-81
-0.1388888888888889 9.554641341421595e-81
-0.14 3.6608178071228096e-80
-0.1411111111111111 1.389366890700112e-79
-0.14222222222222222 5.234746323725006e-79
-0.14333333333333334 1.955709566369812e-78
-0.14444444444444443 7.243047647598247e-78
-0.14555555555555555 2.659893526306426e-77
-0.14666666666666667 9.692514652329589e-77
-0.14777777777777779 3.501642169790623e-76
-0.14888888888888888 1.2549499408495946e-75
-0.15 4.46246277628712e-75
-0.1511111111111111 1.575331734051082e-74
-0.15222222222222223 5.513884092457811e-74
-0.15333333333333332 1.9160714742391493e-73
-0.15444444444444444 6.604499582424031e-73
-0.15555555555555556 2.257510059667073e-72
-0.15666666666666668 7.663069103446615e-72
-0.15777777777777777 2.5814991319026464e-71
-0.15888888888888889 8.625039065852307e-71
-0.16 2.862218274947741e-70
-0.16111111111111112 9.418239042518094e-70
-0.1622222222222222 3.0796562839599966e-69
-0.16333333333333333 9.992672837965703e-69
-0.16444444444444445 3.2177497051192855e-68
-0.16555555555555557 1.0283687313538855e-67
-0.16666666666666666 3.266109596530095e-67
-0.16777777777777778 1.0287930850903616e-66
-0.1688888888888889 3.2189745184482643e-66
-0.17 1.0002932153187242e-65
-0.1711111111111111 3.0868451132431283e-65
-0.17222222222222222 9.467217311854595e-65
-0.17333333333333334 2.8801203788342483e-64
-0.17444444444444446 8.702805968328295e-64
-0.17555555555555555 2.612103943017646e-63
-0.17666666666666667 7.793368584949405e-63
-0.17777777777777778 2.306797756164931e-62
-0.17888888888888888 6.784979496419366e-62
-0.18 1.9822420001632308e-61
-0.1811111111111111 5.7525355281967734e-61
-0.18222222222222223 1.6583109517897582e-60
-0.18333333333333332 4.751921768600518e-60
-0.18444444444444444 1.3515124432979642e-59
-0.18555555555555556 3.8233296342462103e-59
-0.18666666666666668 1.0735353049501603e-58
-0.18777777777777777 2.9966706290467165e-58
-0.18888888888888888 8.309270239691597e-58
-0.19 2.288537185938922e-57
-0.19111111111111112 6.270815571725625e-57
-0.1922222222222222 1.706655812434886e-56
-0.19333333333333333 4.618940365017214e-56
-0.19444444444444445 1.2395386372645456e-55
-0.19555555555555557 3.313240150956357e-55
-0.19666666666666666 8.796659880961919e-55
-0.19777777777777777 2.3199841782597877e-54
-0.1988888888888889 6.08893489259601e-54
-0.2 1.588197428323526e-53
-0.2011111111111111 4.1150607484927567e-53
-0.20222222222222222 1.0610655965676053e-52
-0.20333333333333334 2.7184866539419103e-52
-0.20444444444444446 6.92159112116711e-52
-0.20555555555555555 1.752531669119321e-51
-0.20666666666666667 4.409792812340901e-51
-0.20777777777777778 1.1036169509437562e-50
-0.2088888888888889 2.743445928770623e-50
-0.21 6.785567696734748e-50
-0.2111111111111111 1.6691702727152602e-49
-0.21222222222222223 4.085298013355005e-49
-0.21333333333333335 9.93425949615701e-49
-0.21444444444444444 2.4039582234885753e-48
-0.21555555555555556 5.777379720044026e-48
-0.21666666666666667 1.3823202018842312e-47
-0.21777777777777776 3.288680797659828e-47
-0.21888888888888888 7.780302085369764e-47
-0.22 1.8302558935765146e-46
-0.22111111111111112 4.2848700490774415e-46
-0.2222222222222222 9.967633112857418e-46
-0.22333333333333333 2.3087672710883785e-45
-0.22444444444444445 5.3159395950137424e-45
-0.22555555555555556 1.2173562385701308e-44
-0.22666666666666666 2.775810211423524e-44
-0.22777777777777777 6.291758066272161e-44
-0.2288888888888889 1.4205979820991112e-43
-0.23 3.1864545173337527e-43
-0.2311111111111111 7.112476162910094e-43
-0.23222222222222222 1.5801681875172207e-42
-0.23333333333333334 3.489152569667621e-42
-0.23444444444444446 7.671650349825598e-42
-0.23555555555555555 1.6780855542905706e-41
-0.23666666666666666 3.6525778654011486e-41
-0.23777777777777778 7.909839793293758e-41
-0.2388888888888889 1.704460047403109e-40
-0.24 3.654566179370825e-40
-0.2411111111111111 7.79830507376304e-40
-0.24222222222222223 1.6553153560766966e-39
-0.24333333333333335 3.4986940393881373e-39
-0.24444444444444444 7.352496314097179e-39
-0.24555555555555555 1.539204025205966e-38
-0.24666666666666667 3.207651307484847e-38
-0.2477777777777778 6.649280698457037e-38
-0.24888888888888888 1.3712822660428893e-37
-0.25 2.8166358250459553e-37
-0.2511111111111111 5.7604242483511815e-37
-0.25222222222222224 1.1723321654623441e-36
-0.25333333333333335 2.373940546410205e-36
-0.2544444444444444 4.79030049714846e-36
-0.25555555555555554 9.615817155724161e-36
-0.25666666666666665 1.9201130787272496e-35
-0.2577777777777778 3.8205861071980346e-35
-0.2588888888888889 7.565136393097932e-35
-0.26 1.491336061981754e-34
-0.2611111111111111 2.9254177992540653e-34
-0.26222222222222225 5.713740533968502e-34
-0.2633333333333333 1.1118226367059688e-33
-0.2644444444444444 2.152353135858156e-33
-0.26555555555555554 4.1475662855248545e-33
-0.26666666666666666 7.965956361328162e-33
-0.2677777777777778 1.5218002041588634e-32
-0.2688888888888889 2.8951713507692544e-32
-0.27 5.483880204147201e-32
-0.27111111111111114 1.0347265666051841e-31
-0.2722222222222222 1.9468746289386708e-31
-0.2733333333333333 3.6396431306481554e-31
-0.27444444444444444 6.781932543990184e-31
-0.27555555555555555 1.2578335412513219e-30
-0.27666666666666667 2.3243247929432454e-30
-0.2777777777777778 4.278106198916733e-30
-0.2788888888888889 7.841520984914144e-30
-0.28 1.4313631358818437e-29
-0.2811111111111111 2.603473753852636e-29
-0.2822222222222222 4.714196232311428e-29
-0.2833333333333333 8.497770145391395e-29
-0.28444444444444444 1.526371655640133e-28
-0.28555555555555556 2.730702977425089e-28
-0.2866666666666667 4.866965509928717e-28
-0.2877777777777778 8.633630315712555e-28
-0.28888888888888886 1.5264521310950894e-27
-0.29 2.6872478429348743e-27
-0.2911111111111111 4.7157985467965254e-27
-0.2922222222222222 8.241344820614603e-27
-0.29333333333333333 1.433858379566438e-26
-0.29444444444444445 2.4880574773174682e-26
-0.29555555555555557 4.295761269510259e-26
-0.2966666666666667 7.389737185436856e-26
-0.29777777777777775 1.2671116958317008e-25
-0.29888888888888887 2.163083404407372e-25
-0.3 3.6828606953124585e-25
-0.3011111111111111 6.244389860231296e-25
-0.3022222222222222 1.0546404706686194e-24
-0.30333333333333334 1.7749103983893038e-24
-0.30444444444444446 2.9753770543607425e-24
-0.3055555555555556 4.973828209087708e-24
-0.30666666666666664 8.279273701226727e-24
-0.30777777777777776 1.3727639101343448e-23
-0.3088888888888889 2.2692060485794467e-23
-0.31 3.7382329265348147e-23
-0.3111111111111111 6.132535545467825e-23
-0.31222222222222223 1.0035970228701436e-22
-0.31333333333333335 1.635578822575504e-22
-0.31444444444444447 2.657300921571451e-22
-0.31555555555555553 4.301768618543026e-22
-0.31666666666666665 6.941702914145875e-22
-0.31777777777777777 1.1164100055023802e-21
-0.3188888888888889 1.7891869669551658e-21
-0.32 2.8562090213057063e-21
-0.3211111111111111 4.542359311205428e-21
-0.32222222222222224 7.211351865556468e-21
-0.3233333333333333 1.1392060781416393e-20
-0.3244444444444444 1.7957800158029393e-20
-0.32555555555555554 2.817368515698496e-20
-0.32666666666666666 4.413760027230399e-20
-0.3277777777777778 6.886444630078853e-20
-0.3288888888888889 1.0699236628039354e-19
-0.33 1.6589755060807353e-19
-0.33111111111111113 2.5641323446486674e-19
-0.3322222222222222 3.9464132328294117e-19
-0.3333333333333333 6.061581589760703e-19
-0.33444444444444443 9.281798371843975e-19
-0.33555555555555555 1.4164073781518037e-18
-0.33666666666666667 2.1551191526557765e-18
-0.3377777777777778 3.2669062800891066e-18
-0.3388888888888889 4.935620379697789e-18
-0.34 7.436319064360508e-18
-0.3411111111111111 1.1179927341633198e-17
-0.3422222222222222 1.673361028779194e-17
-0.3433333333333333 2.499658252006068e-17
-0.34444444444444444 3.7213097274643555e-17
-0.34555555555555556 5.523576445559656e-17
-0.3466666666666667 8.177639831402123e-17
-0.3477777777777778 1.2061995304630379e-16
-0.3488888888888889 1.7741305788089224e-16
-0.35 2.6034597265618195e-16
-0.3511111111111111 3.8054833870351923e-16
-0.3522222222222222 5.549650053663465e-16
-0.35333333333333333 8.071133871951736e-16
-0.35444444444444445 1.169589107681984e-15
-0.35555555555555557 1.6912629255435106e-15
-0.3566666666666667 2.437842421865149e-15
-0.35777777777777775 3.5038115773316056e-15
-0.35888888888888887 5.026054059823824e-15
-0.36 7.185749562249366e-15
-0.3611111111111111 1.024288224478083e-14
-0.3622222222222222 1.4560254142096403e-14
-0.36333333333333334 2.0648374962526338e-14
-0.36444444444444446 2.919192432464507e-14
-0.3655555555555556 4.113328197985518e-14
-0.36666666666666664 5.780520264416625e-14
-0.36777777777777776 8.099951154902707e-14
-0.3688888888888889 1.1332019828098035e-13
-0.37 1.5799797244930583e-13
-0.3711111111111111 2.1973868767939397e-13
-0.37222222222222223 3.0503744848393947e-13
-0.37333333333333335 4.218341153936117e-13
-0.37444444444444447 5.819392873656497e-13
-0.37555555555555553 8.014544186620486e-13
-0.37666666666666665 1.1004261341656987e-12
-0.37777777777777777 1.5079753967462685e-12
-0.3788888888888889 2.0585459313281866e-12
-0.38 2.8071882567607237e-12
-0.3811111111111111 3.814526615813141e-12
-0.38222222222222224 5.16768359365156e-12
-0.38333333333333336 6.985432566421457e-12
-0.3844444444444444 9.41786573149254e-12
-0.38555555555555554 1.2682847759970746e-11
-0.38666666666666666 1.7023883897374683e-11
-0.3877777777777778 2.2783691051342935e-11
-0.3888888888888889 3.04269373651966e-11
-0.39 4.054170665364919e-11
-0.39111111111111113 5.390424539224934e-11
-0.39222222222222225 7.146174197204426e-11
-0.3933333333333333 9.453007780612496e-11
-0.39444444444444443 1.2476925221114197e-10
-0.39555555555555555 1.6435120143928486e-10
-0.39666666666666667 2.1588872948999553e-10
-0.3977777777777778 2.8269036203133425e-10
-0.3988888888888889 3.694914074386006e-10
-0.4 4.820871345377295e-10
-0.4011111111111111 6.273301854516286e-10
-0.4022222222222222 8.141313879668565e-10
-0.4033333333333333 1.0551598248495593e-09
-0.40444444444444444 1.363792884673602e-09
-0.40555555555555556 1.757072340119016e-09
-0.4066666666666667 2.262046746912186e-09
-0.4077777777777778 2.9040770121119678e-09
-0.4088888888888889 3.7248320029599397e-09
-0.41 4.760144332246327e-09
-0.4111111111111111 6.0741429793780254e-09
-0.4122222222222222 7.722648930639989e-09
-0.41333333333333333 9.80243654081492e-09
-0.41444444444444445 1.241192134089561e-08
-0.41555555555555557 1.5693995375491466e-08
-0.4166666666666667 1.9818798424812542e-08
-0.4177777777777778 2.4930733363677534e-08
-0.41888888888888887 3.133155939338743e-08
-0.42 3.929470367870684e-08
-0.4211111111111111 4.9137546193333597e-08
-0.4222222222222222 6.134947279362123e-08
-0.42333333333333334 7.645161861745468e-08
-0.42444444444444446 9.50740765724944e-08
-0.4255555555555556 1.1798140938525563e-07
-0.4266666666666667 1.4608792979062641e-07
-0.42777777777777776 1.8050263718997733e-07
-0.4288888888888889 2.2262600918270872e-07
-0.43 2.742554344124303e-07
-0.4311111111111111 3.368731133492304e-07
-0.43222222222222223 4.1320090541816605e-07
-0.43333333333333335 5.054294760768329e-07
-0.43444444444444447 6.173309307301969e-07
-0.43555555555555553 7.528157379681948e-07
-0.43666666666666665 9.160840535730442e-07
-0.43777777777777777 1.112537207497847e-06
-0.4388888888888889 1.3494062770871529e-06
-0.44 1.6310693003041536e-06
-0.4411111111111111 1.9694208649588333e-06
-0.44222222222222224 2.372836970190195e-06
-0.44333333333333336 2.8553186916179424e-06
-0.4444444444444444 3.4274926224092833e-06
-0.44555555555555554 4.108927189174283e-06
-0.44666666666666666 4.91448510972715e-06
-0.4477777777777778 5.870226206975161e-06
-0.4488888888888889 6.992516855297306e-06
-0.45 8.323714039735794e-06
-0.45111111111111113 9.892241083730329e-06
-0.45222222222222225 1.1727911439735725e-05
-0.4533333333333333 1.3868821133265202e-05
-0.45444444444444443 1.6385717994877183e-05
-0.45555555555555555 1.9315633228762076e-05
-0.45666666666666667 2.2752748666944474e-05
-0.4577777777777778 2.6738585352359944e-05
-0.4588888888888889 3.1345523152170556e-05
-0.46 3.669440966432483e-05
-0.46111111111111114 4.292200992721352e-05
-0.4622222222222222 5.009254320821865e-05
-0.4633333333333333 5.841777403745065e-05
-0.46444444444444444 6.796546163333722e-05
-0.46555555555555556 7.899590005459475e-05
-0.4666666666666667 9.152043529790623e-05
-0.4677777777777778 0.00010598182021586013
-0.4688888888888889 0.00012252533137972518
-0.47 0.0001414595831217715
-0.4711111111111111 0.00016309244199206438
-0.4722222222222222 0.00018766920868059657
-0.47333333333333333 0.00021546299504028425
-0.47444444444444445 0.0002470911389583889
-0.47555555555555556 0.00028307757162833615
-0.4766666666666667 0.0003232323975550118
-0.4777777777777778 0.0003687289850810699
-0.47888888888888886 0.0004203948300438182
-0.48 0.0004785993864679266
-0.4811111111111111 0.0005434686237813327
-0.4822222222222222 0.0006166532720432427
-0.48333333333333334 0.0006979635466670932
-0.48444444444444446 0.0007900156557294132
-0.4855555555555556 0.0008921711840978773
-0.4866666666666667 0.00100595417640128
-0.48777777777777775 0.001133278998514715
-0.4888888888888889 0.001273133386147649
-0.49 0.001429374106939209
-0.4911111111111111 0.0016037631691727548
-0.4922222222222222 0.001795708692343813
-0.49333333333333335 0.0020095457439853457
-0.49444444444444446 0.0022428470770148234
-0.4955555555555556 0.002500557677775531
-0.49666666666666665 0.002783177374852865
-0.49777777777777776 0.003091672421483792
-0.4988888888888889 0.003434925656031698
-0.5 0.0038081603151459897
-0.5011111111111111 0.004215107355849284
-0.5022222222222222 0.004659184879302358
-0.5033333333333333 0.0051464625494134384
-0.5044444444444445 0.00567138444610817
-0.5055555555555555 0.006247480430501053
-0.5066666666666667 0.006871554723519687
-0.5077777777777778 0.007544434331816816
-0.5088888888888888 0.008276307182343422
-0.51 0.009055687555444275
-0.5111111111111111 0.00991410898289957
-0.5122222222222222 0.0108287512562709
-0.5133333333333333 0.011801806614861146
-0.5144444444444445 0.012861939844855511
-0.5155555555555555 0.0139909185723503
-0.5166666666666667 0.015203285921957304
-0.5177777777777778 0.016506017497464925
-0.5188888888888888 0.017903367374311915
-0.52 0.019356718618080984
-0.5211111111111111 0.020951760282551274
-0.5222222222222223 0.022614085663460324
-0.5233333333333333 0.024380891170171844
-0.5244444444444445 0.026261727138135686
-0.5255555555555556 0.028276590601938722
-0.5266666666666666 0.030409656830163917
-0.5277777777777778 0.03266839715414734
-0.5288888888888889 0.03502141123145444
-0.53 0.037549837865173866
-0.5311111111111111 0.04015630340387013
-0.5322222222222223 0.04291702159851816
-0.5333333333333333 0.045832781799419645
-0.5344444444444445 0.048895012996964415
-0.5355555555555556 0.052032125043374115
-0.5366666666666666 0.05534889472793618
-0.5377777777777778 0.058798567020964296
-0.5388888888888889 0.06236015346311647
-0.54 0.06617136436673889
-0.5411111111111111 0.070094459459025
-0.5422222222222223 0.07412775594344478
-0.5433333333333333 0.07841873662218311
-0.5444444444444444 0.08289094738230521
-0.5455555555555556 0.08745336492846971
-0.5466666666666666 0.09228382672547307
-0.5477777777777778 0.09707059221281336
-0.5488888888888889 0.10213438168297084
-0.55 0.10731948073648406
-0.5511111111111111 0.11251479781791131
-0.5522222222222222 0.11798865826455822
-0.5533333333333333 0.12353886101390572
-0.5544444444444444 0.1292244243639632
-0.5555555555555556 0.1351608315909946
-0.5566666666666666 0.1411770474837067
-0.5577777777777778 0.14740568848841323
-0.5588888888888889 0.15369112969821294
-0.56 0.16015376196722175
-0.5611111111111111 0.1664780895144205
-0.5622222222222222 0.17293678318682068
-0.5633333333333334 0.17957876574649365
-0.5644444444444444 0.18623685537531046
-0.5655555555555556 0.19295725479143866
-0.5666666666666667 0.1999063804502622
-0.5677777777777778 0.2067649358346684
-0.5688888888888889 0.2138327466050135
-0.57 0.22091549901196234
-0.5711111111111111 0.22778395108867086
-0.5722222222222222 0.23495640662331935
-0.5733333333333334 0.24187532488925587
-0.5744444444444444 0.24890158089277634
-0.5755555555555556 0.25584131591515386
-0.5766666666666667 0.2627146475642538
-0.5777777777777777 0.26974398050814835
-0.5788888888888889 0.2767081190472887
-0.58 0.28340136997196813
-0.5811111111111111 0.2900291672533084
-0.5822222222222222 0.2967137375544447
-0.5833333333333334 0.30330355790742175
-0.5844444444444444 0.30998211458163116
-0.5855555555555556 0.3164216969287285
-0.5866666666666667 0.3226753705906485
-0.5877777777777777 0.328557969868516
-0.5888888888888889 0.3342427224943477
-0.59 0.3400000241647794
-0.5911111111111111 0.34544931653616634
-0.5922222222222222 0.3510755676630623
-0.5933333333333334 0.35615558734283187
-0.5944444444444444 0.36096441706518173
-0.5955555555555555 0.3656514546222282
-0.5966666666666667 0.37025067307278176
-0.5977777777777777 0.3744291709654014
-0.5988888888888889 0.3784991801951636
-0.6 0.3824316545515027
-0.6011111111111112 0.3863377903556378
-0.6022222222222222 0.3893590411743999
-0.6033333333333334 0.3924388654907988
-0.6044444444444445 0.39524194859354145
-0.6055555555555555 0.39816435284549667
-0.6066666666666667 0.40079824105762285
-0.6077777777777778 0.40334837964219133
-0.6088888888888889 0.40533853737448905
-0.61 0.4073658058908278
-0.6111111111111112 0.40851081553526025
-0.6122222222222222 0.40958810894064085
-0.6133333333333333 0.41063564726357216
-0.6144444444444445 0.4113903297748977
-0.6155555555555555 0.41179148092524565
-0.6166666666666667 0.41183438174657633
-0.6177777777777778 0.4113615138039484
-0.6188888888888889 0.4109097339038233
-0.62 0.41050232296179745
-0.6211111111111111 0.4093101903330149
-0.6222222222222222 0.40841593786218877
-0.6233333333333333 0.40691007500946635
-0.6244444444444445 0.4055796455462419
-0.6255555555555555 0.4034238796588572
-0.6266666666666667 0.4017680937287225
-0.6277777777777778 0.39954396643419837
-0.6288888888888889 0.39699788612361786
-0.63 0.3943337910503416
-0.6311111111111111 0.39104998153571024
-0.6322222222222222 0.387779228085161
-0.6333333333333333 0.3844549403335343
-0.6344444444444445 0.3809601323232965
-0.6355555555555555 0.37714071034703467
-0.6366666666666667 0.3734700719983018
-0.6377777777777778 0.36957778404395214
-0.6388888888888888 0.36524718556741964
-0.64 0.36137042232651434
-0.6411111111111111 0.3568235679780088
-0.6422222222222222 0.352450078819643
-0.6433333333333333 0.3478909692590261
-0.6444444444444445 0.34301444275667914
-0.6455555555555555 0.33810180843110366
-0.6466666666666666 0.3335324889071332
-0.6477777777777778 0.32876039270365465
-0.6488888888888888 0.3234589882155657
-0.65 0.31853047075893903
-0.6511111111111111 0.31330015076849155
-0.6522222222222223 0.30788469282761444
-0.6533333333333333 0.30285021957074537
-0.6544444444444445 0.2974498710560521
-0.6555555555555556 0.2920910450176665
-0.6566666666666666 0.28675914157568205
-0.6577777777777778 0.28131957496575644
-0.6588888888888889 0.2758489136815235
-0.66 0.2704580916037677
-0.6611111111111111 0.26522313039530393
-0.6622222222222223 0.2597229686153825
-0.6633333333333333 0.25414379450162017
-0.6644444444444444 0.24883941511254998
-0.6655555555555556 0.24353442957976262
-0.6666666666666666 0.2379509869608682
-0.6677777777777778 0.2326466687552407
-0.6688888888888889 0.22720710195675323
-0.67 0.2218227012644348
-0.6711111111111111 0.21668759375221133
-0.6722222222222223 0.21153845095725984
-0.6733333333333333 0.206522868600643
-0.6744444444444444 0.20135911856159847
-0.6755555555555556 0.1964130879536056
-0.6766666666666666 0.19148341314891604
-0.6777777777777778 0.18662620921545026
-0.6788888888888889 0.18176713399088598
-0.68 0.17696930026845675
-0.6811111111111111 0.17241829816960366
-0.6822222222222222 0.16788655788719023
-0.6833333333333333 0.16334253083217193
-0.6844444444444444 0.15908833225000418
-0.6855555555555556 0.1546009808951732
-0.6866666666666666 0.15039412244943745
-0.6877777777777778 0.14619528133193319
-0.6888888888888889 0.14203326599838947
-0.69 0.13796912807143102
-0.6911111111111111 0.13400181544340795
-0.6922222222222222 0.1299781396538971
-0.6933333333333334 0.12620035851602218
-0.6944444444444444 0.12241864464776787
-0.6955555555555556 0.11873973391752188
-0.6966666666666667 0.11518582608962037
-0.6977777777777778 0.11166892520565166
-0.6988888888888889 0.10826293696104147
-0.7 0.1049499305411396
-0.7011111111111111 0.10174432855344306
-0.7022222222222222 0.0986079953756924
-0.7033333333333334 0.09556045454058723
-0.7044444444444444 0.09255434423519213
-0.7055555555555556 0.08964822164560426
-0.7066666666666667 0.08687071234132167
-0.7077777777777777 0.0840650988292509
-0.7088888888888889 0.08132083406886588
-0.71 0.07869087564128442
-0.7111111111111111 0.07609606225043371
-0.7122222222222222 0.07362996561665225
-0.7133333333333334 0.0711936207337846
-0.7144444444444444 0.06888244504869295
-0.7155555555555555 0.06658597647155937
-0.7166666666666667 0.06433399171879489
-0.7177777777777777 0.06216004694159276
-0.7188888888888889 0.06003811148613481
-0.72 0.05803670023726811
-0.7211111111111111 0.05604108612727761
-0.7222222222222222 0.05415398262330123
-0.7233333333333334 0.052263057734496736
-0.7244444444444444 0.050500532183748816
-0.7255555555555555 0.04874738549222246
-0.7266666666666667 0.047026207254186804
-0.7277777777777777 0.04543094961237472
-0.7288888888888889 0.04380629323276045
-0.73 0.04225687875678588
-0.7311111111111112 0.04075760399634414
-0.7322222222222222 0.03930510968387818
-0.7333333333333333 0.03794516532284128
-0.7344444444444445 0.03655978569505614
-0.7355555555555555 0.035250294132233455
-0.7366666666666667 0.03399675284514631
-0.7377777777777778 0.03278846404759011
-0.7388888888888889 0.03159889158344821
-0.74 0.030494674475353804
-0.7411111111111112 0.02942438365608478
-0.7422222222222222 0.02839210618493343
-0.7433333333333333 0.02735601765484574
-0.7444444444444445 0.026366324951002773
-0.7455555555555555 0.02541695915294716
-0.7466666666666667 0.024497247818713274
-0.7477777777777778 0.02356091052745316
-0.7488888888888889 0.022698507221888292
-0.75 0.021874393846919443
-0.7511111111111111 0.02107266762605134
-0.7522222222222222 0.020308790234997424
-0.7533333333333333 0.019566329481849165
-0.7544444444444445 0.01885150156521543
-0.7555555555555555 0.018165786181248738
-0.7566666666666667 0.01749103598666444
-0.7577777777777778 0.016856716323570817
-0.7588888888888888 0.01623430296496614
-0.76 0.015639031694262017
-0.7611111111111111 0.015052058799529923
-0.7622222222222222 0.014496349714884086
-0.7633333333333333 0.013957687786644928
-0.7644444444444445 0.013433802620460724
-0.7655555555555555 0.01293460949024563
-0.7666666666666667 0.012449852946952441
-0.7677777777777778 0.011999223046729457
-0.7688888888888888 0.011553449739418966
-0.77 0.0111214236951613
-0.7711111111111111 0.010713686071949459
-0.7722222222222223 0.01031565188726853
-0.7733333333333333 0.009942319956734157
-0.7744444444444445 0.009571894487006693
-0.7755555555555556 0.009216148172747615
-0.7766666666666666 0.008882476740442251
-0.7777777777777778 0.008560561488932968
-0.7788888888888889 0.008235599579803701
-0.78 0.007925550983343696
-0.7811111111111111 0.007639175683434856
-0.7822222222222223 0.007357545335015413
-0.7833333333333333 0.007087362453436788
-0.7844444444444445 0.006823634777946791
-0.7855555555555556 0.0065773250598453875
-0.7866666666666666 0.006331851731836422
-0.7877777777777778 0.006099898606397114
-0.7888888888888889 0.00587822828519866
-0.79 0.005664217157355188
-0.7911111111111111 0.005463356037338047
-0.7922222222222223 0.005266262489066479
-0.7933333333333333 0.005075689492234576
-0.7944444444444444 0.004890958617011963
-0.7955555555555556 0.004714127186247771
-0.7966666666666666 0.0045495608696485045
-0.7977777777777778 0.004384069699721295
-0.7988888888888889 0.004223363511467392
-0.8 0.004071209568646492
-0.8011111111111111 0.003925955064433781
-0.8022222222222222 0.003783993281946861
-0.8033333333333333 0.003647437386132042
-0.8044444444444444 0.0035196136911769173
-0.8055555555555556 0.003395706673356324
-0.8066666666666666 0.003275424009876929
-0.8077777777777778 0.003162758432807604
-0.8088888888888889 0.0030508601530608217
-0.81 0.002942561691012086
-0.8111111111111111 0.002839690117481852
-0.8122222222222222 0.002740276585552762
-0.8133333333333334 0.002643936508671839
-0.8144444444444444 0.0025494026557977994
-0.8155555555555556 0.002461068838096611
-0.8166666666666667 0.002375609250453161
-0.8177777777777778 0.0022918765473079867
-0.8188888888888889 0.0022120436020417263
-0.82 0.0021363413309169565
-0.8211111111111111 0.0020622573159537303
-0.8222222222222222 0.001992504416539112
-0.8233333333333334 0.0019233128252601705
-0.8244444444444444 0.0018578559712781777
-0.8255555555555556 0.001795213288546084
-0.8266666666666667 0.0017348309362126759
-0.8277777777777777 0.0016750481398179419
-0.8288888888888889 0.0016191781940302402
-0.83 0.0015650788797633383
-0.8311111111111111 0.0015114241384783923
-0.8322222222222222 0.0014599904881184727
-0.8333333333333334 0.0014110575255323755
-0.8344444444444444 0.001363966036163287
-0.8355555555555556 0.0013184478010109337
-0.8366666666666667 0.0012763260312258634
-0.8377777777777777 0.0012344707061822443
-0.8388888888888889 0.0011934902975016541
-0.84 0.0011555309265893258
-0.8411111111111111 0.0011173286730153669
-0.8422222222222222 0.0010801633132389483
-0.8433333333333334 0.0010466245802617238
-0.8444444444444444 0.0010137092102553138
-0.8455555555555555 0.0009812348618357773
-0.8466666666666667 0.0009507460204587667
-0.8477777777777777 0.0009212723611815862
-0.8488888888888889 0.0008916186626120083
-0.85 0.0008631406428472847
-0.8511111111111112 0.0008353619541388977
-0.8522222222222222 0.000809078945013445
-0.8533333333333334 0.0007834926352465168
-0.8544444444444445 0.0007589666869633433
-0.8555555555555555 0.0007346148825409092
-0.8566666666666667 0.000712179835906999
-0.8577777777777778 0.0006906187814817371
-0.8588888888888889 0.0006688148789626543
-0.86 0.0006479980029362603
-0.8611111111111112 0.0006277934190414685
-0.8622222222222222 0.0006087830744763904
-0.8633333333333333 0.00059025270365133
-0.8644444444444445 0.0005722772639636688
-0.8655555555555555 0.0005550799116857545
-0.8666666666666667 0.0005387003196701373
-0.8677777777777778 0.0005223565323251474
-0.8688888888888889 0.0005066945363022196
-0.87 0.0004914267683288172
-0.8711111111111111 0.0004770648925208465
-0.8722222222222222 0.0004632252519182413
-0.8733333333333333 0.00044912676798548813
-0.8744444444444445 0.0004361609407047256
-0.8755555555555555 0.0004231868686398085
-0.8766666666666667 0.0004109971710711056
-0.8777777777777778 0.0003989748571502929
-0.8788888888888889 0.00038770497935911827
-0.88 0.00037649561448722507
-0.8811111111111111 0.00036609252838580906
-0.8822222222222222 0.00035577194744123116
-0.8833333333333333 0.0003454788519321938
-0.8844444444444445 0.0003358614373577325
-0.8855555555555555 0.00032636820266797816
-0.8866666666666667 0.00031692421008290724
-0.8877777777777778 0.0003081605380569217
-0.8888888888888888 0.00029982944488791675
-0.89 0.0002913310882022105
-0.8911111111111111 0.00028373841317744
-0.8922222222222222 0.000275680055002675
-0.8933333333333333 0.00026822271382201325
-0.8944444444444445 0.0002611331797925445
-0.8955555555555555 0.00025408793206071
-0.8966666666666666 0.0002472322018578909
-0.8977777777777778 0.00024072713358893493
-0.8988888888888888 0.00023439192686780638
-0.9 0.00022821160572214573
-0.9011111111111111 0.00022235139576435415
-0.9022222222222223 0.0002166714577323492
-0.9033333333333333 0.00021107780340523868
-0.9044444444444445 0.00020565411948592635
-0.9055555555555556 0.00020041815765604903
-0.9066666666666666 0.0001952498552573619
-0.9077777777777778 0.0001904369196736057
-0.9088888888888889 0.00018562497264105164
-0.91 0.0001809040260417135
-0.9111111111111111 0.0001764489529467241
-0.9122222222222223 0.00017208223369922956
-0.9133333333333333 0.00016772229920054927
-0.9144444444444444 0.00016385587411620314
-0.9155555555555556 0.00015972802886801926
-0.9166666666666666 0.00015590580342311747
-0.9177777777777778 0.00015218942236005893
-0.9188888888888889 0.0001484317446618304
-0.92 0.00014489851284037866
-0.9211111111111111 0.00014136638278074655
-0.9222222222222223 0.00013802115684002968
-0.9233333333333333 0.00013470656746460038
-0.9244444444444444 0.00013144432779842673
-0.9255555555555556 0.00012841973810743485
-0.9266666666666666 0.00012555872979573354
-0.9277777777777778 0.00012272486373067905
-0.9288888888888889 0.00011997670235639409
-0.93 0.00011728878076244087
-0.9311111111111111 0.00011465420997879205
-0.9322222222222222 0.00011206108599312783
-0.9333333333333333 0.00010974864911114459
-0.9344444444444444 0.00010732230216891982
-0.9355555555555556 0.00010500253718534376
-0.9366666666666666 0.00010279973131641186
-0.9377777777777778 0.00010055431108179396
-0.9388888888888889 9.85150884416943e-05
-0.94 9.64802964840541e-05
-0.9411111111111111 9.450671766762755e-05
-0.9422222222222222 9.261956090327573e-05
-0.9433333333333334 9.071218984896249e-05
-0.9444444444444444 8.886808939872901e-05
-0.9455555555555556 8.709447772728948e-05
-0.9466666666666667 8.53428916524082e-05
-0.9477777777777778 8.364020930307713e-05
-0.9488888888888889 8.204932157599504e-05
-0.95 8.044248712034726e-05
-0.9511111111111111 7.890226166704456e-05
-0.9522222222222222 7.743977951901516e-05
-0.9533333333333334 7.597926879993332e-05
-0.9544444444444444 7.45578876370842e-05
-0.9555555555555556 7.31623694111381e-05
-0.9566666666666667 7.18255200645817e-05
-0.9577777777777777 7.050862665012025e-05
-0.9588888888888889 6.929420775801552e-05
-0.96 6.80434933809043e-05
-0.9611111111111111 6.67646421446196e-05
-0.9622222222222222 6.566036585133292e-05
-0.9633333333333334 6.449774056534008e-05
-0.9644444444444444 6.338884571849527e-05
-0.9655555555555555 6.225918363094514e-05
-0.9666666666666667 6.121405043181473e-05
-0.9677777777777777 6.02295384319066e-05
-0.9688888888888889 5.9198272608720535e-05
-0.97 5.827967493246529e-05
-0.9711111111111111 5.731842699057942e-05
-0.9722222222222222 5.6391490760823394e-05
-0.9733333333333334 5.550052606385837e-05
-0.9744444444444444 5.4654015952446025e-05
-0.9755555555555555 5.382885526661807e-05
-0.9766666666666667 5.305072910761348e-05
-0.9777777777777777 5.230265290646622e-05
-0.9788888888888889 5.155215704140229e-05
-0.98 5.083178418677624e-05
-0.9811111111111112 5.007009682443835e-05
-0.9822222222222222 4.938967621740585e-05
-0.9833333333333333 4.866740871885549e-05
-0.9844444444444445 4.803699786450992e-05
-0.9855555555555555 4.739368257615841e-05
-0.9866666666666667 4.6756830195973786e-05
-0.9877777777777778 4.61312663090538e-05
-0.9888888888888889 4.5574443254940694e-05
-0.99 4.4985584024184805e-05
-0.9911111111111112 4.441685343551027e-05
-0.9922222222222222 4.387745339539758e-05
-0.9933333333333333 4.3389070898794994e-05
-0.9944444444444445 4.2871952143610324e-05
-0.9955555555555555 4.237967455950893e-05
-0.9966666666666667 4.192050158473138e-05
-0.9977777777777778 4.145109989898552e-05
-0.9988888888888889 4.0975772707538356e-05
-1.0 4.052344633654682e-05
-1.001111111111111 4.012230021273017e-05
-1.0022222222222221 3.965787844286692e-05
-1.0033333333333334 3.9234836346746216e-05
-1.0044444444444445 3.887328603802713e-05
-1.0055555555555555 3.850057118556192e-05
-1.0066666666666666 3.8104545868316816e-05
-1.0077777777777779 3.772979059924227e-05
-1.008888888888889 3.7341856572927355e-05
-1.01 3.698631549228971e-05
-1.011111111111111 3.6630615051998176e-05
-1.0122222222222221 3.6323635905229025e-05
-1.0133333333333334 3.5973377211812874e-05
-1.0144444444444445 3.5634027162154156e-05
-1.0155555555555555 3.535420182389714e-05
-1.0166666666666666 3.506964621333235e-05
-1.0177777777777777 3.476347603417923e-05
-1.018888888888889 3.447068197572495e-05
-1.02 3.4195956652442675e-05
-1.021111111111111 3.395172464772666e-05
-1.0222222222222221 3.369110195624919e-05
-1.0233333333333334 3.345035661399322e-05
-1.0244444444444445 3.3186233624098315e-05
-1.0255555555555556 3.2921364068270016e-05
-1.0266666666666666 3.267496382617864e-05
-1.0277777777777777 3.2441814128649116e-05
-1.028888888888889 3.2241089333047434e-05
-1.03 3.201770089263847e-05
-1.031111111111111 3.1797036361406156e-05
-1.0322222222222222 3.155240340274513e-05
-1.0333333333333334 3.1342721188912665e-05
-1.0344444444444445 3.115558507141745e-05
-1.0355555555555556 3.0941845963235655e-05
-1.0366666666666666 3.075099655467527e-05
-1.0377777777777777 3.055143912232937e-05
-1.038888888888889 3.0380889576435708e-05
-1.04 3.019220134385001e-05
-1.041111111111111 3.001803817610657e-05
-1.0422222222222222 2.9868721827356228e-05
-1.0433333333333332 2.9703056411386914e-05
-1.0444444444444445 2.9551941958490567e-05
-1.0455555555555556 2.938890194987483e-05
-1.0466666666666666 2.920776010303796e-05
-1.0477777777777777 2.9063039883985372e-05
-1.048888888888889 2.8926426832389e-05
-1.05 2.878785883250641e-05
-1.051111111111111 2.8654297687662675e-05
-1.0522222222222222 2.8505615978308812e-05
-1.0533333333333332 2.8396457202245454e-05
-1.0544444444444445 2.8276261691376873e-05
-1.0555555555555556 2.8160119671244205e-05
-1.0566666666666666 2.8059074983507356e-05
-1.0577777777777777 2.795654492687902e-05
-1.058888888888889 2.780747877457246e-05
-1.06 2.7714547897283626e-05
-1.0611111111111111 2.7624024966202783e-05
-1.0622222222222222 2.7533196657829373e-05
-1.0633333333333332 2.740731141953417e-05
-1.0644444444444445 2.7342537406390334e-05
-1.0655555555555556 2.723947759695289e-05
-1.0666666666666667 2.712305958161812e-05
-1.0677777777777777 2.7028290452504553e-05
-1.068888888888889 2.6945268947974992e-05
-1.07 2.6867352342830604e-05
-1.0711111111111111 2.6769528982244947e-05
-1.0722222222222222 2.668596446805808e-05
-1.0733333333333333 2.6619466896145353e-05
-1.0744444444444445 2.6553673296986596e-05
-1.0755555555555556 2.6493355450485802e-05
-1.0766666666666667 2.6418819537020007e-05
-1.0777777777777777 2.6338367315775253e-05
-1.0788888888888888 2.628252012420091e-05
-1.08 2.6203900008621476e-05
-1.0811111111111111 2.616984173600642e-05
-1.0822222222222222 2.6122426936876143e-05
-1.0833333333333333 2.6074699962342104e-05
-1.0844444444444445 2.6021029504889333e-05
-1.0855555555555556 2.5966696510679683e-05
-1.0866666666666667 2.5912334218285634e-05
-1.0877777777777777 2.5848722197666257e-05
-1.0888888888888888 2.5815298455545433e-05
-1.09 2.576631763452781e-05
-1.0911111111111111 2.5714421751403656e-05
-1.0922222222222222 2.5670539453110454e-05
-1.0933333333333333 2.563183522712865e-05
-1.0944444444444446 2.5606603167740802e-05
-1.0955555555555556 2.5536949082258148e-05
-1.0966666666666667 2.5484038800678594e-05
-1.0977777777777777 2.54450144534192e-05
-1.0988888888888888 2.5410455295409503e-05
-1.1 2.539740251252803e-05
-1.1011111111111112 2.5363362696512622e-05
-1.1022222222222222 2.5336407079007302e-05
-1.1033333333333333 2.5339971429791262e-05
-1.1044444444444443 2.5325305851540718e-05
-1.1055555555555556 2.5280706034938032e-05
-1.1066666666666667 2.5258104767437904e-05
-1.1077777777777778 2.5213131002670816e-05
-1.1088888888888888 2.5220300399655857e-05
-1.11 2.5181641115338845e-05
-1.1111111111111112 2.515231989200131e-05
-1.1122222222222222 2.51347053361899e-05
-1.1133333333333333 2.5123708480763443e-05
-1.1144444444444443 2.51097991154335e-05
-1.1155555555555556 2.508814924748168e-05
-1.1166666666666667 2.5095933213725866e-05
-1.1177777777777778 2.5093764832613846e-05
-1.1188888888888888 2.5080999108232914e-05
-1.12 2.508321719154627e-05
-1.1211111111111112 2.5086804001619692e-05
-1.1222222222222222 2.5056379671512378e-05
-1.1233333333333333 2.5055048691663643e-05
-1.1244444444444444 2.504198768246655e-05
-1.1255555555555556 2.5039630860013207e-05
-1.1266666666666667 2.5032033114630572e-05
-1.1277777777777778 2.5029292355130675e-05
-1.1288888888888888 2.5057042051455082e-05
-1.13 2.5048723203006e-05
-1.1311111111111112 2.50572914418753e-05
-1.1322222222222222 2.5056999007037002e-05
-1.1333333333333333 2.5053241113243733e-05
-1.1344444444444444 2.505613817862955e-05
-1.1355555555555557 2.505607195598723e-05
-1.1366666666666667 2.507704103431196e-05
-1.1377777777777778 2.5083204727660596e-05
-1.1388888888888888 2.5105928819308972e-05
-1.14 2.5128466221643933e-05
-1.1411111111111112 2.5128118239545796e-05
-1.1422222222222222 2.5113278390035984e-05
-1.1433333333333333 2.5105957168859195e-05
-1.1444444444444444 2.5129635596574673e-05
-1.1455555555555557 2.513039579498289e-05
-1.1466666666666667 2.5144310174623496e-05
-1.1477777777777778 2.5156199070883023e-05
-1.1488888888888888 2.5174338909112982e-05
-1.15 2.5203171919056484e-05
-1.1511111111111112 2.522351100624897e-05
-1.1522222222222223 2.5232807187893496e-05
-1.1533333333333333 2.523469582542523e-05
-1.1544444444444444 2.5259848212187123e-05
-1.1555555555555554 2.5286654451185673e-05
-1.1566666666666667 2.5293507839778124e-05
-1.1577777777777778 2.533461656840215e-05
-1.1588888888888889 2.5367260618070974e-05
-1.16 2.5388561318713978e-05
-1.1611111111111112 2.5421764802553878e-05
-1.1622222222222223 2.5482110339911457e-05
-1.1633333333333333 2.550937072575825e-05
-1.1644444444444444 2.555065812964155e-05
-1.1655555555555555 2.5573477505294346e-05
-1.1666666666666667 2.5621171725968275e-05
-1.1677777777777778 2.563059381709246e-05
-1.1688888888888889 2.5681173438878426e-05
-1.17 2.5741871896003702e-05
-1.1711111111111112 2.5758291863374035e-05
-1.1722222222222223 2.5800007867929392e-05
-1.1733333333333333 2.5856168109098244e-05
-1.1744444444444444 2.5910242747125912e-05
-1.1755555555555555 2.5967876968795265e-05
-1.1766666666666667 2.6015581422147052e-05
-1.1777777777777778 2.6069926554412148e-05
-1.1788888888888889 2.61146768628654e-05
-1.18 2.6167183516484573e-05
-1.181111111111111 2.6211497299080672e-05
-1.1822222222222223 2.627231885918875e-05
-1.1833333333333333 2.6355967517650785e-05
-1.1844444444444444 2.6404236307402604e-05
-1.1855555555555555 2.647771613676032e-05
-1.1866666666666668 2.6553790416434383e-05
-1.1877777777777778 2.6623878682812538e-05
-1.1888888888888889 2.6676149463423334e-05
-1.19 2.6753729032259796e-05
-1.191111111111111 2.6828466555293576e-05
-1.1922222222222223 2.689324532419096e-05
-1.1933333333333334 2.6970603116300772e-05
-1.1944444444444444 2.7052601924236943e-05
-1.1955555555555555 2.7120295399133415e-05
-1.1966666666666668 2.7187824225086913e-05
-1.1977777777777778 2.7272774589251517e-05
-1.198888888888889 2.7363471218633123e-05
-1.2 2.744207459288473e-05
-1.201111111111111 2.7517566697093465e-05
-1.2022222222222223 2.7612869528167065e-05
-1.2033333333333334 2.7691012797215513e-05
-1.2044444444444444 2.7776819094335364e-05
-1.2055555555555555 2.7870552123225133e-05
-1.2066666666666668 2.7952864921187744e-05
-1.2077777777777778 2.80423925517785e-05
-1.208888888888889 2.8141070596919075e-05
-1.21 2.824280409312009e-05
-1.211111111111111 2.834346907568493e-05
-1.2122222222222223 2.8474579095285846e-05
-1.2133333333333334 2.858313792684686e-05
-1.2144444444444444 2.8689033537964072e-05
-1.2155555555555555 2.8823534934139067e-05
-1.2166666666666666 2.8936075935685066e-05
-1.2177777777777778 2.906271694989422e-05
-1.218888888888889 2.918936525080562e-05
-1.22 2.930687335056395e-05
-1.221111111111111 2.941509819253752e-05
-1.2222222222222223 2.952502642441303e-05
-1.2233333333333334 2.9659420152581273e-05
-1.2244444444444444 2.9809444036279495e-05
-1.2255555555555555 2.994308276362788e-05
-1.2266666666666666 3.006849040337803e-05
-1.2277777777777779 3.0215470180038398e-05
-1.228888888888889 3.034338352103931e-05
-1.23 3.047589128745699e-05
-1.231111111111111 3.0608768359335794e-05
-1.2322222222222223 3.075172482954676e-05
-1.2333333333333334 3.09331744077699e-05
-1.2344444444444445 3.109522673475699e-05
-1.2355555555555555 3.126550790369171e-05
-1.2366666666666666 3.1408358840933355e-05
-1.2377777777777779 3.1603475013616876e-05
-1.238888888888889 3.1786757790315846e-05
-1.24 3.1977843055517726e-05
-1.241111111111111 3.2176002776811914e-05
-1.2422222222222221 3.234286962197876e-05
-1.2433333333333334 3.252629123365098e-05
-1.2444444444444445 3.269780529791888e-05
-1.2455555555555555 3.2874113926555856e-05
-1.2466666666666666 3.3096845643955525e-05
-1.2477777777777779 3.3301993092449514e-05
-1.248888888888889 3.3515454390747935e-05
-1.25 3.373272277414685e-05
-1.251111111111111 3.394511187276002e-05
-1.2522222222222221 3.4156332480734e-05
-1.2533333333333334 3.4383249580707513e-05
-1.2544444444444445 3.4606005013696205e-05
-1.2555555555555555 3.480858681537236e-05
-1.2566666666666666 3.502938942644523e-05
-1.2577777777777779 3.529722010663578e-05
-1.258888888888889 3.552508863690576e-05
-1.26 3.579534540373532e-05
-1.261111111111111 3.604495073511492e-05
-1.2622222222222221 3.6301786728123644e-05
-1.2633333333333334 3.659989784654064e-05
-1.2644444444444445 3.6900383150302456e-05
-1.2655555555555555 3.7151728910629016e-05
-1.2666666666666666 3.739214449845277e-05
-1.2677777777777777 3.7700923716800696e-05
-1.268888888888889 3.800910447816014e-05
-1.27 3.829237581418965e-05
-1.271111111111111 3.8598520276254464e-05
-1.2722222222222221 3.8908059130562244e-05
-1.2733333333333334 3.9208861841279e-05
-1.2744444444444445 3.9556608554153635e-05
-1.2755555555555556 3.98952723407649e-05
-1.2766666666666666 4.022702694070903e-05
-1.2777777777777777 4.0594247012668584e-05
-1.278888888888889 4.094998254281126e-05
-1.28 4.136306151579818e-05
-1.281111111111111 4.1696189468292016e-05
-1.2822222222222222 4.205466326169404e-05
-1.2833333333333334 4.244771359421861e-05
-1.2844444444444445 4.283975963011671e-05
-1.2855555555555556 4.3217366666421194e-05
-1.2866666666666666 4.365275506163188e-05
-1.2877777777777777 4.408926990744201e-05
-1.288888888888889 4.452601207613179e-05
-1.29 4.498612235169733e-05
-1.291111111111111 4.544985134506556e-05
-1.2922222222222222 4.590327614318447e-05
-1.2933333333333332 4.637887283339089e-05
-1.2944444444444445 4.686846380136783e-05
-1.2955555555555556 4.7372010660217636e-05
-1.2966666666666666 4.789194493974912e-05
-1.2977777777777777 4.841935244328284e-05
-1.298888888888889 4.8929769397008465e-05
-1.3 4.948815399994531e-05
-1.301111111111111 5.0062560275644356e-05
-1.3022222222222222 5.063680607287459e-05
-1.3033333333333332 5.116219105443753e-05
-1.3044444444444445 5.1792321598010085e-05
-1.3055555555555556 5.238466546640696e-05
-1.3066666666666666 5.297870119775482e-05
-1.3077777777777777 5.3562652606490407e-05
-1.308888888888889 5.419960275246586e-05
-1.31 5.476273427220938e-05
-1.3111111111111111 5.5433806500270473e-05
-1.3122222222222222 5.6091562837979134e-05
-1.3133333333333332 5.679728610952991e-05
-1.3144444444444445 5.751757887497892e-05
-1.3155555555555556 5.8204173341245804e-05
-1.3166666666666667 5.89928488000611e-05
-1.3177777777777777 5.973240870811785e-05
-1.318888888888889 6.045734842497866e-05
-1.32 6.116433536830459e-05
-1.3211111111111111 6.19466506133969e-05
-1.3222222222222222 6.276788651200949e-05
-1.3233333333333333 6.363432390331455e-05
-1.3244444444444445 6.44021713024052e-05
-1.3255555555555556 6.526406806068592e-05
-1.3266666666666667 6.618584179872531e-05
-1.3277777777777777 6.710398333474421e-05
-1.3288888888888888 6.801875421911888e-05
-1.33 6.889866384567407e-05
-1.3311111111111111 6.986900267464923e-05
-1.3322222222222222 7.086831488608457e-05
-1.3333333333333333 7.178649476271771e-05
-1.3344444444444445 7.285250430403026e-05
-1.3355555555555556 7.383143525152062e-05
-1.3366666666666667 7.48636685576884e-05
-1.3377777777777777 7.597556603791727e-05
-1.3388888888888888 7.705759018758415e-05
-1.34 7.823733996136362e-05
-1.3411111111111111 7.934960517438958e-05
-1.3422222222222222 8.052048618712815e-05
-1.3433333333333333 8.164878460220359e-05
-1.3444444444444446 8.285832962843375e-05
-1.3455555555555556 8.408214083614788e-05
-1.3466666666666667 8.535314743617154e-05
-1.3477777777777777 8.665027944658744e-05
-1.3488888888888888 8.799407323992279e-05
-1.35 8.936104395514382e-05
-1.3511111111111112 9.074426219929899e-05
-1.3522222222222222 9.216096555244511e-05
-1.3533333333333333 9.35424031733211e-05
-1.3544444444444443 9.494972145976259e-05
-1.3555555555555556 9.6418855265422e-05
-1.3566666666666667 9.797057570291795e-05
-1.3577777777777778 9.952350701728078e-05
-1.3588888888888888 0.00010113628127920678
-1.36 0.00010267072692797368
-1.3611111111111112 0.00010429277303722426
-1.3622222222222222 0.00010596545359143936
-1.3633333333333333 0.00010769278258727096
-1.3644444444444443 0.0001093654312997449
-1.3655555555555556 0.00011115394131872826
-1.3666666666666667 0.00011296772614964923
-1.3677777777777778 0.00011500458467488756
-1.3688888888888888 0.0001168678839591725
-1.37 0.0001187782496876762
-1.3711111111111112 0.00012081517496641339
-1.3722222222222222 0.00012285097956541587
-1.3733333333333333 0.0001249760161149821
-1.3744444444444444 0.00012718135225849863
-1.3755555555555556 0.0001293458245685856
-1.3766666666666667 0.00013147721744872145
-1.3777777777777778 0.00013372440130033153
-1.3788888888888888 0.00013617825520704474
-1.38 0.00013850037105511527
-1.3811111111111112 0.0001409156964549084
-1.3822222222222222 0.0001434338154814215
-1.3833333333333333 0.00014585660641629859
-1.3844444444444444 0.0001486373696465938
-1.3855555555555557 0.00015133765380761984
-1.3866666666666667 0.00015406222362779107
-1.3877777777777778 0.00015681016161955762
-1.3888888888888888 0.0001597794360497374
-1.39 0.00016283554323157976
-1.3911111111111112 0.0001657692659217883
-1.3922222222222222 0.0001688828122998033
-1.3933333333333333 0.00017190788293870905
-1.3944444444444444 0.00017507926798366233
-1.3955555555555557 0.00017829396105900925
-1.3966666666666667 0.00018178173951142424
-1.3977777777777778 0.00018518872473332525
-1.3988888888888888 0.00018868293737989917
-1.4 0.00019235193519498339
-1.4011111111111112 0.00019605222514787384
-1.4022222222222223 0.0001997940046412795
-1.4033333333333333 0.00020364258818020886
-1.4044444444444444 0.00020754915908007397
-1.4055555555555554 0.00021157603740570234
-1.4066666666666667 0.00021542240382593038
-1.4077777777777778 0.00021969581339859322
-1.4088888888888889 0.0002238333242658783
-1.41 0.00022836748473361562
-1.4111111111111112 0.00023278044477402122
-1.4122222222222223 0.00023737242636945365
-1.4133333333333333 0.00024221618704669396
-1.4144444444444444 0.0002469387252038305
-1.4155555555555555 0.0002520101812784816
-1.4166666666666667 0.00025711342726759354
-1.4177777777777778 0.00026224633161302523
-1.4188888888888889 0.00026768798355349046
-1.42 0.0002730658322252746
-1.4211111111111112 0.0002786645600303868
-1.4222222222222223 0.0002844755561207245
-1.4233333333333333 0.0002906119282438017
-1.4244444444444444 0.00029642789294471474
-1.4255555555555555 0.0003023271247457946
-1.4266666666666667 0.00030843021838874676
-1.4277777777777778 0.00031468812528570697
-1.4288888888888889 0.00032130498172701485
-1.43 0.0003278897148312677
-1.431111111111111 0.0003346126240730679
-1.4322222222222223 0.00034165030117222104
-1.4333333333333333 0.00034870443985664864
-1.4344444444444444 0.0003558556733968095
-1.4355555555555555 0.00036351306177569
-1.4366666666666668 0.0003709359035009088
-1.4377777777777778 0.0003785497777937562
-1.4388888888888889 0.0003865343640269306
-1.44 0.0003948231939407691
-1.441111111111111 0.00040337490473450136
-1.4422222222222223 0.00041231176304936605
-1.4433333333333334 0.00042093048377938805
-1.4444444444444444 0.0004303035966372804
-1.4455555555555555 0.00043967072828126664
-1.4466666666666668 0.00044901398958155684
-1.4477777777777778 0.00045887328162948487
-1.448888888888889 0.00046894039813840467
-1.45 0.00047916430377227596
-1.451111111111111 0.0004893251733165109
-1.4522222222222223 0.0004995490032174244
-1.4533333333333334 0.00051109030214089
-1.4544444444444444 0.0005219867616331412
-1.4555555555555555 0.0005333489284365428
-1.4566666666666668 0.0005454129073085031
-1.4577777777777778 0.0005574602579776291
-1.458888888888889 0.0005695556600798482
-1.46 0.0005825563127558126
-1.461111111111111 0.0005949608952721496
-1.4622222222222223 0.0006088670990174404
-1.4633333333333334 0.000622429227092306
-1.4644444444444444 0.0006369669789808191
-1.4655555555555555 0.0006514568419127034
-1.4666666666666666 0.0006664199175997459
-1.4677777777777778 0.0006819881131507976
-1.468888888888889 0.000697590671085975
-1.47 0.0007132645552303008
-1.471111111111111 0.000729119643375564
-1.4722222222222223 0.0007463892426267272
-1.4733333333333334 0.0007639216982366869
-1.4744444444444444 0.000781716512052855
-1.4755555555555555 0.0007995880608276152
-1.4766666666666666 0.0008177420842506783
-1.4777777777777779 0.0008362848761861887
-1.478888888888889 0.0008565489190382803
-1.48 0.0008767312533136837
-1.481111111111111 0.0008973066647234005
-1.4822222222222223 0.0009194190205043463
-1.4833333333333334 0.0009402081773247377
-1.4844444444444445 0.0009628736992084917
-1.4855555555555555 0.0009855737176095649
-1.4866666666666666 0.0010089977325622088
-1.4877777777777779 0.0010334435258604654
-1.488888888888889 0.0010573338195408101
-1.49 0.001083079131794496
-1.491111111111111 0.0011093448928852516
-1.4922222222222221 0.0011360112200773339
-1.4933333333333334 0.00116446679013468
-1.4944444444444445 0.0011928792388159488
-1.4955555555555555 0.001222536799844871
-1.4966666666666666 0.0012534247007064542
-1.4977777777777779 0.0012857501079137242
-1.498888888888889 0.0013177639885143882
-1.5 0.001349994206622322
-1.501111111111111 0.001383463271957585
-1.5022222222222221 0.001417695409670703
-1.5033333333333334 0.0014523259007159146
-1.5044444444444445 0.001490352805484511
-1.5055555555555555 0.0015289512343252178
-1.5066666666666666 0.0015687743216119465
-1.5077777777777779 0.0016090145182843405
-1.508888888888889 0.0016500429160125052
-1.51 0.0016931156845200789
-1.511111111111111 0.0017360566506065176
-1.5122222222222221 0.0017809090789213384
-1.5133333333333334 0.0018270350244525334
-1.5144444444444445 0.0018755006350523792
-1.5155555555555555 0.0019236722498912032
-1.5166666666666666 0.001973650525203378
-1.5177777777777777 0.0020236439760830363
-1.518888888888889 0.002075633805182805
-1.52 0.002130431519955138
-1.521111111111111 0.002185005049178474
-1.5222222222222221 0.002242746318452991
-1.5233333333333334 0.0023017418898351816
-1.5244444444444445 0.0023632993563547505
-1.5255555555555556 0.0024258209099814834
-1.5266666666666666 0.0024887151718433515
-1.5277777777777777 0.002558331487299895
-1.528888888888889 0.002628052468333711
-1.53 0.0026978472672933677
-1.531111111111111 0.0027687285053619006
-1.5322222222222222 0.002844281085011993
-1.5333333333333334 0.0029200722408114803
-1.5344444444444445 0.003000516605693398
-1.5355555555555556 0.0030810918466305528
-1.5366666666666666 0.0031654869242539354
-1.5377777777777777 0.0032533358412861492
-1.538888888888889 0.0033431513566324674
-1.54 0.003436651396609168
-1.541111111111111 0.0035308330274545613
-1.5422222222222222 0.003628725807441896
-1.5433333333333332 0.0037259873353024625
-1.5444444444444445 0.003828839661097186
-1.5455555555555556 0.003933780719571605
-1.5466666666666666 0.004041416752217384
-1.5477777777777777 0.004157149004730792
-1.548888888888889 0.004276865865610443
-1.55 0.004396263077903695
-1.551111111111111 0.004520708924570267
-1.5522222222222222 0.0046495368751338926
-1.5533333333333332 0.004785084338037691
-1.5544444444444445 0.00491676418200625
-1.5555555555555556 0.005055517954688611
-1.5566666666666666 0.005198700413878457
-1.5577777777777777 0.0053500481726763876
-1.558888888888889 0.0055041383292165225
-1.56 0.0056619728417067455
-1.5611111111111111 0.005829389012986537
-1.5622222222222222 0.005993234307081133
-1.5633333333333332 0.006172240508428828
-1.5644444444444445 0.006358088261488131
-1.5655555555555556 0.006549675791371602
-1.5666666666666667 0.0067413010891882365
-1.5677777777777777 0.006933431370088924
-1.568888888888889 0.007141783044072103
-1.57 0.0073566937947330355
-1.5711111111111111 0.007572624795032628
-1.5722222222222222 0.007800616610928742
-1.5733333333333333 0.008029879172320925
-1.5744444444444445 0.008268855117493071
-1.5755555555555556 0.008524674670637488
-1.5766666666666667 0.008790209485422855
-1.5777777777777777 0.009057736620843351
-1.5788888888888888 0.009340447103057257
-1.58 0.009621317797197432
-1.5811111111111111 0.009915369417882456
-1.5822222222222222 0.010224102800112371
-1.5833333333333333 0.01054201694851436
-1.5844444444444445 0.010867336053710952
-1.5855555555555556 0.011197757124964432
-1.5866666666666667 0.011547309644536121
-1.5877777777777777 0.01189864897669556
-1.5888888888888888 0.012271588691802879
-1.59 0.012659931696356352
-1.5911111111111111 0.013070908164711098
-1.5922222222222222 0.013498729572870082
-1.5933333333333333 0.013924117819022799
-1.5944444444444446 0.014356263695852906
-1.5955555555555556 0.014809040663818548
-1.5966666666666667 0.015277306833924725
-1.5977777777777777 0.015759165820655018
-1.5988888888888888 0.016270477426117237
-1.6 0.016803815188096958
-1.6011111111111112 0.017359859827715617
-1.6022222222222222 0.017914833267116792
-1.6033333333333333 0.018496820576809278
-1.6044444444444443 0.01909498511229863
-1.6055555555555556 0.019727055270946706
-1.6066666666666667 0.0203912335280639
-1.6077777777777778 0.021073202628714233
-1.6088888888888888 0.021785453382567047
-1.61 0.022483771063249215
-1.6111111111111112 0.023241736854434283
-1.6122222222222222 0.024016670814264677
-1.6133333333333333 0.02481159006606205
-1.6144444444444443 0.025644355939345023
-1.6155555555555556 0.026503669951163645
-1.6166666666666667 0.02740844023577586
-1.6177777777777778 0.02835177519358019
-1.6188888888888888 0.02933717470248022
-1.62 0.03035371136393588
-1.6211111111111112 0.03136947790105722
-1.6222222222222222 0.03246385640500894
-1.6233333333333333 0.03358013932284124
-1.6244444444444444 0.034798788799010515
-1.6255555555555556 0.03597708504954679
-1.6266666666666667 0.03723559872081835
-1.6277777777777778 0.038545050604129216
-1.6288888888888888 0.03987910465139318
-1.63 0.041290216514291475
-1.6311111111111112 0.04275169288646124
-1.6322222222222222 0.044240514414905736
-1.6333333333333333 0.04578299479561332
-1.6344444444444444 0.04744616488448097
-1.6355555555555557 0.04911879664058275
-1.6366666666666667 0.05088161858186735
-1.6377777777777778 0.052732409380651525
-1.6388888888888888 0.05466133645083406
-1.64 0.05658780880178017
-1.6411111111111112 0.058627060550581624
-1.6422222222222222 0.060764669232347475
-1.6433333333333333 0.06293270609862156
-1.6444444444444444 0.06518877670692724
-1.6455555555555557 0.06761072684201755
-1.6466666666666667 0.07004951637351253
-1.6477777777777778 0.072569055439605
-1.6488888888888888 0.07521008993861134
-1.65 0.07794390240034416
-1.6511111111111112 0.08084185772588207
-1.6522222222222223 0.08382544278449974
-1.6533333333333333 0.08702381821998198
-1.6544444444444444 0.09031873351436077
-1.6555555555555554 0.0937430084319727
-1.6566666666666667 0.09729456091084188
-1.6577777777777778 0.10084753618099966
-1.6588888888888889 0.1045258770256802
-1.66 0.10841509529741188
-1.6611111111111112 0.11239484075140123
-1.6622222222222223 0.11653758789067453
-1.6633333333333333 0.12089022729090637
-1.6644444444444444 0.12545446815149625
-1.6655555555555555 0.13007143540006663
-1.6666666666666667 0.13489532155155057
-1.6677777777777778 0.1399194900894825
-1.6688888888888889 0.14528487064570528
-1.67 0.15081419312590033
-1.6711111111111112 0.15647718236648614
-1.6722222222222223 0.1624712058575911
-1.6733333333333333 0.16842451171401215
-1.6744444444444444 0.17476155130766663
-1.6755555555555555 0.18141635612013768
-1.6766666666666667 0.18829763689064338
-1.6777777777777778 0.1954271572476543
-1.6788888888888889 0.20280845504359676
-1.68 0.21050833717560344
-1.681111111111111 0.21848977038120332
-1.6822222222222223 0.22666769165405412
-1.6833333333333333 0.23520408840752885
-1.6844444444444444 0.24436532649691842
-1.6855555555555555 0.2535240232810209
-1.6866666666666668 0.26296842464680265
-1.6877777777777778 0.27303266518911506
-1.6888888888888889 0.28371977930949965
-1.69 0.29440248765879506
-1.691111111111111 0.3058743564706841
-1.6922222222222223 0.3174574351331129
-1.6933333333333334 0.32930377991302157
-1.6944444444444444 0.34192872460174173
-1.6955555555555555 0.35489979765111485
-1.6966666666666668 0.36834146651992955
-1.6977777777777778 0.3826345129901521
-1.698888888888889 0.3970020814523139
-1.7 0.4121375703609216
-1.701111111111111 0.42795120797824737
-1.7022222222222223 0.4447344511620162
-1.7033333333333334 0.46102861985476934
-1.7044444444444444 0.4786465327868731
-1.7055555555555555 0.4969885000231768
-1.7066666666666668 0.515675221446428
-1.7077777777777778 0.535740155948972
-1.708888888888889 0.5556660333053163
-1.71 0.5762227272489262
-1.711111111111111 0.5979474845214421
-1.7122222222222223 0.6206972866618876
-1.7133333333333334 0.6441153732116625
-1.7144444444444444 0.6686447396112185
-1.7155555555555555 0.6933313174416419
-1.7166666666666666 0.7197039092298007
-1.7177777777777778 0.7463725431299922
-1.718888888888889 0.7741100317420324
-1.72 0.8028066176223587
-1.721111111111111 0.8330521901240298
-1.7222222222222223 0.8636007173323725
-1.7233333333333334 0.896199149156703
-1.7244444444444444 0.9295086592909352
-1.7255555555555555 0.96424831464943
-1.7266666666666666 0.9989840933080845
-1.7277777777777779 1.0350531874604834
-1.728888888888889 1.0726596146412317
-1.73 1.111946896189399
-1.731111111111111 1.152786291153564
-1.7322222222222223 1.194804690873286
-1.7333333333333334 1.2385368657765288
-1.7344444444444445 1.2827060754144837
-1.7355555555555555 1.3285499037607544
-1.7366666666666666 1.3758296225722717
-1.7377777777777779 1.4245501373645395
-1.738888888888889 1.4766021477511484
-1.74 1.5289419173773495
-1.741111111111111 1.583188640925469
-1.7422222222222221 1.6397079818211027
-1.7433333333333334 1.6950987744704005
-1.7444444444444445 1.755300359914359
-1.7455555555555555 1.8161107230199303
-1.7466666666666666 1.8775148287441175
-1.7477777777777779 1.9414690009425208
-1.748888888888889 2.0069556387888947
-1.75 2.0740391719965356
-1.751111111111111 2.143738769171342
-1.7522222222222221 2.2159644667502745
-1.7533333333333334 2.2879490098740654
-1.7544444444444445 2.362605970017597
-1.7555555555555555 2.4387438592839596
-1.7566666666666666 2.516905290589088
-1.7577777777777779 2.599198565288768
-1.758888888888889 2.680627462129561
-1.76 2.7655693755239037
-1.761111111111111 2.853357065831316
-1.7622222222222221 2.9397535875367935
-1.7633333333333334 3.0286875929523687
-1.7644444444444445 3.1218526734768153
-1.7655555555555555 3.2171510801238536
-1.7666666666666666 3.3122418759337546
-1.7677777777777777 3.4079007919671858
-1.768888888888889 3.5082859824851433
-1.77 3.610687081362753
-1.771111111111111 3.712121414267543
-1.7722222222222221 3.8191322245453345
-1.7733333333333334 3.9265365726553214
-1.7744444444444445 4.036410319105332
-1.7755555555555556 4.1466109929831365
-1.7766666666666666 4.255485039391674
-1.7777777777777777 4.368295196484288
-1.778888888888889 4.485005260294795
-1.78 4.596961349487702
-1.781111111111111 4.71210013439382
-1.7822222222222222 4.8286383937374655
-1.7833333333333334 4.94847840605737
-1.7844444444444445 5.069217794769166
-1.7855555555555556 5.188266052500532
-1.7866666666666666 5.310400307126907
-1.7877777777777777 5.433098267255349
-1.788888888888889 5.559453882626331
-1.79 5.678614097135536
-1.791111111111111 5.806301146792322
-1.7922222222222222 5.930817744553607
-1.7933333333333332 6.050424258538959
-1.7944444444444445 6.169962072828391
-1.7955555555555556 6.296935448767959
-1.7966666666666666 6.423265183338275
-1.7977777777777777 6.554673152381735
-1.798888888888889 6.676878127233908
-1.8 6.79989206643305
-1.801111111111111 6.916821835962052
-1.8022222222222222 7.036859016675482
-1.8033333333333332 7.156802666132577
-1.8044444444444445 7.268312398921802
-1.8055555555555556 7.383498022087096
-1.8066666666666666 7.495694202112424
-1.8077777777777777 7.614940209315936
-1.808888888888889 7.71322898353472
-1.81 7.814164461535624
-1.8111111111111111 7.914399554311714
-1.8122222222222222 8.009136335745936
-1.8133333333333332 8.110836259354606
-1.8144444444444445 8.203535463812253
-1.8155555555555556 8.293298761539194
-1.8166666666666667 8.374769102297497
-1.8177777777777777 8.459478143354376
-1.818888888888889 8.540502091900136
-1.82 8.610061951139683
-1.8211111111111111 8.674360241105658
-1.8222222222222222 8.748392406815755
-1.8233333333333333 8.806546065857242
-1.8244444444444445 8.850435105593109
-1.8255555555555556 8.893072772413989
-1.8266666666666667 8.937559486152201
-1.8277777777777777 8.964767247952185
-1.8288888888888888 8.9936168831287
-1.83 9.020405802576649
-1.8311111111111111 9.02882239883417
-1.8322222222222222 9.041480692549543
-1.8333333333333333 9.034417148626993
-1.8344444444444445 9.021885734290523
-1.8355555555555556 9.008040161192891
-1.8366666666666667 8.987659934585194
-1.8377777777777777 8.967635336568973
-1.8388888888888888 8.92933446092408
-1.84 8.891623262243158
-1.8411111111111111 8.844753992522113
-1.8422222222222222 8.791021443432419
-1.8433333333333333 8.739990338786724
-1.8444444444444446 8.672385039416593
-1.8455555555555556 8.601170489601362
-1.8466666666666667 8.512632823605735
-1.8477777777777777 8.419618286330774
-1.8488888888888888 8.320971100771025
-1.85 8.221797523385447
-1.8511111111111112 8.112145842785155
-1.8522222222222222 8.007689466656629
-1.8533333333333333 7.88217868811476
-1.8544444444444443 7.7503307445658995
-1.8555555555555556 7.619361227544419
-1.8566666666666667 7.481976698038163
-1.8577777777777778 7.3380862549263455
-1.8588888888888888 7.193294442302542
-1.86 7.040800129850648
-1.8611111111111112 6.891540634666122
-1.8622222222222222 6.733147736833181
-1.8633333333333333 6.572002912709012
-1.8644444444444443 6.404707547270531
-1.8655555555555556 6.233807307321547
-1.8666666666666667 6.066907012944739
-1.8677777777777778 5.89773083544604
-1.8688888888888888 5.721261052681486
-1.87 5.549516094145234
-1.8711111111111112 5.375190528538842
-1.8722222222222222 5.190683618586964
-1.8733333333333333 5.016264401749384
-1.8744444444444444 4.835833489582424
-1.8755555555555556 4.660490451258166
-1.8766666666666667 4.488928744450868
-1.8777777777777778 4.316704813729708
-1.8788888888888888 4.148670665321631
-1.88 3.9774235085339162
-1.8811111111111112 3.812920562938845
-1.8822222222222222 3.645617730860818
-1.8833333333333333 3.4753646323991436
-1.8844444444444444 3.3130922645254746
-1.8855555555555557 3.150804479939782
-1.8866666666666667 2.994956997085972
-1.8877777777777778 2.8428522287854863
-1.8888888888888888 2.6954485820120735
-1.89 2.55049764439293
-1.8911111111111112 2.409346385982104
-1.8922222222222222 2.272161639140683
-1.8933333333333333 2.1406527435070997
-1.8944444444444444 2.012253154273927
-1.8955555555555557 1.8880257045087125
-1.8966666666666667 1.7695529307430047
-1.8977777777777778 1.6557706421258995
-1.8988888888888888 1.5459458474886671
-1.9 1.4419538927736315
-1.9011111111111112 1.342191947572981
-1.9022222222222223 1.2475114355563093
-1.9033333333333333 1.155722345993384
-1.9044444444444444 1.069777678581587
-1.9055555555555554 0.9897588443188117
-1.9066666666666667 0.9123509383992244
-1.9077777777777778 0.8387941098274942
-1.9088888888888889 0.7710765052013925
-1.91 0.7074213170301736
-1.9111111111111112 0.6462268669333333
-1.9122222222222223 0.5893321964627537
-1.9133333333333333 0.5385273310430445
-1.9144444444444444 0.49056298291103356
-1.9155555555555555 0.4437055463044562
-1.9166666666666667 0.4012899434347009
-1.9177777777777778 0.3644931550663475
-1.9188888888888889 0.32797354999847145
-1.92 0.29321501428350655
-1.9211111111111112 0.2628033587983236
-1.9222222222222223 0.23730211708976964
-1.9233333333333333 0.21102728067967785
-1.9244444444444444 0.18617826391268674
-1.9255555555555555 0.16598714883554144
-1.9266666666666667 0.14926080312948112
-1.9277777777777778 0.1299845926802779
-1.9288888888888889 0.11331886938633526
-1.93 0.10073919648826402
-1.931111111111111 0.08997676404772716
-1.9322222222222223 0.07633904266555809
-1.9333333333333333 0.06601964576786287
-1.9344444444444444 0.05877012212518336
-1.9355555555555555 0.052024758613358334
-1.9366666666666668 0.04238742745348925
-1.9377777777777778 0.03675902243898974
-1.9388888888888889 0.03286154087940906
-1.94 0.02855213723370103
-1.941111111111111 0.022045646816398094
-1.9422222222222223 0.01955149998749211
-1.9433333333333334 0.01751806646862074
-1.9444444444444444 0.014781895988541861
-1.9455555555555555 0.010624025649336953
-1.9466666666666668 0.009961074018717389
-1.9477777777777778 0.008865463922390819
-1.948888888888889 0.007155022679488402
-1.95 0.004699683413315938
-1.951111111111111 0.0048903992345300275
-1.9522222222222223 0.004226421372455957
-1.9533333333333334 0.003202118146380768
-1.9544444444444444 0.0018809361549698507
-1.9555555555555555 0.00231648028604553
-1.9566666666666668 0.0018730248420739445
-1.9577777777777778 0.0013041512148188497
-1.958888888888889 0.000671269548995313
-1.96 0.0010543303794500825
-1.961111111111111 0.0007558857943918269
-1.9622222222222223 0.0004764741790982417
-1.9633333333333334 0.00020903506906299975
-1.9644444444444444 0.0004544336856162997
-1.9655555555555555 0.0002730912133008622
-1.9666666666666666 0.00015357288385205495
-1.9677777777777778 5.5514594629548255e-05
-1.968888888888889 0.0001813655584412048
-1.97 8.551351749536048e-05
-1.971111111111111 4.255773312267261e-05
-1.9722222222222223 1.2163965820938983e-05
-1.9733333333333334 6.539029763275119e-05
-1.9744444444444444 2.2519162428415457e-05
-1.9755555555555555 9.883925574598946e-06
-1.9766666666666666 2.098426122182465e-06
-1.9777777777777779 2.0509248679396997e-05
-1.978888888888889 4.765535456332791e-06
-1.98 1.8574411809010271e-06
-1.981111111111111 2.6718060193965774e-07
-1.9822222222222223 5.418954763851491e-06
-1.9833333333333334 7.566251531493011e-07
-1.9844444444444445 2.651118664887214e-07
-1.9855555555555555 2.1808442141693165e-08
-1.9866666666666666 1.149385360179085e-06
-1.9877777777777779 8.004283561314308e-08
-1.988888888888889 2.5713057378883017e-08
-1.99 8.383799426853795e-10
-1.991111111111111 1.8213209247473713e-07
-1.9922222222222221 4.213811915124331e-09
-1.9933333333333334 1.2794003516125512e-09
-1.9944444444444445 0.0
-1.9955555555555555 1.9152268918623293e-08
-1.9966666666666666 0.0
-1.9977777777777779 0.0
-1.998888888888889 0.0
-2.0 1.0413991102348627e-09


==> Plots/autocorrelation_time.tex <==
e T
0.0 1.0985714285714288
-0.03125 1.1057142857142856
-0.0625 1.0914285714285719
-0.09375 1.1257142857142863
-0.125 1.1571428571428575
-0.15625 1.2514285714285718
-0.1875 1.3571428571428577
-0.21875 1.5171428571428578
-0.25 1.708571428571429
-0.28125 1.9657142857142869
-0.3125 2.334285714285715
-0.34375 2.8742857142857154
-0.375 3.700000000000001
-0.40625 4.8571428571428585
-0.4375 6.700000000000004
-0.46875 9.602857142857147
-0.5 14.822857142857147
-0.53125 24.220000000000013
-0.5625 42.92857142857144
-0.59375 85.43142857142861
-0.625 169.98571428571435
-0.65625 338.41714285714295
-0.6875 597.5542857142859
-0.71875 982.0257142857147
-0.75 1341.9371428571433
-0.78125 1571.171428571429
-0.8125 1740.6828571428578
-0.84375 1817.3142857142864
-0.875 1838.2342857142864
-0.90625 1998.0542857142864
-0.9375 2008.642857142858
-0.96875 1566.371428571429
-1.0 913.2228571428576
-1.03125 580.377142857143
-1.0625 449.5542857142859
-1.09375 439.4114285714288
-1.125 457.92000000000013
-1.15625 466.7457142857144
-1.1875 469.02000000000015
-1.21875 501.18857142857166
-1.25 515.0600000000003
-1.28125 472.00000000000017
-1.3125 406.3085714285716
-1.34375 332.657142857143
-1.375 314.2114285714287
-1.40625 326.24571428571437
-1.4375 360.01428571428585
-1.46875 387.3257142857144
-1.5 447.32285714285734
-1.53125 500.8742857142858
-1.5625 547.6285714285716
-1.59375 564.837142857143
-1.625 547.337142857143
-1.65625 465.14000000000016
-1.6875 341.4400000000001
-1.71875 225.60285714285723
-1.75 139.3228571428572
-1.78125 94.43714285714289
-1.8125 64.02571428571432
-1.84375 46.451428571428586
-1.875 38.2057142857143
-1.90625 33.17428571428572
-1.9375 24.317142857142798
-1.96875 0.09571428571417823


==> Plots/condensation.tex <==
e c
-1.500625 0.9557401757125134
-1.50125 0.9552046527047967
-1.501875 0.9546298428144278
-1.5025 0.9510122147207837
-1.503125 0.9526314859858026
-1.50375 0.9512859891258612
-1.504375 0.9497467734876806
-1.505 0.9505238691892469
-1.505625 0.9503061747026245
-1.50625 0.9462306129803479
-1.506875 0.9493240560389609
-1.5075 0.951125640377109
-1.508125 0.946788582260705
-1.50875 0.951611386267586
-1.509375 0.9527287316599715
-1.51 0.953323669985064
-1.510625 0.9547444088548017
-1.51125 0.9485453885824379
-1.511875 0.9579901234441976
-1.5125 0.949688604284761
-1.513125 0.9523544910119591
-1.51375 0.9514266230691352
-1.514375 0.9510815022982022
-1.515 0.9526468290901187
-1.515625 0.9554122843265442
-1.51625 0.9568741954769076
-1.516875 0.9572476650841582
-1.5175 0.9568370512500121
-1.518125 0.9529943648173942
-1.51875 0.9549166206288601
-1.519375 0.9582307673067297
-1.52 0.9494547562719159
-1.520625 0.9500131808143863
-1.52125 0.951573671452282
-1.521875 0.9503618213492003
-1.5225 0.9564854026224708
-1.523125 0.9512820850520506
-1.52375 0.949039506135785
-1.524375 0.947031495334057
-1.525 0.9521230784073024
-1.525625 0.9517335808496479
-1.52625 0.9518411893190105
-1.526875 0.9512323417578328
-1.5275 0.9524288224306172
-1.528125 0.9504202499679998
-1.52875 0.9536771705248563
-1.529375 0.9540480119545877
-1.53 0.9535935229142288
-1.530625 0.9526444797896398
-1.53125 0.9495579356071384
-1.531875 0.951466426431498
-1.5325 0.9523079132642392
-1.533125 0.9565799591383429
-1.53375 0.9594637259900649
-1.534375 0.9550028055743264
-1.535 0.9578285058346437
-1.535625 0.9569952146784321
-1.53625 0.957380449740128
-1.536875 0.9538187093704402
-1.5375 0.9589556161503623
-1.538125 0.9497206041625877
-1.53875 0.952154566011287
-1.539375 0.9540077194529419
-1.54 0.9541794380269143
-1.540625 0.95340849303183
-1.54125 0.9535470644725424
-1.541875 0.953930725919757
-1.5425 0.9507256306556766
-1.543125 0.9530543273731292
-1.54375 0.9517075672482389
-1.544375 0.9526045809244769
-1.545 0.9541760083660288
-1.545625 0.9534583851162914
-1.54625 0.9542691268892757
-1.546875 0.954798699071709
-1.5475 0.9498507722090441
-1.548125 0.9490369479054728
-1.54875 0.9510800466427634
-1.549375 0.9518732075884846
-1.55 0.9506676272745727
-1.550625 0.9544590210309031
-1.55125 0.9538594522831416
-1.551875 0.952694882889532
-1.5525 0.9522600590760224
-1.553125 0.9482186747847168
-1.55375 0.9502968414210834
-1.554375 0.948708504522973
-1.555 0.9441390766259289
-1.555625 0.9490502043518606
-1.55625 0.946174161090426
-1.556875 0.9444678253196647
-1.5575 0.9437299297079711
-1.558125 0.9452650224140232
-1.55875 0.9408932539670788
-1.559375 0.9438454942414054
-1.56 0.9432611608802276
-1.560625 0.941524441464466
-1.56125 0.9414544887450275
-1.561875 0.9386326707575484
-1.5625 0.9414123069455833
-1.563125 0.9406490811363691
-1.56375 0.9415438459386002
-1.564375 0.9372438685893031
-1.565 0.9398377533368866
-1.565625 0.936453882114746
-1.56625 0.9376860664791109
-1.566875 0.9406649694220224
-1.5675 0.9410363328481601
-1.568125 0.9391604036324579
-1.56875 0.9355059396105929
-1.569375 0.9349021253963832
-1.57 0.9340617871758414
-1.570625 0.9327653652062731
-1.57125 0.9325964741696033
-1.571875 0.9314018086430581
-1.5725 0.9340819956523476
-1.573125 0.9287225081056598
-1.57375 0.9291761446173213
-1.574375 0.9241963496286583
-1.575 0.9307414158721233
-1.575625 0.9286707173208827
-1.57625 0.9255442134934494
-1.576875 0.9307326091383197
-1.5775 0.9267096643117363
-1.578125 0.9281672011360657
-1.57875 0.9252405690627672
-1.579375 0.9276883443091997
-1.58 0.9255115477752849
-1.580625 0.9287041309654379
-1.58125 0.9339895525035398
-1.581875 0.929598243895847
-1.5825 0.9297347151889533
-1.583125 0.9294819987378393
-1.58375 0.9296482998060864
-1.584375 0.9309895620780793
-1.585 0.9287688157783892
-1.585625 0.9280688201412184
-1.58625 0.9222297973772284
-1.586875 0.9193924395280412
-1.5875 0.919634280653106
-1.588125 0.9176886892103266
-1.58875 0.916890948264448
-1.589375 0.9111767939442189
-1.59 0.9106029006220793
-1.590625 0.9144555377293186
-1.59125 0.9131199978426904
-1.591875 0.9135366987503801
-1.5925 0.909684856454998
-1.593125 0.9113707329195739
-1.59375 0.9071034131625625
-1.594375 0.9021666876151357
-1.595 0.9078258571537555
-1.595625 0.9018904832645369
-1.59625 0.9087810704935266
-1.596875 0.9026902617356906
-1.5975 0.9033363637761211
-1.598125 0.8981981018658356
-1.59875 0.9039145665368095
-1.599375 0.8938894693404217
-1.6 0.8964963816742771
-1.600625 0.8954535293738528
-1.60125 0.891342347132767
-1.601875 0.8941411781066538
-1.6025 0.8882541223552602
-1.603125 0.8902495577147955
-1.60375 0.8883151675059852
-1.604375 0.8816379716246855
-1.605 0.8826540352306438
-1.605625 0.8842213162944769
-1.60625 0.8802796265903169
-1.606875 0.8768336607412748
-1.6075 0.8841263743865385
-1.608125 0.877211752631692
-1.60875 0.8810858553267025
-1.609375 0.8794184875176279
-1.61 0.8715953006092799
-1.610625 0.8709558708388907
-1.61125 0.8646864421209605
-1.611875 0.8690687962471604
-1.6125 0.8630917314466681
-1.613125 0.8583482612916387
-1.61375 0.8651462357095506
-1.614375 0.857657966513442
-1.615 0.8614292520744238
-1.615625 0.8578389540180216
-1.61625 0.8514171745102525
-1.616875 0.8484178779668909
-1.6175 0.8472032823403266
-1.618125 0.8478421272101508
-1.61875 0.8462831861505343
-1.619375 0.8368003397894421
-1.62 0.8394579002446754
-1.620625 0.8393844724794763
-1.62125 0.8317340875045831
-1.621875 0.8220537491993157
-1.6225 0.8265327624836174
-1.623125 0.8250663617418535
-1.62375 0.8283953291716583
-1.624375 0.8187889594549081
-1.625 0.817229323021787
-1.625625 0.8104984159138193
-1.62625 0.8105248163702913
-1.626875 0.8111241763947467
-1.6275 0.8049559214514769
-1.628125 0.8047581439325706
-1.62875 0.7989867952746649
-1.629375 0.7942573935025109
-1.63 0.7903642678376253
-1.630625 0.789253226873217
-1.63125 0.7828443151965819
-1.631875 0.7774935200035475
-1.6325 0.7795414757523383
-1.633125 0.7768508651295936
-1.63375 0.7716827920528443
-1.634375 0.7711927423391943
-1.635 0.7683045984600709
-1.635625 0.7669088505709558
-1.63625 0.7576569611309598
-1.636875 0.7556358102338967
-1.6375 0.7488905539838032
-1.638125 0.7462764708567577
-1.63875 0.7430243351727185
-1.639375 0.7372020354551743
-1.64 0.7344391382078992
-1.640625 0.7321090133586278
-1.64125 0.7309638294327048
-1.641875 0.7234468409132876
-1.6425 0.7166051421366662
-1.643125 0.7122606096253284
-1.64375 0.7033081458187503
-1.644375 0.7072731630853591
-1.645 0.7054833219316234
-1.645625 0.7013472534585001
-1.64625 0.6907908173820141
-1.646875 0.6920085548001205
-1.6475 0.6883679664267186
-1.648125 0.680757796825541
-1.64875 0.6756067660721162
-1.649375 0.6678129622901662
-1.65 0.666814482371147
-1.650625 0.6592620763739343
-1.65125 0.6501755675233574
-1.651875 0.6505223433088066
-1.6525 0.6441119243687311
-1.653125 0.6378539069253303
-1.65375 0.6294909134321663
-1.654375 0.6243946135266611
-1.655 0.6187980119212253
-1.655625 0.6118568660098029
-1.65625 0.6032104018688534
-1.656875 0.6056072290516877
-1.6575 0.5954479407194917
-1.658125 0.5928415408523876
-1.65875 0.5880842722697778
-1.659375 0.5767415297927919
-1.66 0.576409827311768
-1.660625 0.5778111367197778
-1.66125 0.5764964005225365
-1.661875 0.5713234351472323
-1.6625 0.5678434238234444
-1.663125 0.5656716947754602
-1.66375 0.5606428652040122
-1.664375 0.5556324460338862
-1.665 0.5495305568886142
-1.665625 0.5484357343154792
-1.66625 0.5399128271820218
-1.666875 0.5301569676575514
-1.6675 0.5197768030673429
-1.668125 0.5137970766913954
-1.66875 0.5058935896284878
-1.669375 0.5004396880831841
-1.67 0.49029714156383253
-1.670625 0.49303142175017894
-1.67125 0.4819594811307558
-1.671875 0.47903264456883343
-1.6725 0.4744638160440362
-1.673125 0.4631813036486083
-1.67375 0.45920565953303505
-1.674375 0.4586677002756647
-1.675 0.44940693716978525
-1.675625 0.43987479801525864
-1.67625 0.44197493128447773
-1.676875 0.4385082917171298
-1.6775 0.44123384992366516
-1.678125 0.43214314686740013
-1.67875 0.42034978377201027
-1.679375 0.4068637873299916
-1.68 0.39881524975451665
-1.680625 0.38787499891462374
-1.68125 0.3759613533429448
-1.681875 0.3758158322825967
-1.6825 0.3703409843326474
-1.683125 0.360188821015005
-1.68375 0.3507241903697757
-1.684375 0.35038271010799815
-1.685 0.3424592396507461
-1.685625 0.3346814724414026
-1.68625 0.3243387809160337
-1.686875 0.31347489719907123
-1.6875 0.3117254176035623
-1.688125 0.29468429966312626
-1.68875 0.2892871199921855
-1.689375 0.28388324261384557
-1.69 0.27498752201263793
-1.690625 0.2690544970845826
-1.69125 0.2629454720896338
-1.691875 0.2586682189314847
-1.6925 0.2554714159934698
-1.693125 0.237667131238221
-1.69375 0.2339300202164262
-1.694375 0.22914427141770558
-1.695 0.22180820834010226
-1.695625 0.21102894211077186
-1.69625 0.20562215868697642
-1.696875 0.20484823658384937
-1.6975 0.193208444056857
-1.698125 0.19122503263915502
-1.69875 0.18368092858903326
-1.699375 0.17511211063303966
-1.7 0.16638992306959968
-1.700625 0.16757387764479598
-1.70125 0.1548506306804625
-1.701875 0.14569704266047373
-1.7025 0.14227634054625404
-1.703125 0.13162357258521
-1.70375 0.11508842138199289
-1.704375 0.12037688094924684
-1.705 0.11907282407512856
-1.705625 0.09855706375976468
-1.70625 0.09813035828521027
-1.706875 0.0900542227237178
-1.7075 0.09062333498672936
-1.708125 0.07783407680934105
-1.70875 0.07078225383295433
-1.709375 0.07519636038061298
-1.71 0.0615465923294864
-1.710625 0.06214207858955458
-1.71125 0.05735138559350483
-1.711875 0.05177530717143616
-1.7125 0.03913437556144436
-1.713125 0.032017412635612426
-1.71375 0.029443494498166637
-1.714375 0.024760020677798183
-1.715 0.01911073731403131
-1.715625 0.014255463644216964
-1.71625 0.01206511362218715
-1.716875 -6.974904962509215e-05
-1.7175 -0.0019537815416049206
-1.718125 -0.004981547250723068
-1.71875 -0.009746718322831848
-1.719375 -0.021413825155259993
-1.72 -0.027659093819635678
-1.720625 -0.030768712100409108
-1.72125 -0.02945170917295053
-1.721875 -0.041380100233703435
-1.7225 -0.04824259866698936
-1.723125 -0.05860907265504752
-1.72375 -0.051369007942734544
-1.724375 -0.06510738393712125
-1.725 -0.06371806252220265
-1.725625 -0.07029941929723754
-1.72625 -0.0791684485588571
-1.726875 -0.07279470631015082
-1.7275 -0.07533796411344673
-1.728125 -0.08355104161756398
-1.72875 -0.08820294604393397
-1.729375 -0.10092346255137467
-1.73 -0.1087734459170392
-1.730625 -0.10580905956841619
-1.73125 -0.11341606695417188
-1.731875 -0.11481312343860056
-1.7325 -0.11978508095283008
-1.733125 -0.1279001312973377
-1.73375 -0.12797813782399733
-1.734375 -0.13307765247914902
-1.735 -0.13412517676017116
-1.735625 -0.14037131453720095
-1.73625 -0.142917218725674
-1.736875 -0.14485254827095956
-1.7375 -0.14786633804704694
-1.738125 -0.153410338699673
-1.73875 -0.154771360752734
-1.739375 -0.16023615013255338
-1.74 -0.16087297009446397
-1.740625 -0.16679857806100581
-1.74125 -0.1699459698577816
-1.741875 -0.17148712307033703
-1.7425 -0.17330491643428425
-1.743125 -0.18631122862716398
-1.74375 -0.18373594718311329
-1.744375 -0.1742494536584343
-1.745 -0.17277333422707808
-1.745625 -0.18025676882627736
-1.74625 -0.17848620077954752
-1.746875 -0.1817363874056732
-1.7475 -0.1877498071857174
-1.748125 -0.18438993590367192
-1.74875 -0.1855613813505392
-1.749375 -0.18838157399767042
-1.75 -0.18265738424241573
-1.750625 -0.1826453380002812
-1.75125 -0.18131471486695203
-1.751875 -0.1775147748353896
-1.7525 -0.18566170469666202
-1.753125 -0.1869869521091457
-1.75375 -0.18796716688591328
-1.754375 -0.19337038627903738
-1.755 -0.18306464292133875
-1.755625 -0.184485314763828
-1.75625 -0.18302786027582418
-1.756875 -0.18802408541285132
-1.7575 -0.18899821266915176
-1.758125 -0.1877077898786177
-1.75875 -0.18745832319860864
-1.759375 -0.18418264532429826
-1.76 -0.18340689793298873
-1.760625 -0.18345599481340902
-1.76125 -0.18572979802719236
-1.761875 -0.1912805270327339
-1.7625 -0.18737734015685184
-1.763125 -0.18641247558487675
-1.76375 -0.1821448151601475
-1.764375 -0.18466548612067293
-1.765 -0.19165437723010537
-1.765625 -0.18897293047148714
-1.76625 -0.1852055110483019
-1.766875 -0.18763677231487869
-1.7675 -0.1849201498622042
-1.768125 -0.19420144977934234
-1.76875 -0.1892783372205804
-1.769375 -0.19179426851129913
-1.77 -0.1897439333128503
-1.770625 -0.18564458884049406
-1.77125 -0.18896519535345338
-1.771875 -0.18913243424064863
-1.7725 -0.1862980100388585
-1.773125 -0.18528331104810516
-1.77375 -0.18378341963647965
-1.774375 -0.1818957311701964
-1.775 -0.18196958708125224
-1.775625 -0.1751667923052867
-1.77625 -0.17645348776516717
-1.776875 -0.17149048565323502
-1.7775 -0.1656436209404407
-1.778125 -0.16560988103117316
-1.77875 -0.16910651649215633
-1.779375 -0.16323149554197902
-1.78 -0.16119534251539375
-1.780625 -0.15838649339344027
-1.78125 -0.15010288907400446
-1.781875 -0.15406887706884712
-1.7825 -0.15160751925827123
-1.783125 -0.15106550229047716
-1.78375 -0.15052256984585025
-1.784375 -0.1491406676196128
-1.785 -0.15598362606561472
-1.785625 -0.1487944288241558
-1.78625 -0.14875843013665202
-1.786875 -0.14461525644518972
-1.7875 -0.13979782740896834
-1.788125 -0.14294620807963623
-1.78875 -0.14202124142185638
-1.789375 -0.141976081860198
-1.79 -0.13502949619182186
-1.790625 -0.1342961316841304
-1.79125 -0.13114079663883563
-1.791875 -0.13121606755196918
-1.7925 -0.1294273981804198
-1.793125 -0.12953197518482254
-1.79375 -0.12271301595671708
-1.794375 -0.11770519275185376
-1.795 -0.12154496147953636
-1.795625 -0.11598608905691349
-1.79625 -0.11490498971418353
-1.796875 -0.11652630104455827
-1.7975 -0.11541503244829629
-1.798125 -0.11319053978312278
-1.79875 -0.10985935779951586
-1.799375 -0.1087125433884426
-1.8 -0.11190375324613396
-1.800625 -0.11068326811081101
-1.80125 -0.1082678175417131
-1.801875 -0.10365566626935675
-1.8025 -0.10034400624057326
-1.803125 -0.09983607963166807
-1.80375 -0.09822537073812306
-1.804375 -0.09612693776889564
-1.805 -0.09557241319179022
-1.805625 -0.09252854804712646
-1.80625 -0.09036413763364248
-1.806875 -0.08533140923427542
-1.8075 -0.08746379032512819
-1.808125 -0.08466965255154907
-1.80875 -0.08244775558619068
-1.809375 -0.07966758792319864
-1.81 -0.07634640409356074
-1.810625 -0.0715759694401153
-1.81125 -0.07062989833701205
-1.811875 -0.0696581808533253
-1.8125 -0.07207496518447754
-1.813125 -0.07087444813655598
-1.81375 -0.0711252776713973
-1.814375 -0.06958650344395229
-1.815 -0.06695135373310132
-1.815625 -0.065405654198219
-1.81625 -0.06078847711387086
-1.816875 -0.058749852460288306
-1.8175 -0.05950086343617927
-1.818125 -0.05776513637869368
-1.81875 -0.05545163780744824
-1.819375 -0.05348464862678019
-1.82 -0.0528658983113002
-1.820625 -0.05259554382582313
-1.82125 -0.05269467146033786
-1.821875 -0.05130714077079017
-1.8225 -0.05029947163236375
-1.823125 -0.04825073555205112
-1.82375 -0.04742314780974334
-1.824375 -0.04561423438446245
-1.825 -0.045077313034408914
-1.825625 -0.04344774355587901
-1.82625 -0.04340536980105812
-1.826875 -0.039711072964366066
-1.8275 -0.03877383331050457
-1.828125 -0.0353315350382313
-1.82875 -0.03532795322613687
-1.829375 -0.034635265251716486
-1.83 -0.03554812693380314
-1.830625 -0.0312528842597337
-1.83125 -0.030039631625012556
-1.831875 -0.030155894171163936
-1.8325 -0.029854251203561652
-1.833125 -0.02846507610985511
-1.83375 -0.029120330824695215
-1.834375 -0.027240967536731348
-1.835 -0.026881462109478976
-1.835625 -0.026795430798572276
-1.83625 -0.026392450609157177
-1.836875 -0.025246836782860882
-1.8375 -0.02408818989914732
-1.838125 -0.023340473561295406
-1.83875 -0.0222978478162946
-1.839375 -0.020507128529975317
-1.84 -0.02112824572798452
-1.840625 -0.019485680181832242
-1.84125 -0.0190536259742564
-1.841875 -0.019020103662288367
-1.8425 -0.018663122347276972
-1.843125 -0.0178555551455038
-1.84375 -0.01835613635554375
-1.844375 -0.017298315416139184
-1.845 -0.0161871178586853
-1.845625 -0.015111940540868446
-1.84625 -0.015568148481180969
-1.846875 -0.014755343086491918
-1.8475 -0.01276318695997203
-1.848125 -0.011923825487348985
-1.84875 -0.011575154074474882
-1.849375 -0.011494763805534599
-1.85 -0.011277609014005333
-1.850625 -0.010020485522299694
-1.85125 -0.009671438721718204
-1.851875 -0.009369385105066236
-1.8525 -0.009052792462899946
-1.853125 -0.008488329502902297
-1.85375 -0.008947090294011048
-1.854375 -0.00824518954590287
-1.855 -0.00754169433683897
-1.855625 -0.008291250556116294
-1.85625 -0.007279387554592726
-1.856875 -0.00649959056248331
-1.8575 -0.006527968772705999
-1.858125 -0.0060668769763918004
-1.85875 -0.005714557627274616
-1.859375 -0.0057998794040895925
-1.86 -0.005454594513840647
-1.860625 -0.004851838071099155
-1.86125 -0.004941513503634544
-1.861875 -0.0046081069886272814
-1.8625 -0.0045432612748656405
-1.863125 -0.004284177306962363
-1.86375 -0.004498310280569725
-1.864375 -0.003660703522310033
-1.865 -0.0040351527984662326
-1.865625 -0.00398159306299162
-1.86625 -0.003882235208856982
-1.866875 -0.0035054268159073745
-1.8675 -0.0033384242961242054
-1.868125 -0.003114872448502929
-1.86875 -0.0032154872559573716
-1.869375 -0.0026451326892379403
-1.87 -0.0026023119649285346
-1.870625 -0.002436688310389707
-1.87125 -0.002395816852535434
-1.871875 -0.0020569932738182055
-1.8725 -0.001913344902608322
-1.873125 -0.0017897049197649537
-1.87375 -0.0017678020741353447
-1.874375 -0.0015441901785049107
-1.875 -0.0017413330381527898


==> Plots/wrapping.tex <==
e w
0.0 0.0
-0.000625 0.0
-0.00125 0.0
-0.001875 0.0
-0.0025 0.0
-0.003125 0.0
-0.00375 0.0
-0.004375 0.0
-0.005 0.0
-0.005625 0.0
-0.00625 0.0
-0.006875 0.0
-0.0075 0.0
-0.008125 0.0
-0.00875 0.0
-0.009375 0.0
-0.01 0.0
-0.010625 0.0
-0.01125 0.0
-0.011875 0.0
-0.0125 0.0
-0.013125 0.0
-0.01375 0.0
-0.014375 0.0
-0.015 0.0
-0.015625 0.0
-0.01625 0.0
-0.016875 0.0
-0.0175 0.0
-0.018125 0.0
-0.01875 0.0
-0.019375 0.0
-0.02 0.0
-0.020625 0.0
-0.02125 0.0
-0.021875 0.0
-0.0225 0.0
-0.023125 0.0
-0.02375 0.0
-0.024375 0.0
-0.025 0.0
-0.025625 0.0
-0.02625 0.0
-0.026875 0.0
-0.0275 0.0
-0.028125 0.0
-0.02875 0.0
-0.029375 0.0
-0.03 0.0
-0.030625 0.0
-0.03125 0.0
-0.031875 0.0
-0.0325 0.0
-0.033125 0.0
-0.03375 0.0
-0.034375 0.0
-0.035 0.0
-0.035625 0.0
-0.03625 0.0
-0.036875 0.0
-0.0375 0.0
-0.038125 0.0
-0.03875 0.0
-0.039375 0.0
-0.04 0.0
-0.040625 0.0
-0.04125 0.0
-0.041875 0.0
-0.0425 0.0
-0.043125 0.0
-0.04375 0.0
-0.044375 0.0
-0.045 0.0
-0.045625 0.0
-0.04625 0.0
-0.046875 0.0
-0.0475 0.0
-0.048125 0.0
-0.04875 0.0
-0.049375 0.0
-0.05 0.0
-0.050625 0.0
-0.05125 0.0
-0.051875 0.0
-0.0525 0.0
-0.053125 0.0
-0.05375 0.0
-0.054375 0.0
-0.055 0.0
-0.055625 0.0
-0.05625 0.0
-0.056875 0.0
-0.0575 0.0
-0.058125 0.0
-0.05875 0.0
-0.059375 0.0
-0.06 0.0
-0.060625 0.0
-0.06125 0.0
-0.061875 0.0
-0.0625 0.0
-0.063125 0.0
-0.06375 0.0
-0.064375 0.0
-0.065 0.0
-0.065625 0.0
-0.06625 0.0
-0.066875 0.0
-0.0675 0.0
-0.068125 0.0
-0.06875 0.0
-0.069375 0.0
-0.07 0.0
-0.070625 0.0
-0.07125 0.0
-0.071875 0.0
-0.0725 0.0
-0.073125 0.0
-0.07375 0.0
-0.074375 0.0
-0.075 0.0
-0.075625 0.0
-0.07625 0.0
-0.076875 0.0
-0.0775 0.0
-0.078125 0.0
-0.07875 0.0
-0.079375 0.0
-0.08 0.0
-0.080625 0.0
-0.08125 0.0
-0.081875 0.0
-0.0825 0.0
-0.083125 0.0
-0.08375 0.0
-0.084375 0.0
-0.085 0.0
-0.085625 0.0
-0.08625 0.0
-0.086875 0.0
-0.0875 0.0
-0.088125 0.0
-0.08875 0.0
-0.089375 0.0
-0.09 0.0
-0.090625 0.0
-0.09125 0.0
-0.091875 0.0
-0.0925 0.0
-0.093125 0.0
-0.09375 0.0
-0.094375 0.0
-0.095 0.0
-0.095625 0.0
-0.09625 0.0
-0.096875 0.0
-0.0975 0.0
-0.098125 0.0
-0.09875 0.0
-0.099375 0.0
-0.1 0.0
-0.100625 0.0
-0.10125 0.0
-0.101875 0.0
-0.1025 0.0
-0.103125 0.0
-0.10375 0.0
-0.104375 0.0
-0.105 0.0
-0.105625 0.0
-0.10625 0.0
-0.106875 0.0
-0.1075 0.0
-0.108125 0.0
-0.10875 0.0
-0.109375 0.0
-0.11 0.0
-0.110625 0.0
-0.11125 0.0
-0.111875 0.0
-0.1125 0.0
-0.113125 0.0
-0.11375 0.0
-0.114375 0.0
-0.115 0.0
-0.115625 0.0
-0.11625 0.0
-0.116875 0.0
-0.1175 0.0
-0.118125 0.0
-0.11875 0.0
-0.119375 0.0
-0.12 0.0
-0.120625 0.0
-0.12125 0.0
-0.121875 0.0
-0.1225 0.0
-0.123125 0.0
-0.12375 0.0
-0.124375 0.0
-0.125 0.0
-0.125625 0.0
-0.12625 0.0
-0.126875 0.0
-0.1275 0.0
-0.128125 0.0
-0.12875 0.0
-0.129375 0.0
-0.13 0.0
-0.130625 0.0
-0.13125 0.0
-0.131875 0.0
-0.1325 0.0
-0.133125 0.0
-0.13375 0.0
-0.134375 0.0
-0.135 0.0
-0.135625 0.0
-0.13625 0.0
-0.136875 0.0
-0.1375 0.0
-0.138125 0.0
-0.13875 0.0
-0.139375 0.0
-0.14 0.0
-0.140625 0.0
-0.14125 0.0
-0.141875 0.0
-0.1425 0.0
-0.143125 0.0
-0.14375 0.0
-0.144375 0.0
-0.145 0.0
-0.145625 0.0
-0.14625 0.0
-0.146875 0.0
-0.1475 0.0
-0.148125 0.0
-0.14875 0.0
-0.149375 0.0
-0.15 0.0
-0.150625 0.0
-0.15125 0.0
-0.151875 0.0
-0.1525 0.0
-0.153125 0.0
-0.15375 0.0
-0.154375 0.0
-0.155 0.0
-0.155625 0.0
-0.15625 0.0
-0.156875 0.0
-0.1575 0.0
-0.158125 0.0
-0.15875 0.0
-0.159375 0.0
-0.16 0.0
-0.160625 0.0
-0.16125 0.0
-0.161875 0.0
-0.1625 0.0
-0.163125 0.0
-0.16375 0.0
-0.164375 0.0
-0.165 0.0
-0.165625 0.0
-0.16625 0.0
-0.166875 0.0
-0.1675 0.0
-0.168125 0.0
-0.16875 0.0
-0.169375 0.0
-0.17 0.0
-0.170625 0.0
-0.17125 0.0
-0.171875 0.0
-0.1725 0.0
-0.173125 0.0
-0.17375 0.0
-0.174375 0.0
-0.175 0.0
-0.175625 0.0
-0.17625 0.0
-0.176875 0.0
-0.1775 0.0
-0.178125 0.0
-0.17875 0.0
-0.179375 0.0
-0.18 0.0
-0.180625 0.0
-0.18125 0.0
-0.181875 0.0
-0.1825 0.0
-0.183125 0.0
-0.18375 0.0
-0.184375 0.0
-0.185 0.0
-0.185625 0.0
-0.18625 0.0
-0.186875 0.0
-0.1875 0.0
-0.188125 0.0
-0.18875 0.0
-0.189375 0.0
-0.19 0.0
-0.190625 0.0
-0.19125 0.0
-0.191875 0.0
-0.1925 0.0
-0.193125 0.0
-0.19375 0.0
-0.194375 0.0
-0.195 0.0
-0.195625 0.0
-0.19625 0.0
-0.196875 0.0
-0.1975 0.0
-0.198125 0.0
-0.19875 0.0
-0.199375 0.0
-0.2 0.0
-0.200625 0.0
-0.20125 0.0
-0.201875 0.0
-0.2025 0.0
-0.203125 0.0
-0.20375 0.0
-0.204375 0.0
-0.205 0.0
-0.205625 0.0
-0.20625 0.0
-0.206875 0.0
-0.2075 0.0
-0.208125 0.0
-0.20875 0.0
-0.209375 0.0
-0.21 0.0
-0.210625 0.0
-0.21125 0.0
-0.211875 0.0
-0.2125 0.0
-0.213125 0.0
-0.21375 0.0
-0.214375 0.0
-0.215 0.0
-0.215625 0.0
-0.21625 0.0
-0.216875 0.0
-0.2175 0.0
-0.218125 0.0
-0.21875 0.0
-0.219375 0.0
-0.22 0.0
-0.220625 0.0
-0.22125 0.0
-0.221875 0.0
-0.2225 0.0
-0.223125 0.0
-0.22375 0.0
-0.224375 0.0
-0.225 0.0
-0.225625 0.0
-0.22625 0.0
-0.226875 0.0
-0.2275 0.0
-0.228125 0.0
-0.22875 0.0
-0.229375 0.0
-0.23 0.0
-0.230625 0.0
-0.23125 0.0
-0.231875 0.0
-0.2325 0.0
-0.233125 0.0
-0.23375 0.0
-0.234375 0.0
-0.235 0.0
-0.235625 0.0
-0.23625 0.0
-0.236875 0.0
-0.2375 0.0
-0.238125 0.0
-0.23875 0.0
-0.239375 0.0
-0.24 0.0
-0.240625 0.0
-0.24125 0.0
-0.241875 0.0
-0.2425 0.0
-0.243125 0.0
-0.24375 0.0
-0.244375 0.0
-0.245 0.0
-0.245625 0.0
-0.24625 0.0
-0.246875 0.0
-0.2475 0.0
-0.248125 0.0
-0.24875 0.0
-0.249375 0.0
-0.25 0.0
-0.250625 0.0
-0.25125 0.0
-0.251875 0.0
-0.2525 0.0
-0.253125 0.0
-0.25375 0.0
-0.254375 0.0
-0.255 0.0
-0.255625 0.0
-0.25625 0.0
-0.256875 0.0
-0.2575 0.0
-0.258125 0.0
-0.25875 0.0
-0.259375 0.0
-0.26 0.0
-0.260625 0.0
-0.26125 0.0
-0.261875 0.0
-0.2625 0.0
-0.263125 0.0
-0.26375 0.0
-0.264375 0.0
-0.265 0.0
-0.265625 0.0
-0.26625 0.0
-0.266875 0.0
-0.2675 0.0
-0.268125 0.0
-0.26875 0.0
-0.269375 0.0
-0.27 0.0
-0.270625 0.0
-0.27125 0.0
-0.271875 0.0
-0.2725 0.0
-0.273125 0.0
-0.27375 0.0
-0.274375 0.0
-0.275 0.0
-0.275625 0.0
-0.27625 0.0
-0.276875 0.0
-0.2775 0.0
-0.278125 0.0
-0.27875 0.0
-0.279375 0.0
-0.28 0.0
-0.280625 0.0
-0.28125 0.0
-0.281875 0.0
-0.2825 0.0
-0.283125 0.0
-0.28375 0.0
-0.284375 0.0
-0.285 0.0
-0.285625 0.0
-0.28625 0.0
-0.286875 0.0
-0.2875 0.0
-0.288125 0.0
-0.28875 0.0
-0.289375 0.0
-0.29 0.0
-0.290625 0.0
-0.29125 0.0
-0.291875 0.0
-0.2925 0.0
-0.293125 0.0
-0.29375 0.0
-0.294375 0.0
-0.295 0.0
-0.295625 0.0
-0.29625 0.0
-0.296875 0.0
-0.2975 0.0
-0.298125 0.0
-0.29875 0.0
-0.299375 0.0
-0.3 0.0
-0.300625 0.0
-0.30125 0.0
-0.301875 0.0
-0.3025 0.0
-0.303125 0.0
-0.30375 0.0
-0.304375 0.0
-0.305 0.0
-0.305625 0.0
-0.30625 0.0
-0.306875 0.0
-0.3075 0.0
-0.308125 0.0
-0.30875 0.0
-0.309375 0.0
-0.31 0.0
-0.310625 0.0
-0.31125 0.0
-0.311875 0.0
-0.3125 0.0
-0.313125 0.0
-0.31375 0.0
-0.314375 0.0
-0.315 0.0
-0.315625 0.0
-0.31625 0.0
-0.316875 0.0
-0.3175 0.0
-0.318125 0.0
-0.31875 0.0
-0.319375 0.0
-0.32 0.0
-0.320625 0.0
-0.32125 0.0
-0.321875 0.0
-0.3225 0.0
-0.323125 0.0
-0.32375 0.0
-0.324375 0.0
-0.325 0.0
-0.325625 0.0
-0.32625 0.0
-0.326875 0.0
-0.3275 0.0
-0.328125 0.0
-0.32875 0.0
-0.329375 0.0
-0.33 0.0
-0.330625 0.0
-0.33125 0.0
-0.331875 0.0
-0.3325 0.0
-0.333125 0.0
-0.33375 0.0
-0.334375 0.0
-0.335 0.0
-0.335625 0.0
-0.33625 0.0
-0.336875 0.0
-0.3375 0.0
-0.338125 0.0
-0.33875 0.0
-0.339375 0.0
-0.34 0.0
-0.340625 0.0
-0.34125 0.0
-0.341875 0.0
-0.3425 0.0
-0.343125 0.0
-0.34375 0.0
-0.344375 0.0
-0.345 0.0
-0.345625 0.0
-0.34625 0.0
-0.346875 0.0
-0.3475 0.0
-0.348125 0.0
-0.34875 0.0
-0.349375 0.0
-0.35 0.0
-0.350625 0.0
-0.35125 0.0
-0.351875 0.0
-0.3525 0.0
-0.353125 0.0
-0.35375 0.0
-0.354375 0.0
-0.355 0.0
-0.355625 0.0
-0.35625 0.0
-0.356875 0.0
-0.3575 0.0
-0.358125 0.0
-0.35875 0.0
-0.359375 0.0
-0.36 0.0
-0.360625 0.0
-0.36125 0.0
-0.361875 0.0
-0.3625 0.0
-0.363125 0.0
-0.36375 0.0
-0.364375 0.0
-0.365 0.0
-0.365625 0.0
-0.36625 0.0
-0.366875 0.0
-0.3675 0.0
-0.368125 0.0
-0.36875 0.0
-0.369375 0.0
-0.37 0.0
-0.370625 0.0
-0.37125 0.0
-0.371875 0.0
-0.3725 0.0
-0.373125 0.0
-0.37375 0.0
-0.374375 0.0
-0.375 0.0
-0.375625 0.0
-0.37625 0.0
-0.376875 0.0
-0.3775 0.0
-0.378125 0.0
-0.37875 0.0
-0.379375 0.0
-0.38 0.0
-0.380625 0.0
-0.38125 0.0
-0.381875 0.0
-0.3825 0.0
-0.383125 0.0
-0.38375 0.0
-0.384375 0.0
-0.385 0.0
-0.385625 0.0
-0.38625 0.0
-0.386875 0.0
-0.3875 0.0
-0.388125 0.0
-0.38875 0.0
-0.389375 0.0
-0.39 0.0
-0.390625 0.0
-0.39125 0.0
-0.391875 0.0
-0.3925 0.0
-0.393125 0.0
-0.39375 0.0
-0.394375 0.0
-0.395 0.0
-0.395625 0.0
-0.39625 0.0
-0.396875 0.0
-0.3975 0.0
-0.398125 0.0
-0.39875 0.0
-0.399375 0.0
-0.4 0.0
-0.400625 0.0
-0.40125 0.0
-0.401875 0.0
-0.4025 0.0
-0.403125 0.0
-0.40375 0.0
-0.404375 0.0
-0.405 0.0
-0.405625 0.0
-0.40625 0.0
-0.406875 0.0
-0.4075 0.0
-0.408125 0.0
-0.40875 0.0
-0.409375 0.0
-0.41 0.0
-0.410625 0.0
-0.41125 0.0
-0.411875 0.0
-0.4125 0.0
-0.413125 0.0
-0.41375 0.0
-0.414375 0.0
-0.415 0.0
-0.415625 0.0
-0.41625 0.0
-0.416875 0.0
-0.4175 0.0
-0.418125 0.0
-0.41875 0.0
-0.419375 0.0
-0.42 0.0
-0.420625 0.0
-0.42125 0.0
-0.421875 0.0
-0.4225 0.0
-0.423125 0.0
-0.42375 0.0
-0.424375 0.0
-0.425 0.0
-0.425625 0.0
-0.42625 0.0
-0.426875 0.0
-0.4275 0.0
-0.428125 0.0
-0.42875 0.0
-0.429375 0.0
-0.43 0.0
-0.430625 0.0
-0.43125 0.0
-0.431875 0.0
-0.4325 0.0
-0.433125 0.0
-0.43375 0.0
-0.434375 0.0
-0.435 0.0
-0.435625 0.0
-0.43625 0.0
-0.436875 0.0
-0.4375 0.0
-0.438125 0.0
-0.43875 0.0
-0.439375 0.0
-0.44 0.0
-0.440625 0.0
-0.44125 0.0
-0.441875 0.0
-0.4425 0.0
-0.443125 0.0
-0.44375 0.0
-0.444375 0.0
-0.445 0.0
-0.445625 0.0
-0.44625 0.0
-0.446875 0.0
-0.4475 0.0
-0.448125 0.0
-0.44875 0.0
-0.449375 0.0
-0.45 0.0
-0.450625 0.0
-0.45125 0.0
-0.451875 0.0
-0.4525 0.0
-0.453125 0.0
-0.45375 0.0
-0.454375 0.0
-0.455 0.0
-0.455625 0.0
-0.45625 0.0
-0.456875 0.0
-0.4575 0.0
-0.458125 0.0
-0.45875 0.0
-0.459375 0.0
-0.46 0.0
-0.460625 0.0
-0.46125 0.0
-0.461875 0.0
-0.4625 0.0
-0.463125 0.0
-0.46375 0.0
-0.464375 0.0
-0.465 0.0
-0.465625 0.0
-0.46625 0.0
-0.466875 0.0
-0.4675 0.0
-0.468125 0.0
-0.46875 0.0
-0.469375 0.0
-0.47 0.0
-0.470625 0.0
-0.47125 0.0
-0.471875 0.0
-0.4725 0.0
-0.473125 0.0
-0.47375 0.0
-0.474375 0.0
-0.475 0.0
-0.475625 0.0
-0.47625 0.0
-0.476875 0.0
-0.4775 0.0
-0.478125 0.0
-0.47875 0.0
-0.479375 0.0
-0.48 0.0
-0.480625 0.0
-0.48125 0.0
-0.481875 0.0
-0.4825 0.0
-0.483125 0.0
-0.48375 0.0
-0.484375 0.0
-0.485 0.0
-0.485625 0.0
-0.48625 0.0
-0.486875 0.0
-0.4875 0.0
-0.488125 0.0
-0.48875 0.0
-0.489375 0.0
-0.49 0.0
-0.490625 0.0
-0.49125 0.0
-0.491875 0.0
-0.4925 0.0
-0.493125 0.0
-0.49375 0.0
-0.494375 0.0
-0.495 0.0
-0.495625 0.0
-0.49625 0.0
-0.496875 0.0
-0.4975 0.0
-0.498125 0.0
-0.49875 0.0
-0.499375 0.0
-0.5 0.0
-0.500625 0.0
-0.50125 0.0
-0.501875 0.0
-0.5025 0.0
-0.503125 0.0
-0.50375 0.0
-0.504375 0.0
-0.505 0.0
-0.505625 0.0
-0.50625 0.0
-0.506875 0.0
-0.5075 0.0
-0.508125 0.0
-0.50875 0.0
-0.509375 0.0
-0.51 0.0
-0.510625 0.0
-0.51125 0.0
-0.511875 0.0
-0.5125 0.0
-0.513125 0.0
-0.51375 0.0
-0.514375 0.0
-0.515 0.0
-0.515625 0.0
-0.51625 0.0
-0.516875 0.0
-0.5175 0.0
-0.518125 0.0
-0.51875 0.0
-0.519375 0.0
-0.52 0.0
-0.520625 0.0
-0.52125 0.0
-0.521875 0.0
-0.5225 0.0
-0.523125 0.0
-0.52375 0.0
-0.524375 0.0
-0.525 0.0
-0.525625 0.0
-0.52625 0.0
-0.526875 0.0
-0.5275 0.0
-0.528125 0.0
-0.52875 0.0
-0.529375 0.0
-0.53 0.0
-0.530625 0.0
-0.53125 0.0
-0.531875 0.0
-0.5325 0.0
-0.533125 0.0
-0.53375 0.0
-0.534375 0.0
-0.535 0.0
-0.535625 0.0
-0.53625 0.0
-0.536875 0.0
-0.5375 0.0
-0.538125 0.0
-0.53875 0.0
-0.539375 0.0
-0.54 0.0
-0.540625 0.0
-0.54125 0.0
-0.541875 0.0
-0.5425 0.0
-0.543125 0.0
-0.54375 0.0
-0.544375 0.0
-0.545 0.0
-0.545625 0.0
-0.54625 0.0
-0.546875 0.0
-0.5475 0.0
-0.548125 0.0
-0.54875 0.0
-0.549375 0.0
-0.55 0.0
-0.550625 0.0
-0.55125 0.0
-0.551875 0.0
-0.5525 0.0
-0.553125 0.0
-0.55375 0.0
-0.554375 0.0
-0.555 0.0
-0.555625 0.0
-0.55625 0.0
-0.556875 0.0
-0.5575 0.0
-0.558125 0.0
-0.55875 0.0
-0.559375 0.0
-0.56 0.0
-0.560625 0.0
-0.56125 0.0
-0.561875 0.0
-0.5625 0.0
-0.563125 0.0
-0.56375 0.0
-0.564375 0.0
-0.565 0.0
-0.565625 0.0
-0.56625 0.0
-0.566875 0.0
-0.5675 0.0
-0.568125 0.0
-0.56875 0.0
-0.569375 0.0
-0.57 0.0
-0.570625 0.0
-0.57125 0.0
-0.571875 0.0
-0.5725 0.0
-0.573125 0.0
-0.57375 0.0
-0.574375 0.0
-0.575 0.0
-0.575625 0.0
-0.57625 0.0
-0.576875 0.0
-0.5775 0.0
-0.578125 0.0
-0.57875 0.0
-0.579375 0.0
-0.58 0.0
-0.580625 0.0
-0.58125 0.0
-0.581875 0.0
-0.5825 0.0
-0.583125 0.0
-0.58375 0.0
-0.584375 0.0
-0.585 0.0
-0.585625 0.0
-0.58625 0.0
-0.586875 0.0
-0.5875 0.0
-0.588125 0.0
-0.58875 0.0
-0.589375 0.0
-0.59 0.0
-0.590625 0.0
-0.59125 0.0
-0.591875 0.0
-0.5925 0.0
-0.593125 0.0
-0.59375 0.0
-0.594375 0.0
-0.595 0.0
-0.595625 0.0
-0.59625 0.0
-0.596875 0.0
-0.5975 0.0
-0.598125 0.0
-0.59875 0.0
-0.599375 0.0
-0.6 0.0
-0.600625 0.0
-0.60125 0.0
-0.601875 0.0
-0.6025 0.0
-0.603125 0.0
-0.60375 0.0
-0.604375 0.0
-0.605 0.0
-0.605625 0.0
-0.60625 0.0
-0.606875 0.0
-0.6075 0.0
-0.608125 0.0
-0.60875 0.0
-0.609375 0.0
-0.61 0.0
-0.610625 0.0
-0.61125 0.0
-0.611875 0.0
-0.6125 0.0
-0.613125 0.0
-0.61375 0.0
-0.614375 0.0
-0.615 0.0
-0.615625 0.0
-0.61625 0.0
-0.616875 0.0
-0.6175 0.0
-0.618125 0.0
-0.61875 0.0
-0.619375 0.0
-0.62 0.0
-0.620625 0.0
-0.62125 0.0
-0.621875 0.0
-0.6225 0.0
-0.623125 0.0
-0.62375 0.0
-0.624375 0.0
-0.625 0.0
-0.625625 0.0
-0.62625 0.0
-0.626875 0.0
-0.6275 0.0
-0.628125 0.0
-0.62875 0.0
-0.629375 0.0
-0.63 0.0
-0.630625 0.0
-0.63125 0.0
-0.631875 0.0
-0.6325 0.0
-0.633125 0.0
-0.63375 0.0
-0.634375 0.0
-0.635 0.0
-0.635625 0.0
-0.63625 0.0
-0.636875 0.0
-0.6375 0.0
-0.638125 0.0
-0.63875 0.0
-0.639375 0.0
-0.64 0.0
-0.640625 0.0
-0.64125 0.0
-0.641875 0.0
-0.6425 0.0
-0.643125 0.0
-0.64375 0.0
-0.644375 0.0
-0.645 0.0
-0.645625 0.0
-0.64625 0.0
-0.646875 0.0
-0.6475 0.0
-0.648125 0.0
-0.64875 0.0
-0.649375 0.0
-0.65 0.0
-0.650625 0.0
-0.65125 0.0
-0.651875 0.0
-0.6525 0.0
-0.653125 0.0
-0.65375 0.0
-0.654375 0.0
-0.655 0.0
-0.655625 0.0
-0.65625 0.0
-0.656875 0.0
-0.6575 0.0
-0.658125 0.0
-0.65875 0.0
-0.659375 0.0
-0.66 0.0
-0.660625 0.0
-0.66125 0.0
-0.661875 0.0
-0.6625 0.0
-0.663125 0.0
-0.66375 0.0
-0.664375 0.0
-0.665 0.0
-0.665625 0.0
-0.66625 0.0
-0.666875 0.0
-0.6675 0.0
-0.668125 0.0
-0.66875 0.0
-0.669375 0.0
-0.67 0.0
-0.670625 0.0
-0.67125 0.0
-0.671875 0.0
-0.6725 0.0
-0.673125 0.0
-0.67375 0.0
-0.674375 0.0
-0.675 0.0
-0.675625 0.0
-0.67625 0.0
-0.676875 0.0
-0.6775 0.0
-0.678125 0.0
-0.67875 0.0
-0.679375 0.0
-0.68 0.0
-0.680625 0.0
-0.68125 0.0
-0.681875 0.0
-0.6825 0.0
-0.683125 0.0
-0.68375 0.0
-0.684375 0.0
-0.685 0.0
-0.685625 0.0
-0.68625 0.0
-0.686875 0.0
-0.6875 0.0
-0.688125 0.0
-0.68875 0.0
-0.689375 0.0
-0.69 0.0
-0.690625 0.0
-0.69125 0.0
-0.691875 0.0
-0.6925 0.0
-0.693125 0.0
-0.69375 0.0
-0.694375 0.0
-0.695 0.0
-0.695625 0.0
-0.69625 0.0
-0.696875 0.0
-0.6975 0.0
-0.698125 0.0
-0.69875 0.0
-0.699375 0.0
-0.7 0.0
-0.700625 0.0
-0.70125 0.0
-0.701875 0.0
-0.7025 0.0
-0.703125 0.0
-0.70375 0.0
-0.704375 0.0
-0.705 0.0
-0.705625 0.0
-0.70625 0.0
-0.706875 0.0
-0.7075 0.0
-0.708125 0.0
-0.70875 0.0
-0.709375 0.0
-0.71 0.0
-0.710625 0.0
-0.71125 0.0
-0.711875 0.0
-0.7125 0.0
-0.713125 0.0
-0.71375 0.0
-0.714375 0.0
-0.715 0.0
-0.715625 0.0
-0.71625 0.0
-0.716875 0.0
-0.7175 3.90625e-05
-0.718125 0.0
-0.71875 3.90625e-05
-0.719375 0.0
-0.72 0.0
-0.720625 3.90625e-05
-0.72125 3.90625e-05
-0.721875 3.90625e-05
-0.7225 0.0
-0.723125 0.0
-0.72375 0.0
-0.724375 0.0
-0.725 0.0
-0.725625 0.0
-0.72625 0.0
-0.726875 0.0
-0.7275 0.0
-0.728125 0.0
-0.72875 0.0
-0.729375 0.0
-0.73 0.0
-0.730625 0.0
-0.73125 0.0
-0.731875 0.0
-0.7325 0.0
-0.733125 0.0
-0.73375 0.0
-0.734375 0.0
-0.735 0.0
-0.735625 0.0
-0.73625 0.0
-0.736875 0.0
-0.7375 0.0
-0.738125 0.0
-0.73875 0.0
-0.739375 0.0
-0.74 0.0
-0.740625 3.90625e-05
-0.74125 3.90625e-05
-0.741875 0.0
-0.7425 3.90625e-05
-0.743125 0.0
-0.74375 0.0
-0.744375 0.0
-0.745 3.90625e-05
-0.745625 0.0
-0.74625 0.0
-0.746875 0.0
-0.7475 0.0
-0.748125 0.0
-0.74875 0.0
-0.749375 0.0
-0.75 0.0
-0.750625 0.0
-0.75125 0.0
-0.751875 0.0
-0.7525 0.00011718750000000002
-0.753125 3.90625e-05
-0.75375 3.90625e-05
-0.754375 0.0
-0.755 0.0
-0.755625 0.0
-0.75625 0.0
-0.756875 3.90625e-05
-0.7575 0.0
-0.758125 3.90625e-05
-0.75875 0.0
-0.759375 0.0
-0.76 0.0
-0.760625 0.0
-0.76125 7.8125e-05
-0.761875 3.90625e-05
-0.7625 3.90625e-05
-0.763125 0.0
-0.76375 0.0
-0.764375 0.0
-0.765 3.90625e-05
-0.765625 3.90625e-05
-0.76625 3.90625e-05
-0.766875 3.90625e-05
-0.7675 0.0
-0.768125 0.0
-0.76875 3.90625e-05
-0.769375 0.0
-0.77 0.00011718750000000002
-0.770625 0.0
-0.77125 0.0
-0.771875 3.90625e-05
-0.7725 7.8125e-05
-0.773125 3.90625e-05
-0.77375 0.00011718750000000002
-0.774375 3.90625e-05
-0.775 0.00011718750000000002
-0.775625 7.8125e-05
-0.77625 0.00015625
-0.776875 0.00011718750000000002
-0.7775 0.00015625
-0.778125 7.8125e-05
-0.77875 0.00011718750000000002
-0.779375 0.00015625
-0.78 7.8125e-05
-0.780625 0.0
-0.78125 0.0001953125
-0.781875 0.0001953125
-0.7825 7.8125e-05
-0.783125 0.00015625
-0.78375 0.00011718750000000002
-0.784375 0.0
-0.785 3.90625e-05
-0.785625 0.00011718750000000002
-0.78625 0.000234375
-0.786875 0.00015625
-0.7875 0.0001953125
-0.788125 0.00042968749999999995
-0.78875 0.0001953125
-0.789375 3.90625e-05
-0.79 0.00023437500000000005
-0.790625 0.0001953125
-0.79125 0.000234375
-0.791875 0.00011718750000000002
-0.7925 0.00015625
-0.793125 0.00027343749999999997
-0.79375 0.00027343749999999997
-0.794375 0.0004687500000000001
-0.795 0.00042968749999999995
-0.795625 0.00027343749999999997
-0.79625 0.0001953125
-0.796875 0.00027343749999999997
-0.7975 0.00035156250000000004
-0.798125 0.00031249999999999995
-0.79875 0.000234375
-0.799375 0.00031249999999999995
-0.8 0.0003515625
-0.800625 0.000546875
-0.80125 0.000546875
-0.801875 0.000390625
-0.8025 0.000234375
-0.803125 0.00046875
-0.80375 0.0005468749999999999
-0.804375 0.0008984375000000003
-0.805 0.0006640625000000002
-0.805625 0.0005859375000000001
-0.80625 0.0005078125
-0.806875 0.0007031250000000001
-0.8075 0.0009765625000000004
-0.808125 0.000703125
-0.80875 0.0007812500000000002
-0.809375 0.0006640625000000002
-0.81 0.0007812500000000002
-0.810625 0.00078125
-0.81125 0.0007421875
-0.811875 0.0005859375000000001
-0.8125 0.0008984375000000001
-0.813125 0.0009765625000000004
-0.81375 0.0008593750000000002
-0.814375 0.0008984375000000003
-0.815 0.0009765625000000002
-0.815625 0.0008984375000000003
-0.81625 0.0012500000000000005
-0.816875 0.0012500000000000007
-0.8175 0.0011328125000000004
-0.818125 0.0016015625000000001
-0.81875 0.0015625000000000003
-0.819375 0.00109375
-0.82 0.0015234375000000003
-0.820625 0.0018359375000000001
-0.82125 0.0015625000000000007
-0.821875 0.0013281250000000007
-0.8225 0.0012500000000000007
-0.823125 0.0016406250000000002
-0.82375 0.0015625000000000003
-0.824375 0.0021093749999999997
-0.825 0.001484375
-0.825625 0.0018359375000000001
-0.82625 0.0018750000000000004
-0.826875 0.0018359375000000001
-0.8275 0.0016015625000000001
-0.828125 0.0023046875
-0.82875 0.0022656249999999994
-0.829375 0.00265625
-0.83 0.002109375
-0.830625 0.0022656249999999994
-0.83125 0.0017187499999999998
-0.831875 0.0023046875000000003
-0.8325 0.0021874999999999998
-0.833125 0.0024609374999999996
-0.83375 0.0021875
-0.834375 0.0019921875000000005
-0.835 0.0030078124999999996
-0.835625 0.002421875
-0.83625 0.0023437499999999995
-0.836875 0.0033203124999999995
-0.8375 0.002890625
-0.838125 0.0026171874999999993
-0.83875 0.0035546875000000006
-0.839375 0.002734375
-0.84 0.0032812499999999994
-0.840625 0.003515624999999999
-0.84125 0.0032031250000000002
-0.841875 0.0034375000000000005
-0.8425 0.004335937499999999
-0.843125 0.0036328124999999998
-0.84375 0.0041015625
-0.844375 0.004843749999999999
-0.845 0.003984375
-0.845625 0.004374999999999999
-0.84625 0.003984375
-0.846875 0.0044921875000000005
-0.8475 0.0042578124999999994
-0.848125 0.0051171875
-0.84875 0.0057421875
-0.849375 0.004531250000000002
-0.85 0.005117187500000002
-0.850625 0.005898437499999998
-0.85125 0.005742187500000001
-0.851875 0.0058984375
-0.8525 0.005351562500000001
-0.853125 0.006132812499999999
-0.85375 0.004999999999999999
-0.854375 0.005742187500000002
-0.855 0.005664062499999999
-0.855625 0.0062890625
-0.85625 0.0069140625
-0.856875 0.0063281249999999995
-0.8575 0.0065234375000000015
-0.858125 0.0067578125
-0.85875 0.0071874999999999994
-0.859375 0.007031250000000001
-0.86 0.007890625
-0.860625 0.008671874999999999
-0.86125 0.008632812500000003
-0.861875 0.0083203125
-0.8625 0.0087890625
-0.863125 0.008632812499999998
-0.86375 0.009101562499999997
-0.864375 0.0096484375
-0.865 0.0096875
-0.865625 0.009960937500000001
-0.86625 0.009921875
-0.866875 0.0095703125
-0.8675 0.010507812499999998
-0.868125 0.008749999999999999
-0.86875 0.011406249999999998
-0.869375 0.011601562499999999
-0.87 0.011796874999999998
-0.870625 0.011601562499999999
-0.87125 0.010117187500000001
-0.871875 0.010664062499999998
-0.8725 0.011484374999999998
-0.873125 0.012773437500000002
-0.87375 0.0128125
-0.874375 0.0128125
-0.875 0.014374999999999999
-0.875625 0.014960937499999999
-0.87625 0.014921875000000001
-0.876875 0.0159375
-0.8775 0.015703124999999995
-0.878125 0.0158984375
-0.87875 0.017382812500000004
-0.879375 0.016249999999999994
-0.88 0.017578125
-0.880625 0.017499999999999998
-0.88125 0.018632812500000002
-0.881875 0.0184375
-0.8825 0.02015625
-0.883125 0.019648437499999998
-0.88375 0.0185546875
-0.884375 0.020937500000000005
-0.885 0.022460937500000003
-0.885625 0.01984375
-0.88625 0.023046874999999998
-0.886875 0.021406249999999998
-0.8875 0.021406249999999995
-0.888125 0.022617187500000004
-0.88875 0.025546875000000004
-0.889375 0.022460937500000003
-0.89 0.0248828125
-0.890625 0.025976562499999994
-0.89125 0.0278515625
-0.891875 0.028164062499999996
-0.8925 0.028164062499999996
-0.893125 0.028398437499999995
-0.89375 0.02816406250000001
-0.894375 0.028867187500000002
-0.895 0.030000000000000006
-0.895625 0.028203124999999996
-0.89625 0.029726562500000015
-0.896875 0.03203125
-0.8975 0.033320312500000004
-0.898125 0.03449218749999999
-0.89875 0.033671875000000004
-0.899375 0.03445312500000001
-0.9 0.034140624999999994
-0.900625 0.03546875
-0.90125 0.0369140625
-0.901875 0.03515624999999999
-0.9025 0.0365234375
-0.903125 0.039609375
-0.90375 0.0403515625
-0.904375 0.04062500000000001
-0.905 0.04007812500000001
-0.905625 0.04257812500000001
-0.90625 0.043437500000000004
-0.906875 0.045390625000000004
-0.9075 0.047656250000000004
-0.908125 0.0476953125
-0.90875 0.04621093750000001
-0.909375 0.048671874999999996
-0.91 0.0494921875
-0.910625 0.05230468749999999
-0.91125 0.052460937499999985
-0.911875 0.054960937499999994
-0.9125 0.053007812499999994
-0.913125 0.057851574999999975
-0.91375 0.057265625
-0.914375 0.058671875000000005
-0.915 0.05738281250000001
-0.915625 0.0625
-0.91625 0.06039061250000003
-0.916875 0.0646484375
-0.9175 0.06511718749999999
-0.918125 0.065078125
-0.91875 0.06425781250000002
-0.919375 0.06746093750000001
-0.92 0.0653125
-0.920625 0.071328175
-0.92125 0.07414063750000001
-0.921875 0.07609373750000001
-0.9225 0.07531250000000002
-0.923125 0.07843751249999999
-0.92375 0.07773435000000001
-0.924375 0.07863281249999998
-0.925 0.07972656249999997
-0.925625 0.08441408749999998
-0.92625 0.08152345000000001
-0.926875 0.08320312499999998
-0.9275 0.08613277500000004
-0.928125 0.09113282499999996
-0.92875 0.09222653750000002
-0.929375 0.09499998750000002
-0.93 0.09847663749999999
-0.930625 0.09625003750000002
-0.93125 0.09937496250000001
-0.931875 0.10339845
-0.9325 0.10515628750000001
-0.933125 0.10890622500000002
-0.93375 0.1077343875
-0.934375 0.1132421375
-0.935 0.11156255
-0.935625 0.11410161250000003
-0.93625 0.1109765375
-0.936875 0.117773525
-0.9375 0.12003906249999999
-0.938125 0.1185157125
-0.93875 0.12441402500000001
-0.939375 0.12414060000000005
-0.94 0.1252344125
-0.940625 0.12699212499999998
-0.94125 0.12863286250000003
-0.941875 0.13042972500000002
-0.9425 0.13234385
-0.943125 0.13730472499999996
-0.94375 0.14164055000000003
-0.944375 0.1424609375
-0.945 0.14101565
-0.945625 0.14882815
-0.94625 0.14878902500000002
-0.946875 0.15000000000000002
-0.9475 0.152851575
-0.948125 0.156953075
-0.94875 0.15738285
-0.949375 0.1633203
-0.95 0.16667957500000002
-0.950625 0.167812525
-0.95125 0.16898430000000003
-0.951875 0.17566417500000003
-0.9525 0.17265623749999998
-0.953125 0.175273575
-0.95375 0.17871087499999996
-0.954375 0.186093725
-0.955 0.1888671
-0.955625 0.18867189999999998
-0.95625 0.19390632499999996
-0.956875 0.199140625
-0.9575 0.20300772499999997
-0.958125 0.204921875
-0.95875 0.21156247499999994
-0.959375 0.20972660000000004
-0.96 0.21097657499999994
-0.960625 0.21359369999999997
-0.96125 0.21707032500000004
-0.961875 0.227148325
-0.9625 0.22906260000000006
-0.963125 0.22624992500000002
-0.96375 0.23152342499999995
-0.964375 0.2360938
-0.965 0.24222652500000005
-0.965625 0.2426953749999999
-0.96625 0.24445315000000006
-0.966875 0.24980462499999997
-0.9675 0.25699215
-0.968125 0.25664062499999996
-0.96875 0.2596875249999999
-0.969375 0.261250075
-0.97 0.2707422
-0.970625 0.264960925
-0.97125 0.27683595000000005
-0.971875 0.27492190000000005
-0.9725 0.28363277500000006
-0.973125 0.281914025
-0.97375 0.28703124999999996
-0.974375 0.2933203
-0.975 0.293203125
-0.975625 0.29960942500000004
-0.97625 0.30199212499999994
-0.976875 0.30496092499999994
-0.9775 0.31378904999999996
-0.978125 0.31437507500000006
-0.97875 0.319570325
-0.979375 0.32238285
-0.98 0.3296485250000001
-0.980625 0.329140675
-0.98125 0.3359765
-0.981875 0.33949222499999987
-0.9825 0.33972652499999995
-0.983125 0.3392969250000001
-0.98375 0.3413672500000001
-0.984375 0.35257815000000003
-0.985 0.350976575
-0.985625 0.3575781250000001
-0.98625 0.3613281
-0.986875 0.367500075
-0.9875 0.37246095
-0.988125 0.37703127500000005
-0.98875 0.3799608500000001
-0.989375 0.3817187249999999
-0.99 0.387968775
-0.990625 0.389531225
-0.99125 0.3891406
-0.991875 0.3979296750000001
-0.9925 0.40230475
-0.993125 0.41164062499999987
-0.99375 0.41222649999999994
-0.994375 0.4173437250000001
-0.995 0.419414025
-0.995625 0.42472667500000005
-0.99625 0.4263281500000001
-0.996875 0.43152345
-0.9975 0.43433595
-0.998125 0.44148437500000004
-0.99875 0.4416405750000001
-0.999375 0.44644525
-1.0 0.44957027500000013
-1.000625 0.4623827499999999
-1.00125 0.4644141250000001
-1.001875 0.464648575
-1.0025 0.47000000000000003
-1.003125 0.468203175
-1.00375 0.47664065000000005
-1.004375 0.4846483499999999
-1.005 0.491015525
-1.005625 0.4922655749999998
-1.00625 0.49722662499999987
-1.006875 0.5008593000000001
-1.0075 0.5035936750000001
-1.008125 0.514414025
-1.00875 0.5115234749999998
-1.009375 0.5147656000000002
-1.01 0.5216406749999998
-1.010625 0.5246874999999999
-1.01125 0.531171925
-1.011875 0.5401953749999999
-1.0125 0.54175775
-1.013125 0.5460936500000001
-1.01375 0.545898425
-1.014375 0.5459765
-1.015 0.549101575
-1.015625 0.560781275
-1.01625 0.5572265750000001
-1.016875 0.5694140249999999
-1.0175 0.5651562250000001
-1.018125 0.573203175
-1.01875 0.5805077750000001
-1.019375 0.5813281499999998
-1.02 0.5832813000000001
-1.020625 0.58882815
-1.02125 0.5934373749999999
-1.021875 0.5949219249999999
-1.0225 0.6035547499999999
-1.023125 0.6086329
-1.02375 0.6118749
-1.024375 0.618359425
-1.025 0.6178125000000001
-1.025625 0.624335925
-1.02625 0.6296875000000001
-1.026875 0.631679675
-1.0275 0.6344140249999999
-1.028125 0.6322266
-1.02875 0.6411327999999998
-1.029375 0.64468745
-1.03 0.65277345
-1.030625 0.6552734000000001
-1.03125 0.6527343500000002
-1.031875 0.658124975
-1.0325 0.6642968250000001
-1.033125 0.6678906250000001
-1.03375 0.6712890749999999
-1.034375 0.6784765750000001
-1.035 0.6790234500000001
-1.035625 0.6757422249999999
-1.03625 0.683085925
-1.036875 0.6866015999999998
-1.0375 0.687382825
-1.038125 0.6882813
-1.03875 0.6945703249999998
-1.039375 0.6973047
-1.04 0.69656265
-1.040625 0.7051171249999999
-1.04125 0.7099608749999999
-1.041875 0.7091797000000001
-1.0425 0.7149999500000002
-1.043125 0.7208202749999999
-1.04375 0.7201953
-1.044375 0.7304297750000002
-1.045 0.7289844000000001
-1.045625 0.73285155
-1.04625 0.7359374999999999
-1.046875 0.7403125500000001
-1.0475 0.74812495
-1.048125 0.7481641499999998
-1.04875 0.7509374749999999
-1.049375 0.7529295000000003
-1.05 0.756132775
-1.050625 0.7566016249999999
-1.05125 0.7628125250000001
-1.051875 0.76656235
-1.0525 0.7715624999999998
-1.053125 0.7709374999999999
-1.05375 0.769921875
-1.054375 0.772695275
-1.055 0.774570275
-1.055625 0.7817578000000001
-1.05625 0.7813671
-1.056875 0.78765625
-1.0575 0.78406255
-1.058125 0.7925390250000001
-1.05875 0.793164125
-1.059375 0.79789065
-1.06 0.8004687
-1.060625 0.80558595
-1.06125 0.8054688249999998
-1.061875 0.8091016249999999
-1.0625 0.8090625499999999
-1.063125 0.8146875
-1.06375 0.8133593999999998
-1.064375 0.818906325
-1.065 0.8176953500000002
-1.065625 0.8203125499999999
-1.06625 0.8261719000000001
-1.066875 0.82371095
-1.0675 0.8304296749999999
-1.068125 0.8299999999999997
-1.06875 0.8372265000000002
-1.069375 0.8349218749999997
-1.07 0.8403124500000001
-1.070625 0.8422656
-1.07125 0.8443359499999998
-1.071875 0.845507775
-1.0725 0.8446094000000001
-1.073125 0.8533984
-1.07375 0.8508985250000001
-1.074375 0.8540625000000001
-1.075 0.8586718750000003
-1.075625 0.8608593750000002
-1.07625 0.86070315
-1.076875 0.8617578
-1.0775 0.8635546500000002
-1.078125 0.8706640750000002
-1.07875 0.8709375250000002
-1.079375 0.8723438
-1.08 0.87273425
-1.080625 0.8773437249999999
-1.08125 0.88113285
-1.081875 0.8815234750000001
-1.0825 0.8832812249999998
-1.083125 0.8834765750000002
-1.08375 0.8849608249999997
-1.084375 0.8894531500000001
-1.085 0.8891015750000001
-1.085625 0.8904297750000001
-1.08625 0.893515525
-1.086875 0.8993359749999998
-1.0875 0.8976953250000002
-1.088125 0.8980078749999999
-1.08875 0.89812515
-1.089375 0.9028906000000003
-1.09 0.9022655499999999
-1.090625 0.9049219
-1.09125 0.9029686499999998
-1.091875 0.9072655999999999
-1.0925 0.906132825
-1.093125 0.9078123500000002
-1.09375 0.9121484249999996
-1.094375 0.9108203500000001
-1.095 0.91695305
-1.095625 0.9170703999999998
-1.09625 0.9163671499999999
-1.096875 0.9197655500000002
-1.0975 0.92175775
-1.098125 0.9212109500000001
-1.09875 0.9271875250000001
-1.099375 0.9258594
-1.1 0.9261718250000002
-1.100625 0.9250000750000001
-1.10125 0.9281250250000002
-1.101875 0.9310546499999999
-1.1025 0.9320312749999999
-1.103125 0.9317187749999999
-1.10375 0.9355858250000001
-1.104375 0.9367577749999999
-1.105 0.937304575
-1.105625 0.9378905749999997
-1.10625 0.9385156249999997
-1.106875 0.9417577999999999
-1.1075 0.9452344250000001
-1.108125 0.9433985000000004
-1.10875 0.9441796749999998
-1.109375 0.9448436499999999
-1.11 0.9446874249999999
-1.110625 0.9476953250000001
-1.11125 0.9505468249999998
-1.111875 0.9527344500000001
-1.1125 0.9515234749999999
-1.113125 0.9525392250000001
-1.11375 0.9560938000000002
-1.114375 0.9575391000000002
-1.115 0.9540625500000001
-1.115625 0.955078125
-1.11625 0.9589453249999998
-1.116875 0.9602343750000001
-1.1175 0.9605078
-1.118125 0.9600000499999999
-1.11875 0.9632032
-1.119375 0.9641796749999998
-1.12 0.9656249499999999
-1.120625 0.9657030750000002
-1.12125 0.9667578000000001
-1.121875 0.969062475
-1.1225 0.9669141250000001
-1.123125 0.9677734499999999
-1.12375 0.9682812500000002
-1.124375 0.9658594250000003
-1.125 0.9713671500000001
-1.125625 0.9728515250000003
-1.12625 0.9734375249999999
-1.126875 0.9737890750000002
-1.1275 0.9764844500000003
-1.128125 0.9778515749999999
-1.12875 0.97902325
-1.129375 0.9771485000000002
-1.13 0.9794139999999999
-1.130625 0.9814453999999999
-1.13125 0.982030975
-1.131875 0.9845699000000001
-1.1325 0.9819922000000002
-1.133125 0.9809763249999998
-1.13375 0.9829687000000001
-1.134375 0.9841794999999998
-1.135 0.9874218250000004
-1.135625 0.9871874500000004
-1.13625 0.98738285
-1.136875 0.9889450500000001
-1.1375 0.9912105250000002
-1.138125 0.9901561250000004
-1.13875 0.9919527750000002
-1.139375 0.9939058
-1.14 0.9914059999999998
-1.140625 0.9932031250000002
-1.14125 0.9949214750000003
-1.141875 0.995663725
-1.1425 0.9962497499999999
-1.143125 0.9971873750000002
-1.14375 0.9973823750000002
-1.144375 0.9992570249999998
-1.145 1.0007025749999998
-1.145625 1.0026559999999998
-1.14625 0.9994140000000004
-1.146875 1.0043742750000002
-1.1475 1.0086707500000005
-1.148125 1.005077725
-1.14875 1.00769425
-1.149375 1.0086323249999998
-1.15 1.0082020999999999
-1.150625 1.008435875
-1.15125 1.0101559749999998
-1.151875 1.0119139999999998
-1.1525 1.0092184499999999
-1.153125 1.0099601000000002
-1.15375 1.010467625
-1.154375 1.012304425
-1.155 1.0152332749999997
-1.155625 1.0118348
-1.15625 1.014021825
-1.156875 1.0164834999999999
-1.1575 1.015859625
-1.158125 1.0171481249999998
-1.15875 1.019453
-1.159375 1.01851525
-1.16 1.0202337000000001
-1.160625 1.0219917500000002
-1.16125 1.01996
-1.161875 1.02468725
-1.1625 1.0255459999999996
-1.163125 1.025234625
-1.16375 1.02289045
-1.164375 1.0245309999999999
-1.165 1.0281640000000003
-1.165625 1.0280853000000003
-1.16625 1.0273824499999997
-1.166875 1.0294137499999998
-1.1675 1.03113325
-1.168125 1.0314459999999999
-1.16875 1.0317972499999999
-1.169375 1.0316414999999997
-1.17 1.0336337500000001
-1.170625 1.0368352
-1.17125 1.0344140000000004
-1.171875 1.0379297500000004
-1.1725 1.0388277499999998
-1.173125 1.0405460000000002
-1.17375 1.0403522500000002
-1.174375 1.0415625
-1.175 1.0414072500000002
-1.175625 1.0404687499999998
-1.17625 1.043828
-1.176875 1.04703225
-1.1775 1.0445712500000002
-1.178125 1.0461717499999998
-1.17875 1.04785125
-1.179375 1.0473830000000002
-1.18 1.046835
-1.180625 1.0500392499999998
-1.18125 1.0498827499999996
-1.181875 1.050586
-1.1825 1.05336025
-1.183125 1.0514072500000002
-1.18375 1.0555085000000002
-1.184375 1.0568745
-1.185 1.0580469999999997
-1.185625 1.0582032499999998
-1.18625 1.0595700000000001
-1.186875 1.060234
-1.1875 1.0603902500000002
-1.188125 1.0593357500000002
-1.18875 1.06304525
-1.189375 1.06320375
-1.19 1.0662507500000002
-1.190625 1.0679294999999998
-1.19125 1.06644475
-1.191875 1.0722652500000005
-1.1925 1.0711322499999998
-1.193125 1.0688282499999997
-1.19375 1.06980475
-1.194375 1.0744927499999999
-1.195 1.0735160000000004
-1.195625 1.0753509999999997
-1.19625 1.0787499999999999
-1.196875 1.07738275
-1.1975 1.07703125
-1.198125 1.07746175
-1.19875 1.077617
-1.199375 1.084023
-1.2 1.0830475000000002
-1.200625 1.0852340000000003
-1.20125 1.0866017499999998
-1.201875 1.08589825
-1.2025 1.0865617499999998
-1.203125 1.088945
-1.20375 1.0915235000000003
-1.204375 1.09163975
-1.205 1.0918362499999996
-1.205625 1.09367175
-1.20625 1.0949995
-1.206875 1.0974609999999998
-1.2075 1.0964062499999998
-1.208125 1.10058625
-1.20875 1.1027352500000003
-1.209375 1.1044532500000002
-1.21 1.1004295
-1.210625 1.1045695000000002
-1.21125 1.11054725
-1.211875 1.109375
-1.2125 1.1105867500000002
-1.213125 1.1125777500000003
-1.21375 1.1123437499999995
-1.214375 1.1166405000000001
-1.215 1.1187497499999999
-1.215625 1.1171485
-1.21625 1.12043
-1.216875 1.1190620000000002
-1.2175 1.1179692500000002
-1.218125 1.12632875
-1.21875 1.12859325
-1.219375 1.1283992500000002
-1.22 1.1329295
-1.220625 1.13121125
-1.22125 1.1372272500000002
-1.221875 1.1326567499999998
-1.2225 1.13750075
-1.223125 1.13597575
-1.22375 1.1375787500000003
-1.224375 1.14605425
-1.225 1.1452345
-1.225625 1.1493745
-1.22625 1.1479300000000001
-1.226875 1.1518367500000002
-1.2275 1.1499220000000003
-1.228125 1.154726
-1.22875 1.1568742500000002
-1.229375 1.1573435
-1.23 1.1574605
-1.230625 1.1595312499999997
-1.23125 1.16421925
-1.231875 1.1621872500000001
-1.2325 1.1683205000000003
-1.233125 1.1684759999999998
-1.23375 1.1670304999999999
-1.234375 1.1744917499999994
-1.235 1.17585925
-1.235625 1.1759764999999998
-1.23625 1.1780864999999996
-1.236875 1.17718825
-1.2375 1.1857802499999999
-1.238125 1.1847267500000005
-1.23875 1.1856250000000004
-1.239375 1.1850785
-1.24 1.18582
-1.240625 1.1943357499999996
-1.24125 1.1952347499999998
-1.241875 1.18882875
-1.2425 1.2007022499999997
-1.243125 1.2017965
-1.24375 1.2039847500000003
-1.244375 1.207578
-1.245 1.2066012499999998
-1.245625 1.21050775
-1.24625 1.2141802500000003
-1.246875 1.213711
-1.2475 1.215273
-1.248125 1.2243747500000002
-1.24875 1.22183575
-1.249375 1.2255472500000006
-1.25 1.2308984999999995
-1.250625 1.2261710000000001
-1.25125 1.229962
-1.251875 1.2366800000000002
-1.2525 1.2362495
-1.253125 1.2398437500000001
-1.25375 1.24277325
-1.254375 1.2489847500000004
-1.255 1.2497265000000002
-1.255625 1.2534372499999997
-1.25625 1.2460932499999995
-1.256875 1.255078
-1.2575 1.2544135
-1.258125 1.25851475
-1.25875 1.261523
-1.259375 1.2640634999999998
-1.26 1.266562
-1.260625 1.2756634999999998
-1.26125 1.2723827500000002
-1.261875 1.2732425000000003
-1.2625 1.2794534999999994
-1.263125 1.2829300000000003
-1.26375 1.2931254999999997
-1.264375 1.2953127500000001
-1.265 1.29413975
-1.265625 1.2950002500000004
-1.26625 1.29257875
-1.266875 1.3053902500000003
-1.2675 1.2991017500000002
-1.268125 1.3059372500000002
-1.26875 1.308594
-1.269375 1.3125395000000009
-1.27 1.319219
-1.270625 1.3203122500000002
-1.27125 1.3189065
-1.271875 1.328438
-1.2725 1.3263675
-1.273125 1.3310547500000003
-1.27375 1.3360545000000001
-1.274375 1.337774
-1.275 1.3439835
-1.275625 1.3451947499999997
-1.27625 1.34550775
-1.276875 1.35222675
-1.2775 1.353827
-1.278125 1.353437
-1.27875 1.3638679999999999
-1.279375 1.3587107500000004
-1.28 1.3647265000000002
-1.280625 1.3677339999999998
-1.28125 1.3708595
-1.281875 1.37941425
-1.2825 1.3779690000000007
-1.283125 1.38562525
-1.28375 1.3894144999999998
-1.284375 1.39414025
-1.285 1.3892975
-1.285625 1.394922
-1.28625 1.4007425000000002
-1.286875 1.4090224999999998
-1.2875 1.40390625
-1.288125 1.41124925
-1.28875 1.4130860000000003
-1.289375 1.41945275
-1.29 1.4210937499999996
-1.290625 1.42089875
-1.29125 1.4312895000000005
-1.291875 1.4323445000000001
-1.2925 1.4355862499999996
-1.293125 1.4403120000000005
-1.29375 1.43714825
-1.294375 1.441055
-1.295 1.4458587500000002
-1.295625 1.44710925
-1.29625 1.4527352499999995
-1.296875 1.45956925
-1.2975 1.4608212500000004
-1.298125 1.4657810000000002
-1.29875 1.4718352500000003
-1.299375 1.4736334999999996
-1.3 1.4786329999999999
-1.300625 1.4789460000000003
-1.30125 1.4848050000000004
-1.301875 1.49207
-1.3025 1.4917965
-1.303125 1.4899217500000002
-1.30375 1.49351575
-1.304375 1.4989452499999998
-1.305 1.5028902499999997
-1.305625 1.507734
-1.30625 1.5182035
-1.306875 1.5155077499999998
-1.3075 1.5206635
-1.308125 1.5209762500000001
-1.30875 1.5249222500000001
-1.309375 1.5210547500000002
-1.31 1.5281257499999998
-1.310625 1.5371482500000002
-1.31125 1.5320697499999998
-1.311875 1.5480077500000002
-1.3125 1.5478517499999997
-1.313125 1.552618
-1.31375 1.5552345000000003
-1.314375 1.5563282499999995
-1.315 1.55804575
-1.315625 1.565117
-1.31625 1.5704297500000004
-1.316875 1.5788677500000001
-1.3175 1.5798822499999998
-1.318125 1.5769535000000001
-1.31875 1.5804302499999998
-1.319375 1.5857035
-1.32 1.5920312499999996
-1.320625 1.5952735
-1.32125 1.5930079999999998
-1.321875 1.6023045000000002
-1.3225 1.6023435000000004
-1.323125 1.6100782500000002
-1.32375 1.6107427499999996
-1.324375 1.6102727499999994
-1.325 1.6126162499999999
-1.325625 1.6164840000000003
-1.32625 1.6260547500000002
-1.326875 1.6205462499999996
-1.3275 1.6268359999999995
-1.328125 1.6357422500000005
-1.32875 1.63835925
-1.329375 1.6472269999999998
-1.33 1.6484372500000002
-1.330625 1.6488669999999999
-1.33125 1.65433625
-1.331875 1.6553907499999994
-1.3325 1.6546487500000002
-1.333125 1.6618747500000002
-1.33375 1.66331975
-1.334375 1.6656645000000005
-1.335 1.66906325
-1.335625 1.6780459999999997
-1.33625 1.6869532499999997
-1.336875 1.6796867499999997
-1.3375 1.6894525000000002
-1.338125 1.6916014999999998
-1.33875 1.6892577500000001
-1.339375 1.6944129999999997
-1.34 1.69746075
-1.340625 1.7008215
-1.34125 1.70316425
-1.341875 1.7093742499999998
-1.3425 1.7104300000000001
-1.343125 1.7132817500000002
-1.34375 1.71308575
-1.344375 1.72015625
-1.345 1.7226950000000003
-1.345625 1.72331975
-1.34625 1.7229690000000009
-1.346875 1.7269920000000003
-1.3475 1.72726675
-1.348125 1.73640675
-1.34875 1.7347659999999998
-1.349375 1.7407815000000002
-1.35 1.74015575
-1.350625 1.74398425
-1.35125 1.748594
-1.351875 1.7587120000000005
-1.3525 1.76070275
-1.353125 1.7572670000000001
-1.35375 1.76488325
-1.354375 1.7648047500000004
-1.355 1.7650390000000002
-1.355625 1.7655467500000004
-1.35625 1.7739457500000004
-1.356875 1.7769927500000002
-1.3575 1.78203125
-1.358125 1.7806242500000002
-1.35875 1.7801565000000004
-1.359375 1.78437475
-1.36 1.78894625
-1.360625 1.7891020000000004
-1.36125 1.7941022500000003
-1.361875 1.7960547500000004
-1.3625 1.7961327499999995
-1.363125 1.7978512500000001
-1.36375 1.80000125
-1.364375 1.80648425
-1.365 1.80597675
-1.365625 1.80933625
-1.36625 1.8129679999999997
-1.366875 1.811719
-1.3675 1.8150774999999997
-1.368125 1.817266
-1.36875 1.8176169999999998
-1.369375 1.8209370000000002
-1.37 1.8269534999999997
-1.370625 1.83101575
-1.37125 1.8287887499999997
-1.371875 1.8278515
-1.3725 1.8353522499999997
-1.373125 1.83175825
-1.37375 1.8328509999999998
-1.374375 1.83746075
-1.375 1.8417189999999994
-1.375625 1.843593499999999
-1.37625 1.8464064999999994
-1.376875 1.8482422499999995
-1.3775 1.8460157499999998
-1.378125 1.8519925000000002
-1.37875 1.8522264999999998
-1.379375 1.8523832499999997
-1.38 1.8577734999999997
-1.380625 1.85679725
-1.38125 1.8602347499999996
-1.381875 1.8673042499999997
-1.3825 1.8675000000000002
-1.383125 1.8694917499999995
-1.38375 1.8714840000000001
-1.384375 1.8754690000000003
-1.385 1.8757030000000008
-1.385625 1.8764055
-1.38625 1.8719142500000001
-1.386875 1.87863275
-1.3875 1.881993
-1.388125 1.8847652499999996
-1.38875 1.8857417499999998
-1.389375 1.88429675
-1.39 1.8871875000000002
-1.390625 1.8916800000000003
-1.39125 1.8916009999999996
-1.391875 1.88914
-1.3925 1.8946487500000004
-1.393125 1.8955857500000004
-1.39375 1.89527375
-1.394375 1.8971479999999996
-1.395 1.9003909999999997
-1.395625 1.9016405000000005
-1.39625 1.9025387500000008
-1.396875 1.902422249999999
-1.3975 1.9051955
-1.398125 1.9072657499999994
-1.39875 1.9067964999999993
-1.399375 1.9083977500000002
-1.4 1.9106247499999998
-1.400625 1.9111337499999999
-1.40125 1.9128907500000008
-1.401875 1.9134377499999995
-1.4025 1.9112892499999994
-1.403125 1.91859375
-1.40375 1.9188280000000002
-1.404375 1.9191797500000003
-1.405 1.9230075000000002
-1.405625 1.9221487499999994
-1.40625 1.9233597500000006
-1.406875 1.9244537500000003
-1.4075 1.9268354999999993
-1.408125 1.9263675
-1.40875 1.9320709999999999
-1.409375 1.930469
-1.41 1.9299997499999997
-1.410625 1.9330462500000007
-1.41125 1.9313282500000004
-1.411875 1.933828
-1.4125 1.9344532500000002
-1.413125 1.9352729999999998
-1.41375 1.9351955
-1.414375 1.9409765
-1.415 1.9379292499999992
-1.415625 1.9412887500000005
-1.41625 1.9407415000000003
-1.416875 1.9410939999999997
-1.4175 1.9451162500000003
-1.418125 1.9443354999999998
-1.41875 1.9433195
-1.419375 1.9437892499999996
-1.42 1.9465625
-1.420625 1.9487885000000003
-1.42125 1.9485940000000004
-1.421875 1.9507414999999995
-1.4225 1.9515229999999995
-1.423125 1.9516790000000008
-1.42375 1.9516405000000003
-1.424375 1.9524217500000005
-1.425 1.9514452500000001
-1.425625 1.9574995000000004
-1.42625 1.9559762499999997
-1.426875 1.9560542500000004
-1.4275 1.95504
-1.428125 1.9565622499999997
-1.42875 1.9589062499999996
-1.429375 1.9593747499999996
-1.43 1.9580472500000003
-1.430625 1.9572269999999996
-1.43125 1.95964875
-1.431875 1.9630467500000002
-1.4325 1.9621494999999993
-1.433125 1.9616017499999998
-1.43375 1.9626172500000005
-1.434375 1.9632429999999998
-1.435 1.9658205000000002
-1.435625 1.965586
-1.43625 1.96785175
-1.436875 1.9670704999999997
-1.4375 1.9678902499999995
-1.438125 1.9650004999999997
-1.43875 1.9678519999999995
-1.439375 1.9684760000000001
-1.44 1.9692587499999998
-1.440625 1.9696879999999997
-1.44125 1.97109275
-1.441875 1.97242175
-1.4425 1.9722644999999996
-1.443125 1.972773
-1.44375 1.9726162499999997
-1.444375 1.9755069999999997
-1.445 1.9757815
-1.445625 1.9750379999999996
-1.44625 1.9762104999999994
-1.446875 1.9750775
-1.4475 1.9747262499999998
-1.448125 1.9758202500000004
-1.44875 1.9771089999999998
-1.449375 1.9758195000000005
-1.45 1.9771479999999997
-1.450625 1.977499000000001
-1.45125 1.9785547500000003
-1.451875 1.9784377500000006
-1.4525 1.9782030000000002
-1.453125 1.9802342499999999
-1.45375 1.98160125
-1.454375 1.9801170000000003
-1.455 1.9804687500000004
-1.455625 1.9796485000000004
-1.45625 1.9825392500000003
-1.456875 1.98328275
-1.4575 1.9839069999999999
-1.458125 1.982773750000001
-1.45875 1.9821870000000001
-1.459375 1.9830862500000002
-1.46 1.9837112499999996
-1.460625 1.9853137499999995
-1.46125 1.9828125
-1.461875 1.9847664999999999
-1.4625 1.9838682500000004
-1.463125 1.9842980000000001
-1.46375 1.9851182500000006
-1.464375 1.9853525
-1.465 1.9854297500000009
-1.465625 1.9878914999999995
-1.46625 1.9883997500000004
-1.466875 1.9885160000000006
-1.4675 1.9887907500000004
-1.468125 1.9871105000000004
-1.46875 1.9871492500000005
-1.469375 1.9894154999999991
-1.47 1.9877352499999994
-1.470625 1.9876569999999998
-1.47125 1.98902425
-1.471875 1.9884782499999996
-1.4725 1.9883605
-1.473125 1.9888685000000002
-1.47375 1.9898059999999997
-1.474375 1.989024
-1.475 1.990236
-1.475625 1.9902745
-1.47625 1.9901179999999996
-1.476875 1.99089925
-1.4775 1.9906257499999995
-1.478125 1.9902352499999996
-1.47875 1.9901185
-1.479375 1.9905872500000001
-1.48 1.9917199999999995
-1.480625 1.99191525
-1.48125 1.9918752499999992
-1.481875 1.9913292500000002
-1.4825 1.9910165
-1.483125 1.9924229999999998
-1.48375 1.9921885000000004
-1.484375 1.9921105000000001
-1.485 1.9919539999999993
-1.485625 1.9919155
-1.48625 1.9925017499999995
-1.486875 1.9928922499999995
-1.4875 1.9925797499999998
-1.488125 1.9930477500000001
-1.48875 1.9939464999999998
-1.489375 1.99390675
-1.49 1.9944152499999994
-1.490625 1.99328225
-1.49125 1.9944157499999993
-1.491875 1.994454
-1.4925 1.9944157500000004
-1.493125 1.99386875
-1.49375 1.9941812499999994
-1.494375 1.9944539999999997
-1.495 1.9943765
-1.495625 1.9947670000000008
-1.49625 1.9947665000000003
-1.496875 1.9952360000000002
-1.4975 1.9955867499999997
-1.498125 1.9951189999999996
-1.49875 1.9961732500000005
-1.499375 1.9960957500000003
-1.5 1.9946887499999995
-1.500625 1.9960170000000002
-1.50125 1.9952744999999996
-1.501875 1.9953929999999995
-1.5025 1.9953530000000008
-1.503125 1.99621225
-1.50375 1.9961735000000005
-1.504375 1.995822500000001
-1.505 1.9965642500000005
-1.505625 1.996056500000001
-1.50625 1.9970332500000005
-1.506875 1.9965640000000007
-1.5075 1.9971110000000003
-1.508125 1.9966812500000006
-1.50875 1.99703325
-1.509375 1.9975805000000004
-1.51 1.9976187500000002
-1.510625 1.9978135000000006
-1.51125 1.9966425000000008
-1.511875 1.9973460000000003
-1.5125 1.9973447500000003
-1.513125 1.9980100000000007
-1.51375 1.9973844999999997
-1.514375 1.9971505000000005
-1.515 1.9978152499999997
-1.515625 1.9972280000000002
-1.51625 1.997462000000001
-1.516875 1.9982047500000004
-1.5175 1.9981262500000003
-1.518125 1.9981270000000007
-1.51875 1.9983607500000002
-1.519375 1.99785325
-1.52 1.9975020000000003
-1.520625 1.9984782500000005
-1.52125 1.9986735000000002
-1.521875 1.9987130000000004
-1.5225 1.9983222500000006
-1.523125 1.9982045000000006
-1.52375 1.9984392500000001
-1.524375 1.9984000000000002
-1.525 1.9987507500000004
-1.525625 1.9984785000000005
-1.52625 1.9987905000000006
-1.526875 1.998712
-1.5275 1.99871225
-1.528125 1.9988290000000002
-1.52875 1.9983607500000005
-1.529375 1.9988685000000004
-1.53 1.9991025000000004
-1.530625 1.9991027500000005
-1.53125 1.9988687500000002
-1.531875 1.9989467500000004
-1.5325 1.9989077500000003
-1.533125 1.9990637500000001
-1.53375 1.9990247500000002
-1.534375 1.9991415000000003
-1.535 1.9991030000000003
-1.535625 1.9991805000000007
-1.53625 1.9991417500000004
-1.536875 1.9989075000000003
-1.5375 1.9992197500000004
-1.538125 1.99937575
-1.53875 1.9991420000000002
-1.539375 1.9991810000000005
-1.54 1.9992980000000002
-1.540625 1.9992977500000002
-1.54125 1.9995320000000003
-1.541875 1.99961
-1.5425 1.9996490000000002
-1.543125 1.9996880000000004
-1.54375 1.9994537500000003
-1.544375 1.9994930000000004
-1.545 1.99937575
-1.545625 1.9995320000000003
-1.54625 1.9996490000000002
-1.546875 1.999298
-1.5475 1.9994150000000004
-1.548125 1.99960975
-1.54875 1.9994150000000002
-1.549375 1.9995710000000002
-1.55 1.9994150000000002
-1.550625 1.9996490000000002
-1.55125 1.9995707500000002
-1.551875 1.999493
-1.5525 1.9995710000000002
-1.553125 1.9997270000000005
-1.55375 1.9997660000000004
-1.554375 1.999883
-1.555 1.9996100000000006
-1.555625 1.99961
-1.55625 1.9996880000000001
-1.556875 1.999766
-1.5575 1.999766
-1.558125 1.999844
-1.55875 1.9995707500000002
-1.559375 1.9998050000000003
-1.56 1.9998440000000002
-1.560625 1.999727
-1.56125 1.9997270000000005
-1.561875 1.999766
-1.5625 1.9997657500000003
-1.563125 1.999766
-1.56375 1.999766
-1.564375 1.999883
-1.565 1.999766
-1.565625 1.999883
-1.56625 1.9998829999999999
-1.566875 1.9998049999999998
-1.5675 1.9998440000000002
-1.568125 1.9998440000000002
-1.56875 1.999961
-1.569375 1.9998050000000003
-1.57 1.9996880000000001
-1.570625 1.999961
-1.57125 1.9998440000000002
-1.571875 1.999883
-1.5725 1.9998049999999998
-1.573125 1.9998049999999998
-1.57375 1.999727
-1.574375 1.9999220000000002
-1.575 1.999844
-1.575625 1.999961
-1.57625 1.999766
-1.576875 1.9999220000000002
-1.5775 1.9998440000000002
-1.578125 1.9998050000000003
-1.57875 1.999883
-1.579375 1.999883
-1.58 2.0
-1.580625 1.999883
-1.58125 1.999727
-1.581875 1.9999220000000002
-1.5825 1.9998047500000002
-1.583125 1.9998440000000002
-1.58375 1.999766
-1.584375 1.9998049999999998
-1.585 1.9999220000000002
-1.585625 1.999883
-1.58625 1.999883
-1.586875 1.9999220000000002
-1.5875 2.0
-1.588125 1.999961
-1.58875 1.9999220000000002
-1.589375 1.9999220000000002
-1.59 1.999961
-1.590625 1.999883
-1.59125 1.999961
-1.591875 2.0
-1.5925 2.0
-1.593125 1.999961
-1.59375 1.999961
-1.594375 1.9999220000000002
-1.595 1.999961
-1.595625 2.0
-1.59625 1.999961
-1.596875 1.999961
-1.5975 1.9999220000000002
-1.598125 1.999961
-1.59875 1.999961
-1.599375 1.9999220000000002
-1.6 2.0

